Singularity Formation: Synergy in Theoretical, Numerical and Machine Learning Approaches

This thesis develops numerical and theoretical approaches for understanding and analyzing singularity formation in Partial Differential Equations (PDEs). The singularity formation in the Navier-Stokes Equation (NSE) is famously challenging as one of the seven Clay Prize problems. Unlike simpler equations such as the Nonlinear Heat (NLH) or Keller-Segel (KS) equations, where formal asymptotics near blowup are better understood, the intrinsic complexity of NSE makes quantitative analytical treatment difficult, if not impossible, without numerical guidance. Building on numerical insights, we introduce a robust analytical framework to simplify and systematize pen-and-paper proofs for simpler singular PDEs. We present a novel approach based on enforcing vanishing modulation conditions for perturbations around approximate blowup profiles, complemented by singularly weighted energy estimates. We demonstrate the efficacy of our method on PDEs with complicated asymptotics, such as NLH and the Complex Ginzburg-Landau (CGL) equation, and address the open problem of singularity formation in the 3D KS equation with logistic damping. We develop and refine numerical approaches that facilitate deeper insights into singularity formation. We demonstrate that machine learning methods significantly enhance our capability to identify and characterize potential blowup solutions with high precision. We improve on existing Physics-Informed Neural Network (PINN) and Neural Operator (NO) frameworks. Moreover, we present a novel machine learning paradigm, the Kolmogorov-Arnold Network (KAN) architecture, whose interpretability and excellent scaling properties are achieved through learnable nonlinearities.

==> cgl.tex <==
\chapter{Blowups via Local Modulations: Complex Ginzburg-Landau}  
\label{cha:cgl}
\begingroup
\newcommand{\Epsilon}{\mathrm{E}}
\newcommand{\Eta}{\mathrm{H}}
\newcommand{\assign}{:=}
\newcommand{\cdummy}{\cdot}
\newcommand{\mathd}{\mathrm{d}}
\newcommand{\tmop}[1]{\ensuremath{\operatorname{#1}}}
\newcommand{\Rb}{\mathbb{R}}
\newcommand{\Ac}{\mathcal{A}}
\newcommand{\Bc}{\mathcal{B}}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\Dc}{\mathcal{D}}
\newcommand{\Ec}{\mathcal{E}}
\newcommand{\Fc}{\mathcal{F}}
\newcommand{\Gc}{\mathcal{G}}
\newcommand{\Hc}{\mathcal{H}}
\newcommand{\Lc}{\mathcal{L}}
\newcommand{\Oc}{\mathcal{O}}
\newcommand{\Mc}{\mathcal{M}}
\newcommand{\Nc}{\mathcal{N}}
\newcommand{\Qc}{\mathcal{Q}}
\newcommand{\Pc}{\mathcal{P}}
\newcommand{\Rc}{\mathcal{R}}
\newcommand{\Sc}{\mathcal{S}}
\newcommand{\Tc}{\mathcal{T}}
\newcommand{\Uc}{\mathcal{U}}
\newcommand{\Vc}{\mathcal{V}}
\newcommand{\Pb}{\mathbf{P}}
\newcommand{\Wb}{\mathbf{W}}
\newcommand{\Tb}{\mathbf{T}}
\newcommand{\Ub}{\mathbf{U}}
\newcommand{\Vb}{\mathbf{V}}
\newcommand{\Fb}{\mathbf{F}}

%% SIMPLIFIED NOTATIONS
\newcommand{\pa}{\partial}
\newcommand{\pr}{\partial_r}
\newcommand{\py}{\partial_y}
\newcommand{\pxi}{\partial_\xi}
\newcommand{\ps}{\partial_s}
\newcommand{\pt}{\partial_t}
\newcommand{\ptau}{\partial_\tau}
\newcommand{\inn}{\textup{in}}
\newcommand{\out}{\textup{ex}}
%% OPERATOR
\newcommand{\Ls}{\mathscr{L}}
\newcommand{\Ns}{\mathscr{N}}
\newcommand{\Fs}{\mathscr{F}}
\newcommand{\Ms}{\mathscr{M}}
\newcommand{\Ds}{\mathscr{D}}
\newcommand{\Hs}{\mathscr{H}}
\newcommand{\As}{\mathscr{A}}
\newcommand{\Es}{\mathscr{E}}
\newcommand{\Ts}{\mathscr{T}}

\newcommand{\Lst}{\tilde{\mathscr{L}}}

\newcommand{\Uk}{\mathfrak{U}}

% HERE macro
\newcommand\JC[1]{{\color{black}{#1}}}
%\newcommand\red[1]{\textcolor{red}{#1}}
\newcommand\red[1]{{\color{red}{#1}}}
\newcommand\blu[1]{{\color{black}{#1}}}
\newcommand\org[1]{{\color{orange}{#1}}}
\newcommand\vio[1]{{\color{violet}{#1}}}

 \newcommand{\beq}{\begin{equation}}
 \newcommand{\eeq}{\end{equation}}

 \newcommand{\bseq}{\begin{subequations}}
 \newcommand{\eseq}{\end{subequations}}
 \newcommand{\bal}{\begin{aligned} }
 \newcommand{\eal}{\end{aligned}}

 \newcommand{\bali}{\begin{align}}
 \newcommand{\eali}{ \end{align}}
  \newcommand{\tr}{\mathrm{tr}}
   \newcommand{\TT}{\mathbf{T}}

 \newcommand{\RR}{\mathbf{R}}
 \def\cR{{\mathcal R}}
   \let \mfr = \mathfrak
\let\lam=\lambda
 \let\f=\frac
  \let\D=\Delta
  \let \al = \alpha
 \let \les = \lesssim
 \let \gtr = \gtrsim
 \let\Om=\Omega
 \def\na{\nabla}
 \def\la{\langle}
 \def\ra{\rangle}
 \def \mr{\mathring}
  \let\d=\delta
  \let\B = \Big
  \let \kp = \kappa
  \let\e=\epsilon
  \let\td = \tilde
  \let\Ga= \Gamma
  \let\im= \imath
  \let \g = \gamma
  \let \be = \beta
  \let \th = \theta
  \let \Th = \Theta
  \let\Lam=\Lambda
  \def \VV{{\mathbf V}}
  \def\cE{{\mathcal E}}
   \let\s=\sigma
   \def\cH{{\mathcal H}}
 \def\cX{{\mathcal X}}
 \def\cY{{\mathcal Y}}
 \def\cZ{{\mathcal Z}}
  \def\cP{{\mathcal P}}
 \def\one{\mathbf{1}}
 \def \msD{  \mathscr{D}}
\def \msF{  \mathscr{F}}
\def \msN{ \mathscr{N} }
\def \msL{ \mathscr{L} }


 Building upon the idea in \cite{hou20242}, we establish the stability of 
the type-I\footnote{A blowup solution %to \eqref{cgl} 
is of Type I if it satisfies the bound $\lim_{t\to T}(T-t)^{-\frac{1}{p-1}}\|u(t)\|_\infty < \infty$, otherwise, blowup is of Type II.} blowup with log correction for the complex Ginzburg-Landau equation. In the amplitude-phase representation, a generalized dynamic rescaling formulation is introduced, with modulation parameters capturing the spatial translation and rotation symmetries of the equation and novel \JC{anisotropic} modulation parameters perturbing the scaling symmetry. 
This new formulation provides enough degrees of freedom to impose normalization conditions on the rescaled solution, completely eliminating the unstable and neutrally stable modes of the linearized operator around the blowup profile. It enables us to establish the full stability of the blowup by enforcing vanishing conditions via the choice of normalization and using weighted energy estimates, \blu{for a non-variational problem.} No topological argument or spectrum analysis is needed, \blu{opening up the possibility to tackle a wide range of type-I singularities}. The log correction for the blowup rate is \blu{automatically inferred via the local normalization conditions,} captured by the energy estimates and refined estimates of the modulation parameters.  

\section{Introduction}

We consider the complex Ginzburg-Landau equation 
\begin{equation}
    \label{cgl} 
    \psi_t=(1+\imath\beta)\Delta \psi + (1+\imath \delta)|\psi|^{p-1}\psi- \gamma \psi,  \tag{CGL}
\end{equation}
where $\psi(t): \Rb^d \to \mathbb{C}$, $\beta, \delta, \gamma$ are real constants and $p > 1$. The model equation \eqref{cgl} was first derived by Stewardson and Stuart in \cite{SSjfm71} (see also \cite{DHSjfm74}, \cite{PSbook85}) to examine afresh the problem of plane Poiseuille flow in a wave system. The equation is also used to describe various phenomena in many fields, among which are nonlinear optics with dissipation \cite{MHKnonl98}, turbulent behavior \cite{BLNphysd86}, Rayleigh-Bénard convection or Taylor-Couette flow in hydrodynamics \cite{diprima1971non}, \cite{NWjfm69}, \cite{newell1971review}, reaction-diffusion systems \cite{hagan1982spiral}, \cite{iooss1992time}, \cite{scheel1998bifurcation}, \cite{schneider1998hopf}, the theory of superconductivity \cite{bethuel1994ginzburg}, \cite{chapman1992macroscopic}, \cite{du1992analysis}, \cite{ginzburg2009theory}, etc. For further details on the physical background and derivation of the complex Ginzburg-Landau equation, we refer to the surveys \cite{AKaps02}, \cite{Mmono02}, and the references therein.

The local Cauchy problem has been well established through a semigroup approach in the works  \cite{GVphysd96,  GVmr97, GVcmp97}. A solution to \eqref{cgl} blows up in finite time if $\lim_{t \to T} \|\psi(t)\|_{L^\infty(\Rb^d)} = +\infty$ for some $ T < + \infty$.
% there exists $T \in (0, \infty)$ such that
% $$
% \lim_{t \to T} \|\psi(t)\|_{L^\infty(\Rb^d)} = +\infty.
% $$
% It is obvious to see that the nonlinear ODE associated with \eqref{cgl} ($\psi = \psi(t)$ and $\gamma = 0$) 
% \begin{equation}\label{eq:odecgl}
% \psi_t = (1 + \imath \delta)|\psi|^{p-1}\psi, \quad \psi(t = 0) = \psi_0,
% \end{equation}
% admits a blowup solution according to the expression $|\psi(t)| = \big[(p-1)(T-t)\big]^{-\frac{1}{p-1}}$ with  $T = |\psi_0|^{1-p}$. However, when $\psi$ depends on $x$, its blowup behavior is more subtle. Our goal is to derive a better understanding of blowup dynamics for \eqref{cgl}. 
% One of the common features in the study of singularity formation in PDEs is the existence of symmetries. The problem \eqref{cgl} with $\gamma =0$ enjoys the scaling invariance 
% \begin{equation}\label{def:scaling}
% \forall \lambda > 0, \quad \psi_\lambda(x,t) = \lambda^{\frac{2}{p-1}}\psi(\lambda x, \lambda^2 t),
% \end{equation}
% and the trivial phase shift, time, and spatial translation invariance 
% \begin{equation}\label{def:phaseshift}
% \forall \mu \in \Rb, \; x_0 \in \Rb^d, \; t_0 \in \Rb_+, \quad  \psi_{\mu, x_0, t_0}(x,t) = e^{\imath \mu} \psi(x - x_0, t - t_0). 
% \end{equation}
% The scaling symmetry gives rise to the energy- (sub/super)critical notion in the sense that 
% $$ \|\psi_\lambda(t)\|_{\dot{H}^{s_c}} = \|\psi(\lambda^2 t)\|_{\dot{H}^{s_c}} \quad \textup{with} \quad s_c= \frac{d}{2} -\frac{2}{p-1},$$
% so that $s_c = 1$ refers to as the energy-critical case, and $s_c < 1 (s_c > 1)$ the energy-sub(super)critical cases. In this paper, we do not impose any restriction on the power nonlinearity $p > 1$ or the dimension $d \geq 1$ for the study of blowup solutions to \eqref{cgl}. 
Singularity formation has been intensively studied for the two limiting models of \eqref{cgl}: the classical nonlinear heat equation in the limit $\beta, \delta, \gamma \to 0$,
\begin{equation}\label{nlh}
\pa_t \psi = \Delta \psi + |\psi|^{p-1}\psi, \quad \psi(t): x\in \Rb^d \to \Rb, \tag{NLH}
\end{equation}
and the nonlinear Schr\"odinger equation in the limit $\beta, |\delta| \to \infty$,
\begin{equation}\label{nls}
\imath \pa_t \psi + \Delta \psi +\mu |\psi|^{p-1}\psi = 0, \quad \mu = \pm 1. \tag{NLS}
\end{equation}
{We refer to \cite{quittner2019superlinear} and \cite{Fbook15} for intensive
lists of references from the early 1960s concerning blowup results of these two equations.} However, singularities in \eqref{cgl} (collapse, chaotic, or blowup) are much less understood in comparison with what have been established for \eqref{nlh} and \eqref{nls}. The study of singularity in \eqref{cgl}  is a challenging problem due to the lack of variational structure, no maximum principle, non-self-adjoint linearized operator, etc.  Nevertheless, singularity in \eqref{cgl} was experimentally reported in \cite{KBSaps88}, \cite{KSALphysD95} where the authors described an extensive series of experiments on traveling-wave convection in an ethanol/water mixture and collapse solutions were observed. We have a sharp sufficient criterion for collapse in \eqref{cgl} for the case of subcritical bifurcation described in \cite{Taps93}. In \cite{HDphysA98}, the authors used the modulation theory and numerical observations to show that the collapse dynamic is governed in the \eqref{cgl} limit of the $L^2$-critical cubic \eqref{nls}.  For the existence of blowup, there are the results of  \cite{CDFjee14} and \cite{CDFWsiam13} 
in which the authors studied \eqref{cgl} for the case $\beta = \delta$. {In \cite{budd2005multibump,BRWejam13}, %\cite{beck2014nonlinear}, 
\cite{RScpam01}}, the authors gave some evidence for the existence of a radial solution that blows up in a self-similar way, their arguments were based on the combination of rigorous analysis and numerical computations. In \cite{ZAAihn98} and \cite{MZjfa08}, the authors rigorously constructed particular examples of initial data for which the solutions of \eqref{cgl} blow up in finite time  for $(\beta, \delta)$ in the \textit{subcritical} range
\begin{equation}\label{def:subCri}
{\flat_* := p - \delta^2  - \beta \delta (p+1), \quad \flat_* > 0}  \quad \textup{(subcritical range)}.
\end{equation}
The constructed blowup solution in the subcritical case admits the asymptotic behavior 
\begin{equation}\label{eq:asyGLsub}
\psi(x,t) \sim  |\log (T-t)|^{\imath \mu} \Big[(T-t) \big( p -1   +  c_p |Z|^2\big) \Big]^{-\frac{1 + \imath \delta}{p-1}}, \quad Z = \frac{x}{\sqrt{(T-t)|\log (T-t)|}},
\end{equation}
where the constants $c_p$ and $\mu$ are given by
\begin{equation}
\label{def:constcp}c_p = \frac{(p-1)^2}{4\flat_*} > 0\,,\quad \mu = -\frac{\beta(1 + \delta^2)}{2\flat_*}\,.
\end{equation} The spectral analysis for a non-self-adjoint operator developed in \cite{MZjfa08} can be implemented for other problems where an energy-type method is not applicable, see for example \cite{GNZihp18}. The blowup for the critical range, $\flat_* = 0$, was solved in \cite{NZarma18}, \cite{DNZmems23} following the approach of \cite{MZjfa08}. The blowup for \eqref{cgl} in the supercritical range, $\flat_* < 0$, has recently been solved in \cite{DNZarxiv23} for the special choice $\beta = 0$. We remark that in the mentioned works (\cite{ZAAihn98}, \cite{MZjfa08}, \cite{NZarma18}, \cite{DNZmems23}, \cite{DNZarxiv23}), the authors focused on the case of dimension $d=1$, and briefly described the stability properties of constructed blowup solutions through a spectral approach in a restricted (well-prepared) class of initial data. \blu{One can go further in the spectral analysis to establish type II singularities, for example, the energy supercritical case for \eqref{nlh} in \cite{HVpre94} and for \eqref{nls} in \cite{merle2014type}.}


In this  chapter, we aim to develop a new approach based on the dynamical rescaling formulation and 
\JC{the energy method} to study blowup solutions to \eqref{cgl}. 
\JC{
 Compared to the aforementioned works that employ radial scalings to the spatial variable corresponding to the scaling symmetry, our approach has the following  key novelties. 
 We introduce novel \textit{nonradial, anisotropic} scalings to the spatial variable that breaks the scaling symmetry 
 and incorporates it, along with modulation parameters capturing the symmetries of the equations, to develop a novel generalized \textit{anisotropic} rescaling in Step 1 in Subsection \ref{sec:intro_dyn}. %to modulate the instability.}
This new approach allows us to use a purely energy-based method to establish asymptotically self-similar blowup 
in \eqref{cgl} and a clear notion of stability capturing the logarithm correction \eqref{eq:asyGLsub} in the subcritical case for a large class of initial data in all dimensions $d \geq 1$. 
}
%In this paper, we aim to develop a new approach based on the dynamical rescaling formulation and simple vanishing conditions to study blowup solutions to \eqref{cgl}. This new approach allows us to establish asymptotically self-similar blowup and a clear notion of stability capturing the logarithm correction \eqref{eq:asyGLsub} in the subcritical case for a large class of initial data in all dimensions $d \geq 1$. \blu{Compared with the aforementioned works that introduce simply a radial scaling corresponding to the scaling symmetry, general nonradial perturbation is allowed, and we introduce a novel generalized anisotropic rescaling in Step 1 in Subsection \ref{sec:intro_dyn} to modulate its stability.} 
Throughout this  chapter, we use the amplitude-phase representation,  
\begin{equation}\label{eq:intro_rep}
\psi(x,t) = u(x,t) e^{\imath \theta(x,t)},
\end{equation}
where $u$ and $\theta$ are real-valued functions of time and space solving the coupled system 
%\red{
\bseq\label{eq:CGL_intro}
 \begin{align}
 &\pa_t u = \big[\Delta - |\nabla \theta|^2 \big]u - \beta\big(2 \nabla u \cdot \nabla \theta  + u \Delta \theta \big)  + u^p - \gamma u, \label{eq:A_intro}\\
& u \pa_t \theta = \beta \big[\Delta - |\nabla \theta|^2   \big] u + 2 \nabla u \cdot \nabla \theta  + u \Delta \theta + \delta u^p .\label{eq:theta_intro}
% &\pa_t A = \big[\Delta - |\nabla \theta|^2 \big]A - \beta\big(2 \nabla A \cdot \nabla \theta  + A \Delta \theta \big)  + A^p - \gamma A, \label{eq:A_intro}\\
% & A \pa_t \theta = \beta \big[\Delta - |\nabla \theta|^2   \big]A + 2 \nabla A \cdot \nabla \theta  + A \Delta \theta + \delta A^p, \label{eq:theta_intro}
\end{align}
\eseq
The case $\beta = 0$ is related to a class of reaction-diffusion equations appearing in the study of pattern formation, see for example \cite{hagan1982spiral} and references therein. 



\subsection{Main result}
For any $k \geq 1$, we introduce the functional spaces $\mathfrak E_k$ and  $\mfr F_k$ 
 \begin{equation}\label{def:EkFk}
   \mfr E_k = \Big\{ w: \; \|w\|_{\mfr E_k} = \sum_{j = 0}^k\|\nabla ^j w\|_{\rho_j} < +\infty \Big\}, \quad \mfr F_k =\Big\{ \phi: \; \| \phi \|_{\mfr F_k} = \sum_{j = 1}^k \|\nabla^j \phi \|_{\mathring{\rho}_j} < +\infty \Big\},
 \end{equation}
 where $\| \cdot\|_{\rho_k}$ and $\|\cdot\|_{\mathring{\rho}_k}$  stand for the standard weighted $L^2$-norm with $\rho_k$ and $\mathring{\rho}_k$ being defined as in \eqref{wg:rho}. 
Let $\bar U$ be the universal profile 
\begin{equation}\label{def:Ubar}
\bar U(z) = \Big(p-1 + \frac{(p-1)^2}{4\flat_*} |z|^2 \Big)^{-\frac{1}{p-1}}, \quad \forall \ z \in \Rb^d,
\end{equation}
and $V_0$ be a non-degenerate global maximizer of $u_0$ defined by 
 \beq\label{eq:ass_init}
 V_0 = \arg\max u_0(z) , \quad  u_0(V_0)>0, \quad -\na^2 u_0( V_0 ) \succ 0,
 \eeq
 where $A \succ 0$ means that $A$ is a positive definite matrix. The main result of this  chapter is the following theorem.


\begin{theorem}[Existence and stability of blowup solutions to \eqref{cgl}]\label{thm:blp} 
Consider $\beta, \delta$ in the sub-critical range \eqref{def:subCri}, i.e. $\flat_* > 0$, $p > 1$ and $d \geq 1$. Let $K = K(d,p) \in \mathbb{N}$ be defined as in \eqref{K}. There exists an open set $\Oc \subset \mfr E_K \times \mfr F_{K}$ of initial data $\psi_0 = u_0 e^{{\imath}\theta_0}$ with the property \eqref{eq:ass_init} such that the corresponding solution $\psi = u e^{{\imath}\theta}$ to \eqref{cgl} blows up in finite time $T$ and the following asymptotic behaviors hold. \\

\noindent (i) \textup{(The amplitude-phase decomposition)}
\begin{equation} \label{est:asymptoticEKFK}
    \Big\| H(t) u \big( \RR(t) z + V(t), t \big) -  \bar U(z) \Big\|_{\mfr E_K} + \Big\| \theta \big( \RR(t) z + V(t), t \big) -  \mu(t) - \delta \log \bar U(z)\Big\|_{\mfr F_K} \leq \frac{C}{1 + |\log (T-t)|},
\end{equation}
where $H(t)$ and $\mu(t)$ are scalar functions, $\RR(t)$ is an upper triangular matrix and $V(t)$ is a vector in $\Rb^d$, 
\begin{equation} \label{est:limitHRV}
    \lim_{t \to T} \frac{H(t)^{p-1}}{T-t} =1, \quad \lim_{t \to T} \frac{\RR(t)}{\sqrt{(T-t)|\log (T-t)|}} = \textup{I}_d, \quad \lim_{t \to T} V(t) = V_T,
\end{equation}
for some $V_T \in \Rb^d$, and $\mu(t)$   {admits the expansion}\footnote{While the
$\mfr F_K$ norm in \eqref{est:asymptoticEKFK} only involves $\na^i \phi, i \geq 1 $ and $\mu(t)$ does not play a role in \eqref{est:asymptoticEKFK}, we keep $\mu(t)$ in \eqref{est:asymptoticEKFK} to indicate that it captures the phase of $\psi$. See \eqref{est:limitmu}, \eqref{eq:thm_estb}.}
\begin{equation}\label{est:limitmu}
\mu(t) = -\frac{\delta}{p-1} \log (T-t)  - 
\frac{d\beta(1  +\delta^2)}{2\flat_*} \log |\log (T-t)| + \hat \mu(t), \quad \lim_{t\to T} \hat \mu(t) = \hat \mu_T,
\end{equation}
    %\lim_{t \to T} \Big[\mu(t) - \frac{\delta}{p-1}|\log (T-t)| + \frac{d\beta(1  +\delta^2)}{2\flat_*} \log |\log (T-t)|\Big] = \hat \mu_T, 
 for some scalar function $\hat \mu(t)$ and $\hat \mu_T \in \Rb$. \\

\noindent (ii) \textup{($L^\infty$ asymptotic behavior)} 
\begin{equation}\label{eq:thm_estb}
 \Big\| |\log(T-t)|^{\imath  \frac{d\beta (1 + \delta^2)}{2\flat_*}} (T-t)^{\frac{1 + \imath \delta}{p-1}}  e^{ - \imath \hat \mu(t) } \; \psi( \RR(t) z + V(t) , t )  - \bar U^{1 + {\imath} \d} \Big\|_{L^{\infty}}  \leq \frac{C}{1 + |\log( T- t)|^{\sigma'}},
\end{equation}
where %$\lim_{t \to T} \hat \mu(t) = \hat \mu_T$, 
$\sigma' = \min \big\{1, \frac{4}{p-1}\big\}$ and $C = C(u_0, \theta_0) > 0$.
\end{theorem}

\medskip


 

 \begin{remark}
 [Description of the set $\Oc$ of initial data]\label{rem:blowup} For initial data $u_0$ satisfying the property \eqref{eq:ass_init}, we can define an upper triangular matrix $\Mc_0$ with $\Mc_{0,ii} > 0$\footnote{Simple linear algebra shows that $\Mc$ is uniquely determined.} and the rescaled variables $(U_0, \Th_0)$ 
\beq\label{eq:init_res}
\bal
& H_0 = \f{ \kp_0}{ u_0(V_0 )}, \quad 
\Mc_0^T \Mc_0  =  - \f{  \kp_0  \na^2 u_0(V_0)}{ \kp_2 u_0(V_0)  }
= H_0 \f{   \na^2 u_0(V_0)}{ \kp_2   },\quad \kp_0 = \bar U(0), \quad \kp_2 = \pa_1^2 \bar U(0), \\
& U_0(z) = H_0 u_0( \Mc_0^{-1} z + V_0),  \quad  \Th_0(z) =  \th_0( \Mc_0^{-1} z + V_0),
\eal
\eeq
where $\bar U$ is defined in \eqref{def:Ubar}. Since $\na u(V_0, 0) =0$, by definition, \eqref{eq:init_res} implies the following normalization 
 \beq\label{eq:init_res2}
    U_0(0)= \kp_0 = \bar{U}(0)\,,\quad \nabla U_0(0)=0\,,\quad \nabla^2 U_0(0)=\nabla^2 \bar{U}(0)=\kappa_2 I_d\,. 
  \eeq
Let $\nu > 0$ be small,  $\epsilon_2$ and $C_b$ be defined in \eqref{eps} and \eqref{eq:boot_U},  the set of initial data in Theorem \ref{thm:blp} consists of initial data $(u_0, \th_0)$ satisfying \eqref{eq:ass_init} and its rescaled variable $(U_0, \Th_0)$ satisfies 
\beq\label{eq:ass_init2}
U_0 \bar U^{-1- \e_2} > 2C_b , \quad H_0^{p-1} < \nu, \quad  u_0(V_0)^{-p} \tr( \na^2 u_0(V_0) ) < \nu ,
\eeq
and
\begin{equation}\label{def:EKFKbar}
\|W_0\|_{\mfr E_K}= \|U_0 - \bar U\|_{\mfr E_K} < \nu, \quad \|\Phi_0\|_{\bar {\mfr F}_K} := \| \Th_0 - \delta \log \bar U \|_{\mfr F_{K-1}} + \|\langle z \rangle^{K - \frac{d}{2}} \nabla^K (\Th_0 - \delta \log \bar U) \|_{L^2} < \nu.
 \end{equation}
The last quantity in \eqref{eq:ass_init2} is invariant under the parabolic rescaling: $u_{0, l}(z) 
= l^{1/(p-1)} u_0( l^{1/2} z)$. We will use its smallness to show that the viscous terms are small compared to the nonlinear terms. The lower bound $U_0 \bar U^{-1-\e} > 2 C_b$ in \eqref{eq:ass_init2} ensures that $U_0(z) \neq 0$ for any $z$, without which can lead to low regularity of rescaled velocity $|U|^p$ of $u^p$ \eqref{eq:A_intro}.
\end{remark}


\begin{remark}[Positive definiteness of the Hessian of the initial data]\label{rem:shape}
%While we show that in \eqref{eq:thm_est} the blowup solution is asymptotically self-similar with 
%an isotropic blowup profile $\bar U$, 
While the limiting blowup profile $\bar U$ \eqref{def:Ubar} is isotropic near $z=0$, we do not need to assume that the initial data $u_0$ is isotropic near $V_0$, i.e., $\na^2 u_0(V_0)$ is close to $c I_d$ for some $c \neq 0$. By introducing the upper triangular matrix $\RR(t)$ in the rescaling (see \eqref{eq:dyn_scal0}), 
we can handle a much larger class of initial data with non-degenerate global maximizer \eqref{eq:ass_init}. 
\end{remark}


  \begin{remark}\label{rem:1D}
  The asymptotics of the blowup solution \eqref{eq:thm_estb}  recovers the constructed result of Masmoudi-Zaag \cite{MZjfa08} for the case $d = 1$.  
  The set of initial data leading to the blowup solution described in Theorem \ref{thm:blp} contains different elements (see Remark \ref{rem:blowup}) from the one described in \cite{MZjfa08}  which is a subset of $L^\infty(R)$ via spectral analysis of a non-selfadjoint linear operator. We note that there is a free phase-shift $\hat \mu$ in \eqref{eq:thm_estb} corresponding to the phase invariant of \eqref{cgl} that was fixed to be $\hat \mu(t) = 0$ in \cite{MZjfa08} by a specific choice of initial data through a topological argument. We remark that the relaxing asymptotics \eqref{est:limitHRV} and \eqref{est:limitmu} are natural for rigorous stability analysis in all dimensions $d \geq 1$ treated in this  chapter.
\end{remark}

{Note that the asymptotic behavior \eqref{est:asymptoticEKFK}, \eqref{eq:thm_estb} involves the 4 parameter functions $H, \RR, V$ and $\mu$ (or $\hat \mu$) which are responsible for all the symmetries of \eqref{cgl}.\footnote{
Although $H(t)$ is absent in \eqref{eq:thm_estb}, we can replace the factor $(T-t)^{1/(p-1)}$ by $H(t)$ using \eqref{est:limitHRV}.} Theorem \ref{thm:blp} is stated in terms of the rescaled profiles, with a singular weight at the origin. 
We note that the condition \eqref{eq:ass_init} and parameters $\Mc_0, H_0, V_0$ in \eqref{eq:init_res} are $C^2$-stable if the global maximizer is unique.
We can therefore simplify the assumptions in Theorem \ref{thm:blp} to obtain the following stability results with a more explicit description of the open set of initial data. %without a singular weight at the origin.
 }

\begin{theorem}
    [Stability of blowup solutions to \eqref{cgl}]\label{cor:stab}

Let $K = K(d,p) \in \mathbb{N}$ be defined as in \eqref{K}, and $\cH^K, \mfr F_{K-1}$ be the norms defined in \eqref{norm:Hk}, \eqref{def:EkFk}. Suppose that $(u_0, \th_0)$ satisfies the assumptions \eqref{eq:ass_init}, \eqref{eq:ass_init2},
\eqref{def:EKFKbar} and $V_0$ is the unique global maximizer: $u_0(V_0) > u_0(z)$ for all $z \neq V_0$. 
%$u_0(V_0) > \max_{|z| \geq r } u_0(V_0 + z) $
%- \max_{|z| \geq r } u_0(V_0 + z) = b(r)>0$ 
%for any $r>0$. 
There exists {$\epsilon_0 = \e_0(u_0) > 0$} such that if 
\beq\label{eq:ass_cor}
\| \td u_0 - u_0 \|_{\cH^K} + \|(\td u_0 - u_0 ) \bar U^{-1-\e_2} \|_{L^{\infty}} +  \| \td \th_0 - \th_0\|_{\mfr F_{K-1}} + \|\langle z \rangle^{K - \frac d2} \nabla^K (\td \th_0 - \th_0) \|_{L^2}  < \epsilon_0,
\eeq
the solution $\tilde \psi = \td ue^{{\imath}\td \th}$ to \eqref{cgl} with the initial data $ \tilde \psi_0 = \td u_0e^{{\imath}\td \th_0}$ blows up in finite time $\td T$. Moreover, there exists $H(t), \RR(t), V(t), \mu(t)$ satisfying \eqref{est:limitHRV} and \eqref{est:limitmu} such that \eqref{est:asymptoticEKFK} and \eqref{eq:thm_estb} hold for $(\td u(t), \td \th(t))$ with $T$ being replaced by $\tilde T$. 
\end{theorem}

{From the proof of Theorem \ref{cor:stab}, it can be shown that $\e_0$ depends on $u_0$ through 
its certain norms. We do not state the dependence explicitly for simplicity.
}
\begin{remark} 
The assumptions in Theorems \ref{thm:blp},\ref{cor:stab} are satisfied, e.g. for $ u_0 = C \bar U$, $\th_0 = \bar \Th_0$ with $C$ sufficiently large. 
The weighted norms $\|\cdot \|_{\cH^K}$ \eqref{norm:Hk} and $\|\cdot \|_{\mfr F_K}$ \eqref{def:EkFk} are well-defined for sufficiently smooth functions with fast decay. We do not require that $u_0 - \td u_0$ agrees up to $\Oc(|z - V_0|^k), k >0$ near the maximizer $V_0$ of $u_0$. 
\end{remark}


%\subsection{Stability via vanishing conditions and weighted energy estimates}
\subsection{
Dynamic rescaling formulation with extra modulation parameters} 
\label{sec:intro_dyn}

{The dynamic rescaling formulation or the modulation technique was developed to study singularity formation in the nonlinear Schr\"odinger equation  \cite{mclaughlin1986focusing}, \cite{landman1988rate} numerically and various nonlinear PDEs; see the comprehensive references on \eqref{nlh},  \eqref{nls}, and related models in \cite{quittner2019superlinear}, \cite{Fbook15}.}
Recently, researchers also generalized this technique for fluid mechanics 
\cite{chen2019finite2,chen2022stable,chen2025stable}, \cite{elgindi2021finite}.  We can establish singularity in two steps. Firstly, one constructs an approximate steady state of the dynamic rescaling equation (analytically or numerically). Secondly, 
  one performs linear and nonlinear stability analysis for perturbation around the approximate steady state with appropriate normalization conditions. The law of blowup will then be prescribed by the normalizing constants.
  One can establish stability using a $L^2$-based \cite{chen2021finite,chen2021HL} or $L^\infty$-based \cite{chen2022stable} argument. In these arguments, {one of the crucial steps} is to design appropriate singular weights depending on the profile, and then use the weights to derive damping terms for the energy estimates. 
  The approach does not require an explicit profile and is robust to small perturbations, which makes it possible to combine weighted energy estimates for stability analysis,
  a numerical \textit{implicit} profile, and computer-assisted proofs to construct blowup solutions. {See for example,} \cite{chen2022stable,chen2025stable}  for applications in 3D incompressible Euler equations with smooth data and \cite{chen2021finite, chen2021HL}, \cite{chen2020singularity}, \cite{hou2024blowup} for related 1D models.


% Upon imposing pointwise vanishing conditions for the perturbation of the (approximate) profile, one can establish blowup via
% a $L^2$-based \cite{chen2021finite,chen2021HL} or $L^\infty$-based \cite{chen2022stable} stability argument, even if we do not have an explicit (approximate) profile. One can combine the stability argument with rigorous computer-assisted proofs and a numerical profile; see  \cite{chen2021finite, chen2021HL}, \cite{chen2020singularity}, \cite{ hou2024blowup} for applications in various 1D models for the Euler equation and \cite{chen2022stable,chen2025stable} for the 3D axissymmetric Euler equation. \blu{We can establish singularity in two steps: Firstly one solves for an approximate steady state of the dynamic rescaling equation (analytically or numerically) and relates blowup to the stability around the approximate steady state; second, one can perform linear and nonlinear stability estimates to show that upon imposing vanishing conditions the perturbation  still remain small in some suitable functional space. The law of blowup will  then be prescribed by the normalizing constants.}

In \cite{hou20242}, the authors generalized the $L^2$-based methodology to establish a type-I 
 blowup for the semilinear heat equation beyond the self-similar setting where there is a logarithm correction in the self-similar scaling
for the spatial variable. {Compared with previous works \cite{bricmont1994universality}, \cite{HVaihn93}, \cite{merle1997stability}, \cite{dejak2008blow}, \cite{MZjfa08} where the authors heavily relied on a spectral analysis with detailed properties of the associated linearized operator to establish the existence and stability, we simply suppress unstable directions {and neutral modes} via a clear characterization of weighted Sobolev spaces, without using Brouwer's fixed-point theorem or a topological argument.  The correct Type I blowup rate is automatically inferred by enforcing proper vanishing conditions of the perturbation. We remark that for Type I blowup, there is indeed a link between the vanishing conditions at the origin and the vanishing coefficients projected onto the unstable {and neutral} spectral eigenfunctions. %; see for example \cite{hou20242} and \cite{merle1997stability} in the case of the nonlinear heat equation, where the eigenfunctions correspond to Hermite polynomials.
{It is worth mentioning that the method used in \cite{hou20242} shares a similar approach to that of \cite{dejak2008blow}, where the authors employed self-similar variables and derived the blowup law by imposing orthogonality conditions on the perturbation with respect to the eigenfunctions (Hermite polynomials) of the associated linear operator in an exponentially weighted $L^2$
 space. In particular, these orthogonality conditions are analogous to the vanishing conditions at the origin in the correct blowup variables considered in \cite{hou20242}.} A further explanation of this connection is discussed in Step 2 in Section \ref{sec:idea}.} %One can further combine this method with a topological argument to establish singularity with finite codimensional stability; see \cite{liu2025finite} for an open problem on the Keller-Segel equation with logistic damping.

\vspace{0.1in}
\noindent \textbf{A generalized dynamical rescaling formulation with extra modulation parameters\footnote{The modulation parameters are also known as normalization constants in the dynamic rescaling formulation.}.}
In this article, we further generalize the above framework and the ideas in \cite{hou20242}. {In particular, it consists of three main steps:}

\vspace{0.1in}

%\vio{VT: I remove \textit{"artificial scalings"}}

\noindent \textit{Step 1 ({Renormalization with extra modulation parameters}):} {The renormalization is an essential step in the study of nonlinear PDEs with symmetries including incompressible/compressible fluids equations. For the equation \eqref{cgl}, there are trivial symmetries (see Section \ref{sec:res}) from which we introduce the following renormalization in terms of the amplitude-phase representation  $\psi(x,t) = u(x,t)e^{\imath \theta(x,t)}$,} 
%renormalization corresponding to the symmetries of \eqref{cgl}, 
\begin{equation}\label{eq:intro_dyn}
U(z,\tau) = H(\tau) u\big( \RR(\tau) z + V(\tau), t(\tau)\big), \quad \Theta(z, \tau) = 
%\red{\mu(\tau)} + 
 \theta\big( \RR(\tau) z + V(\tau), t(\tau)\big), 
 \quad 
 t(\tau) = \int_0^\tau H^{p-1}(s) ds,
\end{equation}
where $ \RR(\tau) \in \Rb^{d \times d}$ is a upper triangular matrix, $V(\tau) \in \Rb^d$ and $H(\tau) \in \Rb_+$. Here, $H$ is responsible for time, $V$ for spatial translation. %and $\RR$ for rotation invariant and parabolic scaling. 

The key novelty is that in addition to modulation parameters corresponding to the symmetries, we introduce \textit{extra \JC{anisotropic} modulation parameters}. Instead of applying the same rescaling to $z_i$, we rescale $z_i$ with \textit{different but similar} scalings following the ideas  \cite{hou20242}. 
See also a recent work \cite{hou2024nearly} on the generalized Navier-Stokes equations, in which the author developed a generalized dynamic rescaling formulation by using different rescalings for the $r$ and $z$ directions respectively and a self-similar blowup was observed numerically. 
%See also a recent work \cite{hou2024nearly} on the generalized Navier-Stokes equations, where different rescalings for $r$, $z$ are introduced  in the axissymmetric formulation and  upon varying the space dimension dynamically, the ratio of the two scales converges to a constant as the rescaled time approaches to infinity, recovering a self-similar blowup observed numerically. 
In the case of \eqref{cgl}, we rescale $z_i$ with scaling slightly perturbed from the parabolic scaling. We remark that the choices of different scalings for $z_i$ violate the scaling symmetries.
Yet, in the case of \eqref{cgl}, we will show that the violation is asymptotically small and $\RR(\tau)$ converges to $c(\tau) I_d$ asymptotically for some scalar function $c(\tau)$. Therefore, the above renormalization \eqref{eq:intro_dyn} asymptotically agrees with the classical dynamical rescaling formulation \cite{chen2022stable,chen2025stable}, \cite{chen2021finite, chen2021HL}. %The artificial scalings p
These extra parameters provide us extra $d-1$ degrees of freedom, and we have crucial $1 + d + \f{d(d+1)}{2}$ degrees of freedom in total in choosing the dynamic variables $H(\tau), V(\tau), \RR(\tau)$. 
 %While we can 
  A natural idea to represent the scaling in $z_i$ and capture the rotation symmetries is to choose $\RR(\tau) = D(\tau) Q(\tau)$ with a diagonal matrix $D$ and an orthogonal matrix $Q$. Yet, it is challenging to parametrize a time-dependent orthogonal matrix in $\Rb^{d \times d }$. %To overcome this difficulty, 
  \JC{We overcome this difficulty by using} the upper triangular matrix $\RR(\tau)$ with $\f{d(d+1)}{2}$ parameters. 
  %Instead, we use the upper triangular matrix $\RR(\tau)$ with $\f{d(d+1)}{2}$ parameters. 

%To represent the scaling in $z_i$ and capture the rotation symmetries, we use the upper triangular matrix $\RR(\tau)$ with $\f{d(d+1)}{2}$ parameters. 



To determine these modulation parameters, we impose normalization conditions on $\na^i U(0), i=0,1,2$, so that the perturbation of $U$ vanishes $O(|z|^3)$ near $z=0$ and we can perform weighted energy estimates mentioned above.
Note that the number of (different) equations and that of the degrees of freedom are \textit{exactly} the same.
For \eqref{cgl}, these conditions allow us to completely eliminate the unstable and neutrally stable modes of the linearized operator. See Step 2 in Section \ref{sec:idea} for more details.



\vspace{0.1in}

\noindent \textit{Step 2 (Equations of the profiles and modulation parameters)}: We derive the equations of $F = (U, \Th)$ and matrix (or vectors) 
$\Qc(\tau)$ governing the {modulation parameters} $\RR(\tau), V(\tau), H(\tau)$,
\beq\label{eq:intro_full}
 \pa_{\tau} F = \msN_F(F, \Qc), \quad  \f{d}{d \tau} \Qc = \msN_{\Qc}(F, \Qc) ,
\eeq
where $\msN_F$ is a nonlinear function and $\msN_{\Qc}$ is a matrix. Then the rescaling system is completely determined, and we further construct the approximate steady state $(\bar F, \bar \Qc)$ analytically or numerically. 


\vspace{0.1in}

\noindent \textit{Step 3 (Stability analysis and the log correction):} In general, we \textit{do not} know \textit{a-priori} that the approximate steady state $(\bar F, \bar \Qc)$ is stable in some suitable topology. Nevertheless, if we can establish {stability of} $(\bar F, \bar \Qc)$ following the strategy mentioned above and $H(\tau)^{p-1}$ is integrable, then we can obtain finite time blowup using \eqref{eq:intro_dyn} and the law of blowup will then be prescribed by the normalizing constants. 

For \eqref{cgl}, we will use the energy method with an energy $E$ for the perturbation $F - \bar F$ 
to establish 
\[
\f{d}{d \tau} E \leq - c_1 \cdot E + C \tr(\Qc) + l.o.t., \quad 
\quad  \f{d}{d \tau} \tr(\Qc) \leq  - c_2 \cdot \tr(\Qc)^2 + l.o.t.,
\]
for some $c_1, c_2, C >0$, where $\Qc$  is a positive definite matrix and $l.o.t.$ denotes some terms that are very small.
The second ODE of $\tr(\Qc)$ further implies that $|\tr(\Qc)| \les (1 + \tau)^{-1}$. A further refinement of this algebraic decay in the self-similar time implies a log correction $\log(T-t)$ in the blowup rate. We will elaborate more in Step 2 in Section \ref{sec:idea}. 

\

One can thus hope to combine the above method for a log correction and the framework \cite{chen2022stable,chen2025stable} to problems with numerical steady states, while  spectral analysis heavily hinges on a simple and analytical approximate steady state with explicit (nonlinear heat \cite{merle1997stability}) or at least asymptotical spectral information of the linearized operator (Keller-Segel \cite{collot2022refined}). 
%One can hope to combine the method in this paper for a logarithm correction and the framework \cite{chen2022stable,chen2025stable} with computer-assistance to study potential blowup in 3D incompressible Euler or Navier-Stokes equations (NSE). 
%For example, for 3D incompressible Euler or Navier-Stokes equations (NSE), constructing a smooth (approximate) steady state analytically is challenging and remains an open problem. 
For example, constructing a smooth (approximate) steady state \JC{in the dynamic rescaling equations} analytically for 3D incompressible Euler or Navier-Stokes equations (NSE) is challenging and remains an open problem.
On the other hand, constructing a numerical approximate steady state with computer-assistance is much more feasible. See \cite{chen2022stable,chen2025stable}, \cite{wang2022self}, \cite{wang2025high} for the construction in 3D Euler equations. 
For NSE, self-similar blowup with a perfect self-similar scaling has been ruled out \cite{tsai1998leray}, \cite{sverak1996leray}.
 Yet, one can construct a blowup violating these non-blowup results by adding a log correction in the spatial variable. 
See numerical evidence on the singular behavior of NSE with a potential logarithm correction in the potential blowup by the second author \cite{hou2022potentially}.
%\paragraph{Novelties and main contributions:} 
%\vspace{0.1in}
%\paragraph{\textbf{Difficulties and novelties:} }


\subsection{Ideas of the blowup analysis}\label{sec:idea}


{We first discuss some of difficulties in the study of singularity formation in \eqref{cgl}. Then we follow the generalized dynamic rescaling framework to establish the existence and stability of asymptotically self-similar blowup  solutions to \eqref{cgl} by briefly discussing the strategy and main ideas of our analysis.}



\paragraph{\textbf{Difficulties:}} Compared with \eqref{nlh} or \eqref{nls}, the analysis for the complex Ginzburg-Landau equation \eqref{cgl} has the following additional challenges. 


\vspace{0.1in}
  \textbf{1.} The complex Ginzburg-Landau equation \eqref{cgl} is not of a gradient form, rendering energy estimates hard. To overcome this challenge, we use the amplitude-phase representation \eqref{eq:intro_rep}, \eqref{eq:CGL_intro} to analyze \eqref{cgl}.



    \vspace{0.1in}
  \textbf{2.}  
 %\vio{VT: I don't get to the point here, what is a particular difficulty? It'd be better if you could explain more}  
 We remove the even symmetry assumption of the perturbation required in \cite{hou20242} to recover full stability. {%Removing the 
 Without the even symmetry assumption, we have more potentially unstable modes for the linearized operator. We control these unstable modes using the generalized dynamic rescaling formulation in Step 1 in Section \ref{sec:intro_dyn}.
 }

 \vspace{0.1in}
  \textbf{3.}
  We consider the whole range of the nonlinearity $p > 1$. For the analysis of the phase equation \eqref{eq:theta_intro} and the nonlinearity $u^p$ \eqref{eq:A_intro}, \eqref{eq:theta_intro}, we need to bound the rescaled amplitude $U$ from below, which we establish using the maximal principle and a weighted $L^{\infty}$ estimate. Due to the non-integer power $p$ to control $\na^K(U^p)$ in the $H^K$ estimate, which leads to terms like $ U^{p-K} (\na U)^K$, we need to obtain sharp decay estimates for $\na^i U$. This is done by 
  choosing an almost tight power in the far field of the weight for the weighted $H^k$ energy estimates and using interpolation and embedding inequalities following \cite{chen2024Euler}.  
An additional difficulty comes from the coupling between $u, \th$ in the viscous terms in \eqref{eq:A_intro}, \eqref{eq:theta_intro}. 
We design the top order energy with a special algebraic structure to cancel out the top order terms and show that the viscous terms have a good sign. See Step 3(b) in Section \ref{sec:idea}. 

  

\paragraph{Ideas and strategy:} We briefly discuss the strategy and main ideas of our analysis.

\vspace{0.1in}
%\noindent - \underline{Step 1}(Dynamical rescaling formulation):
\noindent \textit{Step 1 (Dynamical rescaling formulation)}:
We follow Step 1 in Section \ref{sec:intro_dyn} to perform the rescaling \eqref{eq:intro_dyn}.
% From the amplitude-phase representation $\psi(x,t) = u(x,t)e^{\imath \theta(x,t)}$,  we introduce the renormalization corresponding to the symmetries of \eqref{cgl}, 
% \begin{equation}\label{eq:intro_dyn}
% U(z,\tau) = H(\tau) u\big( \RR(\tau) z + V(\tau), t(\tau)\big), \quad \Theta(z, \tau) = 
% %\red{\mu(\tau)} + 
%  \theta\big( \RR(\tau) z + V(\tau), t(\tau)\big), 
%  \quad 
%  t(\tau) = \int_0^\tau H^{p-1}(s) ds,
% \end{equation}
% where $ \RR(\tau) \in \Rb^{d \times d}$ is a upper triangular matrix, $V(\tau) \in \Rb^d$ and $H(\tau) \in \Rb_+$. Here, $H$ is responsible for time, $V$ for space translation, and $\RR$ for rotation invariant and parabolic scaling. See Section \ref{sec:res} for more discussions of the symmetries. In addition, instead of rescaling $z$ according to the parabolic scaling, we rescale $z_i$ differently with scaling close to the parabolic scaling following \cite{hou20242}. This provides us crucial $1 + d + \f{d(d+1)}{2}$ degrees of freedom in choosing the dynamic variables $H(\tau), V(\tau), \RR(\tau)$. 
%See Step 2.
Then, we introduce the following factors governing the evolution of these parameters 
\beq\label{eq:intro_Pv}
 \frac{H_\tau}{H}=c_U, 
 \quad c_U = - \frac{1}{p-1} + c_W, 
 %\f{1}{p-1}, 
 \quad 
 \Mc = e^{- \frac{\tau}2} \RR^{-1},
 \quad \Vc = - \RR^{-1} V_{\tau}, 
 \quad \Pc = \Mc_{\tau} \Mc^{-1}.
\eeq

\vspace{0.1in}

\noindent \textit{Step 2 (Normalization and vanishing conditions)}:
{Let $\bar U$ be the profile defined in \eqref{def:Ubar}}. To determine {the law for the parameter functions} $H(\tau), V(\tau), \RR(\tau)$, we enforce the following normalization conditions on the amplitude $U$:
\beq\label{eq:intro_vanish}
k = 0,1,2, \quad \nabla^k U(0, \tau) = \na^k \bar U(0).  %\quad \pa_\tau \nabla W(0, \tau) = 0, %b\quad  \Phi(0) = 0, \;\; 
\eeq
Since $\na^2 U \in \Rb^{d \times d}$ is symmetric, we have $1 + d + \f{d(d+1)}{2}$ different equations, which match the degrees of freedom of the dynamic variables exactly. 
The above conditions determine the initial {modulation parameters} $H(0), \RR(0), V(0)$ and the leading order system of $c_W, \Pc, \Vc$ \eqref{eq:intro_Pv} 
\beq\label{eq:intro_ODE}
\bal
&c_W = \frac{2(1 - \beta \delta)}{4\flat_*} \textup{tr}(\Qc) + O(\cE_0), 
\quad \Vc = O(\cE_0),\quad \Pc =O( |\Qc| + \cE_0), 
\quad  \textup{where} \quad \Qc = H^{p-1} e^{\tau} \Mc \Mc^T, 
  \\
 %&\Qc_\tau = - \big(\QH + \frac{1}{2}\Qc_d \big)\Qc - \Qc\big(\QH^T + \frac{1}{2}\Qc_d \big) + O(|\Qc| \cE_0), \quad   \textup{where} \quad \Qc = H^{p-1} e^{\tau} \Mc \Mc^T, 
\eal
\eeq
%\red{\begin{align*}
% &c_W = \frac{2(1 - \beta \delta)}{4\flat_*} \textup{tr}(\Qc) + o(|\Qc|),  \quad \textup{where} \quad \Qc = C_W^{p-1} \Mc \Mc^T, \\
%  &\Qc_\tau = - \big(\QH + \frac{1}{2}\Qc_d \big)\Qc - \Qc\big(\QH^T + \frac{1}{2}\Qc_d \big) + o(|\Qc|^2),\\
%  &|\Pc| + |\Vc| = \Oc(|\Qc|), \qquad \hat \mu_\tau = - \frac{\beta(1 + \delta^2)}{2\flat_*} \textup{tr}(\Qc) + o(|\Qc|).
%\end{align*}}
where $\cE_0$ tracks some lower order terms depending on the perturbation $(W, \Phi)$ \eqref{eq:W_Intro}, \eqref{eq:Phi_Intro}  and $\Qc$. 
%depending on some $L^{\infty}$ norm of the perturbation $(W, \Phi)$ and $|\Qc|$ and $\QH, \Qc_d$ are the strictly upper part and diagonal part of $\Qc$.  
The main unknown $\Qc \in \Rb^{d\times d}$ (a positive definite matrix) solves the following ODE %(see Remark \ref{rmk1})
\beq\label{eq:intro_ODE2}
\frac{d}{d\tau} \tr(\Qc) = -\tr(\Qc^2) + O(\cE_0 |\Qc|  )
\leq - \f{1}{d} (\tr(\Qc))^2 + O(\cE_0 |\Qc|  ) .
 %\textup{tr}(\Qc^2), \quad \textup{hence}, \quad \Qc \sim \frac{1}{\tau}\textup{I}_d.
% \frac{d}{d\tau} \textup{tr}(\Qc) \sim \textup{tr}(\Qc^2), \quad \textup{hence}, \quad \Qc \sim \frac{1}{\tau}\textup{I}_d.
\eeq
From \eqref{eq:intro_ODE2}, \eqref{eq:intro_ODE}, \eqref{eq:intro_Pv}, we can control all the modulation parameters. A refined estimate using $\tr(\Qc)$ and $\tr(\Qc^{-1})$ yields $\Qc = \frac{1}{\tau}\textup{I}_d + O(\tau^{-3/2 +})$, together with an asymptotic refinement of the phase yield the asymptotics in Theorem \ref{thm:blp}.  See Section \ref{sec:ode} for deriving \eqref{eq:intro_ODE}, Section \ref{sec:refineasym} for the estimates of $\Qc$ and Proposition \ref{prop:linf} for the refinement of the phase.  

Roughly speaking, imposing \eqref{eq:intro_vanish} for $U$ is equivalent to imposing local orthogonality conditions for the perturbation $W = U - \bar U$ to $1, z_i, z_i z_j, 1 \leq i, j \leq d$. These functions are all the neutrally stable and unstable modes of $L =\textup{Id} - \frac{1}{2}z \cdot \nabla$, 
which behaves similarly to the main linearized operator $\msL_{\bar U}$ in \eqref{eq:W_Intro} {for $|z|$ small}.  We then get a damping in the weighted $L^2$ energy estimate. 


\vspace{0.1in}
\noindent \textit{Step 3 (Stability analysis)}: We linearize $(U, \Th)$ around  the approximate steady state  $(\bar U, \bar \Theta)$ defined in \eqref{def:Ubar} and \eqref{ss-} and obtain the equations for the perturbation $W = U - \bar U, \Phi = \Th - \bar \Th$,
%The linearied equations for the perturbation $W = U - \bar U, \Phi = \Th - \bar \Th$  are given by 
\bseq\label{eq:per_Intro}
\begin{align}
{W}_\tau &= \msL_{\bar U} W +\mathscr{F}_{ U}+\mathscr{N}_U+\mathscr{D}_U ,
\quad 
 \msL_{\bar U} W = \big(-\frac{1}{p-1} + p \bar U^{p-1} - \frac{1}{2}z \cdot \nabla \big)W, \label{eq:W_Intro}\\
\Phi_\tau &=-\frac{1}{2}z \cdot \nabla \Phi+\mathscr{F}_\Theta+\mathscr{N}_\Theta+\mathscr{D}_\Theta, \label{eq:Phi_Intro}
\end{align}
\eseq
%where $\mathscr{F}_{\al}, \mathscr{N}_{\al}, \mathscr{D}_{\al}, \al = U, \Phi$ 
where $\mathscr{F}_U, \mathscr{N}_U, \mathscr{D}_U, \mathscr{F}_\Theta, \mathscr{N}_\Theta, \mathscr{D}_\Theta$ are small residue, nonlinear, and viscous terms \eqref{eq:lin}, and will be treated perturbatively. 
Below, we outline the stability estimates and focus on the linear part and the viscous terms.


% A similar observation for the equation \eqref{eq:Phi_Intro} for $\Phi$, where the leading linear part is governed by $-\frac{1}{2}z \cdot \nabla$ which consists a zero eigenvalue (constant eigenfunction) and a negative spectrum, hence, imposing a vanishing condition for $\Phi$, that is equivalent to a local orthogonality condition for $\Phi$ to this zero mode, hence a decay estimate following from a standard weighted $L^2$ energy-estimate. From these observation, we are able to settle down the linear stability analysis by imposing the appropriate vanishing conditions.



\vspace{0.1in}
%\paragraph{Estimates of the amplitude:}
\textit{(a) Estimates of the $(W, \Phi)$} : $\mathscr{L}_{\bar U}$ to the leading order is the linearized equation for the Riccati equation or the semilinear heat equation. With the vanishing conditions $\na^k W = 0, k=0,1,2$ \eqref{eq:intro_vanish}, we obtain its stability using weighted $H^k$ estimates with singular weights. See 
 \cite{hou20242} in the case of $p=2$ and \cite{chen2024stability}, \cite{chen2021finite,chen2021HL}, \cite{chen2020singularity}. 

The right-hand side of \eqref{eq:per_Intro} only involves $\na \Phi$, which enjoys better stability. We estimate $\na \Phi$ by performing a similarly weighted $H^k$ estimate (starting from $k=1$) on \eqref{eq:Phi_Intro} and exploiting the term $-\frac{1}{2}z \cdot \nabla \Phi$.



%(d) Lower bound of the amplitude: 

%\paragraph{Estimates of the lower bound of the amplitude:}
%Finally, as we mentioned before, 
In the nonlinear estimates  and the estimates of the phase, we need to control $1/U$. We use the maximal principle and a weighted $L^{\infty}$ estimate to obtain a lower bound of $U$. 

%which amounts to a lower bound of the amplitude.  We state our bootstrap assumption on the lower bound of $U$ here, which shows that $U$ is almost comparable with $\bar{U}$, up to a small power. To simplify the notations in the nonlinear estimates and to ensure that $\RR, \Mc$ are invertible \eqref{eq:Pv}, \eqref{per_ansatz}, we impose weak assumptions on the energy $E_i, F_j$ and $\det(\Qc)$



% which we have already demonstrated to be stable, once we impose the vanishing conditions, (in the case of $p=2$) in our previous works \cite{hou20242,chen2024stability,chen2021finite} using a family of singular weight $\rho_k$ for $H^k$ estimates. We can say the same about $\mathscr{F}_U$ and $\mathscr{N}_U$.

% \paragraph{Estimates of the phase:}
% {
% Note that all the terms on the right-hand side of \eqref{realp}, \eqref{imaginep} only involve derivatives of $\Theta$, and we can start our estimate at the $H^1$ level. Then it is not hard to demonstrate linear stability, in a similar spirit as the estimates of the amplitude. We will elaborate on this in Subsection \ref{h1sec}.
% }

\vspace{0.1in}
\textit{(b) Estimates of the viscous terms}: 
%\textbf{(b) Viscous terms}: 
%V1
%For the viscous terms $\mathscr{D}_U$ and $\mathscr{D}_\Theta$ \eqref{real_v}, \eqref{im_v},we note that $\Qc$ is small (see Remark \ref{rmk1}) and will treat them perturbatively. 
For the viscous terms $\mathscr{D}_U, \mathscr{D}_\Theta$ \eqref{eq:vis}, the main difficulty %is that there are coupled terms 
is the coupling between $U$ and $\Theta$. At the top $H^K$ estimate, the highest order derivative terms read 
\begin{align*}
    \na^K \msD_{U} &= \D_{\Qc} \na^K U - \be U \D_{\Qc} \na^K \Th + l.o.t. \coloneqq I_1 + I_2 + l.o.t., \\
\ \na^K \msD_{\Th} & = \be \f{\D_{\Qc} \na^K U}{U} + \D_{\Qc} \na^K \Th + l.o.t.
\coloneqq I_3 + I_4 + l.o.t.,
\end{align*}
where $\D_{\Qc} F$ is a weighted elliptic operator defined in \eqref{eq:Del_Q}. 
%In weighted $H^K$ estimate, 
The terms $I_1, I_4$ lead to damping terms of $\nabla^{K+1}U$ and $\nabla^{K+1}\Theta$ via integration by parts. 
To control $I_2, I_3$, we exploit their cancellation using the energy $J_1$ below 
with some weight $\rho_K$ independent of $U, \Th$ and couple their estimates in $J_2$
\begin{equation}  \label{topcouple}
    J_1 =\int(|\nabla^{K}W|^2+{U}^2|\nabla^{K}\Phi|^2)\rho_K,
      \quad  J_2 = \int ( ( - \be U \D_{\Qc} \na^K \Th) \cdot \na^K U + (\be \f{\D_{\Qc} \na^K U}{U}) \cdot U^2  \na^K \Phi) \rho_K.
    %\quad  J_2 = \int ( I_2\cdot \na^K U + U^2 I_3 \cdot \na^K \Phi) \rho_K
\end{equation} 
 Applying integration by parts, $J_2$ reduces to some lower order terms and we can close the viscous estimates. 
For estimates of intermediate-order terms, we use interpolation inequalities following \cite{chen2024Euler}. 



% For the viscous terms $\mathscr{D}_U$ and $\mathscr{D}_\Theta$ \eqref{real_v}, \eqref{im_v},
% we note that $\Qc$ is small (see Remark \ref{rmk1}) and will treat them perturbatively. 
% The main difficult is that there are coupled terms between $U$ and $\Theta$. At the top $H^K$ estimate, we have 
% %the top order terms in terms of derivatives are given by 
% \[
% \na^K \msD_{U} = - \be U \D_{\Qc} \na^K \Th + \cR_1 = I_1 + \cR_1, 
% \ \na^K \msD_{\Th} = \be \f{\D_{\Th} \na^K U}{U} + \cR_2 = I_2 + \cR_2, 
% \]
% where $\cR_i$ denotes terms with a good sign in the energy estimates or involving less derivatives, and $\D_{\Qc} F$ is a weighted elliptic operator defined in \eqref{eq:Del_Q}. 
% %In weighted $H^K$ estimate, the terms $I_1, I_4$ lead to damping terms of $\nabla^{K+1}U$ and $\nabla^{K+1}\Theta$ via integration by parts. 
% To control $I_1, I_2$, we exploit their cancellation using the energy $J_1$ below and its associated coupled estimate in $J_2$
% \begin{equation}  \label{topcouple}
%     J_1 =\int(|\nabla^{K}W|^2+{U}^2|\nabla^{K}\Phi|^2)\rho_K,
%     \quad  J_2 = \int ( I_2\cdot \na^K U + U^2 I_3 \cdot \na^K \Phi) \rho_K
% \end{equation} 
% for some weight $\rho_K$ independent of $U, \Th$. Applying integration by parts, $J_2$ reduces to some lower order terms and we can close the viscous estimates. 
% For estimates of intermediate orders term, we use interpolation inequalities following \cite{chen2024Euler}. 



% We notice that $Q$ is small; see Remark \ref{rmk1}. For the leading order terms in the $H^K$ estimates, we will have damping of terms of order $\nabla^{K+1}U$ and $\nabla^{K+1}\Theta$ via integration by parts. Therefore we can close the viscous estimates in all the intermediate order terms except for terms involving $K+2$ derivatives as $\nabla^{K}(-\beta U\Delta_\Qc \Theta)$ in $\mathscr{D}_U$ and $\nabla^{K}(\beta \frac{\Delta_\Qc  U}{U})$ in $\mathscr{D}_\Theta$. This observation motivates us to consider the energy 
% \begin{equation}
%     \label{topcouple}\int(|\nabla^{K}W|^2+{U}^2|\nabla^{K}\Phi|^2)\rho_K
% \end{equation} 
% to cancel out the {top-order} terms and close the viscous estimates in the leading order estimates. This is a particular challenge only when $\beta$ is nonzero. For estimates of intermediate orders, we use interpolation inequalities. %for simplicity. 
% We will elaborate on the computations in Subsection \ref{hksec}.

\vspace{0.1in}
\textit{(c) {Choosing the weights}}: 
% V1 
% To extract damping in the energy estimates, we design various weights.
% The choices of the weights \eqref{wg:rho} for $W$ are very similar to the case of the semilinear heat equation \cite{hou20242}. They are singular near $z=0$ for the lower order energy estimates and regular for the top order energy estimates so that the viscous terms will have a good sign. See also \cite{chen2021finite,chen2021HL,chen2020singularity}. In addition, we need to choose an almost optimal rate at $\infty$ to obtain sharp decay estimate of the amplitude using interpolation and embedding following \cite{chen2024Euler}.
To extract damping in the energy estimates, we need to design various suitable weights. The weights \eqref{wg:rho} for $W$ are very similar to those of the semilinear heat equation \cite{hou20242}. They are singular near $z=0$ for the lower order energy estimates and regular for the top order energy estimates so that the viscous terms will have a good sign.  In addition, we choose an almost optimal rate at the infinity for these weights to obtain a sharp decay estimate for $(W, \Phi)$ using interpolation and embedding following \cite{chen2024Euler}.


\vspace{0.1in}
\paragraph{{Organization of the chapter:}}

The rest of the  chapter is organized as follows. In Section \ref{sec:dyn}, we introduce the generalized dynamic rescaling formulation using the symmetries of \eqref{cgl} and derive the ODEs governing the modulation parameters. Section \ref{sec:stab} is devoted to the stability analysis of the profile. 
%We refine the estimates to obtain the asymptotics of the blowup rate in Section \ref{sec:refineasym}, and prove Theorem \ref{thm:blp} and Corollary \ref{cor:stab} in Section \ref{sec:thm_proof}.
In Section \ref{sec:refineasym}, we establish the asymptotics of the blowup rate. 
In Section \ref{sec:thm_proof}, %e combine all the estimates to 
we prove Theorem \ref{thm:blp} and Theorem \ref{cor:stab}. 




\vspace{0.1in}
\paragraph{\textbf{Notations:}} {
We use $\imath$ to denote the imaginary number, $\bar{f}$ to denote approximate profiles for the variable $f$, e.g.,$\bar U$, rather than conjugates, and  $(\cdot,\cdot)$ to denote the inner product on $\mathbb{R}^d$: 
$(f,g)=\int_{\mathbb{R}^d}f{g}$. For a weight $\rho$, we denote $\|f\|_{\rho}=(|f|^2,\rho)^{1/2}$. 
}
For matrix notations, we use $\mathrm{tr}(R)$ to denote the trace of a matrix $R$, $\mathbf{T}^u(R)$ to denote the upper triangular part of $R$; namely $(\mathbf{T}^u(R))_{ij}=R_{ij} \one_{ i\leq j}$. %
We use $\delta_{ij} = \one_{i = j}$ to denote the Kronecker delta function, 
and $| \mathbf{T}| := (\sum_{i} \TT_i^2)^{1/2}$ with summation over all entries $\TT_i$ to denote the tensor norm of a tensor $\mathbf{T}$, e.g., higher-order derivatives $\nabla^k f$. We use $C$ to denote an absolute constant only dependent on the constants $p,\beta,\delta,\gamma$ and the dimension $d$, which may vary from line to line. $C(\mu)$ denotes a constant depending on $\mu$. We denote $A=O(B)$ or $A\lesssim B$ if there exists an absolute constant $C>0$, such that $|A|\leq CB$, and denote $A\approx B$ if $A \les B$ and $B \les A$. Furthermore, we denote
\beq\label{eq:intro_nota}
\Lam = z \cdot \na , \quad \langle z\rangle=\sqrt{1+|z|^2}\,.
\eeq

%\quad  \bar \mu = \frac{\delta}{p-1}\tau, 
\noindent \textbf{Parameters and special functions}: We introduce 
 \begin{equation}\label{ss-}
    \bar{\Theta} =  \frac{\delta}{p-1}\tau + \delta\log\bar{U} \,, \quad     c_p=\frac{(p-1)^2}{4\flat_*}, \quad \s = -\f{2}{p-1}.
    \end{equation}
We choose the weights for the $H^k$ estimates as follows:
\begin{equation}
\label{wg:rho}
    \begin{aligned}
        &\rho_k=|z|^{-6+\epsilon-d+2k}+c_0|z|^{- 2 \s -\epsilon-d+2k}, \   0\leq k\leq\frac{d+5}{2}\,, \quad 
    {\rho}_k=1+c_1|z|^{ - 2 \s  -\epsilon-d+2k}, \  \frac{d+5}{2}<k \, , \\
& \mathring{\rho}_k=|z|^{2k-1-d}\,,  \ 0< k\leq\frac{d}{2}\,, \qquad \qquad \ \mathring{\rho}_k=1+|z|^{2k-1-d}\, , \ \frac{d}{2}< k<K\,, \ \qquad \qquad \mathring{\rho}_K=U^2\rho_K\,,
\end{aligned}
\end{equation}
where we determine the constants in the following order: 
\begin{align}
K & =2d+4+2\left \lceil\frac{p+1}{\min\{p-1,c_p\}}\right \rceil\,, \label{K} \\
  \epsilon &{ =\min\{\frac{p-1}{5(p+3)(K+p)},\frac{4}{5(p + 3)(K+p)}\},}
 \quad \e_2 = \f{ (p-1) \e}{4} .
   \label{eps}
 \end{align}
For $c_0, c_1$ used in \eqref{wg:rho}, we determine $c_0$ via \eqref{c0} and $c_1$ via \eqref{defered}. {Note that $c_0, c_1$ only depends on $K, \e, p, \d$. Hence, they are considered as fixed constants throughout the  chapter.}



\section{Generalized dynamical rescaling formulation}\label{sec:dyn}

In this section, we introduce a generalized dynamic rescaling formulation and decompose the complex Ginzburg-Landau equation into the equation of the phase and the amplitude. We will consider a linearization around the approximate profiles and {choose the modulation parameters} based on the vanishing conditions. Finally, we will estimate the ODE of the {modulation parameters}. 
%and provide heuristics of the proof of Theorem \ref{thm:blp}.

\subsection{Symmetries and renormalization}\label{sec:res}


We exploit the following symmetries of equation \eqref{cgl} to study stability for general perturbation, which will motivate our choice of rescaling. 
If $\psi(x,t)$ solves \eqref{cgl}, all of the following also solves \eqref{cgl}:
\begin{enumerate}
    \item Phase shift: $\psi_{a}(x,t)\coloneqq e^{
\imath a}\psi(x,t)$, for $a\in\mathbb{R}$.
  \item Parabolic scaling for $\gamma=0$: $\psi^{l }(x,t)\coloneqq l^{1/(p-1)}\psi( l^{1/2} x, l t)$, for $ l \in\mathbb{R}$. 
    % \item Parabolic scaling for $\gamma=0$: $\psi^{\Gamma}(x,t)\coloneqq\Gamma^{1/(p-1)}\psi(\Gamma^{1/2} x,\Gamma t)$, for $\Gamma\in\mathbb{R}$. 
    \item Translation: $\psi_{{b}}(x,t)\coloneqq \psi(x-{b},t)$, for ${b}\in\mathbb{R}^d$.
    \item Rotation: $\psi^{R}(x,t)\coloneqq \psi(Rx,t)$, for  orthogonal matrix $RR^T=I_d$.
\end{enumerate}
We use the symmetry groups of the parabolic scaling via a rescale in amplitude, of the translation via a shift in space, and of the rotation via a rotation and rescaling in the spatial variable parametrized by an upper triangular matrix. {In sum, we can exploit modulation with $1+d+\frac{(d+1)d}{2}$ degree of freedom.} 
The phase shift invariance corresponding to a constant addition in $\Theta$ is taken care of in \eqref{est:limitmu} and \eqref{eq:thm_estb}. It is irrelevant to the dynamical modulation of stability since the right-hand sides of \eqref{eq:A_intro} and \eqref{eq:theta_intro} only involve the derivatives of $\Theta$. We remark that the modulation of symmetries due to Galilean transformations, including the rotation symmetry, has been used successfully to obtain shock formation in compressible Euler equations with fine characterization \cite{buckmaster2023formation}.  
%cite the compressible Euler paper from Vicol et.al
Below, we will use a general upper triangle matrix, which simplifies the parametrization of the time-dependent orthogonal matrix.


For solution $\psi$ to \eqref{cgl}, we consider the amplitude-phase form $\psi(x,t)= u(x,t)e^{\imath\theta(x,t)}$, where $u(t): x \in \Rb^d \to \Rb_+$ and $\theta(t): x \in \Rb^d \to \mathbb{R}$. For the amplitude $u$ and phase $\psi$, we introduce the generalized dynamic rescaling formulation
\beq\label{eq:dyn_scal0}
U(z,\tau)=H(\tau) u\big( \RR(\tau)z+V(\tau) ,t(\tau)\big)\,,\quad \Theta(z,\tau)= 
%\red{\mu(\tau)} + 
 \theta\big(\RR(\tau)z+V(\tau),t(\tau)\big)\,,
\eeq
where the main unknown parameter functions are $ \RR \in \Cc^1 \big([\tau_0, +\infty), \Rb^{d\times d}\big)$ a non degenerate upper triangular matrix, $V \in \Cc^1 \big([\tau_0, +\infty), \Rb^{d}\big)$ and $H$ is given by
% the renormalization
\beq\label{eq:dyn_scal1}
{H= H(0)\exp{(\int_0^\tau {c}_U(s) ds)}\,, \quad t(\tau) =\int_0^\tau H^{p-1}(s) ds\,.}
\eeq
In a compact form, we have
\begin{equation}\label{drf-nd}
    {U(z,\tau) e^{\imath \Theta(z,\tau) }=H(\tau) (u e^{\imath \theta})\big( \RR(\tau)z+V(\tau),t(\tau)\big), \quad \psi = u e^{\imath\theta}. }
\end{equation}
We decompose the solution into the approximate steady states \eqref{ss-},  with perturbations $W, \Phi$: 
     \begin{equation}\label{per_ansatz}
        U=\bar{U}+W\,,\quad \Theta=\bar{\Theta}+\Phi\,,\quad c_U= -\frac{1}{p-1} + c_W\,,\quad H =
e^{- \f{\tau}{p-1}  } C_W.
    \end{equation}
If $\RR(\tau)$ is a scalar factor and $V = 0$, \eqref{drf-nd} reduces to the standard dynamic rescaling formulation, see e.g., \cite{chen2021HL,chen2021finite,chen2019finite2}. If 
$\RR(\tau)$ is a diagonal matrix and $V = 0$, it reduces to a formulation similar to \cite{hou20242}. We will show that $\RR$ is close to some identity matrix and $V$ is some lower order term. 

We first compute the spatial derivative
$$\nabla U= H  e^{-\imath\Theta}\nabla \psi \RR-\imath H \psi e^{-\imath\Theta}\nabla\Theta \,,$$$$\nabla^2 U=H  e^{-\imath\Theta} \RR^T\nabla^2 \psi \RR-\imath H   e^{-\imath\Theta}(\nabla \psi \RR\nabla\Theta^T+\nabla \Theta \RR^T\nabla \psi^T)-H \psi e^{-\imath\Theta}\nabla\Theta\nabla\Theta^T-\imath H \psi e^{-\imath\Theta}\nabla^2\Theta\,.$$
We then write from \eqref{cgl} the equation for $U$,
\begin{equation*}\begin{aligned}
    %\label{drf-gl}
    {U}_\tau&=-\imath\Theta_\tau U+{c}_U {U}-( \f{1}{2} z+\Pc z+\Vc)\cdot\nabla U-\imath U ( \f{1}{2} z+ \Pc z+\Vc)\cdot\nabla\Theta +(1+\imath\delta){U}^{p}-{C}_U^{p-1}\gamma U\\& \quad +(1+\imath\beta)(\Delta_\Qc U+2\imath\langle\nabla U,\nabla\Theta\rangle_\Qc -U\langle\nabla \Theta,\nabla\Theta\rangle_\Qc+\imath U\Delta_\Qc \Theta)\,,
    \end{aligned}\end{equation*}
where $\Pc, \Vc$ are related to the matrix $\RR$ as  
 \beq \label{eq:Pv} 
 \Mc = e^{-\tau/2} \RR^{-1}, \quad
     %\RR = e^{-\tau /2} \Mc^{-1}\,, \ 
\Vc =- \RR^{-1}{V}{_\tau}, \quad  \Pc={\Mc}{_\tau} \Mc^{-1} , \quad \Qc \coloneqq C_W^{p-1} \Mc \Mc^T\,,
\eeq
and we use the notation 
\begin{equation}\label{eq:Del_Q}
\Delta_\Qc f\coloneqq\text{tr}(\Qc\nabla^2f)\,,\quad \langle x,y\rangle_\Qc \coloneqq x^T\Qc y\,,\, \quad \forall x,y\in\mathbb{R}^d.
\end{equation}
Taking the real and imaginary parts we arrive at the following equations for $U$ and $\Theta$:
    \begin{align}
    \label{real}{U}_\tau & ={c}_U {U}-( \f{1}{2} z+ \Pc z+ \Vc)\cdot\nabla U+{U}^{p}-{C}_U^{p-1}\gamma U+\mathscr{D}_U\,,\\
\label{imagine}\Theta_\tau & =-( \f{1}{2} z+\Pc z+\Vc)\cdot\nabla\Theta+\delta{U}^{p-1}+\mathscr{D}_\Theta\,, 
\end{align}
where $\Ds_U$ and $\Ds_\Theta$ consist of the viscous terms and the nonlinear quadratic term we define  the viscous terms as follows: 
\bseq\label{eq:vis}
\begin{align}
    \label{real_v}
    \mathscr{D}_U & =\Delta_\Qc U-2\beta\langle\nabla U,\nabla\Theta\rangle_\Qc -U\langle\nabla \Theta,\nabla\Theta\rangle_\Qc -\beta U\Delta_\Qc \Theta\,, \\
    \label{im_v}
\mathscr{D}_\Theta & = \beta\frac{\Delta_\Qc  U}{U}+2\frac{\langle\nabla U,\nabla\Theta\rangle_\Qc }{U}-\beta \langle\nabla \Theta,\nabla\Theta\rangle_\Qc +\Delta_\Qc \Theta\,.
\end{align}
\eseq

We will show that the diffusion and $\Qc, c_W, \Vc, \Pc, H^{p-1}$ are lower order terms. See Remark \ref{rmk1}. Dropping these terms and setting $\pa_{\tau} U = 0$, we obtain the leading order parts of \eqref{real} and \eqref{imagine}:
$$
 -\frac{1}{p-1}\bar{U}- \f{1}{2} \Lambda\bar{U}+\bar{U}^p=0\,,\quad \bar{\Theta}_\tau =- \f{1}{2} \Lambda\bar{\Theta} +\delta{\bar{U}}^{p-1}\,,
 $$
 whose solution are given by the approximate profiles  $(\bar U, \bar \Th)$ defined in \eqref{def:Ubar}, \eqref{ss-}.

  \subsection{Initial rescaling and normalization conditions}\label{sec:nom}
    %As was discussed in the previous subsections, 
    We will choose some proper initial modulation parameters $H(0), V(0), \Mc(0)$ and the dynamic variables {$c_W, \Vc, \Pc$} such that the perturbation $W$ vanishes to the third order. We denote the following constants 
    \begin{equation} \label{eq:dU_cons}
       {\kappa_0=\bar{U}(0)=(p-1)^{-\frac{1}{p-1}}\,,\quad \kappa_2=\partial_{1}^2\bar{U}(0)=-\frac{2c_p\kappa_0}{(p-1)^2}\,,\quad \kappa_4={\partial_{1}^4\bar{U}(0)}=\frac{12p c^2_p\kappa_0}{(p-1)^4}\,.}
\end{equation}

Given initial data $(u, \th)$ \eqref{drf-nd} satisfying \eqref{eq:ass_init}, we first define $\Mc_0, V_0, H(0), \Th_0, U_0$ using \eqref{eq:init_res}. Then we determine other initial rescalings and initial data using  
\[
V(0) = V_0, \quad \Mc(0) = \Mc_0, 
\quad \RR(0) = \Mc_0^{-1}, 
\quad \Th(z, 0) = \Th_0(z), \quad 
   U(z, 0) = U_0(z)  .% \quad 
 %=  \theta( \Mc(0)^{-1} z + V(0), 0) .
\]
We impose the following normalization conditions in time as
  $$
    U(0,\tau)=\bar{U}(0)=\kappa_0\,,\quad \nabla U(0,\tau)=\nabla \bar{U}(0)=0\,,\quad \nabla^2 U(0,\tau)=\nabla^2 \bar{U}(0)=\kappa_2 I_d\,. 
  $$
From \eqref{eq:init_res2}, the above holds for $\tau =0$. By the ansatz \eqref{drf-nd}, it reduces a dynamical condition in time $$\partial_\tau \nabla^k U(0,\tau)=0\,,\quad k=0,1,2\,,$$ which we can use \eqref{real} to simplify as
\beq\label{ode:v}
\bal
    & {c}_U+\kappa_0^{p-1}-H^{p-1}\gamma +\frac{\mathscr{D}_U(0)}{\kappa_0} =0 , \\
           & \kappa_2\Vc =\nabla \mathscr{D}_U(0), \\
     & ({c}_U- 1 +p\kappa_0^{p-1}-H^{p-1}\gamma)\delta_{ij}-(\Pc_{ij}+\Pc_{ji})+\frac{\partial_{ij}\mathscr{D}_U(0)-\Vc\cdot\nabla\partial_{ij}U(0)}{\kappa_2} =0\,,
      \eal
\eeq
for any indices $i,j$. Notice that the inverse of an upper-triangular matrix is still upper-triangular, and as a consequence $\Pc={\Mc}_\tau \Mc^{-1}$ is upper-triangular. We can further simplify the equations for $c_U$ and $\Pc$ by the ansatz \eqref{per_ansatz} as follows:
\begin{equation}
    \label{cq}c_W=-\frac{\mathscr{D}_U(0)}{\kappa_0} + H^{p-1}\gamma\,,\quad (1+\delta_{ij})\Pc_{ij}=-\frac{\mathscr{D}_U(0)}{\kappa_0}\delta_{ij}+\frac{\partial_{ij}\mathscr{D}_U(0)-\Vc\cdot\nabla\partial_{ij}W(0)}{\kappa_2}\,,\end{equation}
    for any $i
    \leq j$. We will estimate equations \eqref{cq} and \eqref{ode:v} in the next subsection.

   \subsection{ODE for the {modulation parameters}}\label{sec:ode}
   In this subsection, we simplify equations \eqref{cq} and \eqref{ode:v} to derive a leading order ODE. 
   {
     We will treat the perturbations $W, \Phi$ as low-order terms and estimate them in Section \ref{sec:stab}. Denote
  %We will treat the perturbations as low-order terms and we will show that it is very small in the next section. We define some norm $\Ga$ and lower order terms $\cE_0$
 \begin{equation}
\label{ee}
%\mathcal{E}
\Ga
=\max_{0\leq k\leq 5, 1\leq l\leq 5}(\|\nabla^k W\|_{\infty},\|\nabla^l\Phi\|_{\infty})\, ,
\quad \cE_0 = |\Qc| (\Ga + \Ga^4) + H^{p-1}. 
 \end{equation} 
Clearly, we have $ \Ga^i |Q| \les \cE_0, 1 \leq i \leq 4 $. We use $\cE_0$ to track some lower order terms.
     %We define some norm and lower order term 
%  We will treat the perturbations as low-order terms in the sense that we define 
%  \begin{equation}
% \label{ee}
% %\mathcal{E}
% \Ga
% =\max_{0\leq k\leq 5, 0< l\leq 5}(\|\nabla^k W\|_{\infty},\|\nabla^l\Phi\|_{\infty})\,,
%  \end{equation} and we will show that it is very small in the next section. 
 }
 \begin{lemma}\label{lem1}
     We have the following estimates for the modulation parameters:
     \begin{equation}
         \label{norm_con}
         %c_W=\frac{2(1-\beta\delta)}{(p-1)^2}c_p\textup{tr}(\Qc)+l.o.t._0\,,\quad v=l.o.t._0\,,
           c_W=\frac{2(1-\beta\delta)}{(p-1)^2}c_p\textup{tr}(\Qc)+ \Oc(\cE_0)\,,\quad \Vc = \Oc( \cE_0)\,,
     \end{equation}
and
     \begin{equation}
         \label{norm_p}
         \Pc= \Oc(|\Qc|(1+ \Ga^4)+H^{p-1})\,, \quad
         {\Qc}_\tau=-(\Qc_u+\frac{1}{2}\Qc_d)\Qc-\Qc(\Qc_u^T+\frac{1}{2}\Qc_d)+ \Oc(\Ec_0|\Qc|),
         %{\Qc}_\tau=-\Qc^2+ O(|\Qc| \cE_0).  %|\Qc|l.o.t._0\,.
     \end{equation}
     where $\Qc_u, \Qc_d$ are the strictly upper part and diagonal part of $\Qc$. 
     
     
    %\vio{VT: @Roy @Jiajie: could you please add an estimate for $\Vc$ and an  equation for $\pa_\tau \hat \mu$? }
    
 \end{lemma}
 {
    \begin{remark}\label{rmk1}
    Formally to the leading order when we take the trace, we have 
    $$
    \textup{tr}(\Qc)_\tau\approx-\textup{tr}(\Qc^2)\,,\quad\textup{tr}(\Qc^{-1})_\tau\approx-d\,.
    $$ 
    Recall that $\Qc=C_W^{p-1}\Mc\Mc^T$ is positive. %We can solve the leading order ODE explicitly using eigenvalue decomposition and we have  
    We can estimate $\tr(\Qc), \tr(\Qc^{-1})$ and obtain 
    $\Qc\approx \tau^{-1} \textup{I}_d$. Therefore $\Qc, c_W, \Vc, \Pc$ are indeed small and the viscous terms can be treated perturbatively. We will make this heuristic rigorous by choosing $H(0)=C_W(0)$ small; see Section \ref{sec:boot}. Although we allow anisotropicity in the initial data, the profile will converge to a isotropic one, i.e. $\Qc$ will converge to a diagonal matrix.
    \end{remark}
    }
 % \begin{remark}
 %        If we ignore the $l.o.t.$ terms in \eqref{norm_p}, we can diagonalize the ODE by eigenvalue decomposition. This corresponds to performing a coordinate change for the initial data.
 % \end{remark}
 \begin{proof}
 Notice that by \eqref{real_v}, we have 
\begin{equation}
\label{du_exp}\mathscr{D}_U=\text{tr}(\Qc S_1)\,,\quad S_1=\nabla^2 U-2\beta\nabla U\nabla\Theta^T-U\nabla \Theta\nabla\Theta^T-\beta U\nabla^2\Theta\,.
\end{equation} We can simplify \eqref{cq} by an asymptotic expansion of $S_1$ near the origin up to the second order.
\[
\bal
%$$
\bar{U} & =\kappa_0+\frac{\kappa_2}{2}|z|^2+\frac{\kappa_4}{24}|z|^4+O(|z|^6)\,,\quad \nabla\bar{\Theta}=\frac{\delta}{\bar{U}}{\nabla\bar{U}}=\delta\frac{\kappa_2}{\kappa_0}z+O(|z|^3)\,, \\
%$$
%$$
\nabla^2\bar{U}& =\kappa_2I_d+\frac{\kappa_4}{6}|z|^2I_d+\frac{\kappa_4}{3}zz^T+O(|z|^4)\,, \\
%$$
%$$
\nabla^2\bar{\Theta} & =\frac{\delta}{\bar{U}}{\nabla^2\bar{U}}-\frac{\delta}{\bar{U}^2}{\nabla\bar{U}\nabla\bar{U}^T}=\delta(\frac{\kappa_2}{\kappa_0}I_d+(\frac{\kappa_4}{6\kappa_0}-\frac{\kappa_2^2}{2\kappa_0^2})(|z|^2I_d+2zz^T))+O(|z|^4)\,. 
\eal
\]
{Decomposing $U = \bar U + W, \Th = \bar \Th + \Phi$ \eqref{per_ansatz} and using $\Ga$ \eqref{ee} to control the perturbation $W, \Phi$, we expand}
%Therefore we expand 
$$\begin{aligned}
    S_1&=\kappa_2(1-\beta\delta)I_d+(\frac{\kappa_4}{3}+(-2\beta-\delta)\delta\frac{\kappa_2^2}{\kappa_0}-\beta\delta(\frac{\kappa_4}{3}-\frac{\kappa_2^2}{\kappa_0}))zz^T\\&+(\frac{\kappa_4}{6}-\beta\delta(\frac{\kappa_2^2}{2\kappa_0}+\frac{\kappa_4}{6}-\frac{\kappa_2^2}{2\kappa_0}))|z|^2I_d+O(|z|^4+  \Ga + \Ga^3 )\,.
\end{aligned}$$
{The estimates for $\na^i S_1$ are similar. We have chosen $\Ga$ \eqref{ee} to control $\na^k W, \na^{k+1} \Phi$ with high enough order $k$. In particular, for an error term $I$ in $S_1$ bounded by $|z|^4 + \Ga + \Ga^3$, e.g.,$(U - \bar U) \na^2 (\Theta - \bar \Theta)$, we have 
\[
 |\na^i I| \les |z|^{4-i} + \Ga + \Ga^3, \ i = 1, 2.
\]  
Since we only need the expression at $z=0$, the error term $O(|z|^j), j \geq 1$ vanishes in the following derivations. For this reason, we do not track the constant associated with $|z|^j$. 
}


As a consequence, we have the expressions for derivatives of $\mathscr{D}_U$ as 
\[
\bal
 \mathscr{D}_U(0) & = \kappa_2(1-\beta\delta)\text{tr}(\Qc)+ {O(\cE_0)}
\,,\quad \nabla \mathscr{D}_U(0)= { O(\cE_0)} \,, \\
 \partial_{ij}\mathscr{D}_U(0) & = \delta_{ij}(1-\beta\delta)\frac{\kappa_4}{3}\text{tr}(\Qc)+2((1-\beta\delta)\frac{\kappa_4}{3}-(\beta+\delta)\delta\frac{\kappa_2^2}{\kappa_0})\Qc_{ij}+ { O(\cE_0) }\, .
\eal
\]
%where we use $l.o.t.$ to denote terms of $O(|Q|( \Ga+ \Ga^3))$\,. \JC{l.o.t. here means vanishing order?}

We plug the estimates into \eqref{cq} and \eqref{ode:v} and get 
\[
\bal
  & c_W=-\frac{\kappa_2}{\kappa_0}(1-\beta\delta)\text{tr}(\Qc)+ {O(\cE_0)}\,,\quad v={ O(\cE_0) }\,, \\
%$$ 
%$$
   & \Pc=\mathbf{T}^u\Big[\frac{\kappa_4}{6\kappa_2}(1-\beta\delta)\textup{tr}(\Qc)I_d+((1-\beta\delta)\frac{\kappa_4}{3\kappa_2}-\big(\beta+\delta)\delta\frac{\kappa_2}{\kappa_0}\big)\big(2\Qc-\textup{diag}(\Qc)\big)\Big] \\
   & \qquad \qquad -\mathbf{T}^u(\frac{\kappa_2}{2\kappa_0}(1-\beta\delta)\textup{tr}(\Qc)I_d)+ {O(\cE_0)} \,,
%$$
\eal
\]
where we recall that $\mathbf{T}^u$ is the upper-triangular part of the matrix.   Notice that by \eqref{eq:dU_cons}, we have the relationship $$\frac{\kappa_4}{6\kappa_2}=p\frac{\kappa_2}{2\kappa_0}\,,\quad(1-\beta\delta)\frac{\kappa_4}{3\kappa_2}-(\beta+\delta)\delta\frac{\kappa_2}{\kappa_0}=(p-\delta^2-\beta\delta(1+p))\frac{\kappa_2}{\kappa_0}=-\frac{1}{2}\,.$$
Therefore, we collect 
\begin{equation}
    \label{P} \Pc+\frac{p-1}{2}c_WI_d=-\mathbf{T}^u(\Qc-\frac{1}{2}\textup{diag}(\Qc))+ O(\cE_0)\,.
\end{equation}

Recall that ${\Mc}_\tau=\Pc \Mc$ by definition, and we can compute 
$$
{\Qc}_\tau=(p-1)c_W \Qc+C_W^{p-1}(\Pc \Mc \Mc^T+\Mc \Mc^T\Pc^T)=\big(\Pc+\frac{p-1}{2}c_WI_d\big)\Qc+\Qc\big(\Pc+\frac{p-1}{2}c_WI_d\big)^T\,.
$$
If we decompose $Q$ into the strictly upper, lower, and diagonal parts as $\Qc=\Qc_u+\Qc_u^T+\Qc_d$, then we can simplify 
$$
{\Qc}_\tau=-(\Qc_u+\frac{1}{2}\Qc_d)\Qc-\Qc(\Qc_u^T+\frac{1}{2}\Qc_d)+ \cE_\Qc  \Qc + \Qc \cE_\Qc ^T,
\quad \cE_\Qc  = O(\cE_0).
%O ( \cE_0|Q| )
%=-\Qc^2+ O( \cE_0 |\Qc| )\,,
$$ 
and we conclude the proof of the lemma.
\end{proof}
\begin{remark}
{
In the above ODE of $\Qc$, we get $-1$ for the coefficient of $\Qc^2$ since we have 
normalized the profile \eqref{ss-}. The factor $p-\delta^2-\beta\delta(1+p) > 0$ (corresponding to the subcritical case) appears in the constant $c_p$. 
    %For the subcritical case $p-\delta^2-\beta\delta(1+p) > 0$, we have normalized the profile to get a $-1$ prefactor in the above ODE of $Q$.}
    For the critical case $$p-\delta^2-\beta\delta(1+p)=0\,,$$ without such a normalization}, 
 we can see that if we do something similar, the coefficient %in front of the quadratic term 
of $\Qc^2$ will be zero.  We could keep track of the next order terms of size $\Ga$ to derive a system  of size $|\Qc|^3$. This can potentially help us establish a result similar to \cite{DNZmems23} but we do not pursue it here.
\end{remark}




 \section{Stability analysis and finite time blowup}\label{sec:stab}

{
 In this section, we perform stability analysis and establish nonlinear stability of the perturbation around the approximate steady state following the ideas and strategy outlined in 
 Section \ref{sec:idea}. 

We linearize \eqref{real} and \eqref{imagine} around the approximate profile as in ansatz \eqref{per_ansatz}  and obtain the equations of the perturbations as follows:
\begin{equation}
    \label{realp}{W}_\tau=\mathscr{L}_{\bar{U}}W+\mathscr{F}_U+\mathscr{N}_U+\mathscr{D}_U\,,\end{equation}     
    \begin{equation}
\label{imaginep}\Phi_\tau =- \f{1}{2} \Lambda \Phi+\mathscr{F}_\Theta+\mathscr{N}_\Theta+\mathscr{D}_\Theta\,,\end{equation}
{where we recall from \eqref{real_v} and \eqref{im_v} the definition of $\Ds_U$ and $\Ds_\Theta$, and define the linear, residue, and nonlinear parts respectively as}
\beq\label{eq:lin}
\bal
 \mathscr{L}_{\bar{U}}W & =c_{\bar{U}} W- \f{1}{2} \Lambda W+p\bar{U}^{p-1}W\,,
 \quad \Lambda=z\cdot\nabla , \\
 \mathscr{F}_U & =c_W U-(\Pc z+\Vc)\cdot\nabla U-{C}_U^{p-1}\gamma U\,,\quad\mathscr{N}_U=(\bar{U}+W)^p-\bar{U}^p-p\bar{U}^{p-1}W\,,  \\
\mathscr{F}_\Theta &=-(\Pc z+\Vc)\cdot\nabla {\Theta}\,,\quad\mathscr{N}_\Theta=\delta((\bar{U}+W)^{p-1}-\bar{U}^{p-1})\,. 
\eal
\eeq
%Recall the definition of the viscous terms $\mathscr{D}_U$, $\mathscr{D}_\Theta$ in \eqref{real_v}, \eqref{im_v}, and that they 
We will group the terms by integrability:  $\mathscr{L}_U$ and $\mathscr{N}_U$ vanish to the third order at the origin. Recall that by Lemma \ref{lem1} and Remark \ref{rmk1}, we know that $\Qc, c_W, \Vc, \Pc$ are small. The viscous terms $\mathscr{D}_U$, $\mathscr{D}_\Theta$ are small of order $|\Qc|$ with a typical size of $1/\tau$. 
%$1/\tau$, which is the typical size of $|Q|$; see Remark \ref{rmk1}.
Also obviously $H=C_We^{-\tau/(p-1)}$ is small. 


 We define the weighted $H^k$ energy  as follows 
\begin{equation}\label{norm:Ek}
\bal
    & E_k^2=(|\nabla^k W|^2,\rho_k)\,,\quad 0\leq k\leq K\,, \quad 
    %\quad || f ||_{\cX^k}:= E_k + E_0= || \na^k f ||_{\rho_k} + || f||_{\rho_0} , \\
    %& 
    F_k^2=(|\nabla^k \Phi|^2,\mathring{\rho}_k)\,,\quad 0< k\leq K\,.
    %\quad E_{\Qc} = \tr(\Qc). 
    \eal
\end{equation}
Our goal is to prove the following nonlinear stability results.
  \begin{theorem}\label{thm:stab}
  Denote $E_{\Qc} = \tr(\Qc)$. There exists $ 0< E_* < 1$ sufficiently small and $\mu_3 > 0$, such that for any initial perturbation satisfying 
  \beq\label{eq:thm_stab_ass}
U \rho > 2 C_b, \quad E(0) < E_*, \quad E_{\Qc}  < E_*, \quad H^{p-1}(0) < E_*,
  \eeq
we have the following estimates for all $\tau > 0$
\beq\label{eq:non_stab}
\bal
 & E_\Qc (\tau)  \leq  \min( 2 E_\Qc (0), 4 d / \tau ), \quad U(\tau)  > C_b\bar{U}^{1+\epsilon_2} , 
 \quad H^{p-1}(\tau) < H^{p-1}(0) e^{-\tau / 2} , \\
& E(\tau) \leq e^{-\lam \tau/2} (E(0) + \mu_3 H^{p-1}(0) +\mu_3  E_\Qc (0)) + \mu_3  \min(E_\Qc (0), 1 / \tau).
\eal
\eeq
{Here $C_b, H(\tau), E(\tau),\e_2$ are defined in \eqref{eq:boot_U}, \eqref{eq:dyn_scal1}, \eqref{eneq}, and \eqref{eps}.}
Moreover, the bootstrap assumptions \ref{asss}, \ref{ass:lower}, \ref{ass:refine} (introduced below) hold for all $\tau > 0$. 
  \end{theorem}


Note that the parameters $\mu_1, \mu_2$ will be introduced in the proof in Section \ref{sec:boot}.






We impose the following weak bootstrap assumptions for nonlinear estimates. To control $1/U$, which will appears in the estimate of $\msN_{U}, \msN_{\Th}$, we impose a lower bound on $U$, which is almost comparable with $\bar{U}$, up to a small power. To simplify the notations in the nonlinear estimates and to ensure that $\RR, \Mc$ are invertible \eqref{eq:Pv}, \eqref{per_ansatz}, we impose the following weak assumptions on the energy $E_i, F_j$ and $\det(\Qc)$.
\begin{assumption}
\label{asss}
Let  $\e_2$ be defined in \eqref{eps}. We impose the following bootstrap assumptions
\begin{align}
    & U\geq C_b\bar{U}^{1+\epsilon_2} , \quad  C_b = \min_{|z|\leq 1} \bar U^{-\e_2}(z) / 4 > 0, \label{eq:boot_U}  \\
&  \max(E_K, E_0, F_K, F_1) \leq 1 ,
\quad \quad \det(\Qc) > 0.\label{eq:boot_EE}
\end{align}
\end{assumption}
%We will perform an $L^\infty$ estimate of $ \frac{U}{\bar{U}^{1+\epsilon_2}}$ in Subsection \ref{sec:linfty} to close the bootstrap, inspired by \cite{chen2021HL}.


Below, we will first establish some functional inequalities in Section \ref{sec:ineq}. 
We will start with the $L^2$ analysis of perturbations $W$ and $\nabla\Phi$ in Sections \ref{l2sec}, \ref{h1sec}, and then build higher-order estimates in Section \ref{hksec}. 
We obtain a lower bound of the amplitude $U$ via the maximal principle in Section \ref{sec:linfty}, 
inspired by \cite{chen2021HL}.
Then we close the nonlinear estimates and prove Theorem \ref{thm:stab} via a bootstrap argument in Section \ref{sec:boot}.

}


% In this section, we perform a stability analysis of the perturbation around the approximate steady state, with normalization constants prescribed in \eqref{cq} and \eqref{ode:v}. We will start with the $L^2$ analysis of perturbations $W$ and $\nabla\Phi$, and then build higher-order estimates. Moreover, we obtain a lower bound of the amplitude $U$ via maximal principle. Then we close the nonlinear estimates via a bootstrap argument.


%   \subsection{Strategy of the stability analysis}
%    \label{subsec key}
%     In this subsection, we sketch the high-level ideas of our stability analysis, and then we will conclude our stability analysis in the subsequent three subsections.
    
% We linearize \eqref{real} and \eqref{imagine} around the approximate profile as in ansatz \eqref{per_ansatz}  and obtain the equations of the perturbations as follows:

% \begin{equation}
%     \label{realp}{W}_\tau=\mathscr{L}_{\bar{U}}W+\mathscr{F}_U+\mathscr{N}_U+\mathscr{D}_U\,,\end{equation}     
%     \begin{equation}
% \label{imaginep}\Phi_\tau =- \f{1}{2} \Lambda \Phi+\mathscr{F}_\Theta+\mathscr{N}_\Theta+\mathscr{D}_\Theta\,,\end{equation}
% \blu{where we recall from \eqref{real_v} and \eqref{im_v} the definition of $\Ds_U$ and $\Ds_\Theta$, and define the linear, residue, and nonlinear parts respectively as}
% \beq\label{eq:lin}
% \bal
%  \mathscr{L}_{\bar{U}}W & =c_{\bar{U}} W- \f{1}{2} \Lambda W+p\bar{U}^{p-1}W\,,
%  \quad \Lambda=z\cdot\nabla , \\
%  \mathscr{F}_U & =c_W U-(\Pc z+\Vc)\cdot\nabla U-{C}_U^{p-1}\gamma U\,,\quad\mathscr{N}_U=(\bar{U}+W)^p-\bar{U}^p-p\bar{U}^{p-1}W\,,  \\
% \mathscr{F}_\Theta &=-(\Pc z+\Vc)\cdot\nabla {\Theta}\,,\quad\mathscr{N}_\Theta=\delta((\bar{U}+W)^{p-1}-\bar{U}^{p-1})\,. 
% \eal
% \eeq
% Recall the definition of the viscous terms $\mathscr{D}_U$, $\mathscr{D}_\Theta$ in \eqref{real_v}, \eqref{im_v}, and that they are small of order $1/\tau$, which is the typical size of $|Q|$; see Remark \ref{rmk1}.
% We are grouping terms by integrability:  $\mathscr{L}_U$ and $\mathscr{N}_U$ vanish to the third order at the origin. Recall that by Lemma \ref{lem1} and Remark \ref{rmk1}, we know that $\Qc, c_W, \Vc, \Pc$ are small. Also obviously $H=C_We^{-\tau/(p-1)}$ is small. 


% \paragraph{Estimates of the amplitude:}
% $\mathscr{L}_U$ to the leading order is just the linearized operator of the nonlinear heat equation, or rather the Riccati equation, which we have already demonstrated to be stable, once we impose the vanishing conditions, (in the case of $p=2$) in our previous works \cite{hou20242,chen2024stability,chen2021finite} using a family of singular weight $\rho_k$ for $H^k$ estimates. We can say the same about $\mathscr{F}_U$ and $\mathscr{N}_U$.

% \paragraph{Estimates of the phase:}
% {
% Note that all the terms on the right-hand side of \eqref{realp}, \eqref{imaginep} only involve derivatives of $\Theta$, and we can start our estimate at the $H^1$ level. Then it is not hard to demonstrate linear stability, in a similar spirit as the estimates of the amplitude. We will elaborate on this in Subsection \ref{h1sec}.
% }
%We can not ensure the perturbation of the phase to vanish at the origin, therefore we can not impose a singular weight to extract any damping at the $L^2$ level. Fortunately, all the terms on the right-hand side only involve derivatives of $\Theta$, and we can start our estimate at the $H^1$ level. Then it is not hard to demonstrate linear stability, in a similar spirit as the estimates of the amplitude. We will elaborate on this in Subsection \ref{h1sec}.

% \paragraph{Estimates of the viscous terms and coupling of estimates:}
% For the viscous terms $\mathscr{D}_U$ and $\mathscr{D}_\Theta$ \eqref{real_v}, \eqref{im_v},  there are coupled terms involving both $U$ and $\Theta$. %with top order terms given by 
% We notice that $Q$ is small; see Remark \ref{rmk1}. For the leading order terms in the $H^K$ estimates, we will have damping of terms of order $\nabla^{K+1}U$ and $\nabla^{K+1}\Theta$ via integration by parts. Therefore we can close the viscous estimates in all the intermediate order terms except for terms involving $K+2$ derivatives as $\nabla^{K}(-\beta U\Delta_\Qc \Theta)$ in $\mathscr{D}_U$ and $\nabla^{K}(\beta \frac{\Delta_\Qc  U}{U})$ in $\mathscr{D}_\Theta$. This observation motivates us to consider the energy \begin{equation}
%     \label{topcouple}\int(|\nabla^{K}W|^2+{U}^2|\nabla^{K}\Phi|^2)\rho_K
% \end{equation} to cancel out the {top-order} terms and close the viscous estimates in the leading order estimates. This is a particular challenge only when $\beta$ is nonzero. For estimates of intermediate orders, we use interpolation inequalities. %for simplicity. 
% We will elaborate on the computations in Subsection \ref{hksec}.





% \paragraph{Choices of weights and specification of low-order terms:} 
% The choices of the weights \eqref{wg:rho} for the amplitude are very similar to the case of the semilinear heat equation \cite{hou20242}. 
% {In addition, we need to choose an almost optimal rate at $\infty$ to obtain sharp decay estimate of the amplitude using interpolation and embedding following \cite{chen2024Euler}.} We choose the weights to make sure that they will produce linear damping in the amplitude, that they can close the $L^\infty$ estimates, that the residues are integrable, and that the viscous estimate will have a good sign at the leading order. 
%We define the weighted $H^k$ norms as 

% \begin{equation}\label{norm:Ek}
% \bal
%     & E_k^2=(|\nabla^k W|^2,\rho_k)\,,\quad 0\leq k\leq K\,, \quad 
%     F_k^2=(|\nabla^k \Phi|^2,\mathring{\rho}_k)\,,\quad 0< k\leq K\,.
%     \eal
% \end{equation}

% In addition, we introduce the following norms 
% \beq\label{norm:Hk}
% || f ||_{\dot \cH^k} := || \na^k f g_k^{1/2} ||_{L^2}, \quad 
%  || f ||_{\cH^k} := || f ||_{\dot \cH^k}  + || f ||_{\dot \cH^0}, \quad 
%  g_k = \la z \ra^{ - 2 \s - \e - d + 2k} .
% \eeq
% By definition of $\rho_k$ \eqref{wg:rho}, we have 
% \beq\label{eq:norm_comp}
% g_k \les \rho_k, \quad 
% || f ||_{\dot \cH^k} \les  E_k, 
% \quad  || f ||_{ \cH^k} \les E_0 + E_k.
% \eeq
% We define the low-order terms $\cE_1$, $\cE_2$ that we later show to be small: 
% \beq\label{eq:lot}
% \bal
% \cE_1 & :=   |Q|+H^{p-1}+ \sum_{ i \leq K - 1} E_i + \sum_{ 1\leq j \leq  K-1}  F_j 
% + ( F_K+F_1+E_K+E_0)^2,  \\
% \cE_2  & := |Q|+H^{p-1} .
% \eal
% \eeq
% We treat $\cE_1$  as lower order term since it either contains nonlinear terms or energy with order lower than $E_K, F_K$. Note that $\cE_2$ is the low-order term of order $P$ in Lemma \ref{lem1} after we asuming \eqref{eq:boot_EE}, which implies $\Ga \les 1$. See \eqref{eq:EE_embed}.



% \paragraph{Estimates of the lower bound of the amplitude:}
% Finally, as we mentioned before, in the nonlinear estimates and the estimates of the phase, we need to control $1/U$, which amounts to a lower bound of the amplitude.  We state our bootstrap assumption on the lower bound of $U$ here, which shows that $U$ is almost comparable with $\bar{U}$, up to a small power. To simplify the notations in the nonlinear estimates and to ensure that $\RR, \Mc$ are invertible \eqref{eq:Pv}, \eqref{per_ansatz}, we impose weak assumptions on the energy $E_i, F_j$ and $\det(\Qc)$






% \begin{assumption}
% \label{asss}
% Let  $\e_2$ be defined in \eqref{eps}. We impose the following bootstrap assumptions
% \begin{align}
%     & U\geq C_b\bar{U}^{1+\epsilon_2} , \quad  C_b = \min_{|z|\leq 1} \bar U^{-\e_2}(z) / 4 > 0, \label{eq:boot_U}  \\
% &  \max(E_K, E_0, F_K, F_1) \leq 1 ,
% \quad \quad \det(\Qc) > 0, \label{eq:boot_EE}
% \end{align}
% \end{assumption}


% We will perform an $L^\infty$ estimate of $ \frac{U}{\bar{U}^{1+\epsilon_2}}$ in Subsection \ref{sec:linfty} to close the bootstrap, inspired by \cite{chen2021HL}.



\subsection{Functional inequalities}\label{sec:ineq}


In this section, we establish a few functional inequalities, which will be used to 
estimate the decay of the solution and close the nonlinear estimates. We introduce the following norms 
\beq\label{norm:Hk}
|| f ||_{\dot \cH^k} := || \na^k f g_k^{1/2} ||_{L^2}, \quad 
 || f ||_{\cH^k} := || f ||_{\dot \cH^k}  + || f ||_{\dot \cH^0}, \quad 
 g_k = \la z \ra^{ - 2 \s - \e - d + 2k} .
\eeq
By definition of $\rho_k$ \eqref{wg:rho} and \eqref{norm:Ek} for $E_k$, we have 
\beq\label{eq:norm_comp}
g_k \les \rho_k, \quad 
|| f ||_{\dot \cH^k} \les  E_k, 
\quad  || f ||_{ \cH^k} \les E_0 + E_k.
\eeq
We define the low-order terms $\cE_1$, $\cE_2$ that we later show to be small: 
\beq\label{eq:lot}
\bal
\cE_1 & :=   |\Qc|+H^{p-1}+ \sum_{ i \leq K - 1} E_i + \sum_{ 1\leq j \leq  K-1}  F_j 
+ ( F_K+F_1+E_K+E_0)^2,  \\
\cE_2  & := |\Qc |+H^{p-1} .
\eal
\eeq
We treat $\cE_1$  as a lower order term since it either contains nonlinear terms or energy with order lower than $E_K, F_K$. Note that $\cE_2$ is the low-order term of order $P$ in Lemma \ref{lem1} by asuming \eqref{eq:boot_EE}, which implies $\Ga \les 1$. See \eqref{eq:EE_embed}.



Following Lemma C.4 in \cite{chen2024Euler}, we have the following weighted interpolation and embedding inequalities.


\begin{proposition}[Interpolation]
    \label{prop:inter}
    Let $\s = - \f{2}{p-1}$ and $\e$ be the constants defined in \eqref{eq:dU_cons}, \eqref{eps}. For any $\mu>0$, there exists a constant $C(\mu)$, such that the following interpolation  inequalities hold:    
%     \[
%     \bal
%         E_k & \leq \mu E_K+C(\mu)E_0\,,\quad \forall 0\leq k<K\,,  \\
%     F_k & \leq \mu F_K+C(\mu)F_1\,,\quad \forall 1\leq k<K\,,  \\
%     \|\langle z\rangle^{l+\frac{2}{p-1}-\frac{\epsilon}{2}}\nabla^l W\|_{\infty} & \leq \mu E_K+C(\mu)E_0\,,\quad \forall 0\leq l\leq K/2\,, \\
% \|\langle z\rangle^{l-1/2}\nabla^l\Phi\|_{\infty} & \leq \mu F_K+C(\mu)F_1\,,\quad \forall 1\leq l\leq K/2\,. 
% \eal
% \]
\begin{subequations}\label{eq:inte}
\begin{align}
    %\bal
        E_k &  \leq \mu E_l+C(\mu)E_0\,,\quad \forall 0\leq k< l \leq K\,, \label{eq:inte:1}  \\
     F_k &  \leq \mu F_l+ C( \mu)F_1\,,\quad \forall 1\leq k<l \leq K\,,  \label{eq:inte:2}  \\
     || f  ||_{\dot \cH^k} & \leq \mu || f||_{\dot \cH^l} + C(\mu) || f ||_{\cH^0} , \quad \forall 0\leq k< l \leq K .     \label{eq:inte:Hk}  
\end{align}
\end{subequations}
Moreover, we have the following embedding 
\bseq\label{eq:embed_linf}
\begin{align}
     |\nabla^l W| & \les  \la z \ra^{-l +\s + \e/ 2} \min( E_{l+d} , || W||_{\cH^{l+d}} )   , \ 
\forall 0\leq l\leq K - d \ \label{eq:inte:3} , \\
     %&   \|\langle z\rangle^{l+\frac{2}{p-1}-\frac{\epsilon}{2}}\nabla^l W\|_{\infty}  \les 
     %   E_{l + d} \,,\quad \forall 0\les l\leq K - d \,, \label{eq:inte:3} , \\
 | \nabla^l\Phi | & \les   \langle z\rangle^{-l + 1/2} F_{l + d}  ,\quad \forall 1\leq l\leq K - d-1\, \label{eq:inte:4}  . 
 \end{align}
 \eseq
%     \|\langle z\rangle^{l+\frac{2}{p-1}-\frac{\epsilon}{2}}\nabla^l W\|_{\infty} & \leq \mu E_K+
%     C( \mu)E_0\,,\quad \forall 0\leq l\leq K/2\,, \label{eq:inte:3}  \\
% \|\langle z\rangle^{l-1/2}\nabla^l\Phi\|_{\infty} & \leq \mu F_K+C(  \mu)F_1\,,\quad \forall 1\leq l\leq K/2\, \label{eq:inte:4}  
%\eal



% As a result, we have the following nested property 
% \beq\label{eq:nested}
%  || f ||_{\cH^k} \les_l || f||_{\cH^l},  \quad 
%  \quad  || f ||_{\cX^k} \les_l || f||_{\cX^l}, 
% \eeq
As a result, for $k < l$, we have the following product rule for $i\leq n, j \leq m$ with $ i+ d \leq n$, or $j + d \leq m$,
\beq\label{eq:prod}
|| \na^i F \na^j G g_{i+j}^{1/2} ||_{L^2} 
\les || F ||_{\cH^{n}} || G ||_{\cH^m} .
\eeq


Finally, assuming \eqref{eq:boot_EE}, for $0\leq i\leq K, 1 \leq j \leq K$ and $\Ga$ defined in \eqref{ee}, we have 
\beq\label{eq:EE_embed}
E_i \les 1, \quad F_j \les 1, \quad  \Ga \les 1.
\eeq

% and the following for $2 d \leq l \leq K+1$
% \beq\label{eq:prod2}
%   || f g ||_{\cH^{l}} \les || f||_{\cH^l} || g ||_{\cH^l}
%   \les || f||_{\cX^l} || g ||_{\cH^l}.
% \eeq





%     $$E_k\leq \mu E_K+C(\mu)E_0\,,\quad \forall 0\leq k<K\,,$$
%     $$F_k\leq \mu F_K+C(\mu)F_1\,,\quad \forall 1\leq k<K\,,$$
%     $$\|\langle z\rangle^{l+\frac{2}{p-1}-\frac{\epsilon}{2}}\nabla^l W\|_{\infty}\leq \mu E_K+C(\mu)E_0\,,\quad \forall 0\leq l\leq K/2\,,$$
% $$\|\langle z\rangle^{l-1/2}\nabla^l\Phi\|_{\infty}\leq \mu F_K+C(\mu)F_1\,,\quad \forall 1\leq l\leq K/2\,.$$
\end{proposition}
{Since $K$ \eqref{K} is absolute, $l, k\leq K$, and the parameters $c_0, c_1$ in the weights \eqref{wg:rho} and norms depend on absolute constants $K, \e$ \eqref{eps}, we only need to track the constants related to $\mu$.}

\begin{proof}





\textbf{(a) Interpolation inequalities.}
    %To prove the first two inequalities of the proposition, 
To prove \eqref{eq:inte}, we use integration by parts. For \eqref{eq:inte:1}, we compute for $K>k>0$ that
    $$E_k^2=-\sum_i\int(\partial^2_i\nabla^{k-1}W\cdot\nabla^{k-1}W\rho_k+\partial_i\nabla^{k-1}W\cdot\nabla^{k-1}W\partial_i\rho_k)\,.$$
    Notice that the weights \eqref{wg:rho} satisfy 
    $$
    \rho_k^2\lesssim  \rho_{k+1}\rho_{k-1}\,,\quad(\partial_i\rho_k)^2\lesssim \rho_k\rho_{k-1}\,.
    $$
    Combined with a Cauchy-Schwarz inequality, we obtain  
    $$E_k^2\lesssim  E_{k-1}(E_{k}+E_{k+1})\,.
    $$
    {Since $\e$ only depends on $K$ \eqref{eps},}  by a weighted AM-GM inequality {($ab\leq \nu a^2+1/(4\nu)b^2$)}, for any $\mu>0$, we have 
    $$E_k^2\leq C(\mu)E^2_{k-1}+\mu E^2_{k+1}\,.
    $$
    From here, to conclude the first inequality, since $\mu>0$ is arbitrary, we only need to that show it holds for $k= l-1$, which we can combine the above estimates for $k = 1, 2, .., l-1$ to establish.
    %use induction on $K$ to prove.

    The proof of \eqref{eq:inte:Hk} follows from the same argument.

    For the second inequality \eqref{eq:inte:2}, we can repeat the same procedure to conclude, provided that the weights $\mathring{\rho}_k$ satisfy the same inequalities for $K>k>1$ \eqref{wg:rho}:
    $$\mathring{\rho}_k^2\lesssim  \mathring{\rho}_{k+1}\mathring{\rho}_{k-1}\,,\quad(\partial_i\mathring{\rho}_k)^2\lesssim  \mathring{\rho}_k\mathring{\rho}_{k-1}\,.$$
    When $k+1< K$, this is obvious. For $k=K-1$, we only need to show  
    $$
    \langle z\rangle^{2K-1-d}\lesssim\mathring{\rho}_{K}\approx U^2
        \langle z\rangle^{-2 \s+2K-\epsilon-d}\,,
    %\langle z\rangle^{\frac{4}{p-1}+2K-\epsilon-d}\,,
    $$
    which is true, since by the choice of $\epsilon, \e_2$ \eqref{eps} and the bootstrap Assumption \ref{asss} we have 
    $$
    U\geq C_b\bar{U}^{1+\epsilon_2}\approx \la z \ra^{\s - \e/2} , \quad
    %\langle z\rangle^{-\frac{2+2\epsilon}{p-1}}\,,
    2  \e < 1.
    %\quad \frac{4\epsilon}{p-1}+\epsilon<1\,.
    $$
    
\noindent{\textbf{(b) Embedding \eqref{eq:embed_linf}.}
 To prove the $L^\infty$ estimates \eqref{eq:embed_linf},  one can proceed as in \cite{hou20242} and invoke the weighted Morrey-type inequality. Below, we present a simpler proof. By a density argument, we can assume that $W \in C_c^{\infty}$.  
%We fix $y$ and estimate $\na^i f (y)$. 
Without loss of generality, we fix $z  \in \Rb^d$ with $z_i \geq 0$ and estimate $\na^l W (z)$. 
Consider the region $\Om(z) = \{ y  \in \Rb^d, y_i \geq z_i \}$. We have $|y| \geq |z|$ for any $y \in \Om(z)$. Denote $\d = - 2 \s - \epsilon - d > -d $ \eqref{eps}.
%$\d =  - \kp_1 - d$. 
We have 
\[
\bal
 |\na^l W(Z) | \les_l  \int_{\Om(z)} | \pa_1 \pa_2 .. \pa_d \na^l W (y) | d y
& \les_l || \la y \ra^{ l + d + \d / 2}  \na^{l + d} W ||_{L^2}
 \B( \int_{|y| \geq |z|} \la y \ra^{ - 2 l  -  2 d - \d } d y \B)^{1/2} . \\
 \eal
\]
For $ 0 \leq l \leq K - d - 1$, using $\rho_{ l+ d} \gtr \la y \ra^{ 2 (l+d) + \d}$ \eqref{wg:rho},
$-2 l - d - \d - 1 < -1$, and the first inequality \eqref{eq:inte:1} with $k = l + d < K$, for any $\mu > 0$, we further obtain 
\[
 |\na^l W(y) | \les_K E_{l+d}
 (\int_{ R \geq |y|}  \la R \ra^{-2 l - 2 d - \d } R^{d-1} d R)^{1/2}
\les_K % (\mu E_K + C(\mu) E_0) 
E_{l + d}
 \la y \ra^{- l - (d + \d) /2 } .
\]
%where the integral converges since $-2 l - d - \d - 1 < -1$.
Rearranging the power on both sides, we prove \eqref{eq:inte:3}.

%in the above argument
The proof of \eqref{eq:inte:4} with $ 1 \leq l \leq K- d - 1$ is similar by replacing $W$ by $\na \Phi$  
in the above argument 
%follows a similar argument
and using $\mathring \rho_{ l+ d} \gtr \la y \ra^{ 2 (l+d) + \d_2} $  for $ \d_2 = -d - 1$ 
\eqref{wg:rho} and $ - 2l - d - \d_2 - 1 = - 2 l< -1$ for $l \geq 1$. 
%By definition of $K$ \eqref{K}, we have $ K - d- 1 \geq K / 2 $. We complete the proof of \eqref{eq:inte:3}, \eqref{eq:inte:4}.
}

\noindent \textbf{(c) Other inequalities.}
%The inequalities \eqref{eq:nested} follows from the definition of $\cX^k, \cH^k$ \eqref{norm:Ek}, \eqref{norm:Hk}, and \eqref{eq:inte:1}, \eqref{eq:inte:3}. 
For \eqref{eq:prod}, without loss of generality, we assume that $i+ d \leq n$. Using $g_{i+j}^{1/2} \les \la z \ra^i g_j^{1/2}$, $\s + \f{\e}{2} <0$ \eqref{eq:inte:Hk}, we prove 
\[ 
 || \na^i F \na^j G g_{i+j}^{1/2} ||_{L^2}
 \les || F||_{\cH^{i+d}} || \na^j G g_j^{1/2}||_{L^2}
 \les  || F||_{\cH^{n}} || G||_{\cH^m}.
\]
The inequalities \eqref{eq:EE_embed} follow from \eqref{eq:inte:1}, \eqref{eq:inte:2} and the assumption \eqref{eq:boot_EE}.
%Inequality \eqref{eq:prod2} follows from the Lebiniz rule and the fact that for $i+j = l\geq 2d$, we have $\min(i, j) + d \leq l/2 + d \leq l$.
\end{proof}




{

%for the lower bound
Combining Assumption \ref{asss} and the decay estimates \eqref{eq:inte:3}, \eqref{eq:inte:4}, we have the following estimates.

\begin{corollary}\label{cor:decay}

Denote $W = \bar U - U$. Under the Assumption \ref{asss}, for any $\al \in [0, 1]$ and any $q \in \Rb$ we have 
\beq\label{eq:U_decay}
\bal
  \la z \ra^{ \s - \e / 2} & \les U \les \la z \ra^{\s + \e / 2}, \\
   |(\bar U + \al W)(z)|^q & \les C(|q|) \la z \ra^{ \s q +|\e q| / 2 } , \\
   || \bar U + \al W ||_{\cH^K}, || U ||_{\cH^K} & \les 1 , 
  %(1 + E_{K} + E_0)^{ \max(q, 0)}
  \eal
\eeq
where $\s, \e$ are defined in \eqref{eq:dU_cons}. As a result, 
for $i+j \leq K$, we have the following estimates for the weights
%Furthermore, for $i+j \leq K$,  the weights $\rho_i, \mr{ \rho_i}$ satisfy 
\beq\label{eq:comp_wg}
\bal
& \mr \rho_i  \les \rho_i \la z \ra^{\s + \e/2-1/2},  i\leq K-1,\quad 
\mr \rho_K \les \rho_K \la z \ra^{\s + \e/2},  \\
& \rho_{i+j} \les \rho_i \la z \ra^{2j}, \quad \mr \rho_{i+j} \les \mr \rho_i
 \la z \ra^{2j} .
 \eal
\eeq

\end{corollary}

\begin{proof}

\textbf{(a) Estimate of $U$.} By definition of $\e_2$ \eqref{eps}, we get $- \f{2}{p-1}( 1 +  \e_2)  = - \f{2}{p - 1} -  \f{\e}{2} $. Thus, under Assumption \ref{asss}, we yield 
\[
 U \gtr \bar U^{1 + \e_2} \gtr \la z \ra^{- \f{2}{p-1} - \f{\e}{2} } .
\]

% For the upper bound, using \eqref{eq:inte:3} and triangle inequality, we obtain 
% \[
%  U \les |\bar U| + |W| \les \la z \ra^{\s + \e/2} .
% \]

Since $\bar U + \al W = \bar U + \al( U - \bar U) 
= \al U + (1- \al) \bar U$, which is between $U, \bar U$, and $\bar U, U > 0$, using \eqref{eq:inte:3}, $K > d$ \eqref{K} and the above estimate, we prove
\[
\bal
% |(\bar U + \al W)|^q & \les (\bar U + U)^q \les (1 + E_K + E_0)^q  \la z \ra^{ ( \bar \al  + \e/2) q  } = (1 + E_K + E_0)^q  \la z \ra^{\bar \al  q + | \e q| / 2 } , 
% \ q > 0, \\
% |(\bar U + \al W)|^{-1} & \les \min(\bar U, U )^q \les \la z \ra^{ \bar \al q  - \e q / 2}
% =  ,
% \ q < 0.
|(\bar U + \al W)| & \les \bar U + U \les (1 + E_{K} + E_0)  \la z \ra^{  \s + \e/2  } ,\quad
|(\bar U + \al W)|^{-1}  \les \min(\bar U, U )^{-1} \les \la z \ra^{ -\s  + \e / 2}. 
\eal
\]

The first estimate with $\al = 1$ implies the upper bound for $U$ in \eqref{eq:U_decay}. Raising the above estimates to $|q|$-th power proves the second estimate in \eqref{eq:U_decay}. 

For the last estimate in \eqref{eq:U_decay}, using triangle inequality, $|\na^i \bar U |
\les \la z \ra^{\s -i }$, and \eqref{eq:norm_comp}, we prove 
\[
 || \bar U + \al W ||_{\cH^K}
 +  || \bar U +  W ||_{\cH^K}
\les || \bar U ||_{\cH^K} + || W ||_{\cH^K} 
\les 1 + E_0 + E_K \les 1.
\]
%the proof. 
\textbf{(b) Estimate of weights.}  We consider \eqref{eq:comp_wg}. Using $U  \les \la z \ra^{\s + \e/2}$, clearly, we have 
\[
\bal
& |z| \leq 1: \  \mr \rho_i \les \rho_i \les \rho_i \la z \ra^{ 2 \s + \e - 1} , \\ %|z| \leq 1,    \\
& |z| \geq 1: \ \mr \rho_i \les |z|^{2k-1-d}  \les \rho_i \la z \ra^{ 2 \s + \e-1} ,  i \leq K-1,
\quad \mr \rho_K \les U^2 \rho_K 
\les \rho_K \la z \ra^{ 2 \e + \e}.
\eal
\]
For $(f, \tau) = (\rho, - 2 \s - \e )$ or $( \mr \rho,  -1)$ and $i+j < K$, from the definition of $ f_i$ \eqref{wg:rho}, we have
\[
\bal
 f_{i+j} \les f_i \les f_i \la z \ra^{2j}, \quad |z| \leq 1,
f_{i+j} \approx |z|^{2 i + 2 j + \tau - d} 
\les |z|^{2i + \tau - d} \la z \ra^{2j} \les f_i \la z \ra^{2j}, |z| \geq 1.
 \eal
\]
For $i+j=K$, the above estimate still holds for $f = \rho$. For $ \mr \rho_i$ and $\mr \rho_K$, using $ U \les \la z \ra^{\s + \e/2}$, we obtain 
\[
\mr \rho_K \les \la z \ra^{2 \s + \e  } \rho_K
\les \la z \ra^{2K - 1 - d}
= \la z \ra^{2i-1 - d} \la z \ra^{2j} 
%\les \la z \ra^{2 \s + \e } \rho_i \la z \ra^{2 j}
\les \mr \rho_i \la z \ra^{2 j}.
\]
We complete the proof of \eqref{eq:comp_wg}.
\end{proof}




\begin{proposition}\label{prop:Hk}


Suppose that \eqref{eq:boot_EE} holds true. For $ 0 \leq k \leq K, j_1 + j_2\leq k$ and any $\al \in [0, 1]$, denote 
\[
V = \bar U + \al W , \quad I_{(j_1, j_2)} =  \na^{j_1} W_1 \cdot \na^{ j_2} W_2 \na^{k-j_1-j_2} V^{p-2}.
\]
 We have the following product estimates 
%\begin{subequations}
\beq\label{eq:Hk_est1}  
|| I_{(j_1, j_2 )} ||_{g_k}  \les || W_1 ||_{ \cH^{ \max{ (j_1, K-1)} } } || W_2 ||_{ \cH^{\max(j_2, K-1)} } , %(1 + E_0 + E_K)^{(p+K+2)} ,
\eeq
and 
\begin{subequations}
\begin{align}
  || W_1 W_2 V^{p-2} ||_{\cH^K} & \les ( || W_1 ||_{\cH^{K-1}} || W_2 ||_{\cH^K} 
  +  || W_1 ||_{\cH^{K}} || W_2 ||_{\cH^{K-1}} )  , \label{eq:Hk_est2_Hk} 
  %(1 + E_0 + E_K)^{(p+K+2)}
   \\
 ||W_1 W_2 V^{p-2} ||_{\rho_0} 
& \les || W_2 ||_{\rho_0} || W_1 ||_{\cH^d} 
\label{eq:Hk_est2_L2} . 
%(1 + E_0 + E_k)^{(p+d+2)} 
\end{align}
\end{subequations}

%For $l+m =k \leq K$, we have
Moreover, we have 
%\beq\label{eq:Hk_estU}
\begin{align}
    || \la z \ra^{\s + \e/2}  \na^{l +1} U \na^{m}( U^{-1}) ||_{g_k} & \les || U ||_{\cH^{\max(l+1, m , k)}}, %(1 + E_0 + E_K)^{K},
       \quad l + m = k \leq K , \label{eq:Hk_estU} \\
       | \na^{l +1} U \cdot \na^{m}( U^{-1}) | 
       & \les \la z \ra^{-l-m}  , \quad l , m \leq K-1 - d, 
       %(1 + E_0 + E_K)^K
       \label{eq:Hk_estU_linf}
 \end{align}
%\eeq
\end{proposition}

\begin{proof}
A direct computation yields
\beq\label{eq:Hk_est_pf1}
\bal
I_{j_1, j_2}
 \leq \sum_{2 \leq q \leq k+2,} \sum_{ \sum_{l=1}^q j_l = k, j_l \geq 0} I_{\vec j, q}, \quad 
 I_{\vec j, q} = |V|^{p-q}  \cdot |\na^{j_1} W_1 | |\na^{j_2} W_2|  \prod_{l=3}^q  |\na^{j_l} V| .
 \eal
\eeq {Here $\vec j$ stands for the tuple $(j_1,j_2,\cdots,j_l)$.}
For a fixed $(j, q)$, we denote 
\[
% J_1 = \na^{j_1} W_1, \quad J_2 = \na^{j_2} W_2,
% \quad J_l = \na^{j_l} V, \quad l\geq 3,
% \quad i = \arg\max_{l\leq q} j_l.
J_1 =  W_1, \quad J_2 =  W_2,
\quad J_l =  V, \quad l\geq 3,
\quad i = \arg\max_{l\leq q} j_l.
\]
If there are more than one index $a$ with $ j_a =  \arg\max_{l\leq q} j_l$, we just pick one of them.
% Using \eqref{eq:inte:3} in Proposition \ref{prop:inter} and Corollary \ref{cor:decay}, we obtain 
% \[
%  |I_{\vec j, q}| 
%  \les 
% \]
%Except for at most one of the indices $j_i = \max_{l\leq q} j_l$, 
Clearly, we have $j_l \leq k/2, l \neq  i$ \eqref{K}.
By Proposition \ref{prop:inter}  \eqref{eq:inte:3}, we have
%\eqref{eq:inte:1}, \eqref{eq:inte:3} with $\mu = 1, l = j \leq k /2 \leq k - 1 - d $ and \eqref{ss-}, we have
\[
\bal
|\na^{j_l} J_l | \les \la z \ra^{ - j_l + \s + \e/2}  || J_l ||_{\cH^{j_l + d}}
 % |\na^j W| &  \les ( E_{k} + E_0) \la z \ra^{ \s - j + \e / 2},   \quad j \leq k / 2,  \\
 %  \|  \nabla^{j_{i}}W  \|_{\rho_{j_i}} & \les E_{j_i} \les  E_{k-1 }+ E_0\,,\quad j_{i} \leq k-1, \quad  \|  \nabla^{j_{i}}W  \|_{\rho_{j_i}}   \les     E_{k} \,,\quad j_{i} = k  \\
 %  |\na^j \bar U| & \les_j \la z \ra^{ \s - j } \les_j \la z \ra^{\s - j + \e/2}, \quad 
 %  || \na^j \bar U ||_{g_j} \les_j 1 .
\eal
\]
% Denote $ J =(k,0,0,..,0)$. Then we have $I_{J, q} = \na^k W \cdot V^{p-2}$. Applying the above estimates to $\na^k W \cdot V^{p-2}$ and Corollary \ref{cor:decay} for $V = \bar U + \al W$, we obtain 
% \[
%  I_{J, q} \les |\na^k W| \la z \ra^{(p-2)\s + |p-2| \e / 2} (1 + E_0 + E_k)^{p + K-1}
% \]
%Clearly, we have $j_l \leq k/2, l \neq  i$ \eqref{K}. %and we can use $L^\infty$ bound for $J_l$. 
Applying the above $L^{\infty}$ estimates to $J_l, l\neq i$, and Corollary \ref{cor:decay} for $
V = \bar U + \al W$, we obtain 
\beq\label{eq:Hk_est_pf2}
I_{\vec j, q} \les |\na^{j_i} J_i|  \prod_{l\neq i} \la z \ra^{ - j_l +  \s +  \e / 2}  || J_l ||_{\cH^{j_l + d}}  \la z \ra^{(p-q) \s + |p-q| \e / 2}. %(1 + E_0 + E_k)^{\max(p-q, 0)} 
\eeq
Combining the exponents of the $\la z \ra^{\cdot}$ terms, and using the definitions of $\s = -\f{2}{p-q}$ \eqref{eq:dU_cons}  and $\e$ \eqref{eps}, we yield
\beq\label{eq:Hk_est_pf3}
\bal
\xi & = \sum_{ 1 \leq l \neq i \leq q} ( - j_l + \s +  \e  / 2) + (p-q) \s + |p-q| \e / 2 \\
& = - (k - j_i) + (p-q + q-1) \s + (p+q + q-1) \e / 2
= -(k - j_i) - 2 + ( p + K ) \e <  -(k - j_i).
\eal
\eeq
Since $\rho_k^{1/2} \la z \ra^{ - (k-j_i)} \les \rho_{k-j_i}$ \eqref{wg:rho}, applying weighted $L^2$ bound to $\na^{j_i } J_i$, we further obtain 
\[
I_{\vec j ,q} \les || J_i ||_{\cH^{j_i}} \prod_{l\neq i} || J_l ||_{\cH^{j_l+d}} .%(1 + E_0 +E_k)^{\max(p-q,0)}
\]
Since $j_l + d\leq k /2 + d \leq K-1 $ for $l \neq i, k \leq K$ , $j_i \leq k$, and $ || V ||_{\cH^K} \les 1 + E_0 + E_K$, we obtain $ j_l + d \leq \max( j_l, K-1)$ and thus 
\[
I_{\vec j ,q} \les || W_1 ||_{ \cH^{\max(j_1, K-1)}} 
|| W_2 ||_{ \cH^{\max(j_2, K-1)}} . %(1 + E_0 + E_K)^{ \max(p-q, 0) + q }.
\]
Using $\max(p-q,0) + q \leq p + K + q$ and summing the estimates of $I_{\vec j, q}$, we conclude the proof of \eqref{eq:Hk_est1}. 
%Note that $j_l $



The estimate \eqref{eq:Hk_est2_Hk} follows from summing the estimates of $I_{(j_1, j_2)}$
\eqref{eq:Hk_est1} over $(j_1, j_2) $ with $j_1 + j_2 \leq K$, and using the fact that we have $j_1 \leq K-1$ or $j_2 \leq K-1$. The estimate \eqref{eq:Hk_est2_L2} follows from applying $L^2(\rho_0)$ estimate to $W_2$ and $L^{\infty}$ estimate to $W_1, V$ similar to the above.



For the last estimate \eqref{eq:Hk_estU}, we note that $U = \bar U + W$. Applying the Leibniz rule, we obtain 
\[
%|\na^k (\na U / U)| 
|\na^{l+1} U  \na^{m} (U^{-1} ) | 
\les   \sum_{ 1 \leq q \leq k+1,} \sum_{ \sum_{l=1}^q j_l = k+1 , j_1 \geq 1, j_l \geq 0} T_{\vec j, q}, \quad 
 T_{\vec j, q} = |U|^{-q}  \cdot    \prod_{l=1}^q  |\na^{j_l} U| .
\]
Denote $i = \arg\max_l j_l$. Applying the above estimates of $I_{\vec j, q}$ with $(J_1,.. ,J_l), V, p-q$ replaced by 
$ (U, U,.., U), U, -q$ \eqref{eq:Hk_est_pf1}-\eqref{eq:Hk_est_pf3}, and using $\max(-q, 0) = 0, q \leq K+1 $, we obtain 
\[
|\la z \ra^{\s + \e/ 2} T_{\vec j, q} |
\les |\na^{j_i} U| \la z \ra^{\xi} \prod_{l\neq i} || U ||_{\cH^{j_l + d}}, 
\]
where 
\[
\bal
\xi & =\s + \f{\e}{2} +  \sum_{ 1 \leq l \neq i \leq q} ( - j_l + \s +  \f{\e}{2} ) + (-q) \s + |-q| \f{\e}{2}\\
& = - (k + 1 - j_i) + (-q + q) \s + (q + q) \e / 2
= -(k - j_i) - 1 + ( 1 + K ) \e <  -(k - j_i).
\eal
\]
Using $j_l + d \leq K/2 + d < K, || U||_{\cH^{j_l + d}}  \les || U||_{\cH^K} $ for $l \neq i$, 
$\rho_k^{1/2} \les \rho_{j_i}^{1/2} \la z \ra^{k-j_i}, q, j_i  \leq k+1$, and applying weighted $L^2$ estimate to $\na^{j_i} J_i$, we establish
\[
 ||\la z \ra^{\s + \e/ 2} T_{\vec j, q} ||_{g_k}
\les || U ||_{\cH^{j_i}} (1 + || U ||_{\cH^K})^{q-1}
\les || U ||_{\cH^{k+1}}. %(1 + E_0 + E_K)^{K}.
\]
Combining the estimates for $ T_{\vec j, q} $ with different $\vec j , q$, we  conclude the proof of \eqref{eq:Hk_estU}.

For \eqref{eq:Hk_estU_linf}, denote $k = l + m$. Applying $L^{\infty}$ estimate to each term $\na^{j_l}U$ in $T_{\vec j, q}$ and noting that $j_l \leq \max(l+1, m) \leq K-d$, we prove
\[
T_{{\vec j}, q} \les \la z \ra^{\xi} 
\les \la z \ra^{-k - 1/2} ,
\]
where we have used 
\[
\xi = \sum_{ 1 \leq l  \leq q} ( - j_l + \s +  \f{\e}{2} ) + (-q) \s + |-q| \f{\e}{2}
= - (k+1) + q \e < - k - 1/2.
\]
We complete the proof.
\end{proof}


}


% \paragraph{Interpolation inequalities:} 
% Provided that the bootstrap Assumption \ref{asss} holds,
% we collect the following weighted interpolation $L^2$ and $L^\infty$ inequalities. \textcolor{blue}{To Jiajie: please cite your work here. However, I think at least based on your screenshot, your result can not be directly applied here, although the proof is very similar.}
% \begin{proposition}
%     \label{prop:inter}
%     For any small positive constant $\mu$, there exists a constant $C(\mu)$, such that the following interpolation  inequalities hold:
%     $$E_k\leq \mu E_K+C(\mu)E_0\,,\quad \forall 0\leq k<K\,,$$
%     $$F_k\leq \mu F_K+C(\mu)F_1\,,\quad \forall 1\leq k<K\,,$$
%     $$\|\langle z\rangle^{l+\frac{2}{p-1}-\frac{\epsilon}{2}}\nabla^l W\|_{\infty}\leq \mu E_K+C(\mu)E_0\,,\quad \forall 0\leq l\leq K/2\,,$$
% $$\|\langle z\rangle^{l-1/2}\nabla^l\Phi\|_{\infty}\leq \mu F_K+C(\mu)F_1\,,\quad \forall 1\leq l\leq K/2\,.$$
% \end{proposition}
% \begin{proof}
%     To prove the first two inequalities of the proposition, we use integration by parts. For the first inequality, we compute for $K>k>0$ that
%     $$E_k^2=-\sum_i\int(\partial^2_i\nabla^{k-1}W\cdot\nabla^{k-1}W\rho_k+\partial_i\nabla^{k-1}W\cdot\nabla^{k-1}W\partial_i\rho_k)\,.$$
%     Notice that the weights satisfy $$\rho_k^2\lesssim\rho_{k+1}\rho_{k-1}\,,\quad(\partial_i\rho_k)^2\lesssim\rho_k\rho_{k-1}\,.$$
%     Combined with a Cauchy-Schwarz inequality, we obtain  $$E_k^2\lesssim E_{k-1}(E_{k}+E_{k+1})\,.$$By a weighted AM-GM inequality, for any $\mu>0$, we have $$E_k^2\leq C(\mu)E^2_{k-1}+\mu E^2_{k+1}\,.$$
%     From here, to conclude the first inequality, since $\mu>0$ is arbitrary, we only need to show it holds for $k=K-1$, which we can use induction on $K$ to prove.

%     For the second inequality, we can repeat the same procedure to conclude, provided that the weights $\mathring{\rho}_k$ satisfy the same inequalities for $K>k>1$:$$\mathring{\rho}_k^2\lesssim\mathring{\rho}_{k+1}\mathring{\rho}_{k-1}\,,\quad(\partial_i\mathring{\rho}_k)^2\lesssim\mathring{\rho}_k\mathring{\rho}_{k-1}\,.$$
%     When $k+1< K$, this is obvious. For $k=K-1$, we only need to show  $$\langle z\rangle^{2K-1-d}\lesssim\mathring{\rho}_{K}\approx U^2\langle z\rangle^{\frac{4}{p-1}+2K-\epsilon-d}\,,$$
%     which is true, since by the choice of $\epsilon$ and the bootstrap Assumption \ref{asss} we have $$U\geq C_b\bar{U}^{1+\epsilon}\approx \langle z\rangle^{-\frac{2+2\epsilon}{p-1}}\,,\quad \frac{4\epsilon}{p-1}+\epsilon<1\,.$$
    
%     To prove the $L^\infty$ estimates in the proposition, we proceed as in \cite{hou20242} and invoke the weighted Morrey-type inequality. We borrow the notation from \cite{website}. Define $L^j$ as the differential operator $
% \langle z\rangle \frac{\partial}{\partial z_j}\,.
% $ We consider the weighted Lebesgue space with weight defined by the Japanese brackets: $$
% \|f\|_{\mathcal{L}_s^2}:=\left\|\langle\cdot\rangle^s f\right\|_{2}\,, \quad
% \|f\|_{\mathcal{W}_s^{q, 2}}:=\sum_{j=1}^d\sum_{o=1}^q\left\|(L^j)^{o} f\right\|_{\mathcal{L}_s^2}\,.
% $$
% By the wave type estimates in Theorem 8 of \cite{website}, we have for $m=\left \lfloor{\frac{d}{2}}\right \rfloor$,
% \begin{equation}
% \label{weighted_m}
% \|f\|_{{\infty}} \lesssim\|f\|_{\mathcal{W}_{-d/2}^{m-1,2}}+\|f\|_{\mathcal{W}_{-d/2}^{m, 2}}+\|f\|_{\mathcal{W}_{-d/2}^{m+1,2}}\,.
% \end{equation}
% Since $|L^j\langle z\rangle|\lesssim\langle z\rangle$ for any $j$, we compute $$\|\langle z\rangle^{l+\frac{2}{p-1}-\frac{\epsilon}{2}}\nabla^l{W}\|_{\mathcal{W}_{-d/2}^{q,2}}\lesssim\|{W}\|_{\mathcal{W}_{\frac{2}{p-1}-\frac{\epsilon+d}{2}}^{q+l,2}}\lesssim\sum_{o\leq q+l}E_o\,,$$
% where in the last inequality,
% we use the estimate of the weights $$\langle z\rangle^{o+\frac{2}{p-1}-\frac{\epsilon+d}{2}}\lesssim\sqrt{\rho_o}\,.$$
% Therefore if we apply the weighted Morrey inequality \eqref{weighted_m} and the first interpolation inequality, we conclude the third inequality in the proposition, since $m+1+l\leq\frac{d+3+K}{2}< K$.

% Similarly for the last inequality, we compute $$\|\langle z\rangle^{l-1/2}\nabla^l \Phi\|_{\mathcal{W}_{-d/2}^{q,2}}\lesssim\|{\nabla\Phi}\|_{\mathcal{W}_{1/2-{d}/{2}}^{q+l-1,2}}\lesssim\sum_{o\leq q+l}F_o\,.$$
%  We can apply the weighted Morrey inequality \eqref{weighted_m} and the second interpolation inequality to conclude the last inequality in the proposition.
% \end{proof}



%We remark that $C_b$ is determined before $\epsilon$, but this is not a problem. In fact, we can choose $$C_b=\min\{\inf\{U/\bar{U}\},\inf\{U/\bar{U}^2\}\}\,.$$
%Notice that $1<1+\epsilon<2$, we know that Assumption \ref{asss} will hold.

\subsection{$L^2$ stability analysis of the amplitude}\label{l2sec}

{In this section, we estimate the weighted $L^2$ energy $E_0^2=(W,W\rho_0)\,$ \eqref{norm:Ek}. In the following energy estimates, without specification, we will assume that the bootstrap Assumption \ref{asss} holds true, {Namely \begin{align*}
    & U\geq C_b\bar{U}^{1+\epsilon_2} , \quad  C_b = \min_{|z|\leq 1} \bar U^{-\e_2}(z) / 4 > 0, \label{eq:boot_U}  \\
&  \max(E_K, E_0, F_K, F_1) \leq 1 ,
\quad \quad \det(\Qc) > 0.
\end{align*}}
 We will show that the following lemma holds.

}
\begin{lemma}[Weighted $L^2$ estimate]\label{lem:l2}
Under the bootstrap assumption \ref{asss}, it holds
\begin{equation}
    \label{l2-collecy}
        \frac{1}{2} {  \f{d}{d \tau } } E_0^2\leq (-\frac{\epsilon}{8}+ C \cE_1)E_0^2+ C \cE_2
        E_0\,.
\end{equation}
or some absolute constant $C>0$. 
\end{lemma}
%We consider the weighted $L^2$ norm $E_0^2=(W,W\rho_0)\,.$ 
\begin{proof}
Notice that $W$ vanishes at the origin to the third order so this choice of singular weight induces a well-defined energy. We  have by \eqref{realp} that 
$$\frac{1}{2} { \f{d}{d \tau}} E_0^2=(\mathscr{L}_{\bar{U}}W,W\rho_0)+(\mathscr{N}_U,W\rho_0)+(\mathscr{F}_U+\mathscr{D}_U,W\rho_0)\,.$$

For the leading order linear term, we have via integration by parts %, by the computations in \cite{hou20242} 
 that $$(\mathscr{L}_{\bar{U}}W,W\rho_0)=(d_0 W,W\rho_0)\,,$$
where we calculate the damping 
$$\begin{aligned}
    d_0&\coloneqq c_U+\frac{1}{2\rho_0}\nabla\cdot(d_{\bar{U}}z\rho_0)+p\bar{U}^{p-1}=-\frac{1}{p-1}+p\bar{U}^{p-1}+\frac{1}{4\rho_0}\nabla\cdot(z\rho_0)
    \\&=-\frac{1}{p-1}+\frac{p}{p-1+c_p|z|^2}+\frac{(-6+\epsilon)|z|^{-6+\epsilon}+(\frac{4}{p-1}-\epsilon)c_0|z|^{\frac{4}{p-1}-\epsilon}}{4(|z|^{-6+\epsilon}+c_0|z|^{\frac{4}{p-1}-\epsilon})}\leq-\frac{\epsilon}{8}\,.
\end{aligned}$$
 The last inequality amounts to $$\begin{aligned}&4p(|z|^{-6+\epsilon}+c_0|z|^{\frac{4}{p-1}-\epsilon})+((-6-\frac{4}{p-1}+\frac{3\epsilon}{2})|z|^{-6+\epsilon}-\frac{\epsilon}{2}c_0|z|^{\frac{4}{p-1}-\epsilon})(p-1+c_p|z|^2)\\&\leq-(p-1)|z|^{-6+\epsilon}-\frac{\epsilon}{2}c_0c_p|z|^{2+\frac{4}{p-1}-\epsilon}+4pc_0|z|^{\frac{4}{p-1}-\epsilon}
\leq0\,.\end{aligned}$$ 
The last inequality is implied by a weighted AM-GM inequality provided that \begin{equation}\label{c0}
    \Big(\frac{\epsilon c_0c_p}{2(6+\frac{4}{p-1}-2\epsilon)}\Big)^{6+\frac{4}{p-1}-2\epsilon}(\frac{p-1}{2})^2\geq \Big(\frac{4pc_0}{8+\frac{4}{p-1}-2\epsilon}\Big)^{8+\frac{4}{p-1}-2\epsilon}\,.
\end{equation}
Notice that $\epsilon\leq 1/2$ is fixed to be small. We can choose a sufficiently small constant $c_0 > 0$ such that we can conclude the linear estimate\begin{equation}
    \label{damp-l2}\big(\mathscr{L}_{\bar{U}}W,W\rho_0\big)\leq-\frac{\epsilon}{8}E_0^2\,.
\end{equation} 

The nonlinear estimate is more subtle due to the general nonlinearity $p$. We use Taylor's expansion or Newton-Leibniz's formula twice to derive 
\beq\label{eq:Newton}
\mathscr{N}_U=W^2p(p-1)\int_0^1(1-\alpha)(\bar{U}+\alpha W)^{p-2}d\alpha\,.
\eeq
%Therefore we have the estimate $$(\mathscr{N}_U,W\rho_0)\lesssim \sup_{\alpha\in[0,1]}\|W(1-\alpha)(\bar{U}+\alpha W)^{p-2}\|_{\infty}E_0^2\,.$$
{Using Proposition \ref{prop:Hk} \eqref{eq:Hk_est2_L2} with $(W_1, W_2) = (W, W)$ and $\cE_1$ defined in \eqref{eq:lot}, we obtain 
\[
 || W^2 (\bar{U}+\alpha W)^{p-2} ||_{\rho_0}
 \les || W||_{\cH^d} || W ||_{\rho_0}
\les (E_0 + E_d) E_0
\les \cE_1 E_0,
\]
which implies 
% 	Using Corollary \ref{cor:decay} and \eqref{eq:inte:3} in Proposition \ref{prop:inter} with $ l  =  d$, for $\al \in [0, 1]$, we obtain 
% 	\[
% 	\bal
%  | W(\bar{U}+\alpha W)^{p-2} | 
%  & \les E_d \la z \ra^{ \s + \e / 2} \la z \ra^{ (p-2) \s +  |(p-2)| \e / 2}
%  (1 + E_0 + E_{K} )^{\max(p-2, 0)} \\
% & \les E_d  (1 + E_0 + E_{K} )^{\max(p-2, 0)} \les \cE_1 ,
% \eal
% 	\]
% where we have used $\cE_1$ \eqref{eq:lot}, $\s = -\f{2}{p-1}$, and the smallness of $\e$ \eqref{eps}
% \[
% \s  +  \f{1}{2}\e  +  (p-2) \s + |(p-2)| \f{1}{2} \e 
% = -2 + \f{1}{2} \e (1 + |p-2|) \leq - 2 - \f{1}{2} \e (p+3)  <0
% \]
% in the second inequality. Using the above estimates, we obtain
}


% \red{Using the bootstrap assumption \ref{asss}, we have $U, \bar U > 0$. 
% For $0\leq \alpha\leq 1$, since $\bar{U}+\alpha W$ is between $U, \bar U$, we obtain $(\bar{U}+\alpha W)^{q}\leq \bar{U}^{q}+{U}^{q}$ for any power $q$.} By Proposition \ref{prop:inter} and Assumption \ref{asss}, we have the estimate that
%  \begin{equation}
%      \label{ass-big}\begin{aligned}
%         \|\langle z\rangle^{(\frac{2}{p-1}-\frac{\epsilon}{2})q}(\bar{U}+\alpha W)^{q}\|_{\infty}&\lesssim_\Qc  1+(\mu E_K+C( \mu)E_0)^q\,,\quad \forall 0\leq q\,,\\ 
%      \|\langle z\rangle^{\frac{2q+2q\epsilon}{p-1}}(\bar{U}+\alpha W)^{q}\|_{\infty}&\lesssim_\Qc  \|\langle z\rangle^{\frac{2q+2q\epsilon}{p-1}}\bar{U}^{q(1+\epsilon)}\|_{\infty} \les_\Qc  1\,, \quad \forall 0> q\,.\end{aligned}
%  \end{equation}

%  \red{Since $p$ is an absolute constant, we compute by Proposition \ref{prop:inter} with $\mu = 1$
% that}
%  \begin{equation}
%     \label{non-11}
% \begin{aligned}
% \|W(\bar{U}+\alpha W)^{p-2}\|_\infty&\leq\|\langle z\rangle^{\frac{-\epsilon}{2}+\frac{2}{p-1}}W\|_\infty\|\langle z\rangle^{\frac{\epsilon}{2}-\frac{2}{p-1}}(\bar{U}+\alpha W)^{p-2}\|_\infty\\&
% \les (\mu E_K+C( \mu)E_0)(1+( E_K+E_0)^{p}) \les \cE_1
% %=l.o.t._1
% \,,\end{aligned}\end{equation}
% where in the second inequality, we use the fact that by \eqref{eps}, we have 
% \begin{equation}\label{xi}\xi\coloneqq\frac{\epsilon}{2}-\frac{2}{p-1}-\min\{\frac{2(p-2)+2(p-2)\epsilon}{p-1},(\frac{2}{p-1}-\frac{\epsilon}{2})(p-2)\}\leq -1<0\,.
% \end{equation}


%By \eqref{non-11},  we collect the nonlinear estimate 
\begin{equation}
    \label{non-l2}
    | (\mathscr{N}_U,W\rho_0) | \leq\|\mathscr{N}_U\|_{\rho_0}E_0 
    \les \cE_1 || W ||_{\rho_0} E_0 \les 
        \cE_1 E_0^2\,.
    %l.o.t._1 E_0^2\,.
\end{equation} 

Finally, we estimate the viscous and residue terms together. We group the terms to make them integrable. Consider a fixed 1D smooth cutoff function $\chi$ such that it equals $1$ in $[-1,1]$ and $0$ outside of $[-2,2]$. We use the notation $\widetilde{f}$ to denote functions only differing from $f$ near the origin, where they equal the residue of $f$ when expanded until its second-order Taylor's expansion at the origin, via the cutoff function $\chi$.  For illustrative purposes, we will explicitly write down   $\widetilde{f}$ by the expansions 
$$f=(f(0)+z^T\nabla f(0)+\frac{1}{2}z^T\nabla^2f(0)z)\chi(|z|)+\widetilde{f}\,,$$
where $\widetilde{f}$ vanishes to the third order at the origin.  By the choice of 
{the modulation parameters} in \eqref{ode:v}, it's easy to see that\footnote{Note that $\tilde U$ does not denote the perturbation.} 
\begin{equation} \label{reor}\mathscr{F}_U+\mathscr{D}_U=c_W\widetilde{U}-\cP z\cdot\nabla\widetilde{U}-v\cdot\widetilde{\nabla{U}}-H^{p-1}\gamma\widetilde{U}+\widetilde{\mathscr{D}_U}\coloneqq\widetilde{\mathscr{F}_U}+\widetilde{\mathscr{D}_U}\,.
\end{equation}
Each of the terms in $\widetilde{\mathscr{F}_U}$ vanishes to the third order at the origin. Notice that $\rho_k=\rho_0 |z|^{2k}$, for $k=1,2,3$. Recall the definition of $\cE_1, \cE_2$ from \eqref{eq:lot}. By Lemma \ref{lem1}, we have that 
$$
\|\widetilde{\mathscr{F}_U}\|_{\rho_0}\les {\cE_2} (1+E_0+E_1+\|\widetilde{\nabla{W}}\|_{\rho_0})\,.
$$
We can decompose the integral region into the near field $I=[0,1]^d$ and the rest of the outer region $I^c$ to estimate 
$$\|\widetilde{\nabla{W}}\|_{\rho_0}\lesssim(\int_{z\in I}|z|^{\epsilon-d})^{1/2}\sup_{z\in I}|\widetilde{\nabla{W}}/|z|^3|+\|\widetilde{\nabla{W}}|z|\|_{\rho_0}\les   \Ga +E_1\,.
$$
{Here we recall the definition of $\Gamma, E_k$ in \eqref{ee} and \eqref{norm:Ek}.}
Combined with  Proposition \ref{prop:inter}, we have the residue estimate
\begin{equation}
    \label{res-l2}
     %(\widetilde{\mathscr{F}_U},W\rho_0)  \leq \red{\cE_2}(1+E_0+E_K)E_0\,.
      { | (\widetilde{\mathscr{F}_U},W\rho_0) | \les \cE_2 E_0\,.}
\end{equation} 

For the viscous term, we notice as in \eqref{du_exp}, we can write $$\widetilde{\mathscr{D}_U}=\text{tr}(\Qc\widetilde{S_1})\,,\quad S_1=S_{11}+S_{12}+S_{13}+S_{14}\,.$$
We estimate the four terms respectively. We compute
$$ 
 \|\widetilde{S_{11}}\|_{\rho_0}=\|\widetilde{\nabla^2U}\|_{\rho_0}\les 1 +\|\widetilde{\nabla^2W}\|_{\rho_0}\les 1+ \Ga +E_2 \,,
$$
where in the last inequality we use again the decomposition of the integral into the near and far fields.
For the remaining three viscous terms, we estimate similarly as follows:
{
\[
\bal
 \|\widetilde{S_{12}}\|_{\rho_0}&=2|\beta|\|\widetilde{\nabla U\nabla \Theta^T}\|_{\rho_0}\ \les  2|\beta|\|\widetilde{\nabla W}\widetilde{\nabla \Phi^T}\|_{\rho_0}+ (1+ \Ga)^2 \les  \Ga( \Ga +E_1) + (1+ \Ga )^2\,, \\
  \|\widetilde{S_{13}}\|_{\rho_0}&=\|\widetilde{U\nabla \Theta\nabla \Theta^T}\|_{\rho_0} \les \|\widetilde{W}\widetilde{\nabla \Phi}\widetilde{\nabla \Phi^T}\|_{\rho_0}+ (1+ \Ga)^3\les \Ga^2(\Ga+E_0) +(1+ \Ga)^3 \,, \\
   \|\widetilde{S_{14}}\|_{\rho_0}&=\|\widetilde{U\nabla^2\Theta}\|_{\rho_0} \les 
\|\widetilde{W}\widetilde{\nabla^2\Phi}\|_{\rho_0}+ (1+ \Ga )^2 \les \Ga(\Ga+E_0) +(1+\Ga)^2 .
\eal
\]
}

We can collect the viscous estimate by Proposition \ref{prop:inter} and Assumption \ref{asss}:
\begin{equation}
    \label{vis-l2} { | (\widetilde{\mathscr{D}_U},W\rho_0) | \les \cE_2} (1+E_0+E_1+E_2 + \Ga)^3 E_0\les {\cE_2} (1+E_0+E_K)^3E_0 \les \cE_2 E_0\,.
\end{equation} 
We thereby conclude the proof of Lemma \ref{lem:l2} using \eqref{damp-l2}, \eqref{non-l2}, \eqref{res-l2}, and \eqref{vis-l2}.  
\end{proof}
One sees that we already have leading order damping in the $L^2$ estimates. However, to close the nonlinear estimates, we will need higher order estimates to control the $L^\infty$ norms. 
\subsection{$H^1$ stability analysis of the phase}\label{h1sec}


We consider the weighted $H^1$ norm of the phase $F_1^2=(\nabla\Phi,\nabla\Phi\mathring{\rho}_1)\,$ \eqref{norm:Ek}.  
We choose this norm since $\Phi$ does not decay at the origin. We will show that the following lemma holds. 
\begin{lemma}[Weighted $H^1$ estimate] \label{lem:h1}
    Under the bootstrap assumption \ref{asss}, it holds 
    \begin{equation}    
    \label{h1-collecy}
            \frac{1}{2} \f{d}{d \tau} F_1^2\leq - \frac{1}{8}F_1^2+ { C ( E_{K-1}+E_0)^2
          } + {C \cE_2} F_1\,,   
\end{equation}
for some absolute constant $C>0$.
\end{lemma}\begin{proof}
    We  have by \eqref{imaginep} that 
$$\frac{1}{2} { \f{d}{d \tau} }  F_1^2=(\nabla(- \f{1}{2} \Lambda \Phi)+\nabla\mathscr{N}_\Theta+\nabla\mathscr{F}_\Theta+\nabla\mathscr{D}_\Theta,\nabla\Phi\mathring{\rho}_1)\,.$$

For the leading order linear term, we have via integration by parts
 that 
 $$(\partial_i(- \f{1}{2} \Lambda \Phi),\partial_i\Phi\mathring{\rho}_1)=- \f{1}{4}(\partial_i\Phi,\partial_i\Phi\mathring{\rho}_1)\,.
 $$
 Therefore we have the linear estimate\begin{equation}
\label{lin-theta}
(\nabla(- \f{1}{2} \Lambda \Phi),\nabla\Phi\mathring{\rho}_1)=-\frac{1}{4}F_1^2\,.
 \end{equation}
 
 For the nonlinear estimate, we again use Newton-Leibniz's formula to get 
 \beq\label{eq:newton_th}
 \mathscr{N}_\Theta= 
\d ( ( \bar U + W)^{p-1 } - \bar U^{p-1} )  = \delta(p-1)W\int_0^1(\bar{U}+\alpha W)^{p-2}d\alpha\,.
 \eeq
 % Using the definitions of $\rho_i, \mr{\rho}_i$ \eqref{wg:rho}, we compute that the weights satisfy
 % $$
 % %\frac{\sqrt{\mathring{\rho}_1}}{\sqrt{{\rho}_1}}
 %  \frac{ \mathring{\rho}_1^{1/2}}{ {\rho}_1^{1/2}}
 % \lesssim\frac{1}{|z|^{\frac{-5+\epsilon}{2}}+|z|^{\frac{2}{p-1}+\frac{1-\epsilon}{2}}}\lesssim\langle z\rangle^{\frac{-1+\epsilon}{2}-\frac{2}{p-1}} = \la z \ra^{\s + \f{\e-1}{2} } .
 % $$ 
{It is not difficult to see that $ \la z \ra^{\s  + \f{\e-1}{2}} \in \cH^i$ for any $i\geq 0$ since $\e-1 < 0$. Note that $\mr \rho_1$ \eqref{wg:rho} is locally integrable and $\mr \rho_1
\les \la z \ra^{\s  + \f{\e-1}{2}} g_1$. Applying $L^{\infty}$ estimate for $W, \bar U + \al W$ from Corollary \ref{cor:decay}, \eqref{eq:inte:3} in Proposition \ref{prop:inter},  and Proposition \ref{prop:Hk} \eqref{eq:Hk_est1} with $W_1 =\la z \ra^{\s  + \f{\e-1}{2}} , W_2 = W, j_1 = 0, j_2 = 1, k=1$, we obtain 
\[
\bal
|| \nabla\mathscr{N}_\Theta ||_{\mr \rho_1}
& \les || \nabla\mathscr{N}_\Theta  ||_{L^{\infty}(|z|\leq 1)}
+ || W_1 \nabla\mathscr{N}_\Theta ||_{ g_1}  
  \les  E_0 + E_{K-1} + || W_1 \nabla\mathscr{N}_\Theta ||_{  \rho_1}  \\
 & \les  E_0 + E_{K-1}  + || W_2 ||_{\cH^{K-1}} 
 \les E_0 + E_{K-1}  .
 \eal
\]
% \[
% || \nabla\mathscr{N}_\Theta ||_{\mr \rho_1}
%  \les  || W_1 \nabla\mathscr{N}_\Theta ||_{  \rho_1} 
%  \les || W_2 ||_{\cH^{K-1}} 
%  \les E_0 + E_{K-1} 
% \]
}
%  Therefore, using Proposition \ref{prop:inter} for $W, \na W$ and Corollary \ref{cor:decay}, we can estimate
% \red{
%   $$
%  \begin{aligned}
% & | \na (W(\bar{U}+\alpha W)^{p-2}) \mr{\rho_1}^{1/2} | 
%  \les ( |\na W  \cdot (\bar{U}+\alpha W)^{p-2}| + 
% | W (\bar U + \al W )^{p-3} \cdot \na (\bar U + \al W) | )  \mr{\rho_1}^{1/2} \\
% & \les | \na W| \rho_1^{1/2}
% \la z \ra^{\xi_1} (1 + E_K + E_0)^{\max(p-2, 0)}
% + |W| \rho_0^{1/2} \la z \ra^{\xi_2} (1  +E_K + E_0)^{ \max(p-3, 0) + 1}
%  \end{aligned}
%  $$
%  where the exponents $\xi_1, \xi_2$ satisfy 
%  \[
%  \bal
% & \xi_1 = \s + \f{\e-1}{2} + (p-2) \s + \f{ |(p-2)\e| }{2}
% < (p-1)\s  + \f{(p+3) \e}{2} 
% = -2 + \f{(p+3) \e}{2} < 0,  \\
% & \xi_2 = \s + \f{\e-1}{2} + 1 + 
% (p-3) \s + \f{ |(p-3)\e| }{2}
% + \s - 1 + \f{\e}{2}
% < (p-1) \s + \f{ (p+5)\e}{2}
% = - 2 + \f{ (p+5)\e}{2} < 0.
% \eal
%  \]
% Using the above estimates, $\max(p-2,0) , \max(p-3,0)+1< p+2$, and Proposition \ref{prop:inter} \eqref{eq:inte:1}, we establish 
% \[
% || \na (W(\bar{U}+\alpha W)^{p-2}) \mr{\rho_1}^{1/2} \mr \rho_1^{1/2} ||_{L^2}
% \les ( || \na W ||_{\rho_1}  + || W||_{\rho_0} )
% (1 + E_K + E_0)^p \les (E_0 + E_{K-1}) (1 + E_K + E_0)^{p+2} .
% \]
 %}
% $$
%  \begin{aligned}
% \|\nabla(W(\bar{U}+\alpha W)^{p-2})\|_{\mathring{\rho}_1} & \lesssim E_0\|\langle z\rangle^{1+\frac{2}{p-1}-\frac{\epsilon}{2}}(|\nabla\bar{U}|+|\nabla U|)\|_\infty\|\langle z\rangle^{\frac{-1+2\epsilon}{2}-\frac{4}{p-1}}(\bar{U}+\alpha W)^{p-3}\|_\infty \\
%  & \quad +E_1\|\langle z\rangle^{\frac{-1+\epsilon}{2}-\frac{2}{p-1}}(\bar{U}+\alpha W)^{p-2}\|_\infty \\
%  &\leq  (\mu E_K+C(\mu)E_0)(1+( E_K+E_0)^{p+2})\,,
%  \end{aligned}
%  $$
% where in the last inequality, we use again Proposition \ref{prop:inter}, the estimate \eqref{ass-big} and  inequalities of the indices similar to \eqref{xi}. 
We can collect the nonlinear estimate, via an AM-GM inequality as follows:\begin{equation} \label{non-theta}
|(\nabla\mathscr{N}_\Theta,\nabla\Phi\mathring{\rho}_1) | \leq C \|\nabla\mathscr{N}_\Theta\|_{\mathring{\rho}_1}F_1\leq C (  E_0+ E_{K-1} )^2 +\frac{1}{8}F^2_1\,.\end{equation}

For the residue estimate, we have 
\begin{equation}
\label{res-theta}
| (\nabla\mathscr{F}_\Theta,\nabla\Phi\mathring{\rho}_1) | \leq\|\nabla\mathscr{F}_\Theta\|_{\mathring{\rho}_1}F_1\les  \cE_2(1+F_1+\|\nabla^2\Phi\|_{\mathring{\rho}_1})F_1
\les \cE_2 F_1 
\,.
\end{equation}

For the viscous estimate, we have 
\beq\label{eq:vis_H1_1}
\begin{aligned}
|\nabla\mathscr{D}_\Theta\|_{\mathring{\rho}_1}&\les \cE_2 \B(\|\frac{\nabla^3U}{U}\|_{\mathring{\rho}_1}+\|\frac{\nabla^2U}{U}\|_{\mathring{\rho}_1}\|\frac{\nabla U}{U}\|_{\infty }+\|\frac{\nabla U}{U}\|_{\infty}\|\nabla ^2\Theta\|_{\mathring{\rho}_1}\\&+(\|\frac{\nabla^2U}{U}\|_{\infty}+\|\frac{\nabla U}{U}\|_{\infty}^2)\|\nabla \Theta\|_{\mathring{\rho}_1}+1+F_1+\|\nabla^3\Phi\|_{\mathring{\rho}_1} \B)\,.
\end{aligned}
\eeq
To estimate the integral $L^2(\mr \rho_1)$, we apply $L^{\infty}$ estimate in the region $|z| \leq 1$ and \eqref{eq:Hk_estU} and $ \mr \rho_1 \les \la z \ra^{\s + \e/2} g_1 \les \la z \ra^{\s + \e/2} g_2 $  to the region $|z| \geq 1$: 
\[
\bal
|| \na^l U / U ||_{\mr \rho_1} 
\les || \na^l U / U ||_{L^{\infty}(|z|\leq 1)}
+ || \la z \ra^{\s + \e/2} \na^l U / U ||_{g_1} 
\les 1 +  E_0 + E_{K} \les 1 , \quad l = 2,3 .
\eal
\]
Applying \eqref{eq:Hk_estU_linf} with $(l, m) =(1,0),(0,0)$, we get 
\beq\label{eq:vis_H1_2}
|\na^{l+1} U / U| \les 1.
\eeq
% 	 By Corollary \ref{cor:decay} and the choice of $\e$ \eqref{eps}, for $ l\leq 2$,
% 	 we have the following estimates:
% \begin{equation}
%     \label{h1-gb}
%     \B| \langle z\rangle^{l-1+\epsilon}\frac{\nabla^l U}{U} \B|
%     \les  \la z \ra^{l-1 + \e - l + \s + \f{\e}{2}  - \s + \f{\e}{2}  } 
%     \lesssim  \la z \ra^{-1+\e}
%     \les 1 .
% \end{equation}
% By Proposition \ref{prop:inter} and Assumption \ref{asss} similar to \eqref{xi}, we have the following estimates:
% \begin{equation}
%     \label{h1-gb}
%    \red{
%     \|\langle z\rangle^{l-1+\epsilon}\frac{\nabla^l U}{U}\|_\infty
%     \les (1 + E_K + E_0) || \la z \ra^{l-1 + \e - l - \f{2}{p-1} + \f{\e}{2} + (1 + \e) \f{2}{p-1}  } ||_{\infty} }
%     \lesssim 1+ E_K+E_0\,.
% \end{equation}
As a consequence, we can simplify the viscous estimate as follows:
\begin{equation}
    \label{h1-vis}|\nabla\mathscr{D}_\Theta\|_{\mathring{\rho}_1}\les \cE_2 (1+F_1+\|\nabla ^2\Phi\|_{\mathring{\rho}_1} +\|\nabla^3\Phi\|_{\mathring{\rho}_1})\,.
\end{equation}
% \begin{equation}
%     \label{h1-vis}|\nabla\mathscr{D}_\Theta\|_{\mathring{\rho}_1}\les \cE_2((1+( E_K+E_0)^2)(1+F_1+\|\nabla ^2\Phi\|_{\mathring{\rho}_1})+\|\nabla^3\Phi\|_{\mathring{\rho}_1})\,.
% \end{equation}
Finally, since $\mr \rho_1$ is $L^1$ integrable and $\mr \rho_i \les \la z \ra^{2i-2} \mr \rho_1$
\eqref{eq:comp_wg}, we can decompose the integral region into $I=[0,1]^d$ and the rest of the outer region $I^c$ as in the $L^2$ estimate of the amplitude to compute 
$$\|\nabla^l\Phi\|_{\mathring{\rho}_1} \lesssim\sup_{z\in I}|\nabla^l\Phi|+\|\nabla^l\Phi|z|^{2l-2}\|_{\mathring{\rho}_1} \les \Ga+F_l\,,
          \quad  || \na^l \bar \Th ||_{\mathring{\rho}_1} \les 1, \quad  l=2,3\,.
$$
We use Proposition \ref{prop:inter} and the bootstrap assumption \eqref{eq:boot_EE} to further obtain 
\[
\|\nabla^l\Phi\|_{\mathring{\rho}_1} + || \na \bar \Th \|_{\mathring{\rho}_1}
 \les 1 + F_1 + F_K \les 1.
\]{Here we recall the definition of $\Gamma, F_k$ in \eqref{ee} and \eqref{norm:Ek}.}
Plugging in the estimate in \eqref{h1-vis} and combined with \eqref{lin-theta}, \eqref{non-theta}, and \eqref{res-theta}, we establish Lemma \ref{lem:h1}.
%for any sufficiently small $\mu>0$:
\end{proof}
\subsection{$H^K$ stability analysis}\label{hksec}
%\JC{(Need to explain better the idea of different parameters and decays)}

For the estimate at the highest order, we consider the weighted $H^K$ energies \eqref{norm:Ek}
$$E_K^2=(|\nabla^K W|^2,\rho_K)\,,\quad F_K^2=(|\nabla^K \Phi|^2,U^2\rho_K)\,.$$ 
In this section, we will establish the following lemma.
\begin{lemma}[Weighted $H^K$ estimate]\label{lem:hk}
Under the bootstrap assumption \ref{asss}, we have
    \begin{equation}
     \label{hk-collected}
     \frac{1}{2} \f{d}{d \tau }  (E_K^2+F_K^2)\leq-\frac{\epsilon}{8}(E_K^2+F_K^2)+ \mu_0 \cE_1(E_K+F_K)\,\end{equation}
     for some absolute constant $\mu_0>0$.
\end{lemma}

%\paragraph{Estimates of the amplitude:}
\subsubsection{Estimates of the amplitude}

Recall the definitions of $\Ls_{\bar U}, \Ns_U, \Fs_U$ from \eqref{eq:lin}. We have  
$$\frac{1}{2} \f{d}{d \tau} E_K^2=(\nabla^K (\mathscr{L}_{\bar{U}}W)+\nabla^K \mathscr{N}_U+{\nabla^K\mathscr{F}_U}+{\nabla^K\mathscr{D}_U},\nabla^KW\rho_K)\,.
$$
For the leading order linear term, we can calculate the damping similarly as in the $L^2$ estimates.
{
A direct computation yields $\bar U^{p-1} \in \cH^i$ \eqref{ss-} for any $i \geq 0$. 
Using the Leibniz rule, the product rule \eqref{eq:prod} in Proposition \ref{prop:inter} with $i + j = K, j \leq K-1, m =K-1, n = i + d$, and $g_K \approx \rho_K$ \eqref{wg:rho}, \eqref{norm:Hk}, we yield 
\[
|| \na^K(\bar U^{p-1} W) - \bar U^{p-1} \na^K W ||_{\rho_K}
\les \sum_{ j \leq K-1} \na^{K-j} || \bar U^{p-1}||_{\cH^{i+d}} || W ||_{\cH^j}
\les \sum_{ j \leq K-1} E_j \les \cE_1.
\]
}
% For the leading order linear term, we can calculate the damping similarly as in the $L^2$ estimates. We know that for a canonical term in $\nabla^K(\bar{U}^{p-1}W) $ as $\partial_{i_1}\partial_{i_2}\cdots\partial_{i_j}(\bar{U}^{p-1})\partial_{i_{j+1}}\partial_{i_{j+2}}\cdots\partial_{i_{K}}W$, %it is $l.o.t.$ if $j>0$, 
% \red{it is lower order compared to $E_{K}$ and its $L^2(\rho_K)$ norm is bounded by $C \cE_1 $ \eqref{eq:lot}}, since we have the estimates
% $$
% | \partial_{i_1}\partial_{i_2}\cdots\partial_{i_j}(\bar{U}^{p-1}) | \lesssim | \partial_{i_1}\partial_{i_2}\cdots\partial_{i_j}(\langle z\rangle^{-2}) | \lesssim\langle z\rangle^{-2-j}\,,\quad \rho_K\lesssim\rho_{K-j}\langle z\rangle^{2j}\,.
% $$
Therefore, we can compute 
$$
\nabla^K(\mathscr{L}_{\bar{U}}W)=c_{\bar{U}} \nabla^KW- \f{1}{2} \sum_iz_i\nabla^K\partial_iW-
\f{K}{2} \nabla^KW+p\bar{U}^{p-1}\nabla^KW+ { O(\cR_{\mathscr{L}, K}),  \quad 
|| \cR_{\mathscr{L}, K } ||_{\rho_K} \les \cE_1.}
$$
We can calculate the damping similar to the $L^2$ case as follows:
$$\begin{aligned}
    d_K & \coloneqq-\frac{1}{p-1}-\frac{K}{2}+p\bar{U}^{p-1}+\frac{1}{4\rho_K}\nabla\cdot(z\rho_K)\\&=\frac{p}{p-1+c_p|z|^2}-\frac{1}{p-1}-\frac{K}{2}+\frac{d+(2K+\frac{4}{p-1}-\epsilon)c_1|z|^{\frac{4}{p-1}-\epsilon-d+2K}}{4(1+c_1|z|^{\frac{4}{p-1}-\epsilon-d+2K})}\leq-\frac{\epsilon}{8}\,,
\end{aligned}$$
where the last inequality holds for a sufficiently small $c_1$, which we defer till \eqref{defered} where we combine this damping with the estimates of the nonlinear term in the phase equation. %Fixing such a $c_1$, we conclude that \begin{equation}
    %\label{lin-hk} (\nabla^K(\mathscr{L}_{\bar{U}}W),\nabla^KW\rho_K)\leq-\frac{\epsilon}{8}E_{K}^2+O(\sum_{j<K}E_{j}E_{K})\,.%\leq-\frac{\epsilon}{10}E_{K}^2+O(\sum_{j<K}E_{j}^2)\,.
%\end{equation}

For the nonlinear term, we use Netwon-Leibniz's formula twice as in the $L^2$ estimate \eqref{eq:Newton}, to derive  
$$
 | (\nabla^K\mathscr{N}_U,\nabla^K W\rho_K) | \lesssim \sup_{\alpha\in[0,1]}(1-\alpha)\|\nabla^K(W^2(\bar{U}+\alpha W)^{p-2})\|_{\rho_K}E_K\,.
$$
%We consider a canonical term in the expansion of $\nabla^K(W^2(\bar{U}+\alpha W)^{p-2})$. 
%By the Leibniz rule, it will be bounded by 
Since $|| f||_{\rho_K} \les || f ||_{\cH^K}$  \eqref{wg:rho}, \eqref{norm:Hk}, 
using the product estimate \eqref{eq:Hk_est2_Hk} with $(W_1, W_2) = (W, W)$ and $ || f ||_{\cH^K} 
\les E_0 + E_K$ \eqref{eq:norm_comp}, we obtain 
\beq\label{non-hk} 
\bal
 | (\nabla^K\mathscr{N}_U,\nabla^K W\rho_K) | & \les E_K || W||_{\cH^K} || W ||_{\cH^{K-1}} 
 \les E_K  ( E_K + E_0) ( E_0 + E_{K-1}) 
\les E_K \cE_1. 
\eal
\eeq
% Using the Leibniz rule and expanding the derivative, we can bound it by 
% $$
% I \leq  E_K \sum_{1\leq q \leq K+1} \sum_{ \sum_{l=0}^q j_l = K, j_l \geq 0 } 
% I_{\vec{j}, q}, \
% I_{ \vec{j}, q} :=  |\nabla^{j_{0}}W||\nabla^{j_{1}}W||(\bar{U}+\alpha W)^{p-1-q}|\Pi_{l=2}^q|\nabla^{j_{l}}(\bar{U}+\alpha W)|\,. %\quad \sum_{l=0}^q j_l=K\,, \red{\quad 1 \leq q\leq K+1 }\,.
% $$

% Except for at most one of the indices $j_i$,we have $j_l \leq K/2, l \neq  i$ \eqref{K} and we can use $L^\infty$ bound for those terms. To be precise, we have the following estimates by Proposition \ref{prop:inter} \eqref{eq:inte:1}, \eqref{eq:inte:3} with $\mu = 1, l = j \leq K/2< K- d $ and \eqref{ss-}: 
% \[
% \bal
%  |\na^j W| &  \les ( E_{K-1} + E_0) \la z \ra^{ \s - j + \e / 2},  \quad 
%  |\na^j \bar U| \les \la z \ra^{ \s - j + \e / 2}, 
% \quad j \leq K / 2,  \\
%   \|  \nabla^{j_{i}}W  \|_{\rho_{j_i}} & \les E_{j_i} \les     E_{K-1}+ E_0\,,\quad j_{i} \leq K-1, \quad 
%   \|  \nabla^{j_{i}}W  \|_{\rho_{j_i}}   \les     E_{K} \,,\quad j_{i} = K 
%   .  
% \eal
% \]
% Applying the above estimates to the terms in $I_{\vec{j}, q} $ other than the $j_i$-th term, i.e. $\na^{j_i}W$ or $\na^{j_i}(\bar U + \al W)$, and Corollary \ref{cor:decay} for $\bar U + \al W$, we obtain 
% \beq\label{eq:non_amp}
% \bal
% I_{\vec{j}, q} 
% & \les  ( |\na^{j_i} W|+ |\na^{j_i} \bar U| ) 
% \cdot  \la z \ra^{ \xi} (E_0 + E_{K-1}) (1 + E_0 + E_{K-1} )^{\max(p-1-q, 0) + q-1} \\
% \eal
% \eeq
% where 
% \[
% \bal
% \xi & = (p-1-q) \s + |p-1-q| \e/2 +  \sum_{ l \neq i, 0\leq l \leq q} ( -j_i +  \s + \e / 2) \\
% & = (p-1) \s  + ( |p-1-q| + q ) \e / 2 - (K - j_i) 
% = - 2 + ( |p-1| + 2 q ) \e / 2 - (K - j_i)  < - (K - j_i) ,
% \eal
% \]
% and we have used $\sum_{j_l} = K$ and the smallness of $\e$ \eqref{eps} to get $(|p-1| + 2 q ) \e \leq  (p + K + 1) \e  < 1$. 
% Recall $\cE_1$ from \eqref{eq:lot}. Using \eqref{wg:rho} for the weight, 
% \[
% \rho_K \la z \ra^{2 \xi } \les 
% \rho_K \la z \ra^{- 2(K - j_i)} \les \la z \ra^{- 2 \s - \e - d + 2 j_i}  \les  \rho_{j_i},
% \quad  | \na^{j_i} \bar U |^2 \la z \ra^{- 2 \s - \e - d + 2 j_i} 
% \les %\la z \ra^{ - 2 j_i + 2 \s - 2 \s - \e - d + 2 j_i} = 
% \la z \ra^{-\e - d} \in L^1(\Rb^d),
% \] 
% and $q\leq K+1$, we further obtain 
% \[
% \bal
%   || I_{\vec{j}, q }  ||_{\rho_K} & \les (E_K + E_0) (E_{K-1} + E_0) (1 + E_{K-1} + E_0)^{\max(p-1-q,0) + q-1 + 1} \\
%  & \les (E_K + E_0) (E_{K-1} + E_0 ) (1 + E_{K-1} + E_0)^{\max(p, K)} \les \cE_1 . %(E_K + E_0). 
%  \eal
% \]
% Summing up the estimates, we will get the nonlinear estimate 
% \begin{equation}
% \label{non-hk} 
% (\nabla^K\mathscr{N}_U,\nabla^KW\rho_K) \les  \cE_1 E_{K} . %(E_K + E_0) \, .
% \end{equation}
% {\color{red}
% \paragraph{Ideas of the estimate} The main difficulty in the estimate of $I$ is the decay estimates. We explain the ideas below. 
% If the perturbation $\na^j W$ and $ \na^j (\bar U + \al W)$ has the same decay rates as $|\na^l\bar U(z)| \approx \la z \ra^{\al- l}, \al = - \f{2}{p-1}$, then we get
%  \[
%     |I_{\vec{j}, q}| \approx
% \la z \ra^{\al - j_0  } \cdot \la z \ra^{\al - j_1}
%      \la z \ra^{ (p-1 - q) \al}  \la z \ra^{\sum_{l=2}^q (\al-  j_l)}
%      = \la z \ra^{ p \al - K }
%      = \la z \ra^{- 2 - \f{2}{p-1}- K},
%      \quad     |I_{\vec{j}, q}|^2 \rho_{K}
%      \les \la z \ra^{- 4 - d  - \e}
%  \] 
% which is $L^1$ integrable in $\Rb^d$. We have established the tight decay estimates $ |\na^l W| \les \la z \ra^{-l + \al + \e / 2} $ and $  \la z \ra^{- \f{2}{p-1} - \f{\e}{2}}  \les  \bar U + \al W \les \la z \ra^{-\al + \e / 2} $. 
% Since $K$ is fixed \eqref{K}, by choosing $\e = O(1 / K)$ small \eqref{eps} and using  the extra decay rate $\la z \ra^{-4 + e}$ for the integrability, our estimate for the nonlinear terms are integrable. In the following estimates, the reader can treat $\e$ as if it is $0$.
% }
% {\color{red}
% Using the decays estimates of $\bar{U}$ and $(\bar U + \alpha W)^q$ \eqref{ass-big} and 
% $\rho_{K}\lesssim\rho_{j_i}\langle z\rangle^{2K-2j_i}$ \eqref{wg:rho}, 
% we can bound one summand as follows ...  
% \JC{(This part needs to explain better. A few steps are skipped here.)}
% }
%Notice the integrability of $\bar{U}$ and the fact that $\rho_{K}\lesssim\rho_{j_i}\langle z\rangle^{2K-2j_i}$. Using the bound \eqref{ass-big} and 
% Summing up the estimates, we will get the nonlinear estimate \begin{equation}
% \label{non-hk} 
% (\nabla^K\mathscr{N}_U,\nabla^KW\rho_K)\leq C\mu (1+\mu E_K+C(\mu)E_0)^{p+K-1}(E_K+C(\mu)E_0)^2E_{K}\les \cE_1 E_{K}\,,
% \end{equation}
% where we use the fact that $$\sum_{l\neq i}(j_l+\frac{2}{p-1}-\frac{\epsilon}{2})+\min\{(\frac{2}{p-1}-\frac{\epsilon}{2})(p-1-q),\frac{2(1+\epsilon)(p-1-q)}{p-1}\}\geq K-j_i\,,$$
% which is implied by our choice of $\epsilon$ in \eqref{eps} as we have $2\geq 3\epsilon(K+p)$.
Recall $\cE_2$ from \eqref{eq:lot}. For the residue term, we have via integration by parts that 
%\JC{(Below should be $E_K^2?$ rather than $E_K^2 + E_K?)$}
$$
| (\nabla^K\mathscr{F}_U,\nabla^KW\rho_K) | {\les \cE_2}(E_K^2+ E_K+ (|\nabla^KW|^2,|z\cdot\nabla\rho_K|+|\nabla\rho_K|))\,.
$$
Since we have $|\nabla\rho_K|\langle z\rangle\lesssim\rho_K$, we can conclude the residue estimate
\begin{equation}
    \label{res-hk} | (\nabla^K\mathscr{F}_U,\nabla^KW\rho_K) |\les \cE_2(E_K+E_K^2) {\les \cE_1 } E_K\,.%\leq-\frac{\epsilon}{10}E_{K}^2+O(\sum_{j<K}E_{j}^2)\,.
\end{equation}


%\paragraph{Estimates of the phase:} 
\subsubsection{Estimates of the phase}
We have 
\begin{align*}
     \frac{1}{2} \f{d}{d \tau } F_K^2 & =\Big(\nabla^K (- \f{1}{2} \Lambda \Phi)+\nabla^K \mathscr{N}_\Theta+{\nabla^K\mathscr{F}_\Theta}+{\nabla^K\mathscr{D}_\Theta},\nabla^K\Phi U^2\rho_K\Big) \\
     & \qquad \qquad  \qquad +\Big(\mathscr{L}_{\bar{U}}W+ \mathscr{N}_U+{\mathscr{F}_U}+{\mathscr{D}_U},  U|\nabla^K\Phi|^2\rho_K\Big)\,.
\end{align*}
Notice that the weight is time-dependent.
We remark that it is essential to pair the two linear terms and the two residue terms together to cancel out the leading order term via integration by parts. For the leading order linear term, we have via integration by parts that 
$$
(\nabla^K (- \f{1}{2} \Lambda \Phi),\nabla^K\Phi U^2\rho_K)+(\mathscr{L}_{\bar{U}}W+\mathscr{N}_U,  U|\nabla^K\Phi|^2\rho_K)=(\mathring{d}_{K},|\nabla^K\Phi|^2U^2\rho_K)\,,
$$
where we can calculate the damping $$\mathring{d}_{K}=\frac{-K}{2}+\frac{1}{4\rho_K}\nabla\cdot(z\rho_K)-\frac{1}{p-1}+\frac{{U}^{p}}{U}< d_K+{U}^{p-1}-\bar{U}^{p-1}\,.$$
Notice that by \eqref{eq:Newton}, \eqref{eq:inte:3} in Proposition \ref{prop:inter} with $l = 0$, and Corollary \ref{cor:decay}, we can further estimate
\beq\label{eq:main_Up}
    % |{U}^{p-1}-\bar{U}^{p-1}|\leq\sup_{0\leq\alpha\leq1}|W(\bar{U}+\alpha W)^{p-2}|\leq(\mu E_K+C(\mu)E_0)(1+( E_K+E_0)^{p})\,.
     |{U}^{p-1}-\bar{U}^{p-1}|\les \sup_{0\leq\alpha\leq1}|W(\bar{U}+\alpha W)^{p-2}|\les 
     (E_0 + E_{K-1} ) (1+  E_K+E_0 )^{p + 2}) \les \cE_1.
     %(\mu E_K+C(\mu)E_0)(1+( E_K+E_0)^{p})\,.
    \eeq
For the residue term, similarly via integration by parts, we have \begin{equation}
\label{res_hk1}
\begin{aligned}
     | (\nabla^K \mathscr{F}_\Theta,\nabla^K\Phi U^2\rho_K) | +| (\mathscr{F}_U,  U|\nabla^K\Phi|^2\rho_K) | & {  \les \cE_2}(F_K+F_K^2+(\frac{\nabla\cdot((Pz+v)\rho_K)}{2\rho_K},|\nabla^K\Phi|^2U^2\rho_K))\\ & \les \cE_2(F_K+F_K^2)\les \cE_1F_K\,,
\end{aligned}\end{equation}
where the inequality is again by the fact that $|\nabla\rho_K|\langle z\rangle\lesssim\rho_K$.

	For the nonlinear term, using Newton-Leibniz's formula \eqref{eq:newton_th}, we obtain 
\[
 |  \na^K \Ns_{\Th} | 
\leq I_{0, K} + C \sum_{j\leq K-1} I_{0, j} 
,\quad I_{i, j} = \d(p-1)  \cdot  \na^j W \cdot \na^{K-j} ( U + \al \bar W ) . 
\]
Applying \eqref{eq:Hk_est1} in Proposition \ref{prop:Hk} with $(W_1, W_2, j_1, j_2, k) = (U, W, 0, j, K-j)$ and $\bar U \in \cH^i$ \eqref{eq:U_decay}, we obtain 
\[
|| U I_{0, j} ||_{\rho_K} \les || U ||_{\cH^{K}} || W ||_{\cH^{K-1}} 
\les E_0 + E_{K-1}  \les \cE_1.
% || U I_{0, j} ||_{\rho_K} \les || U ||_{\cH^{K}} || W ||_{\cH^{K-1}} (1 + E_0 + E_K)^{p+K+2}
% \les (E_0 + E_{K-1}) (1 + E_0 + E_K)^{p+K+3} \les \cE_1.
\]
% For the nonlinear term, we estimate similarly as for the amplitude. Using Newton-Leibniz's formula \eqref{eq:newton_th}, a canonical term in $\nabla^K\mathscr{N}_\Theta$ is bounded by 
% $$
% \d (p-1) |\nabla^{j_{1}}W||(\bar{U}+\alpha W)^{p-1-q}|\Pi_{l=2}^q|\nabla^{j_{l}}(\bar{U}+\alpha W)|\,, \quad \sum_{l=1}^q j_l=K\,, \quad q\leq K+1\,.
% $$
% Let $j_i = \max_{l\leq q} j_l$. If $j_i < K$, we bound the weight $\mr \rho_K = U^2\rho_K$ \eqref{wg:rho} via an $L^\infty$ bound of $U$, apply $L^{\infty}$ estimate to the term with derivatives $\na^{j_l}, l \neq i$, and weighted $L^2$ estimate to the term with derivatives $\na^{j_i}$, and obtain similarly as in the amplitude estimate in Section \ref{sec:Hk_W} that its $\mathring{\rho}_K$ norm is bounded by 
% \begin{equation}
%     \label{nonbound} 
%     (1+  E_K+ E_0)^{p+K}( E_{K-1} + E_0) \les \cE_1\,.
% \end{equation}
% If $j_i =\max_{l\leq q} j_l = K$, the term with derivative $\na^{j_i}$ can only be of the form 
% $$ \d (p-1)(\bar{U}+\alpha W)^{p-2}\nabla^K W\,,\quad \text{or}\quad  \d(p-1) W(\bar{U}+\alpha W)^{p-3}\nabla^K(\bar{U}+\alpha W)\,. 
% $$
% The latter case has the same bound \eqref{nonbound} on its  $\mathring{\rho}_K$ norm.
Recall $\mr \rho_K = U^2 \rho_K$ \eqref{wg:rho}. For $ j\leq K-1$, the above estimate implies 
\beq\label{eq:non_HK_Th1}
 ||  I_{0, j} ||_{\mr \rho_K} = || U I_{0, j} ||_{\rho_K} \les \cE_1,
 \quad | ( I_{0, j}, \na^K \Phi \mr \rho_K ) | 
 \les  ||  I_{0, j} ||_{\mr \rho_K}  F_K \les \cE_1 F_K.
\eeq
The term $I_{0, K}$ is trickier and we need to estimate by an AM-GM inequality: 
{
$$\begin{aligned}
    ((\bar{U}+\alpha W)^{p-2}\nabla^K W,\nabla^K\Phi U^2\rho_K)&\leq\frac{1}{2}\| ( U^{\f{1}{2}}(\bar{U}+\alpha W)^{\frac{p-2}{2}}\nabla^K \Phi \|^2_{\mr \rho_K} +\frac{1}{2}\|U^{ \f{1}{2}}(\bar{U}+\alpha W)^{\frac{p-2}{2}}\nabla^K W\|^2_{\rho_K}\, ,
\end{aligned}$$
where we pair one of $U$ in $U^2$ with $\rho_K^{1/2}$ to get $\mr \rho_K^{1/2}$. Applying $U = (1-\al) W + \bar U + \al W$, Newton-Leibniz's rule for $(\bar U + \al W)^{p-1} - \bar U^{p-1}$, Proposition \ref{prop:inter} for $W$, and Corollary \ref{cor:decay} for $\bar U + s W, s \in [0, 1]$, which are similar to the estimate of $\mathscr{N}_{\Th}$ \eqref{eq:newton_th}, we obtain 
\[
\bal
U (\bar U + \al W)^{p-2} 
& \leq (\bar U + \al W)^{p-1} + C |W (\bar U + \al W)^{p-2} |
\leq \bar U^{p-1} + C \sup_{s \in [0, 1]}   |W (\bar U + s W)^{p-2} \\
&\leq \bar U^{p-1} + C (  E_{K-1} + E_0) 
\leq 
  (\min\{p-1,c_p\})^{-1}\langle z\rangle^{-2}+ C \cE_1 ,
%|U(\bar{U}+\alpha W)^{ p-2|& \leq U(\bar{U}^{\frac{p-3}{2}}+{U}^{\frac{p-3}{2}})\leq %	\bar{U}^{p-2}+|W\bar{U}|^{p-2}+{U}^{ p-2 }\,, \\
%\bar{U}^{\frac{p-1}{2}}+|W\bar{U}^{\frac{p-3}{2}}|+{U}^{\frac{p-1}{2}}& \leq (\min\{p-1,c_p\})^{-1/2}\langle z\rangle^{-1}+ C (  E_{K-1} + E_0)(1+( E_K+E_0)^{p})\,,
\eal
\]
% $$\begin{aligned}
%     ((\bar{U}+\alpha W)^{p-2}\nabla^K W,\nabla^K\Phi U^2\rho_K)&\leq\frac{1}{2}\|U(\bar{U}+\alpha W)^{\frac{p-1}{2}}\nabla^K \Phi \|^2_{\rho_K} +\frac{1}{2}\|U(\bar{U}+\alpha W)^{\frac{p-3}{2}}\nabla^K W\|^2_{\rho_K}\,.
% \end{aligned}$$
% We pair the terms with the linear damping in the phase and the amplitude. Similar to  \eqref{ass-big}, %\eqref{non-11}, and \eqref{xi}, 
% we can use Proposition \ref{prop:inter} to estimate  that 
% \[
% \bal]
% |U(\bar{U}+\alpha W)^{\frac{p-3}{2}}|& \leq U(\bar{U}^{\frac{p-3}{2}}+{U}^{\frac{p-3}{2}})\leq \bar{U}^{\frac{p-1}{2}}+|W\bar{U}^{\frac{p-3}{2}}|+{U}^{\frac{p-1}{2}}\,, \\
% |(\bar{U}+\alpha W)^{\frac{p-1}{2}}| & \leq \bar{U}^{\frac{p-1}{2}}+{U}^{\frac{p-1}{2}}\,, \\
% \bar{U}^{\frac{p-1}{2}}+|W\bar{U}^{\frac{p-3}{2}}|+{U}^{\frac{p-1}{2}}& \leq (\min\{p-1,c_p\})^{-1/2}\langle z\rangle^{-1}+ C (  E_{K-1} + E_0)(1+( E_K+E_0)^{p})\,,
% \eal
% \]
}where we extract a decay at the far field for the leading order term.
We can calculate the damping 
\begin{align*}
    &\d(p-1)(\min\{p-1,c_p\})^{-1}\langle z\rangle^{-2}+d_K \\
    & \quad  \leq \frac{ \d(p-1)(p+1) }{\min\{p-1,c_p\}(1+|z|^2)}-\frac{1}{p-1}-\frac{K}{2}+\frac{d+(2K+\frac{4}{p-1}-\epsilon)c_1|z|^{\frac{4}{p-1}-\epsilon-d+2K}}{4(1+c_1|z|^{\frac{4}{p-1}-\epsilon-d+2K})}\,.
\end{align*}
Recall the definition of $K$ in \eqref{K} and
similar to the $L^2$ damping, we can use a weighted AM-GM inequality to conclude for a sufficiently small positive $c_1$, we have  
\begin{equation}
    \label{defered}
   (p-1) \d (\min\{p-1,c_p\})^{-1/2}\langle z\rangle^{-1/2}+d_K\leq-\frac{\epsilon}{8}\,.
\end{equation}
As a consequence, we collect the linear and nonlinear estimates of the phase, and the linear estimate of the amplitude together as follows:
\begin{align}
   \Big(\nabla^K(\mathscr{L}_{\bar{U}}W),\nabla^K W\rho_K\Big)+ \Big(\nabla^K (- \f{1}{2} \Lambda \Phi+\mathscr{N}_\Theta)&+\frac{\mathscr{L}_{\bar{U}}W+\mathscr{N}_U}{U},\nabla^K\Phi U^2\rho_K\Big) \nonumber \\
    & \quad \leq  -\frac{\epsilon}{8}(E^2_K+F^2_K)+C \cE_1( E_K+F_K)%\\&\leq-\frac{\epsilon}{8}E^2_K+\frac{\epsilon}{12}F_K^2+\mu(E_K+C(\mu)E_0)^2(1+( E_K+C(\mu)E_0)^{2p+2K})
    \,. \label{non-hk1}
\end{align}


%\paragraph{Estimates of the viscous terms:}
\subsubsection{Estimates of the viscous terms}
Finally, we estimate the viscous terms. The simpler term  can be estimated as follows: \begin{equation}
    \label{vos-ls}({\mathscr{D}_U},  U|\nabla^K\Phi|^2\rho_K)\leq\|\frac{\mathscr{D}_U}{U}\|_{\infty}F_K^2\les \cE_1 F_K\,.
\end{equation}
The last inequality is derived similarly to the $H^1$ viscous estimates in \eqref{eq:vis_H1_1}, \eqref{eq:vis_H1_2}. 




We group leading order viscous terms as follows and estimate them together: $$(\nabla^K\mathscr{D}_U,\nabla^K W\rho_K)+(\nabla^K\mathscr{D}_\Theta,\nabla^K\Phi U^2\rho_K)\,,$$
and we will use integration by parts to cancel out the leading order terms and extract damping.  
Recall the definition of the viscous terms in \eqref{eq:vis}. For any tensor $f$, we define $$|f|^2_{\Qc}=\sum_{i}(\nabla f_i)^T\Qc\nabla f_i\,,$$ where we sum over its scalar entry components $f_i$. 

Notice that $|\nabla\rho_K|\lesssim\rho_K$. We compute the damping of the amplitude using integration by parts and the Cauchy-Schwarz inequality as 
$$\begin{aligned}
    (\nabla^K\Delta_\Qc  U,\nabla^K W\rho_K) & \leq C \cE_1 E_K -(|\nabla^{K} W|^2_{\Qc},\rho_K) +C|\Qc|^{1/2}\|\nabla^{K} W\|_{\rho_K}\||\nabla^{K} W|_{\Qc}\|_{\rho_K}  \\
    & \leq C \cE_1 E_K-\frac{1}{2}(|\nabla^{K} W|^2_{\Qc},\rho_K)\,.
\end{aligned}$$
Using \eqref{eq:inte:3} from Proposition \ref{prop:inter} and \eqref{eq:U_decay}, we get 
\[
|\na U| \les U % (1 + E_K + E_0) 
, \quad  |\nabla(U^2\rho_K)|\lesssim  
|\na U| U \rho_K + U^2 | \na \rho_K | \les  
U^2\rho_K. 
 \]
Similarly, we compute the damping of the phase as
$$
  (\nabla^K\Delta_\Qc  \Theta,  \nabla^K\Phi U^2\rho_K)\leq C \cE_1F_K-\frac{1}{2}(|\nabla^{K} \Phi|^2_{\Qc},U^2\rho_K)\,.
$$

For the four intermediate terms in the viscous terms 
$$
I_1 = \langle\nabla U,\nabla\Theta\rangle_\Qc \,,\quad I_2 = U\langle\nabla \Theta,\nabla\Theta\rangle_\Qc \,,\quad I_3 = \frac{\langle\nabla U,\nabla\Theta\rangle_\Qc }{U}\,,\quad I_4 = \langle\nabla \Theta,\nabla\Theta\rangle_\Qc \,,
$$
we can simply control their weighted norms using the diffusion term. 

{We consider the most challenging term $I_3$. Using the Leibniz rule, \eqref{eq:Hk_estU} in Proposition \ref{prop:Hk}, we obtain 
\[
|| I_3 ||_{\mr \rho_K}
\les \sum_{0\leq i\leq K} || I_{3, i} ||_{\mr \rho_K}, \quad  I_{3, i} = (\na^i \f{ \na U }{U}, \na^{K-i+1} \Th )_\Qc .
 %\sum_{ 1 \leq i \leq K-1} |\Qc || \na^i \f{\na U}{U} \na^{K-i} \na \Th ||_{\rho_K}
\]
For $ 1 \leq i \leq K-1$, applying  \eqref{eq:Hk_estU_linf} to $\na U / U$ if $i \leq  K/2 + 1 < K-d-1$ and \eqref{eq:inte} to $\Th$ if $ i > K/2$, which implies $K-i+1 \leq K/2+1 < K-d-1$, we obtain
\[
|I_{3, i} |
\les |\Qc| ( \la z \ra^{-i}  | \na^{K-i+1} \Th|
  + \la z \ra^{-(K-i)} |  \na^i (\na U / U)|    ).
% |I_{3, i} |
% \les |\Qc| ( \la z \ra^{-i} (1 + E_0 + E_K)^{p+K+ 2}  | \na^{K-i+1} \Th|
%   + \la z \ra^{-(K-i)} |  \na^i (\na U / U)|   (1 + F_1 + F_K)^{p+K+2})
\]
Since $ i \leq K-1, K-i+1 \leq K$, using the estimate \eqref{eq:comp_wg} for weights
\[
 \mr \rho_K^{1/2} \les \la z \ra^{i-1} \mr \rho^{1/2}_{K-i+1}, \quad \la z \ra^{-(K-i)} \mr \rho_K^{1/2}
 \les \mr \rho_{i}^{1/2}
 \les \la z \ra^{\s + \e/2} \rho_{i}^{1/2}, 
 \]
%the product estimate \eqref{eq:prod}, and \eqref{eq:inte}, 
and \eqref{eq:Hk_estU}, we obtain 
\[
\bal
 ||I_{3, i}||_{ \mr \rho_K}
& \les |\Qc| 
(||\na^{K-i+1} \Th  ||_{ \mr \rho_{K-i}} 
+ || \la z \ra^{\s +\e/2}  \na^i (\na U / U) ||_{\rho_i})  \les |\Qc|  \les \cE_1.
%  ||I_{3, i}||_{ \mr \rho_K}
% & \les |Q| ( 1 + E_0 + E_K + F_1 + F_K)^{p+K+2} 
% (||\na^{K-i+1} \Th  ||_{ \mr \rho_{K-i}} 
% + || \la z \ra^{\s +\e/2}  \na^i (\na U / U) ||_{\rho_i}) \\
% & \les |Q| ( 1 + E_0 + E_K + F_1 + F_K)^{2( p+K+2)} \les \cE_1.
\eal
\]
}
% We take the most challenging term as an example. When we estimate $$\|\nabla^K\frac{\langle\nabla U,\nabla\Theta\rangle_\Qc }{U}\|_{U^2\rho_K}=\|U\nabla^K\frac{\langle\nabla U,\nabla\Theta\rangle_\Qc }{U}\|_{\rho_K}\,,$$
% a canonical term in the expansion is bounded by 
% \begin{equation}\label{can}
% J = |Q||\nabla^{j_{1}}\Theta||\nabla^{j_{2}}U||U^{2-q}|\Pi_{l=3}^q|\nabla^{j_{l}}U|\,, \quad \sum_{l=1}^q j_l=K\,, \quad 3\leq q\leq K\,, \ j_1, j_2 \geq 1.
% \end{equation}
% Similar to the estimates of the nonlinear terms, except for one of the indices $j_i$,  all other indices will be smaller than $K/2$ and we can use $L^\infty$ bound for those terms. 
% Denote $ i = \arg\max j_l$. If $j_i \leq  K-1$, the $\rho_K$ norm of $J$ is bounded by $ \cE_1$, 
% \red{which can be established following \eqref{eq:non_amp}
% \[
% J \les \Ga \la z \ra^{\xi} 
%  (1 + E_0 + E_K)^{q}
% \]
% where 
% \[
% \bal
% \xi &\leq - 1 + \f{1}{2} + \sum_{l \neq i, l\leq q} - j_i 
% - j_1 - 1 + \f{1}{2}, \quad i = 1 \\ 
% \xi &\leq 
% \eal
% \]
% since we count the index similar to \eqref{non-hk} as
% $$
% j_1+\frac{1}{2}+1+\sum_{1<l\neq i}(j_l+\frac{2}{p-1}-\frac{\epsilon}{2})+\frac{2(1+\epsilon)(2-q)}{p-1}\geq K-j_i\,,
% $$
% $$
% j_1+\frac{1}{2}-\frac{d}{2}+\sum_{1<l}(j_l+\frac{2}{p-1}-\frac{\epsilon}{2})+\frac{2(1+\epsilon)(2-q)}{p-1}\geq K+\frac{2}{p-1}-\frac{\epsilon+d}{2}\,,
% $$
% or we can use the estimates \eqref{h1-gb} when $j_1=K-1$. When one of the indices is $K+1$, then $j_1=K$ or $j_2=K$. 
For $I_{3,0}, I_{3, K}$, we use the Cauchy-Schwarz inequality to compute that its $\rho_K$ norm is bounded by $$ \cE_1+|\Qc|^{1/2}(\|\nabla\Theta\|_{\infty}\||\nabla^{K} W|_{\Qc}\|_{\rho_K}+\|\frac{\nabla U}{U}\|_{\infty}\|U|\nabla^{K} \Phi|_{\Qc}\|_{\rho_K})\,.$$
Similarly, we have the estimates for the other three viscous terms $I_1, I_2, I_4$.
Combined with \eqref{eq:vis_H1_2}, we can use the Cauchy-Schwarz inequality to derive that 
\begin{align*}
&\Big(-2\beta\nabla^K\langle\nabla U,\nabla\Theta\rangle_\Qc -\nabla^K(U\langle\nabla \Theta,\nabla\Theta\rangle_\Qc ),\nabla^K W\rho_K\Big)+\Big(2\nabla^K\frac{\langle\nabla U,\nabla\Theta\rangle_\Qc }{U}-\beta\nabla^K{\langle\nabla \Theta,\nabla\Theta\rangle_\Qc },\nabla^K\Phi U^2\rho_K\Big)\\
& \qquad \leq C\cE_1(E_K+F_K)+\frac{1}{8}((|\nabla^{K} W|^2_{\Qc},\rho_K)+(|\nabla^{K} \Phi|^2_{\Qc},U^2\rho_K))\,.
\end{align*}
%$$\begin{aligned}(\nabla^K\langle\nabla U,\nabla\Theta\rangle_\Qc ,\nabla^K W\rho_K)&\leq l.o.t._1E_K\\&+\frac{1}{20}((|\nabla^{K} W|^2_{Q},\rho_K)+(|\nabla^{K} \Phi|^2_{Q},U^2\rho_K))\,.\end{aligned}$$
%$$\begin{aligned}(\nabla^K(U\langle\nabla \Theta,\nabla\Theta\rangle_\Qc ),\nabla^K W\rho_K)&\leq l.o.t._1E_K\\&+\frac{1}{20}((|\nabla^{K} W|^2_{Q},\rho_K)+(|\nabla^{K} \Phi|^2_{Q},U^2\rho_K))\,.\end{aligned}$$
%A canonical term in the expansion of $U\nabla^K\langle\nabla \Theta,\nabla\Theta\rangle_\Qc $ is bounded by $$|Q||\nabla^{j_{1}+1}\Theta||\nabla^{j_{2}+1}\Theta||U|\,, \quad j_{1}+ j_2=K\,. $$
%We can count the index as before using \eqref{h1-gb} when one of $j_1, j_2\geq K-1$, or when $j_1, j_2<K-1$ by: $$j_1+\frac{1}{2}-\frac{d}{2}+j_2+\frac{1}{2}+\frac{2}{p-1}-\frac{\epsilon}{2}\geq K+\frac{2}{p-1}-\frac{\epsilon+d}{2}\,,$$
%to conclude the estimate 
%$$\begin{aligned}  (\nabla^K{\langle\nabla \Theta,\nabla\Theta\rangle_\Qc },\nabla^K\Phi U^2\rho_K)&\leq l.o.t._1F_K\\&+\frac{1}{20}((|\nabla^{K} W|^2_{Q},\rho_K)+(|\nabla^{K} \Phi|^2_{Q},U^2\rho_K))\,.
%\end{aligned}$$

Finally, for the last two viscous terms, we use integration by parts to cancel out the leading order terms. 
{
Applying estimates similar to the those for $I_3$ in the above, we can extract the leading order terms, which involve $\na^{K+2} U$ or $\na^{K+2} \Th$,
%we obtain 
\[
\bal
-\beta \B(\nabla^K(U\Delta_\Qc  \Theta),\nabla^K W\rho_K \B)
& = - \beta ( U  \Delta_\Qc  \na^K \Th, \na^K W \rho_K) + O(\cE_1 E_K) + \f{1}{16} (|\nabla^{K} \Phi|^2_{\Qc},U^2\rho_K) , \\
\beta\B(\nabla^K\frac{\Delta_\Qc  U}{U},\nabla^K \Phi U^2\rho_K\B)& = \beta \B( \f{ \D_\Qc  \na^K U }{U} , \na^K \Phi U^2 \rho_K \B) + O(\cE_1 F_K) + \f{1}{16} (|\nabla^{K} U|^2_{\Qc},\rho_K)
.  \\
\eal
\]
}
% To be precise, we notice that 
% a canonical term in $U\nabla^K\frac{\Delta_\Qc  U}{U}$ is bounded by $$|Q||\nabla^{j_{1}+2}U||U^{1-q}|\Pi_{l=2}^q|\nabla^{j_{l}}U|\,, \quad \sum_{l=1}^q j_l=K\,, \quad q\leq K\,.$$
% Except for the case when $j_1=K$, we can bound its $\rho_K$ norm as what we did in \eqref{can}. Likewise, we can do the same for $\nabla^K(U{\Delta_\Qc  \Theta})$. We can conclude that  $$\begin{aligned}
%     &-\beta(\nabla^K(U\Delta_\Qc  \Theta),\nabla^K W\rho_K)+\beta(\nabla^K\frac{\Delta_\Qc  U}{U},\nabla^K \Phi U^2\rho_K)
%     \les \cE_1(E_K+F_K)\\&+\frac{1}{16}((|\nabla^{K} W|^2_{Q},\rho_K)+(|\nabla^{K} \Phi|^2_{Q},U^2\rho_K))+\beta(-(\nabla^K\Delta_\Qc  \Theta,\nabla^K WU\rho_K)+({\nabla^K\Delta_\Qc  U},\nabla^K \Phi U\rho_K))\,.
% \end{aligned}$$
Now, we use $U = \bar U + W,  \Th = \bar \Th + \Phi$ and integration by parts to cancel out the leading order terms. 
$$
\begin{aligned}
    &-(\nabla^K\Delta_\Qc  \Theta,\nabla^K WU\rho_K)+({\nabla^K\Delta_\Qc  U},\nabla^K \Phi U\rho_K) \\
 = &  -(\nabla^K\Delta_\Qc  \Phi,\nabla^K WU\rho_K)+ ({\nabla^K\Delta_\Qc  W},\nabla^K \Phi U\rho_K) + O(\cE_1(E_K+F_K)) \\
 = & \sum_{i,j} \B(  \Qc_{ij} ( -\pa_i ( \pa_j \na^K \Phi \cdot \na^K W)  + \pa_j ( \pa_i \na^K W \cdot \na^K \Phi ) ), U \rho_K \B) \\
     \leq &  C \cE_1(E_K+F_K)+\frac{1}{16\beta}((|\nabla^{K} W|^2_{\Qc},\rho_K)+(|\nabla^{K} \Phi|^2_{\Qc},U^2\rho_K))\,.
\end{aligned}
$$ 
We notice that the remaining terms from integration by parts are controlled since $|\nabla(U\rho_K)|\lesssim U\rho_K$.

Combining the viscous estimates with the estimates \eqref{non-hk}, \eqref{res-hk}, \eqref{res_hk1}, and \eqref{non-hk1}, we conclude the proof of Lemma \ref{lem:hk}.
 %\paragraph{Collection of the estimates:} 
\subsubsection{Summary of the $H^K$ estimates}
 Using \eqref{eq:inte:1}, \eqref{eq:inte:2} in Proposition \ref{prop:inter}, for any $\mu > 0$, we obtain 
\[
\cE_1 \leq |\Qc| + H^{p-1}
+ C(\mu)(E_0 + F_1) + \mu( E_K + F_K) +( E_0 + F_1 +E_K + F_K)^2. 
\]
By Lemma \ref{lem:hk},
choosing $\mu < \f{\e}{16 \mu_0}$ and then collecting \eqref{hk-collected}, \eqref{h1-collecy}, and \eqref{l2-collecy}, we obtain that there exists a sufficiently small constant $1 > \nu_1>\nu_2>0$, $\nu_2$ determined after $\nu_1$, such that for the energy \begin{equation}   \label{eneq}E^2=E_K^2+F_K^2+1/\nu_1 F_1^2+ 1/\nu_2 E_0^2\,,
 \end{equation}
 %we can collect the 
 the following estimate holds 
 \begin{equation}
 \label{booten}\frac{1}{2} \f{d}{d \tau} E^2\leq-\frac{\epsilon}{16}E^2+C(|\Qc|+H^{p-1})
E+CE^3 \,, 
\iff 
 \f{d}{d \tau} E \leq-\frac{\epsilon}{16}E +\mu_1(|\Qc|+H^{p-1})
+\mu_1 E^2 \,, 
% \label{booten}\frac{1}{2} \f{d}{d \tau} E^2\leq-\frac{\epsilon}{16}E^2+C(|\Qc|+H^{p-1})
% E+CE^3+CE^{3p+3K+3}\,, 
 \end{equation}
 for some absolute constant $\mu_1>0$. Here, the constant $C$ would depend on $\nu_1, \nu_2$. Once we fix $\nu_1, \nu_2$, then $C$ becomes a fixed constant $\mu_1$. The estimate holds provided that Assumption \ref{asss} is valid.

\subsection{Lower bound of the amplitude}\label{sec:linfty}

% We now prove the bootstrap Assumption \ref{asss} by estimating the upper bound of $U^{-1}\rho$,
% for the weight $\rho=\bar{U}^{1+\epsilon_2}$. The reason that we estimate $U^{-1}$ instead of $U$ is due to the outgoing property of the flow $ d_U z \na U$ \eqref{real-gl}, which allows us to localize the estimate of $U^{-1}$. See \JC{below}. Firstly, we derive the equation of $\Om = U^{-1} g$ using \eqref{real} for some function $g$. Then we will localize the estimate and apply the maximal principle to prove the desired estimate.



% Multiplying $-U^{-2}$ on both sides of \eqref{real}, we get 
% %A direct computation yields 
% \[
%  \pa_{\tau} U^{-1}
%   = - (c_U + U^{p-1} - H^{p-1} \gamma) U^{-1} 
%   - (d_{\bar U} z + P z + v) \na U^{-1}  - U^{-2} \Ds_U.
% \]

% Recall $\Om = U^{-1} g$. Note that 
% \[
% \na U^{-1} = \f{1}{g} 
% \]






We now prove the bootstrap Assumption \ref{asss} by estimating the lower bound of $U\rho$,
for the  weight $\rho=\bar{U}^{-1-\epsilon_2}$. We will proceed with a maximal principle argument and a barrier argument.  Notice that $$\nabla U=\frac{\nabla(U\rho)-U\nabla\rho}{\rho}\,,\quad\nabla^2 U=\frac{\nabla^2(U\rho)-U\nabla^2\rho}{\rho}-\frac{\nabla(U\rho)\nabla\rho^T+\nabla\rho\nabla(U\rho)^T-2U\nabla\rho\nabla\rho^T}{\rho^2}\,. $$ 
We compute by \eqref{real} that 
\begin{equation}\label{max-p}
\bal
& \partial_\tau(U\rho)= \cP_U (U \rho) ,
\quad \cP_U  f = A_0 f + A_1 \cdot \na f + \tr( Q \na^2 f ) .  \\
%& L_0 U\rho-(d_{\bar{U}}z+Pz+v+2\frac{Q\nabla\rho}{\rho}+2\beta Q\nabla \Theta)\cdot\nabla( U\rho)+\text{tr}(Q\nabla^2(U\rho))\,,
\eal
 \end{equation}
where the coefficients $A_0, A_1$ of the parabolic operator $\cP_U$ are:  
$$
\begin{aligned}
A_0 &=c_U-H^{p-1}\gamma+U^{p-1}+( \f{1}{2} z+\Pc z+\Vc)\cdot\frac{\nabla\rho}{\rho}-\frac{\Delta_\Qc \rho-2\beta\langle\nabla \rho,\nabla\Theta\rangle_\Qc }{\rho}+2\frac{\langle\nabla \rho,\nabla\rho\rangle_\Qc }{\rho^2}-\langle\nabla \Theta,\nabla\Theta\rangle_\Qc -\beta\Delta_\Qc \Theta\,, \\
A_1 & = -(  \f{1}{2} z+\Pc z+\Vc+2\frac{\Qc\nabla\rho}{\rho}+2\beta \Qc ), 
\end{aligned}$$


Notice that $\bar{U}$ is the approximate steady state and $|\nabla\rho|\langle z\rangle\lesssim\rho$. We can calculate the damping using the nonlinear estimate \eqref{eq:main_Up} and Lemma \ref{lem1}
that:
\[
A_0= O(\cE_1)-\epsilon_2 \frac{z\cdot\nabla\bar{U}}{\bar{U}}\,,
\quad A_1 = - ( \f{1}{2} z + \Pc z) + O(\cE_1)  ,\quad |\Pc| \les \cE_1.
\]
Next, we define a barrier function $F = \bar U^{ - 4 \e_2}$.  
%for $b$ to be chosen so that $\cP_U F \leq 0$. 
Since $|z \cdot \na F | \les F, |\na^i F| \les F, i=1,2 $, we get
%A direct computation yields
\[
\bal
\cP_U F & = ( O(\cE_1)- \e_2 \f{z \cdot \na \bar U}{\bar U}  
+ \f{ A_1 \cdot \na F }{F} ) F  + \tr(\Qc \na^2 F ) \\
& = (  O(\cE_1)   -\e_2 \f{ z \cdot \na \bar U}{\bar U} - \f{1}{2} \f{z \cdot \na F}{F}  ) F
=  ( O(\cE_1) -  (\e_2 - 2 \e_2) \f{z \cdot \na \bar U}{\bar U} )F 
= (O(\cE_1) + \e_2 \f{z \cdot \na \bar U}{\bar U} )F.
\eal
\]
- For $|z|\geq 1$, we derive by the form of $\bar{U}$ in \eqref{ss-}  the lower bound $-\frac{z\cdot\nabla\bar{U}}{\bar{U}}\geq \mu_{U,2}$ for some positive constant $\mu_{U,2}$\,. Recall the definition of $\cE_1$ \eqref{eq:lot} and $E \les 1$ from \eqref{eneq} and Assumption \eqref{eq:boot_EE}. Since $|\Qc| \les \tr(\Qc)$, for some positive constant $\mu_{U,1}$, we have 
\begin{equation}\label{max-g1}
%A_0\geq C_1\epsilon_2 - C_2(|Q|+H^{p-1}) \,.
A_0\geq \mu_{U,2}\epsilon_2 - \mu_{U,1}( \tr(\Qc)+H^{p-1} + E) \,,
\quad \cP_U F \leq (  \mu_{U,1}( \tr(\Qc)+H^{p-1} + E) - \mu_{U, 2} \e_2 ) F.
 \end{equation}

\noindent - For $|z|\leq 1$, since $\rho$ is bounded on the interval and we recall the definition of $\Gamma$ \eqref{ee}, we can estimate 
\begin{equation}\label{max-l1}
U\rho=\bar{U}^{-\epsilon_2}+W\rho\geq 4 C_b-C\Gamma\geq 4 C_b- \mu_{U,3} E\,,
 \end{equation}
for some positive constant $\mu_{U,3}$. Here we use the definition of $C_b$ in Assumption \ref{asss}.

Hence, by enforcing $E, |\Qc|+H^{p-1}$ sufficiently small, we will verify the following bootstrap assumption.

\begin{assumption}\label{ass:lower}
\beq\label{eq:boot_lower}
A_0 > 0, \  \cP_U F < 0, \quad  |z| \geq 1, \quad   \ U \rho > 2 C_b,  \ |z| \leq 1.
\eeq

\end{assumption}

Now, we consider $\Om_{ c} = U \rho + c F$ for $c >0$. From Corollary \ref{cor:decay} and the choice of $\e_2$, we obtain 
\[
 U \rho \les \la z \ra^{\s + \e /2} \la z \ra^{-\s + \e / 2 } 
 = \la z \ra^{\e},
 \quad F = \bar U^{-4 \e_2} \gtr \la z \ra^{ 8 \e_2/(p-1)} \gtr \la z \ra^{2 \e}.
\]

%and $\bar U^{-4 \e_2} \approx \la z \ra^{ 8 \e_2/(p-1)} = \la z \ra^{2 \e}$
Under the assumption \eqref{eq:boot_lower} and \ref{asss},  for any $c > 0$, we have 
\[
\Om_c(z) > 2 C_b,\quad  |z| \leq 1, \quad \lim_{|z| \to \infty} \Om_c = \infty.
\]

Using the above estimates of $\cP_U$, we get 
\[
\pa_{\tau} \Om_c = \pa_{\tau} (U \rho) 
= \cP_U( U\rho + c F) - c \cP_U F = \cP_U \Om_c - c \cP_U F > \cP_U \Om_c.
\]

By choosing initial data with $ U \rho > 2 C_b$ and then applying the maximal principle to the operator $\cP_U$ on $|z| \geq 1$, we obtain 
\[
\Om_c > 2 C_b, \quad U \rho + c F \geq 2 C_b,\quad |z| \geq 1.
\]

Since $c$ is arbitrary, taking $c \to 0$, we prove $U \rho > 2 C_b$ for $|z| \geq 1$, which along with \eqref{eq:boot_lower} for $U \rho$ concludes 
$U \rho \geq 2 C_b, \forall z \in \Rb^d$ and strengthens \eqref{eq:boot_U} in Assumption \ref{asss}.  
 

In Section \ref{sec:boot}, we prove Assumption \ref{ass:lower}. 



%As a consequence, by enforcing $E, |Q|+H^{p-1}$ sufficiently small, we can derive that $L_0$ is positive on $|z|\geq 1$ and $U\rho\geq C_b$ on $|z|\leq 1$. \JC{We can then use the maximal principle on $|z|\geq 1$ to conclude.} We will make this rigorous and close the bootstrap of Assumption \ref{asss} together with the bootstrap of upper bound of the energy in the next subsection.

\subsection{Bootstrap argument and blowup}\label{sec:boot}



In this section, we prove Theorem \ref{thm:stab} by combining previous estimates and use a bootstrap argument.

%We establish the standard bootstrap argument.

%\begin{proof}
Recall the ODE of $Q$ from Lemma \ref{lem1} and $\cE_0, \Ga$ from \eqref{ee}
\beq\label{eq:EE_ODE}
  %\pa_{\tau} Q = - Q^2 + O(|Q| \cE_0), \quad \cE_0 = |Q|(\Ga + \Ga^4) + H^{p-1}. 
  {\Qc}_\tau=-(\Qc_u+\frac{1}{2}\Qc_d)\Qc-\Qc(\Qc_u^T+\frac{1}{2}\Qc_d)+ \Oc(|\Qc| \Ec_0), \quad \cE_0 = |\Qc|(\Ga + \Ga^4) + H^{p-1}. 
\eeq
% Since all matrices norm are equivalent, for a positive semi-definite matrix $A$, we define its norm using the trace
% \[
% |A| := \tr(A) 
% \]

Since the parameters $\nu_i$ in the energy $E$ \eqref{eneq} have been chosen as some absolute constants, under the bootstrap assumption \ref{asss}, we get 
 \beq\label{eq:EE_ga}
E \les 1, \quad 
\Ga \les E_0 + E_K \les E \les 1,  \quad \cE_0 \les |\Qc| \Ga + H^{p-1}
\les |\Qc| E + H^{p-1}.
\eeq

Taking trace on both side of \eqref{eq:EE_ODE} and then using $\Qc = \Qc_u + \Qc_u^T + \Qc_d$,
\[
\bal
& \tr( (\Qc_u + \f{1}{2} \Qc_d) \Qc + \Qc(\Qc_u + \f{1}{2} \Qc_d )^T )
= \tr( (\Qc_u + \f{1}{2} \Qc_d + \f{1}{2} \Qc_d + \Qc_u^T  )  \Qc ) = \tr(\Qc^2), \\
 & |\Qc| \approx \tr(\Qc), \quad 
\tr(\Qc^2) = %\sum_{i=1}^d 
\sum \lambda_{\Qc,i}^2 \geq \f{1}{d}( \sum \lambda_{\Qc,i})^2 =
 \f{1}{d} ( \tr (\Qc))^2  ,
 \eal
 \]
 where $\lambda_{\Qc, i}$ is the eigenvalue of $\Qc$,  and the above estimates, we get for a constant $\mu_2$:
%It follows 
\beq\label{eq:EE_ODE2}
\pa_{\tau} \tr (\Qc) \leq - \tr(\Qc^2) + \mu_2 ( E \tr(\Qc)^2  + H^{p-1} \tr(\Qc))
\leq  - \f{1}{d}  (\tr \Qc)^2 + \mu_2 ( E (\tr \Qc)^2 + H^{p-1} \tr(\Qc) ).
\eeq

Recall $c_W$ from \eqref{per_ansatz}. To simplify the nonlinear estimates, in addition to bootstrap assumption \ref{asss}, we impose the following assumption 

\begin{assumption}\label{ass:refine}
\beq\label{eq:boot_refine}
|c_W| < \f{1}{2} \min( (p-1)^{-1}, 1), \quad E(\tau) < \min( \f{1}{ 4 d \mu_1} , \f{\e}{ 32 \mu_2} ) , 
\eeq
where $\mu_1$ is the constant in \eqref{eneq}. We denote 
%Under the Assumptions \ref{asss} and 
\beq\label{eq:EE_nota}
 \e_1 = \mu_2 H^{p-1}, \quad a(\tau) = \exp( \mu_2 \int_0^\tau H^{p-1}(s) ds),
 \quad \lam = \f{\e}{32}. 
\eeq
\end{assumption}


\noindent 
\textbf{Consequence of bootstrap assumptions.} 
We perform the energy estimates under the assumptions \eqref{eq:boot_refine} and \ref{asss} and show that these estimates can be strengthened.

%Assuming \eqref{eq:boot_refine} and 
Using \eqref{eq:dyn_scal1}, \eqref{per_ansatz}, we obtain 
$(p-1) c_U(s) = -1 + (p-1) c_W(s) \leq -\f{1}{2}$ and 
\beq\label{cUUU}
H^{p-1}(\tau) \leq H^{p-1}(0) \exp(\int_0^{\tau} (p-1)c_U(s) d s)
%\leq H^{p-1}(0) \exp(\int_0^{t} (-1 + \f{1}{10} )d s)
\leq H^{p-1}(0) \exp( - \tau / 2),
\quad - \f{1}{d} + \mu_2 E(\tau) < - \f{1}{2 d}.
\eeq

%Denote $E_\Qc  = \tr(Q)$. 
%Denote $E_\Qc  = \tr(Q)$. 
We can solve the ODE of $(\tr(Q))^{-1}$ using the above estimate and \eqref{eq:EE_ODE2} to obtain 
\[
\pa_{\tau} E_\Qc ^{-1} \geq \f{1}{2d} - \mu_2 H^{p-1} E_\Qc ^{-1},\quad E_\Qc  := \tr(\Qc). 
\]



By choose $H^{p-1}(0)$ small enough such that $ \exp(2  \e_1 )  < 2$, for any $0\leq s \leq \tau$, we get 
\[
a(\tau) a(s)^{-1} \leq e^{ \e_1 \int_0^\tau \exp(-s/2) d s  } \leq e^{ 2 \e_1}  < 2,
\quad a(\tau)^{-1} a(s) > \f{1}{2},  \quad a(0) = 1.
\]

Solving the above ODE, we yield 
\beq\label{eq:EE_ODE3}
\bal
  E_\Qc ^{-1}(\tau) & \geq a(\tau)^{-1} E_\Qc ^{-1}(0) + \f{1}{2 d} \int_0^\tau a(\tau)^{-1}  a(s)  d s 
\geq \f{1}{2} ( E_\Qc ^{-1}(0) + \f{1}{2 d} \tau  ) ,\\
 E_\Qc (\tau) & \leq  \min( 2 E_\Qc (0), 4 d / \tau ).
\eal
\eeq

Using \eqref{eq:boot_refine}, the above estimates, and $-\f{\e}{16} + \mu_1 E < - \f{\e}{32} = \lam$ \eqref{eq:EE_nota}, we obtain 
\[
 \f{d}{d \tau} E \leq -\lam E + C ( E_\Qc   + H^{p-1}(0) e^{-\tau / 2} ).
\]


Solving the ODE and using \eqref{eq:EE_ODE3}, we obtain 
\[
E(\tau) \leq e^{-\lam \tau} E(0) 
+ C \int_0^\tau e^{-\lam(\tau-s)} ( \min( E_\Qc (0) , \f{1}{s}) + H^{p-1}(0) e^{-s / 2} ) d s  ,
\]
where $C$ is some absolute constant and can depend on $\e, \lam$. Since $\lam < 1/2$, by decomposing the integral into $s < \tau / 2$ and $s \geq \tau/2$, we obtain 
\beq\label{eq:EE_E}
\bal
E(\tau) & \leq e^{-\lam \tau} ( E(0) + C H^{p-1}(0) )
+ C \B( E_\Qc (0) \int_0^{\tau/2} e^{-\lam(\tau- s)} d s +  \int_{\tau/2}^\tau e^{-\lam(\tau-s)} \min(E_\Qc (0), 1 / \tau) d s \B) \\
& \leq e^{-\lam \tau/2} (E(0) + \mu_3 H^{p-1}(0) +\mu_3  E_\Qc (0)) + \mu_3  \min(E_\Qc (0), 1 / \tau)
\eal
\eeq
for some absolute constant $\mu_3 > 0$. 


Plugging the above estimates and \eqref{eq:EE_ga} into Lemma \ref{lem1}, and using $E \les 1$ \eqref{eq:boot_refine}, we get for some $\mu_4>0$:
\beq\label{eq:EE_cw}
|c_W(\tau)| < C ( E_\Qc (\tau) + E_\Qc (\tau) E(\tau) + H^{p-1}(\tau) ) 
< \mu_4 ( \min( E_\Qc (0), 1/ \tau) + H^{p-1}(0) e^{-\tau/2}).
\eeq


\noindent 
\textbf{Continuation of the bootstrap assumptions.} For initial data satisfying 
\beq\label{eq:cond_init1}
E(0) < E_*, \quad  E_\Qc (0) < E_*, \quad  H^{p-1}(0) < E_* ,
\eeq
with $E_*$ sufficiently small, we obtain from \eqref{eq:EE_ODE3}, \eqref{eq:EE_E}, \eqref{eq:EE_cw}  the following estimates 
\[
\bal
E(\tau) & \leq e^{-\lam \tau/2} E_* (1 + 2\mu_3) + \mu_3 \min(E_* , 1/\tau) < E_*(1 + 3 \mu_3),\quad 
E_\Qc (\tau)  < 2 E_* , \quad  |c_W| < \mu_4 E_* , \\
H^{p-1}(\tau) & \leq H^{p-1}(0) < E_*,
\quad E(\tau) + \tr(\Qc) + H^{p-1} < (4 + 3 \mu_3 ) E_*. 
\eal
\]

Therefore, there exists $\nu_3 >0$ such that for $E_* < \nu_3$, the bootstrap assumption \eqref{eq:boot_refine} can be strengthened and continued. Plugging the above estimates into \eqref{max-g1}, \eqref{max-l1}  we obtain 
\[
A_0 \geq \mu_{U,2} \e_2 - \mu_{U, 3}(  3 \mu_3 + 4 ) E_*,
\quad \cP_U F \leq ( \mu_{U,2} (4 + 3 \mu_3) E_* - \mu_{U,2} \e_2 ) F,
\quad U \rho \geq 4 C_b- \mu_{U,3} (1 + 3 \mu_3) E_*.
\]

By further requiring $E_*$ to be sufficiently small, the Assumption \ref{ass:lower}  can be strengthened and continued. The $L^{\infty}$ estimate in Section \ref{sec:linfty} 
strengthens \eqref{eq:boot_U} in the Assumption \ref{asss}. Using the definition \eqref{eneq} and the above estimate for $E$, we obtain 
\[
(E_0 + E_K + F_1 + F_K)(t) \leq C(\nu_1, \nu_2) E_*,
\]
which strengthens the first inequality in \eqref{eq:boot_EE} in Assumption \ref{asss} by further choosing $E_*$ to be small enough. 

For the second inequality in \eqref{eq:boot_EE}, applying the Jacobi's formula 
$ \f{d}{d \tau} \det( \Qc(\tau)) = \det (\Qc(\tau)) \tr( \Qc^{-1} \f{d}{d\tau} \Qc)$ to \eqref{norm_p} and using $\tr(A B) = \tr(B A), \Qc = \Qc_u +\Qc_d + \Qc_u^T$, we obtain 
\[
 \pa_{\tau} \det(\Qc)  = \det(\Qc) \cdot \tr(  - \Qc + O(\cE_{0}) ) .
\]
From the above estimates,  $|\Qc|$ and $\cE_0$ remain uniformly bounded for all $\tau>0$. Since $\det(\Qc(0)) > 0$, we prove $\det(\Qc) \geq \det(\Qc(0)) e^{-C \tau}$, which 
strengthens the second inequality in \eqref{eq:boot_EE}. This concludes the proof of Theorem \ref{thm:stab}.

%\end{proof}

%In summary, there exists $\nu_4 > 0$ small enough, such that for $E_* < \nu_4$ and any initial data satisfying \eqref{eq:cond_init1} and $U \rho \geq 2 C_b$, we can continue  the bootstrap assumptions \ref{asss}, \ref{ass:lower}, \ref{ass:refine}, and establish the nonlinear estimates
%\eqref{eq:EE_E}, \eqref{eq:EE_ODE3}, \eqref{eq:EE_cw}.

















% As discussed in the previous sections, we want to demonstrate that $E$ is uniformly small in time, and therefore we can close the bootstrap of Assumption \ref{asss} at the same time. 

% 	Recall the ODE of $Q$ from Lemma \ref{lem1} and $\cE_0, \Ga$ from \eqref{ee}
% 	\[
%   \pa_{\tau} Q = - Q^2 + O(|Q| \cE_0), \quad \cE_0 = |Q|(\Ga + \Ga^4) + H^{p-1}. 
% 	\]
% Since the parameters $\nu_i$ has been fixed in \eqref{eneq}, which are some absolute constants, 
% under the bootstrap assumption \ref{asss}, we get 
% \beq\label{eq:EE_ga}
% E \les 1, \quad 
% \Ga \les E_0 + E_K \les E \les 1,  \quad \cE_0 \les |Q| \Ga + H^{p-1}
% \les |Q| E + H^{p-1}.
% \eeq






% \textbf{Size of variables.} Below, we will show that $E(\tau) \leq c \la \tau \ra^{-1}$ with small $c$, $ Q(\tau) \sim \la \tau \ra^{-1} I_d, H^{p-1} \approx e^{\tau}$, which is extremelly small compared to other variables. The reader can treat as if $H^{p-1} = 0$. 



% Provided that Assumption \ref{asss} holds, applying Lemma \ref{lem1} for $c_W, Q$, 
% \[
% \bal
%  \pa_{\tau} Q^{-1} & =- Q^{-1} \cdot  \pa_{\tau} Q \cdot Q^{-1}, \quad 
% \pa_{\tau} |Q^{-1}|  = \f{1}{2} |Q^{-1}|^{-1} \pa_{\tau} \tr( Q^{-1} \cdot Q^{-1})
% = O( |\pa_{\tau} Q^{-1} |), \\
% %= |Q^{-1}|^{-1} \tr( \pa_{\tau} (Q^{-1}) \cdot Q^{-1})  ,  \\
%  \pa_{\tau} e^{\tau / 2} & = \f{1}{2} e^{\tau / 2},
% \quad \pa_{\tau} H^{p-1} = (p-1) (\bar c_u + c_W) H^{p-1} = (- 1  + O( |Q | + \cE_0) ) H^{p-1} ,
% \eal
% \]
% and \eqref{per_ansatz}, and \eqref{booten}, we obtain that 
%  %that %the ODEs for 
% $Q^{-1}$, $e^{\tau/p}H^{p-1}|Q^{-1}|$, and $G\coloneqq E|Q^{-1}|$ satisfy:
% \[
% \bal
%  \partial_\tau Q^{-1} & = I_d+O(|Q^{-1}||Q|(|Q|E +H^{p-1})|Q^{-1}|) 
% = I_d + O(E +H^{p-1}|Q^{-1}|)\,, \\
%  \partial_\tau (e^{\tau/ 2}H^{p-1}|Q^{-1}|) & = (\frac{1}{2}- 1
%  + O(|Q| + \cE_0)  )  e^{\tau/p}H^{p-1}|Q^{-1}| + (1 + E + H^{p-1} |Q^{-1}| ) e^{\tau/2} H^{p-1}
%  \\
%  & =   (\frac{1}{2}- 1
%  + O(|Q| + \cE_0 + E + H^{p-1})  )  e^{\tau/p}H^{p-1}|Q^{-1}| .
%  %\quad + O( E +H^{p-1}|Q^{-1}| )  e^{\tau/ 2} H^{p-1}
% \eal
% \]
% %where $A \succeq B$ for two symmetric matrices $A , B \in \Rb^{d \times d}$ means that $A - B $ is a positive semi-definite matrix. 
% Notice that we use $|Q^{-1}||Q|\approx 1$. This is true since $Q, Q^{-1}$ are symmetric and positive, all matrix norms are equivalent, and their $L^2$ matrix norms are their largest eigenvalues, which are reciprocal. Combining the estimate for $E$ \eqref{booten} and $Q^{-1}$, we obtain the ODE for $G = E |Q^{-1}|$
% \[
% \bal
% \partial_\tau G& \leq-\frac{\epsilon}{16}G+C( ( |Q|+H^{p-1}) |Q^{-1}| +G E )+E\partial_\tau |Q^{-1}|\\&
% \leq -\frac{\epsilon}{16}G+ C( 1+H^{p-1}|Q^{-1}| 
% + G E 
% + E+  H^{p-1} E |Q|^{-1}   )
% \leq 
% -\frac{\epsilon}{16}G+ C( 1+H^{p-1}|Q^{-1}| + G E  +   H^{p-1} G  )
%  \,.
% \eal
% \]

% Now from the ODEs, we can immediately use the bootstrap argument to conclude that there exist positive constants $C_4, C_5$ and a small positive constant $\nu_3$, such that if initially, we have $$|Q(0)|+ H^{p-1}(0)|Q^{-1}(0)|\leq \nu_3\,,\quad E(0)|Q^{-1}(0)|\leq C_5\,,$$ as long as Assumption \ref{asss} holds, we have the bootstrap bounds \begin{equation}\label{boot-b} |Q^{-1}|\geq C_4 |Q^{-1}(0)|\,,\quad H^{p-1}|Q^{-1}|\leq e^{-\tau/p}H^{p-1}(0)|Q^{-1}(0)|\,,\quad  E|Q^{-1}|\leq C_5\,.\end{equation}  

% Finally, we finish the bootstrap on Assumption \ref{asss}. By \eqref{max-g1} and  \eqref{max-l1}, we know that there exists a constant $0<\nu_4< \nu_3$, such that if initially, we have $$|Q(0)|+ H^{p-1}(0)|Q^{-1}(0)|\leq \nu_4\,,\quad E(0)|Q^{-1}(0)|\leq C_5\,,$$ then we have the estimates $L_0> 0$ on $|z|\geq 1$ and $U\rho\geq C_b$ on $|z|\leq 1$. By the maximal (minimal) principle in \eqref{max-p}, since $Q$ is positive, we derive the bootstrap bound $U\rho\geq C_b$ for all time, provided that $U(0)\rho\geq C_b$. Therefore Assumption \ref{asss} and \eqref{boot-b} holds for all time, given the initial conditions, defined in \eqref{eqn:ini}, satisfy \begin{equation}
%     \label{boot-end}|Q(0)|+ H^{p-1}(0)|Q^{-1}(0)|\leq \nu_4\,,\quad E(0)|Q^{-1}(0)|\leq C_5\,,\quad U(0)\rho\geq C_b\,.
% \end{equation}


\section{Refined asymptotics} \label{sec:refineasym}


%In this section, we establish the blowup rate of the amplitude and phase stated in Theorem \ref{thm:blp}. 
In this section, building on Theorem \ref{thm:stab}, we obtain sharp asymptotics stated in Theorem \ref{thm:blp}. %We estimate the asymptotics for the amplitude in Section \ref{sec:asym_amp}, and the asymptotics for the phase and prove $L^{\infty}$ convergence in Section \ref{sec:asym_phase}.
In Section \ref{sec:asym_amp}, we estimate the sharp blowup rates for the amplitude similarly as in \cite{hou20242}. In Section \ref{sec:asym_phase}, we estimate the asymptotics related to the phase and prove $L^{\infty}$ convergence. %We focus on initial data $(U, \Th, \Qc, H)$ satisfying  assumptions in Theorem \ref{thm:stab}. 
In Section \ref{sec:thm_proof}, we combine Theorem \ref{thm:stab}, Propositions \ref{prop:asym} and \ref{prop:linf} to prove Theorem \ref{thm:blp}. 



\subsection{Asymptotics of the amplitude and blowup rate}\label{sec:asym_amp}

We use $O_{in}$ and $C_{in}$ to track any constant depending on the norm of the initial data $\tr(\Qc(0)), \tr(\Qc^{-1}(0))$. We have the following results for the asymptotics.
\begin{proposition}\label{prop:asym}
Suppose that the initial data $(U, \Th, \Qc, H)$ satisfy the assumption in Theorem \ref{thm:stab}. We have the following asymptotics for the {modulation parameters}
\beq\label{eq:rate_asym1}
%\lim_{\tau \to \infty}  \f{H^{p-1}(\tau)}{T-t(\tau) } = 1,
%\lim_{\tau \to \infty}  
\B| \f{H(\tau)^{p-1}}{T-t(\tau) } - 1 \B| \les C_{in} \la \tau \ra^{-1}, 
\quad \lim_{\tau \to \infty} \f{\tau}{|\log( T-t(\tau))|}
= 1,
\quad \lim_{t\to T}\frac{\RR(t)}{\sqrt{(T-t)|\log(T-t)|}}= I_d .
\eeq

\end{proposition}


{%We assume that the initial data satisfies the assumptions in Theorem \ref{thm:stab}. 
%Below, 
%Since the initial data satisfies the assumptions in Theorem \ref{thm:stab}, 
%We will use the stability estimates in Theorem \ref{thm:stab} to derive the sharp blowup rate similarly as in \cite{hou20242}. 
We consider $\tau \geq 2$. %and use $O_{in}$ and $C_{in}$ to track any constant depending on the norm of the initial data $\tr(\Qc(0)), \tr(\Qc^{-1}(0))$.
Note that $E_* < 1$. We focus on the asymptotics as $\tau \to \infty$ and the decay rate in $\tau$. 

}
% We assume initial data satisfies \eqref{eq:cond_init1} and $U \rho \geq 2 C_b$, by the bootstrap argument in the previous subsection, the bootstrap assumptions \ref{asss}, \ref{ass:lower}, \ref{ass:refine}, and the nonlinear estimates
% \eqref{eq:EE_E}, \eqref{eq:EE_ODE3}, \eqref{eq:EE_cw} hold for all time. 
%  Now we derive the blowup rate similarly as in \cite{hou20242}. 

\paragraph{Refined estimate of $\Qc$.}
By inserting \eqref{eq:EE_E} and \eqref{cUUU} into \eqref{eq:EE_ODE2}, we get 
$$
\pa_{\tau} E_\Qc  \leq - \f{1}{d}  E_\Qc ^2+ C((\frac{1}{\tau}+  e^{-\lambda\tau/2}  )E_\Qc ^2+  E_\Qc e^{-\tau/2})\,,
$$
for some absolute constant $C>0$. 
% $$
% \pa_{\tau} E_\Qc  \leq - \f{1}{d}  E_\Qc ^2+\mu_2((\frac{\mu_3}{\tau}+e^{-\lambda\tau/2}E_*(1+2\mu_3))E_\Qc ^2+ E_* E_\Qc e^{-\tau/2})\,,
% $$
Since $E_Q > 0$, we arrive at the ODE 
$$
\pa_{\tau} E_\Qc ^{-1} \geq  \f{1}{d}  - C (  \frac{1 }{\tau}+e^{-\lambda\tau/2}  )- C  E_\Qc^{-1}e^{-\tau/2}\,.
% \pa_{\tau} E_\Qc ^{-1} \geq  \f{1}{d}  -\mu_2(\frac{\mu_3}{\tau}+e^{-\lambda\tau/2} E_* (1+2\mu_3))-\mu_2 E_* E_\Qc ^{-1}e^{-\tau/2}\,.
$$

{
  By introducing the integrating factor $a(\tau) = \exp( -C E_* \int_1^{\tau} e^{-s /2 } d s )$, and using the fast convergence $|a(\tau) / a(s) - 1| \les E_* e^{-s/2}, a(\tau) \geq e^{-C E_*} $ for $1\leq s < \tau$, we can solve the above ODE and obtain 
}
%As a consequence, we have the estimate that as $\tau\to\infty$, 
$$
{E_\Qc ^{-1}}\geq \frac{1}{d}\tau+O(\log\tau) 
+ E_{\Qc}^{-1}(2) e^{- C E_*} 
\geq \frac{1}{d}\tau + O_{in}(\log \tau).
$$

Since $\tr(\Qc) = \sum \lam_{\Qc, i}$, 
%By the eigenvalue decomposition, 
we know that 
\beq\label{trq}
\min(\lambda_{\Qc,i})\leq\frac{1}{d}E_\Qc \leq \frac{1}{\tau}+O_{in}(\frac{\log\tau}{\tau^2}  ).
\eeq

Next we estimate $\text{tr}(\Qc^{-1})$. From \eqref{eq:EE_ODE}, we have by \eqref{eq:EE_ga} that 
$$
\pa_{\tau}\text{tr}(\Qc^{-1})=d-2\text{tr}(\cE_\Qc  \Qc^{-1})\leq d+\mu_2(EE_\Qc +H^{p-1})\text{tr}(\Qc^{-1}).
$$
By the above estimates of $E_\Qc $, and the same estimates of $E$ and $H^{p-1}$ in \eqref{eq:EE_E} and \eqref{cUUU}, we have that for sufficiently large $\tau$, there exists a $\mu_5$ such that 
$$
\pa_{\tau}\text{tr}(\Qc^{-1})\leq d+\frac{C}{\tau^2}\text{tr}(\Qc^{-1}).
$$
We conclude that %as $\tau\to\infty$, 
$$
\tr(\Qc^{-1}) \leq {d}\tau+O(\log\tau) + \tr(\Qc^{-1}(2))
\leq {d}\tau+O_{in}(\log\tau) 
$$
Using $\tr(\Qc^{-1}) = \sum_i \lam_{\Qc, i}^{-1}$, we obtain
\beq\label{trq-1}
\max(\lambda_{\Qc,i})\geq\frac{d}{\text{tr}(\Qc^{-1})}\geq \frac{1}{\tau}+O_{in}(\frac{\log\tau}{\tau^2}).
\eeq

%Namely, we collect that as $\tau\to\infty$, 
Combining the above estimates, we obtain 
$$
{\text{tr}(\Qc^{-1})}\text{tr}(\Qc)\leq d^2+O_{in}(\frac{\log\tau}{\tau}).
$$ 
%Notice that by the eigenvalue computation, 
Using $\tr(\Qc^{\al}) = \sum \lam_{\Qc, i}^{\al}, \al = 1, -1$, we derive
$$
\text{tr}(\Qc^{-1})\text{tr}(\Qc)=\sum \lambda_{\Qc,i}\sum \lambda^{-1}_{\Qc,i}=d^2+\sum_{i<j}(\sqrt{\frac{\lambda_{Q,i}}{\lambda_{\Qc,j}}}-\sqrt{\frac{\lambda_{\Qc,j}}{\lambda_{\Qc,i}}})^2.
$$
%For any $i<j$, 
It follows 
$$\Big(\sqrt{\frac{\lambda_{\Qc,i}}{\lambda_{\Qc,j}}}-\sqrt{\frac{\lambda_{\Qc,j}}{\lambda_{\Qc,i}}}\Big)^2=O_{in}\Big(\frac{\log\tau}{\tau}\Big), \quad \forall i < j, 
\quad  \f{\max(\lambda_{\Qc,i})}{\min(\lambda_{\Qc,i})}=1 + O_{in}( (\frac{\log\tau}{\tau})^{ 1/2 } ).
$$
% In particular, we establish
% $$
%  \f{\max(\lambda_{\Qc,i})}{\min(\lambda_{\Qc,i})}=1 + O_{in}( (\frac{\log\tau}{\tau})^{ 1/2 } ).
% $$
Combining the above estimate with \eqref{trq} and \eqref{trq-1}, we have that  each one of the eigenvalue satisfies 
$$
\lambda_{\Qc,i}=\frac{1}{\tau}+ O_{in}(\tau^{-3/2}\sqrt{\log \tau} )
= \frac{1}{\tau} +  O_{in}(a_{\tau}),\quad a_{\tau} = \tau^{-3/2 + \e_3},
\quad \e_3 = \f{1}{10}.
 %(\log \tau)^{1/2} \tau^{-3/2}
$$

{
  Since $\Qc$ is symmetric and $\Qc(\tau) = R(\tau) \Lam R(\tau)^T$ for $\Lam = \mathrm{diag}(\lam_{\Qc, 1}, .., \lambda_{\Qc, d})$ and some orthogonal matrix $R$, which satisfies 
 $| R(\tau)| \leq C$ for $C$ independent in $\tau$, the above estimates further imply, 
 \beq\label{eq:asymp_Q}
 \Qc= R(\tau) \B( \f{1}{\tau} I_d + O_{in}(a_{\tau})  \B) R(\tau)^T =  \frac{1}{\tau}I_d+O_{in}(a_{\tau}) .
% \Qc= R(\tau) \B( \f{1}{\tau} I_d + O_{in}(\frac{ ( \log\tau )^{1/2} }{\tau^{3/2}}) \B) R(\tau)^T =  \frac{1}{\tau}I_d+O_{in}(\frac{ ( \log\tau )^{1/2} }{\tau^{3/2}}) . 
 \eeq
}

\paragraph{Estimate of $\RR$ and blowup rate.}
%As a consequence and by 
Recall from \eqref{per_ansatz}, \eqref{eq:Pv} 
\[
\Mc = e^{- \tau / 2}
\RR^{-1}, \quad 
\Qc = C_W^{p-1} \Mc \Mc^T = C_W^{p-1} e^{-\tau/2}  \RR^{-1} ( e^{-\tau/2} \RR^{-1})^T =
M_Q M_Q^T, \quad M_Q : = {C}_U^{(p-1)/2} \RR^{-1}.
\]
Note that $\RR, \Mc,  M_Q$ are upper triangular matrices. Due to $M_{Q, ii}(0) > 0$ and 
the non-degeneracy $ 0 < \det(\Qc) = \det(M_Q)^2 = \prod M_{Q, ii}^2 $ for all $\tau$ from \eqref{eq:boot_EE}, by continuity, we have $M_{Q, ii}(\tau) > 0$, which are the eigenvalues of $M_Q, M_Q^T$. For each real eigenpair $(\lam, v)$ of $M_Q^T$ with $ || v||_{l^2}^2 = 1$, we obtain 
\[
\lam^2 = \lam^2 || v||_{l^2}^2 =  v^T M_Q M_Q^T v = v^T \Qc v 
= \tau^{-1} || v||_{l^2}^2 + O_{in}( a_{\tau} )
= \tau^{-1} +  O_{in}( a_{\tau} ).
\]


Since $M_{Q, ii} > 0$ is a eigenvalue of $M_Q$, we obtain 
\[
M_{Q, ii} =  \tau^{-1/2} ( 1 + \tau O(a_{\tau}))^{1/2}
= \tau^{-1/2} + O( \tau^{1/2} a_{\tau})
= \tau^{-1/2} + O( (\log \tau)^{1/2} / \tau).
\]
%Since $M_{Q, ii} > 0$ is a eigenvalue of $M_Q$, 

Next, we estimate the strictly upper part of $M_Q$: $M_{\Qc}^u$. Taking {the} trace, we get 
\[
 \sum_{i \neq j} M_{Q, ij}^2
= \tr( M_Q M_Q^{T}) - \sum_i M_{Q, ii}^2
 = \tr(\Qc) -\sum_i M_{Q, ii}^2 = d /\tau - d / \tau + O(a_{\tau}) = O(a_{\tau})
\]
which implies $M_{\Qc}^u = O( a_{\tau}^{1/2})$.
%, where $M_{\Qc}^u$ is the strictly upper part of $M_{\Qc}$. 
%Finally, 
Comparing the strictly upper part $\Qc = (M_{Q,d} + M_{Q}^u) 
  (M_{Q,d} + M_{Q}^u)^T$, we get 
\[
  M_{Q}^u  M_{Q, d}  =   \Qc^u -  (M_{Q, u} M_{Q, u}^T )^u
  = O(a_{\tau}), \quad  M_Q^u =  O( a_{\tau}  ) M_{Q, d}^{-1}
  =  O( a_{\tau}  \tau^{1/2} ) .
\]

Therefore, we conclude,
\beq\label{eq:asym_M}
{C}_U^{(p-1)/2} \RR^{-1} = M_Q=\frac{1}{\sqrt{\tau}}I_d+ O_{in}( \tau^{1/2} a_{\tau})
= \frac{1}{\sqrt{\tau}}I_d+ O_{in}( \tau^{-1 +\e_3}) .
%M_Q^T M_Q = \tau^{-1} I_d + O_{in}(\tau^{-3/2 +\e_3}).
%O_{in}(\frac{\sqrt{\log\tau}}{\tau}).
\eeq





% Let $V_i \in \Rb^d$ be the $i-th$ row vector of $M_Q$ and $\la \cdot, \cdot \ra$ is the inner product. Then $ V_{k, l} = 0, l < k$. Applying the identities 
% \[
% M_Q M_Q^{T}= \Qc, \quad \Qc_{i j} = \la V_i, V_j  \ra, \quad V_{k, l} = 0, l < k,
% \]
% with $(i, j) = (d, d), (d-1, d), .., (1, d)$ in order, we obtain $V_d = 1 / \tau^{1/2} e_d + O(\e_3), \e_3 = (\log \tau)^{1/2} / \tau$,


% in the order of $(i, j) =  (d, d),(d-1, d), (d-1, d-1)..$, i.e. for $i=d, d-1, d-2,.., 1$, we use the above identities in the order of $j = d, d-1, ., 1$, 


% we have  
% $$
% {C}_U^{(p-1)/2}M_U^{-1}=\frac{1}{\sqrt{\tau}}I_d+ O_{in}(\frac{\sqrt{\log\tau}}{\tau})
% $$ 

{
% HERE
Using \eqref{eq:dyn_scal1}, we define the blowup time as $T = t(\infty)$. Using \eqref{eq:dyn_scal1} for $t(\tau)$, Lemma \ref{lem1} and \eqref{eq:boot_refine} for $c_W$, and \eqref{eq:EE_cw}, \eqref{eq:non_stab}, \eqref{eq:asymp_Q} for $\tr(\Qc), \cE_0$, we obtain 
\begin{equation}\label{tau-t}
t_{\tau} = H^{p-1}, % \quad \tau_t = H^{-(p-1)}, 
\quad (p-1) c_W =  \f{\mu_5}{\tau}  + O_{in}(a_{\tau}),  
\quad |(p-1) c_W| < \f{1}{2}, \quad a_{\tau} = \tau^{-3/2 + \e_3}, 
 \quad \mu_5 = \f{ 2(1 - \be \delta) d c_p}{p-1} .
% \quad (p-1) c_U =  (p-1)(\bar c_U + c_W)=
% -1 + \f{\mu_5}{\tau}  + O_{in}(a_{\tau}),   \quad
% \mu_5 = \f{ 2(1 - \be \delta) d c_p}{p-1} .
\end{equation}

Using \eqref{eq:dyn_scal1}, \eqref{per_ansatz}, for $\tau \geq 2, s>0$, we obtain
%using $\int_{\tau}^{\tau + s} a_z d z = O( (\log \tau)^{1/2} \tau^{-1/2} ) = O(a_{\tau} \tau)$,  we obtain
\[
\f{H^{p-1}(\tau +s) }{ H^{p-1}(\tau) }
%= e^{-s} \f{C_W^{p-1}(\tau+s)}{C^{p-1}_W(\tau)}
= e^{-s} F(\tau, s), 
\quad F(\tau, s) := e^{ (p-1) \int_{\tau}^{\tau+s} c_W(z) d z }. %\leq e^{s/2}.
\]

Since $|(p-1)c_W(s)| < \min( \f{1}{2}, C  \tau^{-1})$, using $|e^x - 1| \les |x| (e^x + 1),
\pa_s F(\tau, s) = (p-1) c_W(\tau + s) F(\tau, s), F(\tau, 0)=1$, for $0\leq z  \leq s$,  we obtain 
\[
\bal
 |F(\tau , s) -1| & \les s / \tau ( F(\tau, s) + F(\tau,0)) \les e^{s/2} s / \tau, \\
 |c_W(\tau+z) - \mu_5 \tau^{-1} |
& \les | (\tau + z)^{-1} - \tau^{-1}| + a_{\tau}
\les z \tau^{-2} + a_{\tau}, 
\eal
\]
which implies 
\[
\bal
 | c_W(\tau + z) F(\tau, z) - \mu_5 \tau^{-1}|
& \les | c_W(\tau + z) ( F(\tau, z) - 1) + (c_W(\tau+z) - \mu_5 \tau^{-1})|
\les a_{\tau} + e^{z/2} z \tau^{-2} + z\tau^{-2} , \\
 |F(\tau, s) - 1  - s \mu_5 \tau^{-1}| 
&\les s \max_{0\leq z \leq s}  | c_W(\tau + z) F(\tau, z) - \mu_5 \tau^{-1}|
\les e^{s/2} s^2 \tau^{-2} + s \tau^{-3/2 + \e_3}.
\eal
% | F(\tau, s) - 1 - s \pa_s F(\tau , 0)|
%  \les | \int_0^{s} ( c_W^(\tau + z) F(\tau, z) - c_W(\tau) ) d z |
\]

Therefore, integrating $\f{H^{p-1}(\tau +s) }{ H^{p-1}(\tau) }$  for $s$ from $0$ to $\infty$ and using the above estimates, we get 
\beq\label{eq:t_tau}
\bal
\f{T-t(\tau) }{H^{p-1}(\tau)}
 & = \int_{0}^{\infty} \f{H^{p-1}(\tau +s) }{ H^{p-1}(\tau) } d s
= \int_{0}^{\infty} e^{-s} F(\tau, s) d s
=  \int_0^{\infty}  (1 + \mu_5 s \tau^{-1}) e^{-s} d s 
+O_{in}(\tau^{-3/2 + \e_1}) \\
& = 1 + \mu_5 \tau^{-1} +O_{in}(\tau^{-3/2 + \e_1}),
\eal
\eeq
where we use $\int_0^{\infty} s e^{-s} ds=1$. Since $(p-1) c_U = (p-1) (\bar c_U + c_W ) = - 1 + O(\tau^{-1})$, we further obtain 
\beq\label{eq:t_tau2}
\log ( T-t(\tau))
= (1 + O(\tau)^{-1}) \log( H^{p-1})
= (1 + O(\tau)^{-1} ) ( O_{in}( 1 ) + \int_0^{\tau} (p-1) c_U ) 
%= (1 + O(\tau)^{-1} ) ( O_{in}( 1 ) - \tau + O_{in}(\log(\tau)) ) 
= - \tau + O_{in}(\log(\tau)) .
\eeq

Combining \eqref{eq:asym_M}, \eqref{eq:t_tau}, \eqref{eq:t_tau2}, we prove \eqref{eq:rate_asym1} and Proposition \ref{prop:asym}.
%  we conclude
% \[
% \lim_{\tau \to \infty}  \f{H^{p-1}(\tau)}{T-t(\tau) } = 1,
% \quad \lim_{\tau \to \infty} \f{\tau}{|\log( T-t(\tau))|}
% = 1,
% \quad \lim_{t\to T}\frac{\RR}{\sqrt{(T-t)|\log(T-t)|}}= I_d .
% \]
% This renders the correct blowup rate of the amplitude in Theorem \ref{thm:blp}.


% Integrating the above esitmates for $s$ from $0$ to $\infty$ and using integration by parts, we yield 
% \[
% \bal
% J &=\f{T-t(\tau) }{H^{p-1}(\tau)}
%  = \int_{0}^{\infty} \f{H^{p-1}(\tau +s) }{ H^{p-1}(\tau) } d s
% = \int_{0}^{\infty} e^{-s} F(\tau, s) d s
% = \int_{0}^{\infty}  F(\tau, s) d (- e^{-s})
% = 1 + \int_0^{\infty} \pa_s F(\tau, s) e^{- s} d s ,
% \eal
% \] 
% where we have used $F(\tau, 0) = 1$. Since $ \pa_s F(\tau, s)
% = (p-1)  c_W(\tau + s) F(\tau, s)
% = (\f{\mu_5}{\tau +s} + O(a_{\tau })) F(\tau, s), F(\tau, s) e^{-s} \leq e^{s/2}$, we get
% \[
% J = 1 + I_1  + I_2, \ |I_1| \les   a_{\tau} \int_0^{\infty}  F(\tau, s) e^{-s} d s  \les a_{\tau},
% \quad I_2 = \mu_5 \int_0^{\infty} \f{1}{\tau + s} F(\tau, s) e^{-s} d s .
%  \]

% Applying integration by parts to $I_2$, we get 
% \[
% I_2 = \mu_5 \int_0^{\infty} \f{1}{\tau + s} F(\tau, s) d -e^{-s}
% = \f{\mu_5}{\tau} + \mu_5 \int_0^{\infty} \pa_s(\f{1}{\tau + s} F(\tau, s) ) e^{- s} d s
% = \f{\mu_5}{\tau} +  \int_0^{\infty} O(\tau^{-2}) F(\tau, s) e^{- s} d s
% = \f{\mu_5}{\tau} +  \int_0^{\infty} O(\tau^{-2}) e^{- s/2} d s
% =  \f{\mu_5}{\tau} + \tau^{-2}.
% \]


% Using \eqref{eq:dyn_scal1} again, we conclude that 
% \begin{equation}
%     \label{eq:t_tau}
%     \lim_{t\to T} \f{T-t}{ H^{p-1} }
%     = \lim_{\tau \to \infty} \int_{\tau}^{\infty}  H^{p-1}(s) /H^{p-1}(\tau) d s    
%     \quad\lim_{t\to T}\frac{\tau}{|\log(T-t)|}=1\,,
% \end{equation} 
}

% We can conclude that there exists a blowup time $T>0$, such that 
% \begin{equation}
%     \label{eq:t_tau}\lim_{t\to T}\frac{{C}_U^{p-1}}{T-t}=1\,,\quad\lim_{t\to T}\frac{\tau}{|\log(T-t)|}=1\,,
% \end{equation} 
% which implies 
% $$
% \lim_{t\to T}\frac{M_U}{\sqrt{(T-t)|\log(T-t)|}}= I_d\,.
% $$
% This renders the correct blowup rate of the amplitude in Theorem \ref{thm:blp}.


\subsection{Asymptotics of phase and $L^{\infty}$ convergence}\label{sec:asym_phase}



{
In this section, our goal is to prove the following convergence.

\begin{proposition}\label{prop:linf}

Suppose that the initial data $(U, \Th)$ satisfy the assumption in Theorem \ref{thm:stab}. We have 
\beq\label{eq:linf_conv}
| U(z, \tau) e^{ \imath (\Th -  A(\tau))  } - \bar U^{1 + \imath \d} |   \les 
 \min( \la z\ra^{\s +\e/2} \la \tau \ra^{-\e}, \la \tau \ra^{\max(-1, 2 \s)} ).
\eeq
where $A(\tau)$  satisfies the following estimate for some constant $C_{in}$ depending on the initial data
\beq\label{eq:phi0_asym1}
|A -  \bar A| \leq C_{in} ,
\quad 
A(\tau) := \frac{\delta}{p-1}\tau+\Phi(\tau, 0) ,
\quad 
\bar A(\tau):= - \frac{\delta \log (T-t(\tau))}{p-1}-\frac{d\beta(1+\delta^2)\log|\log (T-t(\tau))|}{2 
\flat_*} .
\eeq

\end{proposition}

}




\begin{proof}

We will first estimate $\Phi(0)$ and then prove convergence. 
%We assume that $ T - t(\tau) < 1$ since we only need to prove \eqref{eq:linf_conv} for large $\tau$. Then we have $\log( T- t(\tau)) < 0$.

\paragraph{Estimate of $\Phi(0)$.}


% For the phase $\Theta=\bar{\Theta}+\Phi$, we have weighted estimates for the gradient of $\Phi$ and recall the definition of $\bar{\Theta}$ in \eqref{ss-}. Below, our goal is to obtain the following asymptotics
% \beq\label{eq:phi0_asym1}
% |A - B| \leq C_{in} ,
% \quad 
% A := \frac{\delta}{p-1}\tau+\Phi(0) ,
% \quad 
% B:=  \frac{\delta|\log (T-t(\tau))|}{p-1}-\frac{d\beta(1+\delta^2)\log|\log (T-t(\tau))|}{2 
% \flat_*} .
% %L.H.S.\coloneqq\frac{\delta}{p-1}\tau+\Phi(0)\to\frac{\delta|\log (T-t)|}{p-1}-\frac{d\beta(1+\delta^2)\log|\log (T-t)|}{2(p-\delta^2-\beta\delta(1+p))}\coloneqq R.H.S\,.
% \eeq
%We compute the derivative in $\tau$.  %For the left hand side, 
Firstly, we compute $A_{\tau}, \bar A_{\tau}$. Using \eqref{imaginep}, we perform similar computations to the proof of Lemma \ref{lem1} to compute that 
$$
\Phi_\tau(0)=-v\cdot\nabla\Phi(0)+\mathscr{D}_\Theta(0)= O( \cE_0)+(\beta+\delta)\frac{\kappa_2}{\kappa_0}\text{tr}(Q)\,.
% \Phi_\tau(0)=-v\cdot\nabla\Phi(0)+\mathscr{D}_\Theta(0)= O( \cE_0)+(\beta+\delta)\frac{\kappa_2}{\kappa_0}\text{tr}(Q)\,.
$$

Applying \eqref{eq:asymp_Q} and the estimates \eqref{eq:non_stab}, \eqref{eq:EE_ga} for $\cE_0$, we yield
\[
\bal
%& A_\tau=\frac{\delta}{p-1} + \frac{d(\beta+\delta) \kp_2}{ \kp_0 \tau}+O(\frac{ (\log\tau)^{1/2} }{\tau^{3/2}}),  \\
%& B_\tau=\frac{\delta}{p-1}\frac{t_\tau}{T-t}-\frac{d\beta(1+\delta^2)t_\tau}{2(p-\delta^2-\beta\delta(1+p))|\log (T-t)|(T-t)}\,.
 & A_{\tau}(\tau)=\frac{\delta}{p-1}-\frac{d(\beta+\delta)}{2 \flat_* \tau}+
 O_{in}(\tau^{-3/2 + \e_1}), \quad 
  \bar A_{\tau}(\tau)=\frac{\delta}{p-1}\frac{t_\tau}{T-t}-\frac{d\beta(1+\delta^2)t_\tau}{2 \flat_* |\log (T-t)|(T-t)}\,.
\eal
\]

{
Using $t_{\tau} = H^{p-1}$  \eqref{tau-t}, \eqref{eq:t_tau}, and \eqref{eq:t_tau2}, we yield 
\[
 \f{t_{\tau}}{ T- t(\tau)}
 = \f{H^{p-1}}{T- t(\tau)}
  = 1 - \f{\mu_5} {\tau} + O_{in}(\tau^{-3/2 + \e_1}),  \quad
   \f{t_{\tau}}{ (T-t)\log( T- t)}
   = \f{1}{\tau} + O_{in}(\log(\tau) \tau^{-2}).
\]
} 
Using the definition of $\mu_5$ \eqref{tau-t}, $c_p$ \eqref{ss-}, we conclude
\begin{align*}
A_{\tau} - \bar A_{\tau} &=  ( - \f{ d( \beta + \d)}{2 \flat_*} + \f{\mu_5 \d}{p-1} 
 + \f{ d \beta(1 + \d^2) }{2 \flat_*} ) \f{1}{\tau} + O_{in}(\tau^{- \f{3}{2} + \e_3})\\
 &= \f{\d}{\tau}( \f{2 (1 - \beta \d) d c_p }{(p-1)^2} - \f{d (1-\be \d)}{2 \flat_*} ) 
 + O_{in}(\tau^{- \f{3}{2} + \e_3}).
\end{align*}
The first term vanishes due to \eqref{ss-} for $c_p$. Since the error term is integrable in $\tau \geq 2$, we conclude the asymptotics of the phase \eqref{eq:phi0_asym1}.

%We finally discuss the implications of the initial conditions \eqref{boot-end}, where we recall the initial normalizing conditions are defined in \eqref{eqn:ini}.
%\end{proof}

% \subsubsection{Special case: $d=1$}

% For $d=1$, $\Qc$ reduces to a scalar and $\Qc_u = 0$. We estimate $\Qc$ directly using \eqref{eq:EE_ODE} and applying \eqref{eq:non_stab}, \eqref{eq:EE_ga} for the error term $\cE_0$, we obtain 
% \[
% \pa_{\tau} \Qc^{-1} = 1 + O( E ) + O( e^{ - \tau / 2 } \Qc^{-1} ).
% \]

\paragraph{$L^{\infty}$ convergence.}

%Recall the decomposition 
Recall $ \Th = \bar \Th + \Phi$ \eqref{per_ansatz}. Integrating \eqref{eq:inte:4} with $l=1$, we obtain 
\beq\label{eq:linf_phi}
|\Phi(z) - \Phi(0)| \les \int_0^{1}  |\na \Phi( t z ) | d t 
\les E \int_0^1 \la t z \ra^{-1/2} d t \les E \la z \ra^{1/2}.
\eeq

Using $U = \bar U + W$ \eqref{per_ansatz}, we decompose
\[
J := U e^{ \imath (\Th - \bar \Th - \Phi(0))} - \bar U
 = U e^{ \imath (\Phi - \Phi(0))} - \bar U
 = W e^{ \im (\Phi - \Phi(0))} 
 + \bar U (e^{ \im (\Phi - \Phi(0)) }  - 1) =  I + II.
\]

Appyling \eqref{eq:inte:3} to $I$, \eqref{eq:linf_phi} and $|e^{\im x } - 1| \les \min(|x|, 1)$ to $II$, and $E \les \la \tau \ra^{-1}$ \eqref{eq:non_stab}, we prove
\[
\bal
|J| & \les \la z \ra^{\s + \e/2} E 
+ \la z \ra^{\s} \min( E \la z \ra^{1/2}, 1)
\les \min( \la z \ra^{\s + \e/2} ( E + E^{ \e} )  , E + E^{- 2\s})  \\
& \les 
 \min( \la z\ra^{\s +\e/2} \la \tau \ra^{-\e}, \la \tau \ra^{\max( -1, 2 \s)} ).
%\min( \la z\ra^{\s +\e/2} (1 + \tau)^{-\e}, (1 + \tau)^{\min(1, -2 \s)} ).
\eal
\]
Since $\Th - \bar \Th - \Phi(0) + \d \log \bar U 
= \Th - A(\tau)$ \eqref{ss-} and \eqref{eq:phi0_asym1}, we get $ U^{ \imath \d} J  =   U e^{ \imath (\Th - A(\tau))} - \bar U^{1 + \imath \d} $. Since $| U^{ \imath \d}| = 1$, the above estimate conclude the proof of \eqref{eq:linf_conv}.
\end{proof}

\subsection{Proof of Theorem \ref{thm:blp}}\label{sec:thm_proof}

In this section, we prove Theorem \ref{thm:blp} with the open set $\Oc$ prescribed in Remark 
\ref{rem:blowup}. 

\

\noindent \textbf{Verification of assumptions in Theorem \ref{thm:stab}.} We first choose $\nu < 1$ in \eqref{eq:ass_init2} for Theorem \ref{thm:blp}. Following the proof of Corollary \ref{cor:decay}, we obtain $U_0 \les \la z \ra^{\s + \e/2}$. Using the definitions \eqref{norm:Ek} of $F_K$ and  \eqref{def:EKFKbar} of the norm {$\bar {\mfr F}_K$}, and \eqref{wg:rho}, we get 
\[
%U_0 \geq C \la z \ra^{\s - \e/2},\quad 
 \mr \rho_K = \rho_K U^2 \leq  C \la z \ra^{2 \s + \e}\rho_K \geq C (1 + |z|^{ - d - 2 K } ),\quad
F_K \leq C {\|\Phi\|_{\bar {\mfr F}_K} }.
\]
From  \eqref{def:EkFk}, \eqref{eneq}, we obtain $E \leq C E_{in}$. 
%Since $E_{sim}$ \eqref{eq:E_sim} and $E$ \eqref{eneq} are equivalent, 
By choosing $\nu = c E_*$ in \eqref{eq:ass_init2} with $c>0$ sufficiently small, the assumptions \eqref{eq:ass_init2} implies the assumptions \eqref{eq:thm_stab_ass} in Theorem \ref{thm:stab} except for $E_{\Qc} < E_*$. Using the definitions of $\Mc_0, H(0)$ \eqref{eq:init_res} 
$\cR_0, \Qc$ \eqref{eq:Pv},  and $C_W(0) = H(0)$ \eqref{per_ansatz}, we obtain 
\[
\tr(\Qc(0)) = H(0)^{p-1} \tr(\Mc \Mc^T) = 
H(0)^{p-1} \tr( \Mc^T \Mc) =  C u_0(V_0)^{-p} \tr( \na^2 u_0(V_0))
\]
for some absolute constant $C$. Therefore, by further choosing $ c$ small in $\mu = c E_*$, we obtain $|E_{\Qc}| < E_*$ from the last assumption in \eqref{eq:ass_init2}.  
We verify the assumptions in Theorem \ref{thm:stab} and can use the results in Theorem \ref{thm:stab}, and Propositions \ref{prop:asym} and \ref{prop:linf}.


For the time $t$ in Theorem \ref{thm:blp}, we use the change of variables $t = t(\tau)$ \eqref{eq:dyn_scal1}. Then we only need to prove Theorem \ref{thm:blp} in terms of the self-similar time $\tau$.

\

\noindent \textbf{Proof of estimates \eqref{est:asymptoticEKFK}, \eqref{eq:thm_estb}.}
Using Theorem \ref{thm:stab}, we obtain the estimates \eqref{eq:non_stab}, which along with the relation between $(U , \Th), (u, \th)$ and $W = U - \bar U, \Phi = \Th - \bar \Th$ prove \eqref{est:asymptoticEKFK} in Theorem \ref{thm:blp}. 

To obtain \eqref{eq:thm_estb} and \eqref{est:limitmu}, we choose $\mu(t(\tau)) = A(\tau), \hat \mu(t) = A(\tau) - \bar A(\tau) $. Using 
$ \Th - A = \Th - \bar A -  \hat \mu $ and the formula of $\bar A$ \eqref{eq:phi0_asym1}, we obtain  
\[
\bal
J: & = |\log(T-t)|^{\imath  \frac{d\beta (1 + \delta^2)}{2\flat_*}} (T-t)^{\frac{1 + \imath \delta}{p-1}}  \psi( \RR(t) z + \Vc(t) , t )  e^{ -\imath \hat \mu(t) }
= (T-t)^{ \f{1}{p-1} } H^{-1} U(z, \tau) e^{ \imath ( \Th(z, \tau) - \bar A - \hat \mu ) }\\
& = (T-t)^{ \f{1}{p-1} } H^{-1} U(z, \tau) e^{ \imath ( \Th(z, \tau) - A(\tau) ) } .%:=  (T-t)^{ \f{1}{p-1} } H^{-1} J_2. 
 \eal
\]

We denote
\[
J_2 =  U(z, \tau) e^{ \imath ( \Th(z, \tau) - A(\tau) ) } .
\]


Using the limits $H(\tau) / (T-t)^{1/(p-1)} \to 1$ and $\tau / |\log(T-t(\tau))| \to 1$ as $\tau \to \infty$ \eqref{eq:rate_asym1},  and the estimate \eqref{eq:linf_conv}, we prove 
\begin{align*}
|J  - \bar U^{1 + {\imath} \d}|
&\les | (T-t)^{ \f{1}{p-1} } H^{-1} - 1| \cdot 
 |\bar U^{1 + {\imath} \d}| 
 + (T-t)^{ \f{1}{p-1} } H^{-1} |J_2 -\bar U^{1 + {\imath} \d} | \\
 &\les C_{in}  (1 + \tau)^{\eta}
 \les C_{in}(1 + |\log( T-t(\tau))| )^{\eta},
\end{align*}
where $\eta = \max(-1, 2 \s)$. 

\ 

\noindent \textbf{Proof of rates \eqref{est:limitHRV}, \eqref{est:limitmu}.} {Next, we show that $V(\tau)$ converges as $\tau \to \infty$ in \eqref{est:limitHRV}. From Lemma \ref{lem1} for $\Vc$, the decay estimates for $\Qc, E$ in Theorem \ref{thm:stab}, and $\RR(\tau) \to 0$ as $\tau \to \infty$ in Proposition \ref{prop:asym}, we obtain 
\[
 | \RR(\tau) \Vc(\tau) | \les (1 + \tau)^{-2}.
\]
Since the upper bound is integrable in $\tau$, using $|  V_{\tau}(\tau) | = | \RR(\tau) \Vc(\tau)| $ \eqref{eq:Pv}, we prove that $V(\tau)$ converges as $\tau \to \infty$.} The asymptotics \eqref{est:limitmu} follows from the definition of $\mu$ and \eqref{eq:rate_asym1}.This ends the proof of Theorem \ref{thm:blp}. 


\subsection{Proof of Theorem \ref{cor:stab}}\label{sec:cor_pf}

To prove Theorem \ref{cor:stab}, we only need to show that for $\e_0 = \e_0(u_0)$, assumption \eqref{eq:ass_cor} implies that $\td u_0$ is in the open set $\Oc$ in Theorem \ref{thm:blp}. 

\

\noindent  \textbf{Estimates of $\td V_0, \td \Mc_0, \td H_0$.}  Since $V_0$ is the unique maximizer and $\na^2 u_0(V_0) \succ 0$, for $\d_1$ sufficiently small, 
we obtain that $\td u_0$ admits a global non-degenerate maximizer $\td V_0$ close to $V_0$ 
\footnote{Since for any $\d > 0$, there exists a $r > 0$, such that 
$u_0(V_0) > u_0(V_0 + z) + \d, |z| > r$, we obtain $|\td V_0 - V_0| < r$ when $\d_1 < \d / 2$.
}
with $|V_0 - \td V_0| \to 0$ as $||\td u_0 - u_0||_{L^{\infty}} \to 0$. Using embedding \eqref{eq:inte:3} in Proposition \ref{prop:inter}, we obtain 
\[
||u_0 - \td u_0||_{C^2} \les || u_0 - \td u_0 ||_{\cH^K} . 
\]
Denote 
\[
\d_1 := || u_0 - \td u_0 ||_{\cH^K} ,
\quad \d_2 := |V_0 - \td V_0| .
\]
%where $\td V_0$ is a global maximizer of $\td u_0$ to be defined. 
Using continuity and the above embedding, we obtain
\bseq
\beq\label{eq:cor_small1}
\lim_{\e_0 \to 0}  |\td V_0 - V_0| = 
\lim_{\e_0 \to 0}  \d_2 =0, \quad | \td u_0(\td V_0) - u_0(V_0) | \les \d_1 + \d_2, 
%|\td V_0 - V_0|, 
\quad | \na^2 \td u_0(\td V_0) - \na^2 u_0(V_0) | \les \d_1  + \d_2. 
%|\td V_0 - V_0|. 
\eeq




Upon choosing $\e_0 > 0$ small, we can define the initial {modulation parameters} \eqref{eq:init_res} $\td H_0, \td \Mc_0$ associated with $\td u_0$ and obtain 
\beq\label{eq:cor_small2}
\lim_{\e_0 \to 0} |\td \Mc_0 - \Mc_0 | + | H_0 - \td H_0| = 0.
\eeq

\eseq


We denote by $\td U_0$ the rescaled variables for $\td u_0$: 
\beq\label{eq:cor_pf1}
\td U_0 = \td H_0 \td u_0( \td \Mc_0^{-1} z + \td V_0 ) .
\eeq


\noindent  \textbf{Verification of assumptions.}  We show that $( \td u_0, \td U_0)$ satisfies assumptions \eqref{eq:ass_init2}. The implicit constants can depend on $u_0$. 



Firstly, assumptions \eqref{eq:ass_init}, \eqref{eq:ass_init2} for $\td u_0$ except for 
\beq\label{eq:cor_pf2}
\td U_0 \bar U^{-1 - \e_2} > 2 C_b
\eeq
follow from continuity and choosing $\d_1$ small. Condition \eqref{eq:cor_pf2} follows from 
the assumption \eqref{eq:cor_pf2} for $U_0$, \eqref{eq:ass_cor}, the triangle inequality, and choosing $\e_0$ small.

Next, we verify \eqref{def:EKFKbar} for $\td U_0$, i.e. 
 \beq\label{eq:cor_small0}
|| \td U_0 - \bar U_0 ||_{\mfr E_K} < \nu .
 \eeq
 Using the definition \eqref{eq:cor_pf1}, we decompose $\td U_0 - \bar U$ as follows 
\beq\label{eq:cor_J}
 \td U_0 - \bar U
=  \td H_0 \B(  \td u_0( \td \Mc_0^{-1} z + \td V_0 )
 - u_0( \td \Mc_0^{-1} z + \td V_0 ) \B)  
 + \B( \td H_0 
  u_0( \td \Mc_0^{-1} z + \td V_0 ) - \bar U_0  \B) := J_1 + J_2. 
\eeq

For $J_1$, using a change of variable, \eqref{eq:cor_small1}, the assumption \eqref{eq:ass_cor} for $u_0 - \td u_0$, and the embedding \eqref{eq:inte:3}, we obtain 
\beq\label{eq:cor_J1}
|| J_1 ||_{\cH^K} \les || u_0 - \td u_0 ||_{\cH^K} \les \e_0,
\quad \lim_{\e_0 \to 0} \max_{|z| \leq 1} | \na^i J_1 |  = 0, \quad \mathrm{for \ } i = 0,1, 2,3.
\eeq

Denote $H_1 =\td H_0 H_0^{-1}, \Mc_1 = \Mc_0 \Mc_0^{-1}, V_1 = \Mc_0 ( \td V_0 - V_0 ) $. For $J_2$, using $u_0(z) = H_0^{-1}U_0( \Mc_0 ( z - V_0))$ \eqref{eq:init_res} and a change of variable, we obtain 
\[
\bal
%J_2 = \td H_0 H_0^{-1} U_0( \Mc_0 \Mc_0^{-1} z  + \Mc_0 ( \td V_0 - V_0 ) ) - \bar U_0
J_2 & = \td H_0 H_0^{-1} U_0( \Mc_0 \Mc_0^{-1} z  + \Mc_0 ( \td V_0 - V_0 ) ) - \bar U_0
= H_1 U_0( \Mc_1 z + V_1) - \bar U \\
& =  H_1 (U_0 - \bar U) (\Mc_1 z + V_1)
+ \B( H_1 \bar U(\Mc_1 z + V_1) - \bar U \B) := J_{21} + J_{22}. 
\eal
\]

From \eqref{eq:cor_small2}, we obtain that $\Mc_1 - 1 =o(1), H_1 - 1 = o(1), V_1 = o(1)$. 
Since $|| U_0 - \bar U_0 ||_{\mfr E_K} < \nu$, by choosing $\e_0$ small enough, we yield 
\beq\label{eq:cor_J21}
|| J_{21} ||_{\mfr E_K} < \nu .
\eeq

Using the smoothness of $\bar U$ and the embedding \eqref{eq:inte:3}, we obtain 
\beq\label{eq:cor_J22}
\lim_{\e_0 \to 0} || J_{22} ||_{\cH^K} + \max_{|z| \leq 1, i\leq 3} | \na^i J_{22} |   = 0.
\eeq

Next, we show that  for $f$ with $\na^j f(0) = 0, j \leq 2$ and $i\leq K$, we have 
\beq\label{eq:cor_pf3}
 %|| f ||_{\cE_K} 
 || \na^i f ||_{\rho_i} \les || f ||_{\cH^K} .
\eeq

Using the definition of {$\rho_K$ \eqref{wg:rho}, $\mfr E_K$ \eqref{def:EkFk},  $g_k, \cH^K$ \eqref{norm:Hk}}, and embedding \eqref{eq:inte:3}, for $f$ with $\na^j f(0) = 0, j \leq 2$, we have 
\[
\bal
 & ||  \na^i f ||_{\rho_i}
 \les || \na^3 f ||_{L^{\infty}} || \ |x|^{ 3 - i } \one_{|x| \leq 1} ||_{\rho_i}
  +  ||  \na^i f ||_{g_i}
  \les  || f ||_{\cH^K} , \quad i \leq 3,  \\
  & ||  \na^i f ||_{\rho_i} 
\les ||  \na^i f ||_{L^{\infty}} || \one_{|x| \leq 1} ||_{\rho_i}
 +  ||  \na^i f ||_{ g_i} \les || f||_{\cH^K}, \quad i \leq (d+5)/2. 
\eal
\]

For $ \f{d+5}{2} < i \leq K$, $\rho_i$ and $g_i$ are equivalent and \eqref{eq:cor_pf3} follows from \eqref{eq:inte:Hk}. From the definition of $\td U_0$ and $J_i$, for $l\leq 2,i=1,2$, we obtain $\na^l J_{21}(0) = 0, \na^l( J_1 + J_{22})(0) = 0 $. Applying \eqref{eq:cor_pf3}, we obtain 
\[
 || J_1 + J_{22} ||_{\mfr E_K} \les || J_1 + J_{22} ||_{\cH^K} ,
 \]
 which goes to $0$ as $\e_0 \to 0$. Since the inequality \eqref{eq:cor_J21} is strict, for $\e_0$ small enough, we prove \eqref{eq:cor_small0}. Condition \eqref{def:EKFKbar} follows from a similar argument, we conclude the proof of Theorem \ref{cor:stab}.


\endgroup

==> ks.tex <==
\chapter{Blowups via Local Modulations: Keller-Segel}\label{cha:ks}
\begingroup
    

\newcommand{\be}{\begin{equation}}
	\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
	\newcommand{\eea}{\end{eqnarray}}
\newcommand{\bee}{\begin{eqnarray*}}
	\newcommand{\eee}{\end{eqnarray*}}
 \newcommand{\la}{\left\langle}
\newcommand{\ra}{\right\rangle}
\def\div{{\rm div \;}}
\def\grad{{\rm grad \;}}
\def\Tr{{\rm Tr \;}}
\def\tr{{\rm tr \;}}
\def\pa{\partial}
\def\pr{\partial}
\def\na{\nabla}
\def\Eq{\mbox{Eq}}
\def\Ai{\mathbf{Ai}}
%
\def\CC{\mathbb{C}}
\def\NN{\mathbb{N}}
\def\RR{\mathbb{R}}
\def\ZZ{\mathbb{Z}}
\def\TT{\mathcal{T}}
\def\La{\Lambda}
\def\SS{\mathcal{S}}
%
\def\ds{\displaystyle}
\def\wegde{\wedge}
\def\ni{\noindent}
\def\bs{\bigskip}
\def\ms{\medskip}
\def\ss{\smallskip}
\def\eps{\vare}
\def\etah{\hat{\eta}}
\def\wt{\tilde{w}}
\def\sigmat{\tilde{\sigma}}
\def\ga{\gamma}
\def\b{\beta}
\def\de{\delta}
\def\om{\omega}
\def\ep{\varepsilon}
\def\LL{\mathcal{L}}
\def\gammah{\hat{\gamma}}
\def\psih{\hat{\psi}}
\def\fref#1{{\rm (\ref{#1})}}
\def\pref#1{{\rm \ref{#1}}}
\def\im{{\mathcal I} \hspace{-2pt}{\textit m}\,}
\def\real{{\mathcal R} \hspace{-2pt}{\textit e}\,}
\def\uh{\hat{u}}
\def\calC{{\mathcal C}}
\def\calB{{\mathcal B}}
\def\calA{{\mathcal A}}
\def\calD{{\mathcal D}}
\def\calE{{\mathcal E}}
\def\calF{{\mathcal F}}
\def\calG{{\mathcal G}}
\def\calH{{\mathcal H}}
\def\calI{{\mathcal I}}
\def\calJ{{\mathcal J}}
\def\calK{{\mathcal K}}
\def\calL{{\mathcal L}}
\def\calM{{\mathcal M}}
\def\calN{{\mathcal N}}
\def\calO{{\mathcal O}}
\def\calP{{\mathcal P}}
\def\calQ{{\mathcal Q}}
\def\calR{{\mathcal R}}
\def\calS{{\mathcal S}}
\def\calT{{\mathcal T}}
\def\calU{{\mathcal U}}
\def\calV{{\mathcal V}}
\def\calW{{\mathcal W}}
\def\calX{{\mathcal X}}
\def\calY{{\mathcal Y}}
\def\calZ{{\mathcal Z}}
\def\ltl{\frac{\l_\tau}{\l}}
\def\calo{{\mathcal o}}
\def\tphi{\tilde{\phi}}
\def\tPsi{\tilde{\Psi}}

\def\calU{{\mathcal U}}
\def\calV{{\mathcal V}}
\def\etaloc{\eta^{\rm loc}}
\def\calX{{\mathcal X}}
\def\calT{{\mathcal T}}
\def\calS{{\mathcal S}}
\def\G{{\Gamma}}
\def\Hd{\dot{H}^1_r}
\def\ft{\tilde{f}}
\def\X{\dot{H}^1_{r}}

\def\tPhi{\tilde{\Phi}}
\catcode`@=11
\def\supess{\mathop{\operator@font Sup\,ess}}
\catcode`@=12

\def\un{{\mathbbmss{1}}}
\def\curl{{\rm curl \;}}
\def\Diag{{\rm Diag}}
\def\div{{\rm div \;}}
\def\grad{{\rm grad \;}}
\def\Yt{\tilde{Y}}
\def\bt{\tilde{b}}
\def\bb{b}
\def\Tr{{\rm Tr \;}}
\def\tr{{\rm tr \;}}
\def\vol{{\rm vol}}

\def\CC{\mathbb{C}}
\def\MM{\mathbb{M}}
\def\NN{\mathbb{N}}
\def\OO{\mathbb{O}}
\def\RR{\mathbb{R}}
\def\CC{\mathbb{C}}
\def\LL{\mathbb{L}}
\def\EE{\mathbb{E}}
\def\etab{\overline{\eta}}
\def\PP{\mathbb{P}}
\def\At{\tilde{A}}
\def\Bt{\tilde{B}}
\def\ZZ{\mathbb{Z}}
\def\II{\mathbb{I}}
\def\TT{\mathbb{T}}

\def\e{\varepsilon}
\def\rhopa{{\rho_{pa}}}
\def\upa{{u_{pa}}}
\def\wpa{{w_{pa}}}
\def\rhoin{\rho_{in}}
\def\uin{u_{in}}
\def\win{w_{in}}
\def\epz{{\varepsilon^0}}
\def\epp{{\varepsilon^\perp}}
\def\Dein{\Delta^{-1}}
\def\chif{\chi_{\frac{\zeta^*}{4}}}
\def\chit{\chi_{\frac{\zeta^*}{2}}}
\def\barm{\bar{m}_\varepsilon}
\def\Lwei{{_{L_{\frac{w_\nu}{\zeta}}^2}}}
\def\Lweibar{{_{L_{\frac{\bar w_\nu}{\zeta}}^2}}}
\def\dtau{\partial_\tau}
\def\ds{\partial_s}
\def\dr{\partial_r}
\def\rr{r}
\def\drr{\partial_r}
\def\dzeta{\partial_{\zeta}}
\def\mar{m_{\rho,pa}}
\def\marin{m_{\rho,in}}
\def\pnu{P_{1,\nu}}
\def\pnutwo{P_{2,\nu}}
\def\meppa{m_{\e,pa}}
\def\mepin{m_{\e,in}}
\def\Anull{\mathscr{A}_0}
\def\Lweiin{{_{L_{\frac{w_0}{\rr}}^2}}}
\def\epa{{\ep_{pa}}}
\def\ein{{\ep_{in}}}
\def\einr{{\ep_{in}^{(0)}}}
\def\einp{{\ep_{in}^{\perp}}}
\def\teinr{{\tilde \ep_{in}^{(0)}}}
\def\teinp{{\tilde \ep_{in}^{\perp}}}
\def\rhopap{\rho_{pa}^\perp}
\def\eppa{\ep_{pa}^\perp}
\def\epino{\ep_{in,1}}
\def\Dtepino{D^2 \ep_{in,1}}
\def\Azeta{\mathscr{A}^\zeta}
\def\mzero{m_{\ep,0}}
\def\mone{m_{\ep,1}}
\def\mtwo{m_{\ep,2}}
\def\tmepin{\tilde m_{\ep,in}}
\def\ctmepin{\tilde m_{\ep,in}^*}
\def\trhoin{\tilde \rho_{in}}
\def\tuin{\tilde u_{in}}
\def\tr{\tilde r}
\def\tnu{\tilde \nu}
\def\teta{\tilde \eta}
\def\tmarin{\tilde m_{\rho,in}}
\def\epae{\ep_{pa}}
\def\epaer{\ep_{pa}^0}
\def\epaep{\ep_{pa}^\perp}
\def\chiz{\chi_{\frac{\zeta_*}{4}}}
\def\chizt{\chi_{\frac{\zeta_*}{2}}}
\def\Lwtwo{L_{\frac{w_\nu}{\zeta}}^2}
\def\epc{\ep_c}
\def\hw{\hat w}
\def\bw{\bar w}
\def\Lni{\calL_0^{-1}}
\def\mass{m_\rho}
\def\ma{\bar m_\rho}
\def\cin{c_{in}}
\def\eps{\varepsilon_s}
\def\epu{\varepsilon_u}
\def\dg{\delta_g}
\def\txi{\tilde \xi}
\def\teta{\tilde \eta}
\def\bep{\bar{\varepsilon}}
\def\dfa{d_{fake}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}



The Keller-Segel equation, a classical chemotaxis model, and many of its variants have been extensively studied for decades. In this work, we focus on $3$D Keller-Segel equation with a quadratic logistic damping term $-\mu \rho^2$ (modeling density-dependent mortality rate) and show the existence of finite-time blowup solutions with nonnegative density and finite mass for any $\mu \in \big[0,\frac{1}{3}\big)$. This range of $\mu$ is sharp; for $\mu \ge \frac{1}{3}$, the logistic damping effect suppresses the blowup as shown in \cite{Kang_Stevens_globalexistence_p,Tello_Winkler_globalexi_for_p}.
    A key ingredient is to construct a self-similar blowup solution to a related aggregation equation as an approximate solution, with subcritical scaling relative to the original model.
    Based on this construction, we employ a robust weighted $L^2$ method to prove the stability of this approximate solution, where modulation ODEs are introduced to enforce local vanishing conditions for the perturbation lying in a singular-weighted $L^2$ space. As a byproduct, we exhibit a new family of type I blowup mechanisms for the classical $3$D Keller-Segel equation.

        \section{Introduction}
Chemotaxis is a widespread natural phenomenon, and it occurs when organisms, such as body cells or bacteria, detect and move toward chemical signals in their surroundings. A principal mathematical description of chemotaxis is provided by the Keller-Segel system:
\be
\begin{cases}
\partial_t \rho  = \Delta \rho - \na \cdot (\rho \na c), \\
\Delta c + \rho = 0,
\end{cases}
\tag{KS}
\label{equation, Keller-Segel}
\ee
 where $\rho$ represents the density of the bacteria and $c$ denotes the concentration of the self-emitted chemical substance. The model captures two key processes: the diffusive effect of random bacterial motion and the directed movement of bacteria toward the highest concentration of the chemical. For a broader introduction to chemotaxis, see \cite{MR3932458, MR2013508, MR2073515}.

 Biologically, beyond the competition between diffusion and bacterial aggregation, the limitation of resources and overcrowding necessitate introducing the bacterial mortality rate that further suppresses the aggregation process. In particular, we consider the following $3$D coupled parabolic-elliptic Keller-Segel system with logistic damping
\be
\begin{cases}
\partial_t \rho = \Delta \rho -  \na \cdot (\rho \na c) - \mu \rho^2, \\
\Delta c +\rho = 0,
\end{cases}
\label{equation: KS with damping}
\tag{KS-D}
\ee
where $-\mu \rho^2$ ($\mu \ge 0$)  represents the logistic damping rate. For additional background on \eqref{equation: KS with damping} and related models, we refer the interested readers to \cite{Fuest_blowup_optimal_2021,MR2448428,MR1788983,MR540951,Tello_Winkler_globalexi_for_p}.

        \subsection{Background}

    \subsubsection{Classical Keller-Segel equation: global existence v.s. finite-time blowup}

\mbox{}

\vspace{0.1cm}

    For the classical Keller-Segel equation \eqref{equation, Keller-Segel}, the total mass $M(t) = \int \rho(t,x) dx$ is conserved for all time.  
Additionally, the system \eqref{equation, Keller-Segel} admits a one-parameter family of scaling invariance: 
\be
\rho(t,x)\to \frac{1}{\lambda^2} \rho\left(\frac{t}{\lambda^2}, \frac{x}{\lambda} \right), \ c(t,x)\to c\left( \frac{t}{\lambda^2}, \frac{x}{\lambda} \right), \quad \forall \; \lambda>0.
\label{scaling invariance}
\ee
We remark that this scaling invariance also holds for \eqref{equation: KS with damping}. 

In two dimensions, the total mass $M=8\pi$ serves as a crucial quantity determining the global existence and finite-time blowup of the system \eqref{equation, Keller-Segel}. Specifically,  it has been shown that finite-time blowup occurs whenever $M> 8 \pi$ with initial data $\rho_0 \in L_+^1((1+|x|^2),dx)$, while global-in-time existence with a uniform $L^\infty$ bound holds when $M<8\pi$, see \cite{Blanchet_Dolbeault_Perthame_globalexistence06, Dolbeault_Perthame_globalexistence04}.

Nevertheless, the critical mass threshold does not exist for the three-dimensional model \eqref{equation, Keller-Segel}. In fact, even with a tiny total mass, there is a radial solution that develops a finite-time singularity found by Nagai \cite{MR1361006}. Beyond the radial case, Corrias, Perthame, and Zaag \cite{MR2099126} demonstrated that blowup occurs whenever the second moment of the initial density is sufficiently small in comparison to the total mass, while weak solutions exist globally if the initial density has a suitably small $L^\frac{3}{2}$ norm. Interested readers can refer to \cite{MR4201903, MR3411100, MR3438649, MR3936129} for more results.

\subsubsection{Classical Keller-Segel equation: singularity formation}
\label{subsub: singularity formation of KS}

\mbox{}

\vspace{0.1cm}

Over the last several decades, the singularity formation for the classical Keller-Segel equation \eqref{equation, Keller-Segel} has been well studied. For the $2$D case, since the model is in the $L^1$ critical sense, Naito and Suzuki \cite{Naito_Suzuki_typeIIblowup} verified that any finite-time blowup solution to \eqref{equation, Keller-Segel} is of type II\footnote{The solution of \eqref{equation, Keller-Segel} exhibits type I blowup at $t=T$ if 
\begin{equation*}
    \limsup_{t \to T} (T-t) \| \rho(t) \|_{L^\infty} < \infty.
\end{equation*}
Otherwise, the blowup is of type II.
}.
In particular, Rapha\"{e}l and Schweyer \cite{raphael2014stability} provided a precise construction of a radially stable finite-time blowup solution of the form
\be
\rho(t,x) \approx \frac{1}{\lambda^2(t)} U\left(\frac{x}{\lambda(t)} \right), \quad U(x) = \frac{8}{(1+|x|^2)^2}, \label{type II blowup: profile}
\ee
where the blowup rate
\[
\lambda(t) = \sqrt{T-t} e^{-\sqrt{\frac{|\ln (T-t)|}{2}}+ O(1)}, \quad t \to T.
\]
Subsequently, this result has been extended to several refined scenarios, including nonradial blowup, multi-bubble blowup without collision, and the simultaneous collision of two collapsing bubbles. For further details, we refer the interested reader to \cite{buseghin2023existence, collot2022refined, 2DKSmultibubble}.


Unlike the $2$D case, the $3$D Keller-Segel system exhibits a large variety of blowup mechanisms. 
Notably, there is a countable family of radial self-similar blowup solutions of the form
\be
\rho_s(t,x) = \frac{1}{T-t} Q_s\left( \frac{x}{\sqrt{T-t}} \right), \; 
\footnote{It exactly matches the scaling invariance \eqref{scaling invariance} of the classical Keller-Segel system \eqref{equation, Keller-Segel}.}
\label{ansatz: self-similar blowup solution usual scaling}
\ee
which have been identified in \cite{Brenner_Constantin_Leo_Schenkel_Venkataramani_steady_state_99, MR1651769,nguyen2025infinitely}.
In particular, there is an explicit self-similar solution given by
\be
\rho_{s*}(t,x) = \frac{1}{T-t}Q_{s*}\left( \frac{x}{\sqrt{T-t}} \right), \quad \text{ with } \quad Q_{s*}(x) = \frac{4(6+|x|^2)}{(2 + |x|^2)^2},
\label{profile}
\ee
whose radial stability has been verified by Glogi\'c and Sch\"orkhuber \cite{stable3DKS}. Recently, Li and the third author \cite{ksnsblowup,lizhou2025nonradial} extended this stability theory to the nonradial setting.
Beyond self-similar blowup solutions, other non-self-similar formations have also been identified. For example, Collot, Ghoul, Masmoudi, and Nguyen \cite{Collot_Ghoul_Masmoudi_Nguyen_3Dblowup_Collasping-ring_blowup23} discovered a collapsing-ring blowup solution, and
Nguyen, Nouaili, and Zaag \cite{nguyen2023construction} found a type I blowup solution with a log correction on the shrinking rate. Additionally, Hou, Nguyen, and Song \cite{hou2025axisymmetric} recently found a type II blowup solution under axisymmetry, whose local leading-order profile coincides with the rescaled stationary solution of the two-dimensional Keller-Segel equation as given in \eqref{type II blowup: profile}.


    \subsubsection{Blowup or no blowup with logistic damping}
    \label{subsub: logistic damping}

    \mbox{}

    \vspace{0.1cm}

    To detect the core mechanism behind the bacterial aggregation, we can rewrite the aggregation term in \eqref{equation, Keller-Segel} or \eqref{equation: KS with damping} as
\begin{equation*}
    \nabla \cdot (\rho \nabla \Dein \rho)  = \nabla \Dein \rho \cdot \nabla \rho + \rho^2.
\end{equation*}
In this expression, $\na \Dein \rho \cdot \na \rho$ is the advection term, which, along with the effect of the diffusion term, cannot lead to the finite-time blowup. Consequently, the main factor causing the blowup is $\rho^2$.



If the logistic damping term $-\mu \rho^2$ in \eqref{equation: KS with damping} is replaced by a stronger term of the form $-\mu \rho^p$ with $\mu>0$ and $p >2$, then the aggregation effect is always suppressed. Precisely, the smooth solution always exists globally in time, regardless of how concentrated the initial density is, see \cite{Tello_Winkler_globalexi_for_p}. 

In the scenario of quadratic damping
$-\mu \rho^2$ (corresponding to \eqref{equation: KS with damping}), Tello and Winkler \cite{Tello_Winkler_globalexi_for_p} proved that the global existence is guaranteed for any $\mu >0$ in two dimensions.
For higher dimension $d\geq 3$, they further demonstrated that global existence holds provided $\mu > \frac{d-2}{d}$. Subsequently, Kang and Stevens \cite{Kang_Stevens_globalexistence_p} verified the global existence in the critical case $\mu = \frac{d-2}{d}$ with $d \ge 3$. In the subcritical regime with $\mu \in \left(0, \frac{d-2}{d}\right)$, Fuest \cite{Fuest_blowup_optimal_2021} partially bridged the gap by proving that finite-time blowup occurs in a bounded domain for $\mu \in \left( 0, \frac{d-4}{d} \right)$ in higher dimensions $d \ge 5$. However, to the best of the authors' knowledge, 
prior to the present work, it remained an \textit{open problem} whether blowup occurs for $\mu \in (\frac{d-4}{d}, \frac{d-2}{d})$ with $d \ge 5$ and $\mu \in (0, \frac{d-2}{d})$ with $ 3 \le d \le 4$.


Regarding the weaker damping term $-\mu \rho^p$ with $1<p<2$, for higher dimensions $d \ge 5$, Winkler \cite{Winkler_blowup} verified the existence of finite-time blowup solution when $1 <p < \frac{3}{2} + \frac{1}{2d-2}$. Subsequently, for dimensions $d \in \{3,4\}$, Winkler \cite{Winkler_blowup_N} demonstrated finite-time blowup for $1< p < \frac{7}{6}$. This range was later significantly extended by Fuest \cite{Fuest_blowup_optimal_2021}, where the author established the finite-time blowup for $1 < p< \frac{3}{2}$ in dimensions $d=3$ and for  $1 < p< 2$ in dimensions $d \ge 4$.%, thereby completing the finite-time blowup theory in the high-dimensional regime  $d \ge 4$.


    


    \subsection{Main result}

    \mbox{}
    
    The principal objective of this work is to establish the \textit{optimal blowup result} to \eqref{equation: KS with damping} in three dimensions. Specifically, we establish the existence of a smooth finite-time blowup solution to \eqref{equation: KS with damping} with nonnegative density and finite mass for any $0 \le \mu < \frac{1}{3}$ in three dimensions.

    In the literature, most blowup results for chemotaxis equations are obtained either by tracking the evolution of some appropriate functional (such as the second moment) to obtain a contradiction  \cite{Blanchet_Dolbeault_Perthame_globalexistence06, MR2099126, Dolbeault_Perthame_globalexistence04}, or by working in the radial setting where the mass accumulation function satisfies an ODE  \cite{Fuest_blowup_optimal_2021}. However, the damping term $-\mu \rho^2$ in \eqref{equation: KS with damping} destroys the structures that these proofs rely on. In particular, it \textit{leads to a time-decreasing mass} and \textit{breaks the divergence form structure} that the classical Keller-Segel equation \eqref{equation, Keller-Segel} enjoys, thereby making these classical methods too limited to obtain the sharp blowup result for \eqref{equation: KS with damping}.

    Motivated by the various singularity formation results, 
     ranging from the nonlinear heat equation \cite{bricmont1994universality,CollotsuperHeateq,hou20242,merle1997stability}, nonlinear wave equation \cite{MR3537340,kim2022self}, nonliear Schr\"odinger equation \cite{MerleblowupNLSdefocusing,MR2729284}, incompressible fluids \cite{chen2022stable, chen2025stable,chen2021finite,hou2024blowup,elgindi2019finite,elgindi2021finite}, compressible fluids \cite{Javierblowup3DNS,chen2024Euler,MRRSam22a},  we adopt a strategy based on the direct construction of finite-time blowup solutions via the stability analysis of an approximate blowup solution. And the precise statement of the main theorem is as follows: 
    
\begin{theorem}[Existence of finite-time blowup to \text{\eqref{equation: KS with damping}} with finite mass]
\label{thm: existence of blowup}
For any fixed $0 \le \mu < \frac{1}{3}$, let $j_0$ be an integer such that
\be 
j_0 \ge J:= \frac{3(1-\mu)}{1-3\mu} +1 >1,
\label{J: def}
\ee
it then follows that
\be
\beta = \beta(j_0,\mu) := \frac{1}{3(1-\mu)} + \frac{1}{2j_0} < \frac{1}{2}.
\label{beta: def, thm}
\ee
In addition, under these choices, there exists a radially nonnegative $\rho_0 \in C_0^\infty (\RR^3)$  \footnote{Since $\rho_0 \in C_0^\infty(\RR^3)$, the total mass of the system is necessarily finite. Additionally, with the nonnegativity of initial data $\rho_0$, an argument analogous to \cite[Theorem A.1]{ksnsblowup} ensures that the corresponding solution remains nonnegative in its lifespan.
}
such that the related smooth solution to \eqref{equation: KS with damping} 
exhibits finite-time blowup at $t=T<\infty$. Moreover,
the solution satisfies
\be
\rho(t,x) = \frac{1}{T-t} \left[ Q \left( \frac{x}{(T-t)^\beta} \right) + \ep \left( t, \frac{x}{(T-t)^\beta} \right) \right], \quad x \in \RR^3, \; t \in [0,T),
\label{blowup KS with damping}
\ee

\noindent where 

\noindent $\bullet$ (Existence of profile). $Q$ is a unique smooth
radial decreasing solution to the equation:
\be
    Q+\beta y \cdot \nabla_y Q = \nabla_y Q \cdot \nabla_y\Delta^{-1}_yQ + (1-\mu)Q^2,
    \label{PDE Q}
\ee
with the initial data
 \be
    Q(0) = \frac{1}{1-\mu} \quad \text{ and } \quad \partial_r^{(2j_0)} Q(0) = -(2j_0)!  <0.
    \label{smooth profile: initial data -1}
\ee

\noindent $\bullet$ (Smallness of error term).
There exists $s=s(\mu) \in \ZZ_{\ge 1}$ sufficiently large and constants $C>0$ and $\bar \epsilon >0$ such that the error term $\ep$ satisfies
\[
\| \ep(t) \|_{H^s(\RR^3)} \le C \left( T-t \right)^{\bar \epsilon}, \quad \forall \; 0 \le t <T.
\]
    
\end{theorem}



\vspace{0.15cm}

\noindent \textit{Comments on Theorem \ref{thm: existence of blowup}.}
\label{ref:com}

\vspace{0.08cm}


\noindent \textit{$1.$ Optimality in blowup results for Keller-Segel equation with logistic damping.}

\vspace{0.1cm}

Theorem \ref{thm: existence of blowup} shows the existence of a finite-time blowup solution to $3$D Keller-Segel equation with logistic damping \eqref{equation: KS with damping} for any fixed $0 \le \mu < \frac{1}{3}$. This result provides the optimal blowup threshold for \eqref{equation: KS with damping} and completes the long-standing conjecture proposed in \cite{Fuest_blowup_optimal_2021,Tello_Winkler_globalexi_for_p} as mentioned in Subsection \ref{subsub: logistic damping}.


Moreover, our method is robust enough to extend naturally to higher dimensions $d \ge 3$, resulting in an analogous sharp blowup regime. Specifically, for $\mu \in \Big[ 0, \frac{d-2}{d} \Big)$ with $d \ge 3$, there always exists a finite-time blowup solution to \eqref{equation: KS with damping}.

When the damping term is weakened to $-\mu \rho^p$ with $\mu>0$ and $1 \le p <2$, the problem becomes simpler, as this term can also be viewed primarily as a perturbation of the dominant aggregation effect. Concretely, one could use $\frac{1}{T-t}Q\big(\frac{x}{(T-t)^\beta}\big)$ with $Q$ constructed in Theorem \ref{thm: existence of blowup} with $\mu=0$ as an approximate solution. Alternatively, one may use the self-similar solution \eqref{profile} of the classical Keller-Segel equation \eqref{equation, Keller-Segel} as an approximate solution. Then, we could apply the stability theory developed in this work or \cite{stable3DKS,lizhou2025nonradial} to establish the existence of finite-time blowup for any $\mu > 0$ and $p \in [1,2)$ in three dimensions. Since this problem is easier to handle, we do not pursue this in detail and only study \eqref{equation: KS with damping} with essential difficulty.

\vspace{0.2cm}

\noindent \textit{$2.$ New blowup mechanism for classical Keller-Segel equation in $3$D.}

\vspace{0.1cm}

For $3$D classical Keller-Segel equation \eqref{equation, Keller-Segel}, by applying Theorem \ref{thm: existence of blowup} with $\mu=0$, we have constructed a countably infinite family of blowup solutions, whose asymptotic behavior is given by
\[
\rho(t,x) \approx \frac{1}{T-t} Q_{\beta_j} \left( \frac{x}{(T-t)^{\beta_j}} \right), \qquad \forall \; t \in (0,T),
\]
where $\beta_j = \frac{1}{3} + \frac{1}{2j}< \frac{1}{2}$ for all $ j \ge 4$ and each $Q_{\beta_j}$ solves \eqref{PDE Q} with $\beta =\beta_j$. This blowup is an "abnormal" Type I blowup, in the sense that it does not match natural scaling \eqref{scaling invariance} \footnote{
We take the ansatz $\rho(t,x) = \frac{1}{(T-t)^a} Q \left( \frac{x}{(T-t)^b} \right)$ and plug it into \eqref{equation: KS with damping}. Requiring that all terms in the resulting equation have the same strength, the exponents must satisfy $a=2b=1$. This choice precisely coincides with the scaling symmetry \eqref{scaling invariance} of the equation. We refer to blowup solutions satisfying this form as exhibiting natural self-similar blowup, in analogy with \eqref{equation: KS with damping}.

}. Consequently, as a by-product of Theorem \ref{thm: existence of blowup}, we establish a new family of blowup mechanisms for $3$D classical Keller-Segel equation \eqref{equation, Keller-Segel}.



\vspace{0.2cm}


\noindent \textit{$3.$ Extension of Theorem \ref{thm: existence of blowup}.}

\vspace{0.1cm}
Theorem \ref{thm: existence of blowup} establishes the precise blowup mechanism for the density but does not address its stability. Nevertheless, by following the standard approach outlined in \cite{CollotsuperHeateq, lizhou2025nonradial}, one can construct a finite-codimensional Lipschitz stable manifold of radial initial data such that the corresponding solutions to \eqref{equation: KS with damping} exhibit blowup dynamics similar to in \eqref{blowup KS with damping}.

Besides, a natural extension to the nonradial blowup can be expected by using the spectral method from \cite{nonradialblowupNS, nonradialblowupNLS, chen2024vorticityhigherdimension, chen2024Euler}. Alternatively, following the argument in \cite{chen2024stability}, one might introduce a matrix system of modulation ODEs to realize it. 
Furthermore, noting that the blowup solution constructed in Theorem \ref{thm: existence of blowup} is highly localized, one can expect a finite-time blowup solution in a bounded domain by adapting the cut-off technique from \cite{nonradialblowupNS, nonradialblowupNLS}. However, as the main focus of this work is on the existence of finite-time blowup solutions to \eqref{equation: KS with damping}, we do not pursue these generalizations in detail here.




In addition, our method is expected to be sufficiently robust to potentially shed light on other models, such as the nonlinear heat equations. As a further motivation for the linear and nonlinear analysis for the Keller-Segel equation \eqref{equation: KS with damping} in Section \ref{sec: linear theory} and Section \ref{sec: nonlinear sta}, we briefly outline this in Section \ref{sec:slh} for $1$D semilinear heat equation.

\vspace{0.23cm}

\subsection{Proof strategy and related key highlights.}

\vspace{-0.1cm}

\subsubsection{Key idea of the construction: diffusion term as a perturbation.}

\mbox{}

\vspace{0.08cm}

Motivated by the explicit self-similar blowup solution \eqref{profile} to the classical Keller-Segel equation \eqref{equation, Keller-Segel}, a direct idea is to seek an analogous self-similar solution matching the natural scaling for the damped system \eqref{equation: KS with damping}. Specifically, since \eqref{equation: KS with damping} satisfies the scaling invariance \eqref{scaling invariance}, one is led to consider special solutions of form
\vspace{-0.05cm}
\[
\rho_\mu(t,x) = \frac{1}{T-t} Q_{\mu} \left( \frac{x}{\sqrt{T-t}} \right),
\]
where $Q_\mu$ solves
\be
Q_\mu + \frac{1}{2} y \cdot \na Q_\mu = \Delta Q_\mu + \na \cdot (Q_\mu \na \Dein Q_\mu) - \mu Q_\mu^2.
\label{self-simiar profile: equation}
\ee
However, the damping term $-\mu \rho^2$ significantly complicates the problem by breaking the divergence structure of \eqref{equation, Keller-Segel}. In particular, the partial mass 
\be
m_\rho (r) := \int_{B(0,r)} \rho(x) dx,
\label{partial mass: def}
\ee
is invalid to simplify the equation \eqref{self-simiar profile: equation} into a second order local differential equation, resulting \eqref{self-simiar profile: equation} essentially a third-order differential equation for general $\mu \in \left( 0, \frac{1}{3} \right)$, which, to the best of authors' knowledge, is quite difficult to analyze and is still open.

Instead, we adopt an alternative approach inspired by \cite{chen2024stability,hou20242,MRRSam22a,MRRSam22b,nguyen2023construction,MR4752990}, 
where the first step is to neglect the diffusion term
and construct a self-similar blowup solution for the following $3$D aggregation equation
\be
    \pa_t \rho = \nabla \rho \cdot \nabla\Delta^{-1}\rho + (1-\mu)\rho^2,
    \label{aggregation eq}
\ee
in the form
\be
    \rho(t,x) = \frac{1}{T-t} Q\left( \frac{x}{(T-t)^\beta} \right), \;  \text{ with } \beta < \frac{1}{2},
    \label{abnormal blowup}
\ee
where the profile $Q$ satisfies \eqref{PDE Q}. We then choose \eqref{abnormal blowup} as an approximate solution to the original system \eqref{equation: KS with damping}, which breaks the natural scaling of \eqref{equation: KS with damping}, thus making the diffusion term
$\Delta \rho$ subcritical and allowing it to be treated as a perturbation relative to the dominant aggregation term. 

Compared to \eqref{self-simiar profile: equation}, the equation \eqref{PDE Q} is effectively second-order and much more tractable. 
By restricting to radial solutions and introducing the averaged mass of $Q$ in the ball $B(0,r)$ 
\be
    f_Q(r) := \frac{1}{r^3}\int_0^r Q(s)s^2 ds, 
    \label{f: definition}
\ee  
\eqref{PDE Q} can be reformulated as an ODE system in terms of $(Q,f_Q)$ (see \eqref{ODE system}).
The formation of solutions to \eqref{ODE system} is through the dynamical system and a standard phase portrait analysis (See Figure \ref{fig3} and Lemma \ref{lem: solve ODE}). These methods have been instrumental in recent developments concerning the construction of smooth profiles for implosion, gravitational collapse, and collapsing-expanding shocks \cite{Javierblowup3DNS,ghj21,guoMahirJangpolytropicgap,jls2025,jang2023selfsimilarconvergingshockwaves,MRRSam22a}. The regularity of self-similar solutions serves as a fundamental criterion for solution admissibility and plays a crucial role in ensuring the existence of a nontrivial solution in the context of the present problem.

\subsubsection{Compatibility of $\mu < \frac{1}{3}$: insights from the phase portrait analysis.}

\mbox{}

\vspace{0.1cm}

One of the main goals of our  chapter is to figure out the existence of the smooth nontrivial radial solution to \eqref{PDE Q} for some $\beta < \frac{1}{2}$, which can be further simplified into finding a smooth curve connecting \be
P_0 := \left( \frac{1}{1-\mu}, \frac{1}{3(1-\mu)} \right), \footnote{
With the singular term $\frac1r$ appearing on the right-hand side of the ODE system \eqref{ODE system},
the choice of initial data $(Q(0),f_Q(0))=P_0$ should be required to ensure that $Q$ is smooth near $r =0$.
}
\label{P_0: def}
\ee
and the origin $O$ under the ODE system for $(Q,f_Q)$ given by \eqref{ODE system}. We classify the problem into three cases based on the relative position between $f_Q = \beta$ and $P_0$, and analyze the corresponding phase portraits:

\vspace{0.1cm}

\noindent \textit{\textbf{Case I.} $P_0$ lies strictly above the line $\{f_Q=\beta\}$: $\beta < \frac{1}{3(1-\mu)}$ (See Figure \ref{fig1}).}
\vspace{-0.2cm}
\begin{figure}[ht]
\centering
\includegraphics[width=0.69\textwidth]{ks/smallbeta.jpeg}
\caption{$Qf_Q$-plane with $P_0$ above the line $f_Q=\beta$. In this case, there is only a trivial solution solving \eqref{ODE system} with $(Q(0),f_Q(0))=P_0$.
}
\label{fig1}
\vspace{-2mm}
\end{figure}

\vspace{0.05cm}

We remark here that in \textit{Case I} $\big(\beta < \frac{1}{3(1-\mu)} \big)$, motivated by the related phase portrait (see Figure \ref{fig1}), the flow field around $P_0$ is directed toward $P_0$. Consequently, $P_0$ is a stagnant point in this case and $Q(r) \equiv \frac{1}{1-\mu}$ is the only smooth solution to \eqref{ODE system} with $(Q(0),f_Q(0))=P_0$ that can be obtained. 
Therefore, to obtain a nontrivial solution to \eqref{ODE system}
with $(Q(0),f_Q(0))=P_0$, it is necessary  
for $\beta$ to satisfy
\be
\frac{1}{3(1-\mu)} \le \beta < \frac{1}{2}.
\label{beta: range of choice}
\ee
This requires that $\mu< \frac{1}{3}$, which aligns exactly with the \textit{optimal range of $\mu$} provided in Subsection \ref{subsub: logistic damping} and Theorem \ref{thm: existence of blowup}. 


\vspace{0.1cm}

\noindent \textit{\textbf{Case II.} $P_0$ lies on the line $\{f_Q=\beta\}$: $\beta = \frac{1}{3(1-\mu)}$ (See Figure \ref{fig2}).}

\begin{figure}[ht]
\centering

\includegraphics[width=0.69\textwidth]{ks/middlebeta.jpg}
\caption{$Qf_Q$-plane with $P_0$ on the line $f_Q=\beta$. In this case, though it seems possible to have a solution curve connecting between $P_0$ and the origin $O$ from the phase portrait, with the overwhelming singularity on the right-hand side of \eqref{ODE system}, after some careful analysis, the only possible smooth solution starting from $P_0$ to should be the trivial one: $(Q(r),f_Q(r)) \equiv P_0$.}
\label{fig2}
\end{figure}


\vspace{0.1cm}

\noindent \textit{\textbf{Case III.} $P_0$ lies strictly below the line $\{f_Q=\beta\}$: $\beta > \frac{1}{3(1-\mu)}$ (See Figure \ref{fig3}).}

\begin{figure}[ht]
\centering

\includegraphics[width=0.69\textwidth]{ks/largebeta2.jpg}
\caption{$Qf_Q$-plane with $P_0$ below $f_Q = \beta$. In this case, we can always choose countably many $\{ \beta_j \}_j$  (see Theorem \ref{thm: existence of blowup} and Lemma \ref{lem: solve ODE} for more details) such that there exists a smooth solution curve (the red curve in the figure) lying in $\calM$ and connecting $P_0$ and the origin $O$ simultaneously, we will discuss this case in more details later in Lemma \ref{lem: solve ODE}.
}
\label{fig3}
\end{figure}





\subsubsection{Stability analysis beyond the spectral theory.}

\mbox{}

\vspace{0.1cm}

After selecting the self-similar blowup solution \eqref{abnormal blowup} of the aggregation equation \eqref{aggregation eq} as an approximate solution to \eqref{equation: KS with damping}, we then proceed to study the perturbation dynamics near the profile $Q$ under the self-similar coordinate \eqref{ss coordinte}, which constitutes the key to our stability analysis. 

In the literature, one of the natural approaches to address this problem is to analyze the spectral properties of the associated linearized operator. Such analysis typically relies on compactness arguments \cite{Javierblowup3DNS, nonradialblowupNLS, engel2000one, jiaSverakillposedness, ksnsblowup,  MerleblowupNLSdefocusing, MRRSam22a} or other more intricate operator theory, e.g. studying the precise or approximated spectrum of the linearized operator \cite{Collot_Ghoul_Masmoudi_Nguyen_3Dblowup_Collasping-ring_blowup23, hou2025axisymmetric, lizhou2025nonradial, merle1997stability, nguyen2023construction}.  For problems with an explicit profile available, studying the spectrum of the linearized operator around the profile yields useful information for stability, e.g. \cite{Collot_Ghoul_Masmoudi_Nguyen_3Dblowup_Collasping-ring_blowup23,lizhou2025nonradial, merle1997stability}.
However, for more complicated dynamics with only implicit or numerically approximate profiles, as is our case, obtaining the spectral information becomes significantly more challenging. 


Alternatively, we adopt a robust approach based on energy estimates with a singular weight appropriately chosen. Linear stability can be extracted via enforcing local vanishing conditions of the perturbation at the origin, using only limited information of the profile. The idea was first demonstrated via the seminal works of \cite{chen2022stable,chen2021finite} in the self-similar case, and later on generalized by the second author with collaborators to type I singularities beyond self-similarity \cite{chen2024stability,hou20242} with the blowup law automatically inferred. Such a stability argument via singular weights will be further amenable to computer-assisted proofs. In this  chapter, we further generalize the idea to the finite-codimensional stability case by studying this open problem.





\subsection{Structure of the  chapter.}

\mbox{}

\vspace{0.1cm}
In Section \ref{sec:slh}, we briefly discuss the approach for handling the finite-codimensional stability of blowup solutions to the $1$D semilinear heat equation by introducing the singular weights. Motivated by this illustrative example, 
we then focus on the Keller-Segel equation with logistic damping term \eqref{equation: KS with damping}. In Section \ref{sec: ODE}, given any fixed $\mu \in \left[ 0, \frac{1}{3} \right)$, we establish the existence of nontrivial solutions to equation \eqref{PDE Q} with an appropriate choice of $\beta \in \left( \frac{1}{3(1-\mu)},\frac{1}{2} \right)$, the quantitative properties of the approximate profiles will be investigated as well. 
For the stability analysis, we first examine the coercivity of the linearized operator in the $L_w^2$ sense with $w$ being sufficiently singular at the origin, as detailed in Section \ref{sec: linear theory}. Finally, in Section \ref{sec: nonlinear sta}, we will study the nonlinear stability to complete the proof of Theorem \ref{thm: existence of blowup}. 



\subsection{Notations.} 
We denote 
\[
\la r \ra = \sqrt{1+r^2}.
\]
And we define a radial smooth cut-off function $\chi$ on $B(0,1)$ by
\be
\chi(x) 
= \begin{cases}
    1, & \text{if } |y| \le 1, \\
    0, & \text{if } |y| \ge 2.
\end{cases}
\label{def: cut-off function}
\ee
Based on this, we define the smooth cut-off function on $B(0,R)$ by
\be
\chi_R(x) : = \chi \left( \frac{x}{R} \right).
\label{def: cut-off on B(0,R)}
\ee

For any given weighted function $w:\RR^3 \to \RR$, we define $L_w^2(\RR^3)$ the weighted inner product by
\[
(g_1,g_2)_{L_w^2(\RR^3)} = \int_{\RR^3} g_1(x) g_2(x) w(x) dx,
\]
and the weighted $L^2$ space $L_w^2(\RR^3)$ by the collections of all functions of $g$ satisfying $\| g \|_{L_w^2}^2:= (g,g)_{L_w^2} <\infty$.

Furthermore, we define $C_0^\infty(\Omega)$ as the collection of all $C^\infty(\RR^3)$ functions with compact support in $\Omega \subset \RR^3$.


For any fixed $m \in \ZZ_{\ge 0}$, we define $\dot H^{2m}$ the collection of all functions satisfying
\[
\| g \|_{\dot H^{2m}}^2 = \int_{\RR^3} |\Delta^m g|^2 dx < \infty,
\]
and define $\dot H^{2m+1}$ the collection of all functions satisfying
\[
\| g \|_{\dot H^{2m+1}}^2 = \int_{\RR^3} |\na \Delta^m g|^2 dx < \infty.
\]
In addition, we denote $H^k(\RR^3)$ for the collection of all functions with finite $\dot H^m$ norm for all $0\le m\le k$. And $H_{rad}^{k}$ is the collection of all radial functions lying in $H^{k}$. Moreover, wewrite $H^\infty(\RR^3) := \cap_{k=0}^\infty H^k(\RR^3)$.


If $h(x)=h \left( |x| \right)$ is a smooth radial function on $\RR^3$, then $h(r)$ can be approximated by the Taylor expansion at the origin: 
\be
h(r) = \sum_{j=0}^M [h]_j r^{2j} + O(r^{2M+2}), \; \text{ with } \; [h]_j := \frac{\partial_r^{(2j)} h}{(2j)!} \Bigg|_{r=0},
\label{Taylor coefficient: def}
\ee
where $[h]_j$ is the $2j$-th order coefficient of Taylor expansion of $h(r)$ at the origin.

\mbox{}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Motivating example of 1D semilinear heat equation}\label{sec:slh}


In this section, to illustrate the ideas of proof more clearly, we first consider the simpler $1$D semilinear heat equation as a motivating example.
Precisely, we will briefly sketch the high-level idea to study high-order vanishing type-I blowup for the $1$D semilinear heat equation under \textit{radial (even symmetric)} setting:
\be
u_t=u_{xx} + u^2.
\label{PDE: nonlinear heat}
\tag{HEAT}
\ee

\subsection{Self-similar renormalization and the approximate solution} For any fixed $m \in \ZZ_{> 1}$, we introduce the self-similar coordinate
\be
y = \frac{x}{\lambda^{\frac{1}{m}}}, \quad \frac{d\tau}{dt} = \frac{1}{\lambda^2}, \quad \tau\Big|_{t=0} =0, \quad 
\frac{\lambda_\tau}{\lambda} = -\frac{1}{2},
\label{ss coordinate: heat eq}
\ee
and corresponding renormalization
\be
u(t,x) = \frac{1}{\lambda^2} U \left( \tau, y \right),
\label{ss renormalization: heat eq}
\ee
then $\lambda(\tau) = \lambda_0 e^{-\frac{1}{2} \tau}$ and $U$ solves the equation
\be
\partial_\tau U = \lambda^{2-\frac{2}{m}} U_{yy} - U - \frac{1}{2m} y \cdot \na U + U^2,
\label{eq: heat renormalized setting}
\ee
where the diffusion term can be regarded as a perturbation since $2- \frac{2}{m} >0$. This, in turn, motivates us to find an approximate solution to the equation
\be
-U - \frac{1}{2m} y \cdot \na U + U^2=0.
\label{sec: PDE U*}
\ee
In particular, this equation can be explicitly solved by
\be
U_* (y)= (1+ c y^{2m})^{-1}.
\label{sec3: profile}
\ee
Here $c>0$ is a constant, and $m>1$ describes the vanishing order of the next order expansion of $U_*$ near the origin.

\subsection{Linear stability}
We fix $m>1$ and $c=1$ in \eqref{sec3: profile}, and plug the ansatz  $U = U_* + \ep$ into \eqref{eq: heat renormalized setting}, it then follows that $\ep$ solves
\[
\partial_\tau \ep = \lambda^{2-\frac{2}{m}} U_{yy} + \calL \ep + \ep^2,
\]
where the linearized operator reads
\be
\mathcal{L}\varepsilon=-\varepsilon-\frac{1}{2m}y \partial_y \varepsilon +2U_*\varepsilon.
\label{sec: L}
\ee
Next, we introduce a weighted $L_\Theta^2$ space with singular weight $\Theta(y) = y^{-4m-4}$ near the origin to extract damping, which is the essential step to close the nonlinear stability. Via the integration by parts, we have the coercivity near the origin
\be
\left( \calL \ep, \ep \right)_{L_\Theta^2}
= \left( \left( -1 + 2U_* + \frac{(\Theta y)_y}{4 m \Theta} \right) \ep, \ep \right)_{L_{\Theta}^2} 
\approx  - \frac{3}{4m} \left(\ep, \ep \right)_{L_{\Theta}^2}.
\label{sec3: cor L 1}
\ee
In particular, with careful analysis, there is a small constant $0< \kappa = \kappa(m,U_*) \ll 1$ such that \eqref{sec3: cor L 1} can be extended to
\be
\left( \calL \ep, \ep \right)_{L_{\Theta+\kappa}^2}
 \le - \frac{1}{4m} \left(\ep, \ep \right)_{L_{\Theta+\kappa}^2}.
\label{sec3: cor L 2}
\ee

Additionally, we need to introduce the higher Sobolev norm $\dot H^{\bar K}$ to close the bootstrap argument. Precisely,
\begin{align}
\left( \calL \ep, \ep \right)_{\dot H^{\bar K}}
& =\left( \left(-1-\frac{\bar K}{2m}+2U_*+\frac{1}{4m} \right)\partial_y^{\bar K}\varepsilon, \partial_y^{\bar K}\varepsilon \right)_{L^2} + O(\| \ep \|_{H^{\bar K-1}} \| \ep \|_{\dot H^{\bar K}}) \notag \\
& \le - \frac{2\bar K-4m-1}{4m} \| \ep \|_{\dot H^{\bar K}}^2 + O(\| \ep \|_{H^{{\bar K}-1}} \| \ep \|_{\dot H^{\bar K}}),
\label{sec3: cor L 3}
\end{align}
where the leading order enjoys damping once we choose $\bar K = \bar K(m) \gg 1$.

\subsection{Modulation ODEs and nonlinear stability} With the singular weight $\Theta(y) = |y|^{-4m-4}$ given previously, we further \textit{radially} decompose $\ep$ into
\be
\ep (\tau,y)= \epu(\tau,y) + \eps(\tau,y), \quad \text{ with }  \quad \epu = \sum_{j=0}^{m} c_j(\tau) \chi(y) y^{2j},
\ee
such that $\eps(\tau,y) = O(y^{2m+2})$ near the origin, which yields an ODE system for modulation parameters $\{ c_j \}_{j=0}^m$:
\be
\begin{cases}
    \dot c_j = \left( 1- \frac{j}{m} \right) c_j + [\epu^2]_j + \lambda^{2- \frac{2}{m}} [U_{yy}]_j, & 0 \le j < m-1,
    \vspace{0.1cm} \\
    \dot c_{m} = [\epu^2]_m - 2c_0 + \lambda^{2- \frac{2}{m}}[U_{yy}]_m, & j=m.
\end{cases}
\ee
Additionally, $\eps = O(y^{2m+2})$ solves the equation
\[
\partial_\tau \eps =   \calL \eps  + 2 \epu \eps + \eps^2 + G[\lambda,U,\epu],
\]
with the modulation term $G[\lambda,U,\epu]= O(y^{2m+2})$ given by 
\[
G[\lambda,U,\epu]= \left( \lambda^{2-\frac{2}{m}} U_{yy} + \calL \epu + \epu^2 \right) - \sum_{j=0}^K \left[\lambda^{2-\frac{2}{m}} U_{yy} + \calL \epu + \epu^2 \right]_j \chi  y^{2j}.
\]
Finally, we can use the standard topological argument together with \eqref{sec3: cor L 1} and \eqref{sec3: cor L 3} to derive the nonlinear stability with finite codimension $m+1$. 

\begin{remark}
    We expect that this nonlinear stability result can be improved to finite-codimension $m-1$, which is two dimensions lower than our previous findings. 
    The key underlying reason is the presence of two degrees of freedom, namely, the choice of the blowup time $T>0$ and the shrinking rate. These degrees of freedom can be utilized through a matching argument to recover the corresponding unstable directions as in \cite{Limodestability, lizhou2025nonradial}.
    
   
    Alternatively, one may employ a method of dynamical rescaling to establish stability with finite codimension $m-1$. 
    Specifically, we modify the coordinate \eqref{ss coordinate: heat eq} as
    \[
    y = \frac{x}{\mu^\frac{1}{m}}, \quad  \frac{d\tau}{dt} = \frac{1}{\lambda^2}, \quad \tau\big|_{t=0}=0, \quad \frac{\lambda_\tau}{\lambda} = -\frac{1}{2} + \frac{1}{2} c_a, \quad \frac{\mu_\tau}{ \mu} = - \frac{1}{2}  - mc_s.
    \]
    We then define the corresponding renormalization
    \[
    u(t,x) = \frac{1}{\lambda^2} U (\tau,y).
    \]
    Under this coordinate transformation, $U$ satisfies
    \[
    \partial_\tau U = \lambda^2 \mu^{-\frac{2}{m}} U_{yy} + \left( -1 + c_a \right) U -\left( \frac{1}{2m} + c_s \right) y \partial_y U + U^2,
    \]
    where the parameters $(c_a,c_s)$ are determined by the modulation conditions
    \[
    U(\tau, 0) = U_*(0) \qquad \text{ and } \qquad  [U(\tau,0)]_{m}= [U_*]_{m},
    \] 
    and we eliminate neutral modes by fixing $c_0=c_m=0$.
    By applying a similar argument of modulation ODEs, we obtain the nonlinear stability with finite codimension $m-1$. Notably, introducing extra scaling parameters to perturb the scaling symmetry is crucial for extending the argument to the nonradial setting; see previous works by the second author and collaborators \cite{chen2024stability,hou20242}.
\end{remark}

\begin{remark}

Compared with the semilinear heat equation \eqref{PDE: nonlinear heat}, analyzing the Keller-Segel equation with logistic damping \eqref{equation: KS with damping} involves several additional challenges. For example, 
the profile $U_*$ 
introduced in \eqref{sec3: profile} is an explicit solution to 
the first-order and separable local equation \eqref{sec: PDE U*}. 
In contrast, for \eqref{equation: KS with damping} with $\mu\in \left( 0, \frac{1}{3} \right)$, the associated profile equation \eqref{PDE Q} is inherently nonlocal and cannot be trivially solved. 
This nonlocality requires a more delicate analysis, which will be carried out in Section \ref{sec: ODE}.

    
    Moreover, since there is no explicit nontrivial solution to \eqref{PDE Q} with \eqref{smooth profile: initial data -1}, additional effort is required to derive quantitative properties of the profile $Q$. Combined with the nonlocal nature of \eqref{equation: KS with damping}, these complexities make the establishment of linear coercivity of the Keller-Segel equation more intricate than in the case of the semilinear heat equation \eqref{PDE: nonlinear heat}.  Detailed strategies to handle these obstacles will be presented in Section~\ref{sec: linear theory}.
    
    
    
\end{remark}

    \section{Existence of profile via phase-portrait method}
    \label{sec: ODE}
This section is devoted to the existence of smooth profile solving \eqref{PDE Q} when $\mu< \frac{1}{3}$ with the appropriate choices of $\beta$. Firstly, note that for any radially symmetric function $R(y)$ satisfying $R(y) \to 0$ as $|y| \to \infty$,
\be
    \nabla\Delta^{-1}R (y) = \frac{y}{|y|^3} \int_0^{|y|} R(s)s^2 ds,
    \label{nonlocal term: formula}
\ee
Then, under the radial symmetric assumption, \eqref{PDE Q} becomes 
\be\label{ode Q}
    \left(\frac{1}{r^2}\int_0^r Q(s)s^2 ds-\beta r \right) Q'(r) -Q + (1-\mu)Q^2=0.
\ee
If $f_Q \not = \beta$, by introducing $f_Q$ (cf. \eqref{f: definition}), then we obtain an ODE system of $(Q(r),f(r))$ for $r >0$:
\be
\begin{cases}
   Q'(r) = \frac{1}{\beta -f_Q} \frac{(1-\mu) Q^2 - Q}{r},\vspace{0.2cm} \\
   f_Q'(r) = \frac{Q-3f_Q}{r}.
\end{cases}
\label{ODE system}
\ee

\begin{remark}
    For notational simplicity, in the subsequent discussion of this section, we introduce the following notations: we write $f :=f_Q$, and $Q_i := [Q]_i$ and $f_i := [f]_i$ for any $i \in \ZZ_{\ge 0}$, where $f_Q$ is given in \eqref{ODE system}, $[Q]_i$ and $[f]_i$ are the $2i$-th order coefficients of Taylor expansion of $f$ and $Q$ at the origin respectively (cf. \eqref{Taylor coefficient: def}).
\end{remark}

Our main result of this section is as follows, which gives the existence of the nontrivial smooth solutions to \eqref{ODE system} and the asymptotic behavior of the related solutions when $r=0$ and $r \to \infty$.


\begin{lemma}
\label{lem: solve ODE}
    For any fix $\mu\in[0,\frac13)$, let $\beta:=\beta(j_0,\mu) = \frac{1}{3(1-\mu)}+\frac{1}{2j_0}$ with arbitrarily fixed $j_0\geq J>1$ where $J$ is defined in \eqref{J: def}. Then, for any $Q_{j_0}<0$, there exists a unique smooth solution $(Q(r),f(r))$ to \eqref{ODE system} on $r \ge 0$ with initial conditions:
    \begin{align}
    (Q(0),f(0)) = \left( \frac{1}{1-\mu}, \frac{1}{3(1-\mu)} \right) \quad \text{ and } \quad 
    \partial_r^{2j_0} Q(0) = (2j_0)! Q_{j_0}.
    \label{ODE: initial assumption}
    \end{align}
  
    Moreover, the solution  $(Q(r),f(r))$ satisfies
    \begin{enumerate}
    \item  $(Q(r),f(r))$ is analytic near the origin. Precisely, there exists $\epsilon>0$ such that $(Q(r),f(r))$ can be expressed as Taylor series
\be
	Q(r) =\sum_{j =0}^{\infty} Q_{j}r^{2 j} \quad \text{and}\quad f(r) = \sum_{j =0}^{\infty} f_{j}r^{2 j}, \quad \forall \; r \in [0,\epsilon],
    \label{(Q,f), expansion}
\ee
where $\{Q_j\}_{j\geq 0}$ and $\{ f_j \}_{j\geq 0}$ satisfy the following recurrence relations
\be
\quad f_j = \frac{1}{2j+3} Q_j, \quad  \forall \; j \ge 0,
\label{recurrence relation 1}
\ee
and
\be
Q_j
=
\begin{cases}
\frac{1}{1-\mu}, & j=0, \vspace{0.1cm} \\
0, & 0< j < j_0, \vspace{0.1cm} \\
\frac{ \sum_{i=1}^{j-1} \left( \frac{2i}{2(j-i)+3} + (1-\mu)  \right)Q_i Q_{j-i} }{2j \left( \beta -\frac{1}{2j} - \frac{1}{3(1-\mu)} \right)}, & j >j_0.
\end{cases}
\label{recurrence Qj}
\ee
\item Both $Q(r),f(r)>0$ are strictly positive for $r\in[0,\infty)$ and monotonically decrease from $Q_0=\frac{1}{1-\mu}$ \big(respectively, $f_0 = \frac{1}{3(1-\mu)}$\big) to 0 as $r \to +\infty$. 
\item For any $j \ge 0$, there exists a constant $C=C(\beta,Q,j)>0$ such that
\be\label{decay estimates of Q}
|\partial_r^{(j)}Q(r)| + |\partial_r^{(j)}f(r)|\le C \la r \ra ^{-2-j} \quad \text{for} \quad  r \in \overline{\RR^+}.
\ee
In particular, $Q \in H^\infty (\RR^3)$.
    \end{enumerate}
\end{lemma}
\begin{proof}
\textit{Step 1. Solve \eqref{ODE system} via Taylor expansion.}
We assume that $(f(r),Q(r))$ can be expanded into the following forms:
\[
f(r) = \sum_{j=0}^\infty f_j r^{2j}, \quad Q(r) = \sum_{j=0}^\infty Q_j r^{2j},
\]
which yields that
\[
r f'(r)= \sum_{j=0}^\infty 2j f_j r^{2j}, \quad rQ'(r) = \sum_{j=0}^\infty 2j Q_j r^{2j}.
\]
Next, we substitute these expressions into the ODE system \eqref{ODE system} and match coefficients to establish \eqref{recurrence relation 1} and \eqref{recurrence Qj}. Precisely, we first expand the second equation in \eqref{ODE system} to get that
\[
\sum_{j=0}^\infty 2j f_j r^{2j} = \sum_{j=0}^\infty \left( Q_j -3 f_j \right) r^{2j}.
\]
which directly induces \eqref{recurrence relation 1}. 

Next, we expand $(\beta-f) r \partial_r Q = (1-\mu) Q^2- Q$, the first equation in \eqref{ODE system}. Using the identity
\[
\left( \sum_{j=0}^\infty h_j r^{2j} \right) \left( \sum_{j=0}^\infty k_j r^{2j} \right) = \sum_{j=0}^\infty \left( \sum_{i=0}^j k_i h_{j-i} \right) r^{2j},
\]
the left-hand side of the equation becomes
\begin{align*}
    \left( \beta -  \sum_{j=0}^\infty f_j r^{2j} \right) \left( \sum_{j=0}^\infty 2j Q_j r^{2j} \right) 
    & = \beta \sum_{j=0}^\infty 2j Q_j r^{2j} - \sum_{j=0}^\infty \left( \sum_{i=0}^j 2iQ_i f_{j-i} \right) r^{2j} \\ &= \sum_{j=0}^\infty \left(2 \beta j - \sum_{i=0}^j 2i Q_i f_{j-i} \right) r^{2j},
\end{align*}
and the right-hand side of the equation becomes
\begin{align*}
(1-\mu)\sum_{j=0}^\infty \left( \sum_{i=0}^j Q_i Q_{j-i} \right) r^{2j} - \sum_{j=0}^\infty Q_j r^{2j}  
 = \sum_{j=0}^\infty \left( (1-\mu) \sum_{i=0}^j Q_i Q_{j-i} -Q_j \right) r^{2j}.
\end{align*}
Comparing the coefficients on both sides, we obtain that
\[
2 \beta j Q_j - \sum_{i=0}^j 2i Q_i f_{j-i} = (1-\mu) \sum_{i=0}^j Q_i Q_{j-i} -Q_j, \quad \forall \;  j \ge 0.
\]
Replacing $f_{j-i}$ by using \eqref{recurrence relation 1}, we decouple the recurrence relations for $\{Q_j\}_{j=0}^\infty$ into
\[
2 \beta j Q_j - \sum_{i=0}^j \frac{2i}{2(j-i)+3} Q_i Q_{j-i} = (1-\mu) \sum_{i=0}^j Q_i Q_{j-i} -Q_j, \quad \forall \;  j \ge 0.
\]
In particular,
\[
(1-\mu) Q_0^2 -Q_0 =0, \quad \text{for } \; j=0,
\]
and $Q(0) = Q_0 = \frac{1}{1-\mu}$ exactly solves this equation. For $j\geq 1$, we isolate the highest index term $Q_j$ to obtain
\[
2j \Big(  \beta  - \frac{1}{2j} - \frac{1}{3(1-\mu)} \Big) Q_j = \sum_{i=0}^{j-1} \left( \frac{2i}{2(j-i)+3} + (1-\mu)  \right)Q_i Q_{j-i}.
\]
In particular, applying $j=1$ to the equation together with the fact that $\beta< \frac{1}{2}$ and $1+\frac{1}{3(1-\mu)}>1$, it induces
\[
2\left(  \beta  - \left(\frac{1}{2} + \frac{1}{3(1-\mu)} \right) \right) Q_1=0, \quad \Rightarrow \quad Q_1 =0.
\]
Iteratively, with the choice of $\beta = \frac{1}{3(1-\mu)}+ \frac{1}{2j_0}$,
\[
\beta- \frac{1}{2j} - \frac{1}{3(1-\mu)} = \frac{1}{2j_0} - \frac{1}{2j} \not =0, \quad \Rightarrow \quad Q_j=0, \quad \forall \; 2 \le j < j_0.
\]
Similarly, with $\partial_r^{2j_0} Q(0) =Q_{j_0}<0$ determined in \eqref{ODE: initial assumption},
\[
\beta- \frac{1}{2j} - \frac{1}{3(1-\mu)} \not =0, \; \Rightarrow \; Q_j =\frac{ \sum_{i=1}^{j-1} \left( \frac{2i}{2(j-i)+3} + (1-\mu)  \right)Q_i Q_{j-i} }{2j \left( \beta -\frac{1}{2j} - \frac{1}{3(1-\mu)} \right)}, \quad \forall \; j > j_0.
\]
Hence, we obtain the recurrence relation \eqref{recurrence Qj}.

We remark here that under the previous argument, if $\beta - \frac{1}{2j} - \frac{1}{3(1-\mu)} \not= 0$ for all $j \ge 1$, then $Q_j =0$ for all $j \ge 1$. In this case, $Q(r) \equiv \frac{1}{1-\mu}$, which is a constant solution and not our focus. Hence, to obtain a non-constant solution, we must give the vanishing condition that $\beta - \frac{1}{2j_0} - \frac{1}{3(1-\mu)} = 0$ for some $j_0 \ge 2$, which exactly matches the choice of $\beta$.

\mbox{}

\noindent \textit{Step 2. Analyticity of $(Q,f)$ near the origin.}
First of all,  recalling \cite[Lemma B.1]{guoMahirJangpolytropicgap}, there exists a universal constant $a>0$ such that for all $L\in\NN$,
\be
    \sum_{\substack{i+j=L \\ i,j>0}} \frac{1}{i^2 j^2} \le \frac{a}{L^2},    
    \label{combinatorics ineq}
\ee
which, by using the fact that $Lj \ge i$ for any $1 \le  i,j \le L-1$, yields that
\be\label{combinatorics ineq 1}
    \sum_{\substack{i+j=L \\ i,j>0}} \frac{1}{i j^3} \leq \sum_{\substack{i+j=L \\ i,j>0}} \frac{L}{i^2 j^2} \leq \frac{a}{L}.
\ee
Next, we are devoted to the estimates of coefficients of the Taylor expansion determined in \eqref{recurrence Qj}. Precisely, we claim that there exists $K, \alpha >0$, such that 
\be
|Q_j| \le \frac{K^{j-\alpha}}{j^2}, \quad \forall \; j \ge j_0,
\label{bound for Q_j}
\ee
where $K, \alpha>0$ satisfy
\be
|Q_{j_0}| \le \frac{K^{j_0 -\alpha}}{j_0^2} \quad \text{ and } \quad \frac{a K^{-\alpha}}{\frac{1}{2j_0} - \frac{1}{2(j_0+1)}} < \frac{1}{2}.
\label{initial Q_j}
\ee

In fact, we proceed by induction. For $1 \le j \le j_0$, it automatically holds with \eqref{recurrence Qj} and \eqref{initial Q_j}. We now assume that \eqref{bound for Q_j} holds for any $j_0 \le j \le L$, then by using \eqref{recurrence Qj}, \eqref{combinatorics ineq}, \eqref{combinatorics ineq 1}, \eqref{bound for Q_j} and \eqref{initial Q_j}, we obtain
\begin{align*}
     Q_{L+1} &= \frac{1}{2(L+1) \left( \beta - \frac{1}{2(L+1)} - \frac{1}{3(1-\mu)} \right)} \sum_{\substack{i+j=L+1 \\ i,j>0}} \left( \frac{2i}{2j+3} + (1-\mu) \right) Q_i Q_j
     \\
    &\le \frac{1}{2(L+1)\left( \frac{1}{2j_0} - \frac{1}{2(j_0+1)} \right)}\sum_{\substack{i+j=L+1 \\ i,j>0}}  \left( \frac{2i}{2j+3} + (1-\mu) \right) \frac{K^{L+1 -2 \alpha}}{i^2 j^2} \\
    & \le \frac{K^{L+1-2 \alpha} }{2(L+1)\left( \frac{1}{2j_0} - \frac{1}{2(j_0+1)} \right)}\sum_{\substack{i+j=L+1 \\ i,j>0}} \left( \frac{1}{ij^3} + \frac{1}{i^2j^2} \right) \le \frac{K^{L+1-\alpha}}{(L+1)^2},
\end{align*}
which yields the validity of \eqref{bound for Q_j} with $j=L+1$, hence we have closed the induction and verified the claim.

The analyticity of $Q$ at the origin then follows from Cauchy's convergence criterion for power series. Precisely, there exists $\epsilon = \epsilon(K) \ll 1$ such that the series
\[
Q(r) =  \sum_{j=0}^\infty Q_{j} r^{2j}, \quad \text{ with } Q_j \text{ determined in \eqref{recurrence Qj},} 
\]
is absolutely convergent on $[0,\epsilon]$. The analyticity of $f(r) =\sum_{j=0}^\infty f_j r^{2j}$ on $r \in [0,\epsilon]$ simply follows \eqref{recurrence relation 1} and the analyticity on $[0,\epsilon]$ of $Q$.

\mbox{}

\noindent \textit{Step 3. Extend $(Q,f)$ to $[0,+\infty)$.} 
At this stage, our objective is to extend the previously constructed solution to $\overline{\RR^+}$, and verify that both $f(r)$ and $Q(r)$ will asymptotically decay to $0$ and the solution curve (see the red curve in Figure \ref{fig3})) remains within $\calM$ with
\[ \mathcal M :=\left\{(Q,f) \Big| \;  0< Q<Q_0, \; \frac{Q}{3}<f<\beta\right\}.\]
Here, recalling \eqref{ODE system} or Figure \ref{fig3}, we observe that both $(Q(r)$ and $f(r))$ are strictly decreasing once the solution curve stays within $\calM$, i.e.
\be 
Q'(r) < 0, f'(r)<0 \quad \text{ if} \quad (Q(r),f(r)) \in \text{ $\mathcal M$}.
\label{M: decreasing}
\ee
We first claim that there exists $\nu \in (0,\epsilon)$ such that $(Q(r),f(r)) \in \calM, \; \forall \; r \in (0,\nu]$. To verify this, since
\[
\frac{d^j}{dr^j} Q(0) = 0, \quad \forall \; 1 \le j < 2j_0  \qquad \text{ and } \qquad
\frac{d^{2 j_0}}{dr^{2j_0}} Q(0) = (2j_0)! Q_{j_0} <0,
\]
it follows that both $Q(r)$ and $f(r)$ are strictly decreasing on $[0,\nu]$ for some $0<\nu \le  \epsilon \ll 1$. Consequently, the portion of the solution curve for $r \in [0,\nu]$, which begins at $P_0$ \eqref{P_0: def}, remains within the lower-left area of $P_0$. Furthermore, it continues to be representable as a graph, meaning that there is a smooth function $\calF$ with 
\[
f = \calF(Q)  \quad \text{ on } \quad  Q \in \left[Q_0 - \nu_Q, Q_0 \right],
\]
for some $0 <\nu_Q \ll 1$. By chain rule, \eqref{ODE system}, \eqref{(Q,f), expansion}, \eqref{recurrence relation 1}  \eqref{recurrence Qj} and $j_0 \ge J >1$,
\begin{align*}
    \mathcal F'(Q_0)
    &=\frac{df}{dQ}\Big|_{(Q,f)=P_0}
    = \lim_{r \to 0^+}\frac{(Q(r)-3f(r))(\beta-f(r))}{(1-\mu)Q^2(r)-Q(r)} 
    \\
    &
    = \frac{\beta - f_0}{(1-\mu) Q_0} \frac{Q_{j_0} -3f_{j_0}}{Q_{j_0}}
    = \frac{1}{2j_0} \left( 1- \frac{3}{2j_0 +3} \right) < \frac{1}{2j_0} \le \frac{1}{4} < \frac{1}{3}.
\end{align*}
Thus, the slope of the solution curve at $P_0$ is strictly less than that of the line $f= \frac{1}{3} Q$, which contains the lower boundary of $\calM$. So by adjusting $0< \nu \ll 1$ if necessary and using the smoothness of $\calF$, we conclude that the curve $\{(Q(r), f(r))\}_{r \in(0,\nu]}$ lies above $f = \frac{1}{3} Q$. This has verified the claim.
\vspace{2mm}

Next, we prove that the solution curve remains in $\mathcal M$ for all $r\in(0,\infty)$. In fact, ensured by the Cauchy-Lipschitz theory, with the strict decay property of the solution within $\calM$ (see \eqref{M: decreasing}), there are only three possible scenarios:
\begin{enumerate}
    \item there exists $r_{E1} \in (0,\infty]$, such that the solution exits the region $\mathcal M$ at a point $\left( Q_{E1},\frac{Q_{E1}}{3} \right)$ through the line $f=\frac{Q}{3}$, where $Q_{E1} = Q(r_{E1})\in \left(0, Q_0 \right)$;
    \item there exists $r_{E2} \in (0,\infty]$, such that the solution exits the region $\mathcal M$ at a point $(0,f_{E2})$ through the $f$-axis, where $f_{E2} = f(r_{E2})\in(0,f_0)$;
    \item the solution escapes $\mathcal M$ at the origin $O$.
\end{enumerate}

We now eliminate scenarios $(1)$ and $(2)$ by contradiction arguments. 

For the scenario $(1)$, we assume that it occurs. Since $(Q(r),f(r))$ is strictly decreasing before reaching the line $f=\frac{Q}{3}$, together with Cauchy-Lipschitz theory, the solution curve can be further extended on $Q\in[Q_{E1},Q_0]$ and represented as $Q \mapsto \calF(Q)$ with $\calF$ a smooth function.

On the one hand, since $\{(Q(r),f(r))\}_{r \in (0,r_{E_1})} \subset \calM $, it follows that $f(r) > \frac{1}{3} Q(r)$ for any $r \in (0,r_{E_1})$ and $f(r), Q(r)$ is strictly decreasing on $r \in (0,r_{E_1})$, thus together with $f(r_{E_1}) = \frac{1}{3}Q(r_{E_1})$,
\[
\calF'(Q_{E1})
= \lim_{r \to r_{E_1}^-} \frac{f(r) - f(r_{E_1})}{Q(r)-Q(r_{E_1})}
\ge \lim_{r \to r_{E_1}^-} \frac{\frac{1}{3}Q(r) - \frac{1}{3} Q(r_{E_1})}{Q(r) - Q(r_{E_1})} = \frac{1}{3}.
\]

On the other hand, recalling the ODE system \eqref{ODE system} together with $f(r_{E_1}) = \frac{1}{3}Q(r_{E_1})$ again, we compute
\begin{align*}
    \mathcal F'(Q_{E1}) = 
    \lim_{r \to r_{E1}^-}\frac{(Q(r)-3f(r))(\beta-f(r))}{(1-\mu)Q^2(r)-Q(r)} =0< \frac{1}{3},
\end{align*}
which contradicts our assumption and hence we have ruled out the scenarios $(1)$.

Regarding the second scenario $(2)$, by an argument analogous to that of the first case, the solution curve can be extended on $f \in [f_{E2}, f_0]$ and represented as $f \mapsto \calQ(f)$ with $\calQ$ a smooth function, and thus
\be
\{ \left(Q(r), f(r) \right) \}_{r \in \big(0,r_{E_2} \big)} 
=\{ \left( \calQ(f), f \right) \}_{f \in \big(f_{E_2}, f_0 \big)}
\subset \calM.
\label{case 2: one hand}
\ee
Recall \eqref{ODE system} again, $\calQ(f)$ is governed by the equation
\be
\calQ'= \frac{(1-\mu) \calQ^2 - \calQ}{(\calQ -3f) (\beta -f)}, \quad \forall\; f  \in  [f_{E2}, f_{0}],
\label{case 2: ODE}
\ee
whose local wellposedness near $f=f_{E_2}$ is well established by the Cauchy-Lipschitz theory. Nevertheless, besides the nontrivial solution curve given in \eqref{case 2: one hand}, we observe that $\{ (0, f)\}_{f\in [f_{E_2}, f_0]}$ is also a satisfied solution curve, which leads to a contradiction and hence we have ruled out the scenario $(2)$.


Consequently, we have shown that the solution curve could only exist $\mathcal M$ at the origin $O$, i.e. in scenario $(3)$. To conclude this step, it suffices to verify that 
\be
\lim_{r\to \infty}(Q(r),f(r))=(0,0).
\label{Step 3: decay of Q,f}
\ee
In fact, similar to the previous argument, the solution curve can be further smoothly extended and represented as $Q \mapsto \calF(Q)$ on $[0,Q_0]$. Additionally, using \eqref{M: decreasing} again, the function $r \mapsto Q(r)$ is one-to-one and thus $r$ can be expressed by $r= \calR(Q)$ on $Q \in [0,Q_0]$, with $\calR$ solving
\[
    \mathcal R'(Q) = \mathcal R(Q) \frac{\beta-\mathcal F(Q)}{(1-\mu) Q^2- Q},
\]
which follows from the inverse function theorem and \eqref{ODE system}. Then, a direct computation together with \eqref{ODE: initial assumption}, \eqref{recurrence relation 1}, \eqref{M: decreasing} and the fact that $\mathcal R(\frac{Q_0}{2})\in(0,\infty)$ yields that 
\begin{align*}
    \lim_{Q \to 0^+}\ln \mathcal R(Q) &=\ln \mathcal R\left(\frac{Q_0}{2} \right) +\lim_{Q \to 0^+}\int_{\frac{Q_0}{2}}^{Q} \frac{\beta-\mathcal F(\tilde Q)}{(1-\mu)\tilde Q^2-\tilde Q} \ d\tilde Q \\
    &> \ln \mathcal R\left(\frac{Q_0}{2}\right) +(\beta - f_0)\lim_{Q \to 0+}\int_{\frac{Q_0}{2}}^{Q} \left( \frac{1}{\tilde Q-\frac{1}{1-\mu}}-\frac{1}{\tilde Q} \right) \ d\tilde Q 
    = + \infty,
\end{align*}
and thus we have verified \eqref{Step 3: decay of Q,f} and finished this step.

\mbox{}

\noindent \textit{Step 4. Uniqueness.} Assume that there exist two smooth solutions $(Q^{(1)},f^{(1)})$ and $(Q^{(2)},f^{(2)})$ solving the system \eqref{ODE system} with the same initial conditions \eqref{ODE: initial assumption}, then by the $C^\infty$ continuity of $Q$ at the origin and a similar argument as in \textit{Step 1} and \textit{Step 3}, it can be verified that $(Q^{(i)},f^{(i)})$ satisfies
\begin{align}\label{condition to unique}
    Q_0^{(1)} = Q_0^{(2)} = \frac{1}{1-\mu},
\quad 
Q_j^{(1)} = Q_j^{(2)} = 0 \quad \left( \text{with } 1 \le j < j_0-1 \right), \quad 
Q_{j_0}^{(1)} = Q_{j_0}^{(2)}  < 0,
\end{align}
and both $Q^{(i)}(r)$ and $f^{(i)}(r)$ are strictly decreasing on $\RR^+$ for both $i=1,2$. Next, we study the difference between these two solutions. Denote
\[
(\triangle Q,\triangle f) := (Q^{(1)}-Q^{(2)}, f^{(1)} -f^{(2)}),
\]
which solves the following ODE system:
\[
\begin{cases}
    (\triangle Q)' = \frac{1}{\beta -f^{(1)}} \frac{(1-\mu)(Q^{(1)}+Q^{(2)}) \triangle Q - \triangle Q}{r} - \frac{(1-\mu) (Q^{(2)} )^2 -Q^{(2)}}{r} \frac{\triangle f}{(\beta-f^{(1)})(\beta-f^{(2)})}, \vspace{0.1cm}\\
    (\triangle f)' = \frac{\triangle Q - 3\triangle f}{r}.
\end{cases}
\]
We define
\[
\calE(r)  : = |\triangle Q(r)|^2 + |\triangle f(r)|^2,
\]
and compute
\begin{align*}
         \;\; \calE' &= I+II, \\
      \text{ with } \ \ I &= 2 \frac{\triangle f \triangle Q -3 (\triangle f)^2}{r} 
    + 2\frac{(1-\mu) (Q^{(1)}+Q^{(2)}) -1}{(\beta -f^{(1)})r} (\triangle Q)^2, \\
        \; II&=  -2 \frac{(1-\mu) (Q^{(2)})^2 -Q^{(2)}}{r} \frac{1}{(\beta -f^{(2)})(\beta-f^{(1)})} \triangle f \triangle Q,
     \end{align*}
By using Cauchy inequality, strictly decreasing fact of $Q^{(i)}(r)$ and $f^{(i)}(r)$, \eqref{ODE: initial assumption} and \eqref{recurrence relation 1}, we bound $I$ by
\begin{align*}
    I \leq  \Big(1+ 2\frac{(1-\mu) (Q^{(1)}(0)+Q^{(2)}(0)) -1}{(\beta -f^{(1)}(0))}\Big) \frac{\mathcal E(r)}{r} = (4j_0+1)\frac{\mathcal E(r)}{r}.
\end{align*}
Applying condition \eqref{condition to unique} along with the Cauchy's inequality, there exists constant $M= M(j_0,\mu, Q^{(1)}, Q^{(2)})>0$ such that
\begin{align*}
    II \le  M |\triangle f \triangle Q| \leq M \calE(r),
\end{align*}
which yields that
\[
    \calE'(r) = I+II \leq (4j_0 + 1) \frac{\calE(r)}{r} + M \calE(r).
\]
Applying Gronwall's inequality,
\begin{align*}
    0 \le \calE(r) \le  \calE(\delta)\left( \frac{r}{\delta} \right)^{4 j_0 +1}  e^{M(r-\delta)}, \quad \text{ uniformly for } r,\delta>0.
\end{align*}
Since $(Q^{(i)},f^{(i)})$ (with $i=1,2$) satisfy the same initial conditions \eqref{condition to unique}, it follows that
\[
\partial_r^{j} \calE(r) \Big|_{r=0} =0, \quad \forall \; 0 \le j \le 4j_0+2,
\]
which implies that
\[
\lim_{\delta \to 0+} \frac{\calE(\delta)}{\delta^{4j_0+1}} e^{-M \delta} = 0.
\]
By the squeezing theorem, it follows that $\calE(r) \equiv 0$ for any $r \ge 0$. Consequently, we conclude $Q^{(1)} \equiv Q^{(2)}$ and this completes the uniqueness.


\mbox{}

\noindent \textit{Step 5. Decay estimate of $Q$ and its derivative.} 
Based on the discussion in \textit{Step 3}, both $Q(r)\searrow 0$ and $f(r)\searrow 0$ as $r\to \infty$. Next for any fixed $\nu_0>0$, recalling the choice of $\beta= f_0+ \frac{1}{2j_0}$, there exists $M_0 = M_0(\nu_0)\gg 1$ such that
\begin{align*}
    & \qquad \quad 0<(1-\nu_0)Q(r)\leq Q(r)-(1-\mu)Q^2(r)\leq Q(r), \quad \forall \; r \ge M_0, \\
    & \text{ and } \; \; -2j_0\leq -\frac{1}{\beta-f}\leq -\frac1\beta <0.
\end{align*}
From the ODE \eqref{ODE system} satisfied by $Q(r)$, these inequalities imply
\[
- \frac{2j_0Q}{r} \le Q'(r) \le -\frac{(1-\nu_0) Q}{\beta r}, \quad \quad \forall \; r \ge M_0,
\]
hence
\[
Q(r) \le  Q(M_0) \left( \frac{r}{M_0} \right)^{-\frac{1}{\beta}(1-\nu_0)}, \quad \forall \; r \ge M_0.
\]
In particular, since $\beta < \frac{1}{2}$, we can choose $\nu_0 >0$ sufficiently small such that $\frac{1-\nu_0}{\beta}< 2$. This allows us to find a constant $C=C(\beta,M_0) > 0$ such that
\be
Q(r) \le C \la r \ra^{-2}, \quad \forall \; r \ge 0.
\label{Lemma 2.2 decay 1}
\ee
Moreover, using the second equation in \eqref{ODE system}, there exists a constant $C= C(\beta,M_0)>0$ such that
\be
0< f(r) = \frac{1}{r^3} \int_0^r Q(s) s^2 ds \le \frac{C}{r^3} \int_0^r \frac{s^2}{\la s \ra^2} ds \le C \la r \ra^{-2}, \quad \forall \; r \ge 0.
\label{lemma 2.2 decay 2}
\ee
For the derivatives of $Q(r)$ and $f(r)$, applying $\partial_r^{j-1}$ (with $j \ge 1$) to \eqref{ODE system} and using the base decay estimates \eqref{Lemma 2.2 decay 1} and \eqref{lemma 2.2 decay 2}, a straightforward induction then shows that
\begin{align}
|\partial_r^{(j)}Q(r)| \le C \la r \ra^{-2-j},
\label{asym Q higer order}
\end{align}
for some constant $C=C(\beta,M_0,j)>0$.

Finally, combining the $C^\infty$ smoothness of $Q$, the above decay bound on $\partial_r^{(j)}Q$ (cf. \eqref{Lemma 2.2 decay 1} and \eqref{asym Q higer order}), and the standard identity $D g= \frac{x}{|x|} \cdot \na g$ for radial function $g$, we can verify that $Q \in H^\infty(\RR^3)$. This completes the proof of the lemma.
\end{proof}



Based on Lemma \ref{lem: solve ODE}, one naturally obtains the existence of a smooth profile satisfying \eqref{PDE Q}. More precisely, we have the following result.

\begin{corollary}[Existence of smooth self similar profile]
\label{thm: existence of the profile}
Under the assumptions of Lemma \ref{lem: solve ODE}, for any fixed $[Q]_{j_0} <0$, there exists a unique smooth radial symmetric solution $Q\in H^\infty(\RR^3)$ to \eqref{PDE Q} satisfying
    \be
    Q(0) = \frac{1}{1-\mu}, \quad \text{ and } \partial_r^{(2j_0)} Q(0) = (2j_0)! [Q]_{j_0} <0.
    \label{smooth profile: initial data}
    \ee
    In particular, $Q(r)$ is strictly radially decreasing with respect to $r \ge 0$ and satisfies the decay estimates \eqref{decay estimates of Q}.
\end{corollary}




\section{Linear theory}
\label{sec: linear theory}
Starting from this section, we fix $\mu\in[0,\frac{1}{3})$ and a positive integer $j_0\geq \frac{3(1-\mu)}{1-3\mu} +1>1$, then we have
\be
\beta =  \frac{1}{3(1-\mu)} + \frac{1}{2j_0}\in \left(0,\frac{1}{2} \right).
\label{beta: def}
\ee
We now introduce the self-similar coordinate:
\be
 y =\frac{x}{\lambda^{2\beta}}, \quad \frac{d\tau}{dt} = \frac{1}{\lambda^2}, \quad 
 \tau\Big|_{t=0} = 0, \quad \frac{\lambda_\tau}{\lambda} = -\frac{1}{2},
 \label{ss coordinte}
\ee
and the corresponding renormalization
\be
\rho(t,x) = \frac{1}{\lambda^2} \Psi \left( \tau, y \right).
\label{ss renormalization}
\ee
The equation \eqref{equation: KS with damping} can be mapped into the renormalization system of $\Psi$:
\be
\partial_\tau \Psi = \lambda^{2-4\beta} \Delta \Psi - \Psi - \beta y \cdot \na \Psi + \na \Psi \cdot \na \Dein \Psi + (1-\mu) \Psi^2,
\label{renormalization KS}
\ee
where, from \eqref{ss coordinte}, the function $\lambda$ is
\be
\lambda(\tau) = \lambda_0 e^{-\frac{1}{2} \tau}, \quad \forall \; \tau \ge 0,
\label{lambda: form}
\ee
with initial data given by $\lambda \Big|_{\tau=0}=\lambda_0>0$. 

Next, we consider a solution to the above equation in perturbative form
\[
    \Psi = Q+ \ep,
\]
where $Q$ is a solution to the PDE \eqref{PDE Q}, corresponding to the fixed parameters $\mu$ and $j_0$, whose existence is established in Lemma \ref{lem: solve ODE}. Direct computation shows 
the residue $\ep$ solves
\be
\partial_\tau \ep  =  \calL \ep + \lambda^{2-4\beta} \Delta \Psi + N(\ep),
\label{linearized eq}
\ee
where $\calL$ is the linear operator
\be
\calL \ep = -(\ep + \beta y \cdot \na  \ep) + \na \ep \cdot \na \Dein Q + \na Q \cdot \na \Dein \ep + 2(1-\mu) Q \ep,
\label{linearized op}
\ee
and $N(\ep)$ is the nonlinear term
\be
N(\ep) = \na \ep \cdot \na \Dein \ep  + (1-\mu) \ep^2.
\label{nonlinear term}
\ee
For the linear operator $\calL$ given in \eqref{linearized op}, we will prove its coercivity in the sense of $L_w^2$ for some weight $w$ sufficiently singular at the origin. Precisely, we have the following result:
\begin{proposition}[Coercivity of $\calL$ in $L_w^2$]
\label{prop: coer}
    For $\calL$ given in \eqref{linearized op}, there exists a weight defined by
    \be
    w(y) :=  |y|^{-A} + B,
    \label{singular weight}
    \ee
    where $(A,B) \in \ZZ_+ \times \RR_+$ satisfy $A \gg 4 j_0 +3$ and $\frac{A}{4} \in  \ZZ_{>0}$, such that $\calL$ satisfies the coercivity in the following sense:
    \be
    \left( \calL g,g \right)_{L_w^2} \le - \frac{1}{8} \|g\|_{L_w^2}^2, \quad \forall \; g \in L_w^2(\RR^3) \quad \text{radially symmetric}.
    \label{L: coer}
    \ee
\end{proposition}

\begin{remark}
    Due to the limited quantitative properties of $Q$ available from Lemma \ref{lem: solve ODE} and the nonlocal structure of the operator $\mathcal{L}$, it is difficult to identify the optimal value of $A$ explicitly, in contrast with the situation for the heat equation discussed in Section \ref{sec:slh}. Nevertheless, the existence of some $A$ satisfying \eqref{L: coer} is sufficient for our subsequent analysis.
\end{remark}

\begin{proof}[Proof of Proposition \ref{prop: coer}]
    First of all, for any $g \in L_w^2$, by integration by parts, 
    \eqref{nonlocal term: formula} and the fact that $y \cdot \na w = -A |y|^{-A}$,
    \begin{align*}
      -\beta \int (y \cdot \na g) g w dy
        = \frac{\beta}{2}\left( -A + 3 \right)\int g^2 |y|^{-A} dy 
        +\frac{3B \beta}{2} \int g^2 dy,
    \end{align*}
    and
    \begin{align}
    \int \left( \na g \cdot \na \Dein Q \right) g w dy 
     = -\frac{1}{2} \int Q g^2 w dy + \frac{A}{2} \int g^2 f_Q |y|^{-A}dy,
     \label{coercivity: IBP method}
    \end{align}
    with which, recalling the definition of $\calL$ ( see \eqref{linearized op}),  we split $(\calL g,g)_{L_w^2}$ into the following three parts:
    \be
    (\calL g,g)_{L_w^2}
    = I_{SI} + I_{LO} + I_{NLO},
    \label{(Lg,g) L2 form}
    \ee
    where
    \begin{align*}
        & I_{SI} : =\left( -1 + \frac{\beta}{2} (-A+3) \right) \int g^2 |y|^{-A} dy + \frac{A}{2} \int g^2 f_Q |y|^{-A}dy + \left( \frac{3}{2} -2 \mu \right) \int g^2 Q |y|^{-A} dy , \\
        & I_{LO} :=\left( -B + \frac{3B \beta}{2} \right) \int g^2 dy + \left(\frac{3}{2}-2\mu \right) B \int g^2 Q dy, \quad I_{NLO}:=\int \left( \na Q \cdot \na \Dein g \right) g w dy.
    \end{align*}
     Here $I_{SI}$ denotes the sum of local terms involving the singular weight $|y|^{-A}$, $I_{LO}$ denotes the sum of local terms without singular weight, and $I_{NLO}$ denotes the sum of nonlocal terms.

   \mbox{}
   
    \noindent \underline{\textit{Estimate of $I_{SI}$}.} 
    By Lemma \ref{lem: solve ODE},  $Q$ and $f_Q$ are both radially decreasing. Moreover, recalling the initial conditions of $(Q(0),f_Q(0))$ given in \eqref{ODE: initial assumption} and the definition of $\beta$ in \eqref{beta: def}, $I_{SI}$ can be estimated by
\begin{align}
    I_{SI} 
     & \le \left( -1 + \frac{\beta}{2} (-A+3) \right) \int g^2 |y|^{-A} dy 
     + \left( \frac{A}{2} f_Q(0) + \left(\frac{3}{2}-2\mu \right) Q(0) \right) \int g^2 |y|^{-A} dy \notag\\
     & = \left( -1 + \frac{\frac{1}{3(1-\mu)}+ \frac{1}{2j_0}}{2} (-A+3) + \frac{A}{6(1-\mu)} + \left(\frac{3}{2}-2\mu \right) \frac{1}{1-\mu} \right) \int g^2 |y|^{-A} dy \notag\\
     & = \left( 1 + \frac{-A+3}{4j_0} \right) \int g^2 |y|^{-A} dy,
     \label{coer: singularity weight estimate 1}
\end{align}
where the coercivity becomes linearly stronger as $A \gg 1$ grows.

We remark here that the derivation of \eqref{coer: singularity weight estimate 1} is rather delicate. Precisely, one might naturally expect that the term $g + \beta y \cdot \na g$ alone provides enhanced coercivity with increasing $A$. However, this gain is offset by the contribution $\frac{A}{2} \int g^2 f_Q |y|^{-A} dy$, which greatly diminishes the coercivity originating from the scaling term. Nevertheless, with the estimate given in \eqref{coer: singularity weight estimate 1}, we find that this essential obstacle can be almost exactly controlled via the fact that $\beta -f_Q(r) \ge \beta -f_Q(0) = \frac{1}{2j_0}>0$.

\mbox{}

\noindent \underline{\textit{Estimate of $I_{LO}$}.} Again, by Lemma \ref{lem: solve ODE}, $Q$ is radially decreasing and $\Big\| |y|^{-\frac{1}{2}} \partial_r Q  \Big\|_{L^2} <\infty$, so there exists $R_1 = R_1(Q) \gg 1$ such that
\be
\frac{3}{2} Q(R_1) \le \frac{1}{1000} \quad \text{ and } \quad 
\Big\| |y|^{-\frac{1}{2}} \partial_r Q  \Big\|_{L^2(|x| \ge R_1)} \le \frac{1}{5000}.
\label{R1: choice linear sta}
\ee
Noting that $\beta< \frac{1}{2}$, we may now estimate the lower-order term $I_{LO}$ as follows:
    \begin{align}
        I_{LO} 
        & \le  \left( -B + \frac{3}{4} B \right) \int g^2 dy + \left(\frac{3}{2}-2\mu \right) B  \left( \int_{|y| \le R_1} g^2 Q dy   + \int_{|y| \ge R_1} g^2 Q dy \right) \notag \\
        & \le -\frac{B}{4} \int g^2 dy + \left( \frac{3}{2} -2\mu \right)B Q(0) R_1^A \int_{|y| \le R_1} g^2 |y|^{-A} dy
        + \left( \frac{3}{2} -2 \mu \right) B  Q(R_1) \|g \|_{L^2}^2 
        \notag \\
        & = -\frac{3B}{16}  \| g \|_{L^2}^2 +  \left( \frac{3}{2} -2 \mu \right)  B Q(0) R_1^A \| g\|_{L_{|y|^{-A}}^2}^2.
        \label{I LO}
    \end{align}
   Given the limited qualitative information about $Q$, the term involving $Q$ cannot be directly controlled, especially the integral of $\int_{|y| \le R_1}\int g^2 Qdy$, where $Q(y) = O(1)$ on $B(0,R_1)$. To address this, we will absorb this term using the previous coercivity \eqref{coer: singularity weight estimate 1} by choosing $0< B\ll 1$ sufficiently small.

\mbox{}

\noindent \underline{\textit{Estimate of $I_{NLO}$}.} By Cauchy's inequality, the nonlocal term involving in $I_{NLO}$ can be  controlled pointwise by
\begin{align}
    & \quad \frac{1}{r^2} \int_0^r |g(s)| s^2 ds
     = \frac{1}{ 4\pi r^2} \int_{B(0,r)} |g(y)| dy = \frac{1}{4 \pi r^2}\int_{B(0,r)} |g(y)| |y|^{-\frac{A}{2}} |y|^{\frac{A}{2}} dy \notag\\
    & \le \frac{1}{4 \pi r^2} \left( \int_{B(0,r)} g^2(y) |y|^{-A} dy \right)^\frac{1}{2} \left( \int_{B(0,r)}  |y|^{A} dy \right)^\frac{1}{2}  = \sqrt{\frac{1}{4 \pi(A+3)}} r^{\frac{A}{2} - \frac{1}{2}} \| g \|_{L_{|y|^{-A}}^2},
    \label{linear estimate: nonlocal 1}
\end{align}
and this induces that
\begin{align}
    & \quad \Bigg| \int \left( \na Q \cdot \na \Dein g \right) g |y|^{-A} dy \Bigg|
     = \int |\partial_r Q| \left(  \frac{1}{|y|^2}  \int_0^{|y|} |g(s)| s^2 ds \right) |g||y|^{-A} dy \notag\\
    & \le \sqrt{\frac{1}{4 \pi(A+3)}} \| g \|_{L_{|y|^{-A}}^2}  \int |\partial_rQ|  |g| |y|^{-\frac{A}{2} - \frac{1}{2}} dy 
     \le  \sqrt{\frac{1}{4 \pi(A+3)}} \Big\| |y|^{-\frac{1}{2}} \partial_r Q \Big\|_{L^2} \| g \|_{L_{|y|^{-A}}^2}^2,
     \label{I NLO 1}
    \end{align}
which, by choosing $A \gg 1$ sufficiently large, can be absorbed in \eqref{coer: singularity weight estimate 1}. Similarly, repeating the previous argument, together with the choice of $R_1 \gg 1$ (see \eqref{R1: choice linear sta}), the $L^2$ component of $I_{NLO}$ can be controlled by:
    \begin{align}
         & \quad B\int \left( \na Q \cdot \na \Dein g \right) g dy  
        \le B \| g \|_{L^2} \left(  \int_{|y| \le R_1} |\partial_r Q| |y|^{-\frac{1}{2}} |g| dy + \int_{|y| \ge R_1} |\partial_r Q| |y|^{-\frac{1}{2}} |g| dy  \right) \notag \\
        & \le \frac{B}{100} \| g \|_{L^2}^2 + 50 B R_1^A \big\| \partial_r Q |y|^{-\frac{1}{2}} \big\|_{L^2}^2 \| g \|_{L_{|y|^{-A}}^2}^2 + 50 B \big\| \partial_r Q |y|^{-\frac{1}{2}} \big\|_{L^2(|y| \ge R_1)}^2 \| g \|_{L^2}^2 \notag \\
        & \le \frac{B}{50} \| g \|_{L^2}^2 
        + 50 B R_1^A \big\| \partial_r Q |y|^{-\frac{1}{2}} \big\|_{L^2}^2 \| g \|_{L_{|y|^{-A}}^2}^2.
        \label{I NLO 2}
    \end{align}
    The idea of handling this term is similar to $I_{LO}$, and we can use the smallness of $0< B \ll 1$ to absorb $B \int_{|y| \le R_1} \left( \na Q \cdot \na \Dein g \right) g dy$ by the coercivity \eqref{coer: singularity weight estimate 1}.
    Hence combining \eqref{I NLO 1} and \eqref{I NLO 2} yields
    \begin{align}
        I_{NLO}
        & \le  \left( \sqrt{\frac{1}{4 \pi(A+3)}} \big\| |y|^{-\frac{1}{2}} \partial_r Q \big\|_{L^2}  + 50 B R_1^A \big\| |y|^{-\frac{1}{2}} \partial_r Q  \big\|_{L^2}^2  \right)\| g \|_{L_{|y|^{-A}}^2}^2 
        + \frac{B}{50} \| g \|_{L^2}^2.
        \label{I NLO}
    \end{align}

    \mbox{}

    \noindent \underline{\textit{Conclusion of coercivity}.} Combining the estimates \eqref{coer: singularity weight estimate 1}, \eqref{I LO} and \eqref{I NLO}, we obtain that
    \begin{align*}
        \left( \calL g, g \right)_{L_w^2}
        & \le 
        -\frac{1}{8} B \| g \|_{L^2}^2
        +  \left( 1 + \frac{-A+3}{4j_0}  + \sqrt{\frac{1}{4 \pi(A+3)}} \Big\| |y|^{-\frac{1}{2}} \partial_r Q \Big\|_{L^2} \right) \int g^2 |y|^{-A} dy \\
        & \quad + \left( \left( \frac{3}{2} -2 \mu \right) B R_1^A Q(0)  + 50 B R_1^A \big\| |y|^{-\frac{1}{2}} \partial_r Q  \big\|_{L^2}^2  \right)\| g \|_{L_{|y|^{-A}}^2}^2,
    \end{align*}
    with $R_1 = R_1(Q) >0$ chosen as in \eqref{R1: choice linear sta}. Next, we choose 
    $A \gg 4j_0 +4$ with $\frac{A}{4} \in \ZZ_{>0}$ such that
    \begin{align}
        1 + \frac{-A+3}{4j_0} \le -1, \quad \text{ and } \quad 
        \sqrt{\frac{1}{4 \pi(A+3)}} \Big\| |y|^{-\frac{1}{2}} \partial_r Q \Big\|_{L^2}
        \le  \frac{1}{100},
        \label{A: choice range}
    \end{align}
    then we choose $0< B=B(A,R_1,\mu) \ll 1$ sufficiently small such that
    \[
    \left( \frac{3}{2} -2 \mu \right) B R_1^A Q(0) +  50 B R_1^A \big\| |y|^{-\frac{1}{2}} \partial_r Q  \big\|_{L^2}^2  \le \frac{1}{100},
    \]
   so that we obtain that
    \begin{align*}
         \left( \calL g, g \right)_{L_w^2}
         \le -\frac{1}{8} \| g \|_{L_{|y|^{-A}}^2}^2
         - \frac{1}{8} B \| g\|_{L^2}^2 = -\frac{1}{8} \| g \|_{L_w^2}^2,
    \end{align*}
    which completes the proof of \eqref{L: coer}.
\end{proof}

In addition, to study the nonlinear stability of $Q$ in Section \ref{sec: nonlinear sta}, it is necessary to establish the coercivity properties of the linearized operator $\calL$ in a higher order Sobolev space $\dot H^{2K+4}$ with $K = \frac{A}{4}$. The precise statement is as follows:

\begin{proposition}[Coercivity of $\calL$ in $\dot H^{2K+4}$]
\label{prop: core H^K}
    Let $A >0 $ be as given in Proposition \ref{prop: coer}, and define $K := \frac{A}{4} \in \ZZ_{\ge 1}$. Then there exists constant $C=C(Q,A,B,j_0,\mu)>0$ such that
    \be
    (\calL g ,g)_{\dot H^{2K+4}} 
    \le - \frac{1}{8} \| g \|_{\dot H^{2K+4}}^2 + C \| g \|_{L^2}^2, \quad \forall \; g \in H_{rad}^{2K+4}.
    \label{coercivity in H^K}
    \ee
\end{proposition}

\begin{proof}
    By the definition of $\calL$ given in \eqref{linearized op},
    \be
    \left( \calL g,g \right)_{\dot H^{2K+4}} 
    = I + II + III + IV,
    \label{HK estimate: expression}
    \ee
    with
    \begin{align*}
        &  I: = -\left( \Delta^{K+2} \left( (g + \beta y \cdot \na  g)  \right),  \Delta^{K+2} g\right)_{L^2}, 
        \quad II:= \left( \Delta^{K+2} \left( \na g \cdot \na \Dein Q \right),  \Delta^{K+2} g\right)_{L^2}, \\
        & III:=\left( \Delta^{K+2} \left( \na Q \cdot \na \Dein g  \right),  \Delta^{K+2} g\right)_{L^2}, 
        \quad IV := \left( \Delta^{K+2} \left(  2(1-\mu) Q g \right),  \Delta^{K+2} g\right)_{L^2}.
    \end{align*}
    First, observe that by scaling invariance, the term $I$ can be computed as
    \begin{equation}\label{5.2.1}
    \begin{aligned}
    I &= 
    -\frac{1}{2}\frac{d}{d\lambda}\Bigg|_{\lambda =1} \Big\| \Delta^{K+2} \left( \lambda g(\lambda^\beta y) \right)\Big\|_{L^2}^2
    = -\left( \frac{\beta}{2} \left( 4K+5 \right)  +1 \right) \| \Delta^{K+2} g \|_{L^2}^2.
    \end{aligned}
    \end{equation}

    For the term $II$, recalling \eqref{nonlocal term: formula}, we rewrite $\na \Dein Q = rf_Q \mathbf{e}_r$ with $\mathbf{e}_r = \frac{y}{|y|}$. Then by Lemma \ref{lem: solve ODE}, \cite[Lemma A.$4$]{Javierblowup3DNS}, integration by parts, Gagliardo-Nirenberg inequality, and Young's inequality, there exists a uniform constant $C= C(K,Q)>0$ such that
    \begin{align}
        II
         \leq  &\left( \left( \na  \Delta^{K+2}g \cdot \na \Dein Q \right), \Delta^{K+2}g \right)_{L^2}
        + 2(K+2) \left( (\partial_r (rf_Q))  \Delta^{K+2}g , \Delta^{K+2}g \right)_{L^2} \notag \\
        &+C \big\| r f_Q \big\|_{W^{2K+4,\infty}} \| g \|_{H^{2K+3}} \| g \|_{\dot H^{2K+4}}   \notag \\
         \leq& 
          2(K+2) \left( (\partial_r(rf_Q) )  \Delta^{K+2}g , \Delta^{K+2}g \right)_{L^2} 
      + \frac{1}{100} \norm{g}_{\dot H^{K+2}}^2 + C \norm{g}_{L^2}^2.
      \label{Hk estimate: 1}
    \end{align}
   Since $Q(r)$ is radially decreasing by Lemma \ref{lem: solve ODE},
    \begin{align*}\label{3fQ>Q}
    f_Q(r) = \frac{1}{r^3} \int_0^r Q(s) s^2 ds \ge \frac{1}{r^3} Q(r) \int_0^r s^2 ds = \frac{1}{3} Q(r),
    \end{align*}
  which yields that
    \[
    \partial_r (r f_Q(r)) = Q(r) -2f_Q(r) \le 3f_Q(r) -2 f_Q(r) = f_Q(r), \quad \forall \; r >0.
    \]
    Hence, by the decreasing fact of $f_Q$ given by Lemma \ref{lem: solve ODE}, \eqref{Hk estimate: 1} can be improved to
    \begin{align}
        II & \le 
       \left(  2(K+2) f_Q(0) + \frac{1}{100} \right) \| g \|_{\dot H^{2K+4}}^2 + C \| g \|_{L^2}^2.
        \label{5.2.2}
    \end{align}

 For the term $III$, following the argument in \eqref{linear estimate: nonlocal 1}, we first compute
 \begin{align*}
 & \quad  \int \left( \na \Delta^{K+2} Q \cdot \na \Dein g \right) \Delta^{K+2} g dy
   = \int \big| \partial_r \Delta^{K+2}Q \big| \left( \frac{1}{r^2} \int_0^r |g(s)| s^2 ds \right) \big| \Delta^{K+2} g \big| dy \\
  & \le \left( \int |\partial_r \Delta^{K+2} Q| |y|^{-\frac{1}{2}} |\Delta^{K+2} g| dy \right) \| g \|_{L^2} \le \Big\| |y|^{-\frac{1}{2}} \partial_r \Delta^{K+2} Q \Big\|_{L^2} \| g \|_{L^2} \| g \|_{\dot H^{2K+4}},
 \end{align*}
 which, by Lemma \ref{lem: solve ODE}, Gagliardo-Nirenberg inequality, and Young's inequality, yields that there exists $C=C(K,Q)>0$ such that
\begin{align}
    III
    & \le \int \left( \na \Delta^{K+2} Q \cdot \na \Dein g \right) \Delta^{K+2} g dy
    + C \left( \sum_{j=1}^{2K+4} \| \na^{2K+5-j} Q \|_{L^{\infty}} \| \na^{j+1} \Dein g \|_{L^2} \right) \| g \|_{\dot H^{2K+4}} \notag\\
    & \le C \| g \|_{H^{2K+3}} \| g \|_{\dot H^{2K+4}} 
    \le \frac{1}{100} \| g \|_{\dot H^{2K+4}}^2 + C \| g \|_{L^2}^2.
      \label{5.2.3}
\end{align}

Finally, for $IV$, by Lemma \ref{ODE system}, Gagliardo-Nirenberg inequality and Young's inequality again,
\begin{align}
    IV
    & \le  2(1-\mu) \int Q |\Delta^{K+2} g|^2 dy + C\sum_{j=0}^{2K+3} \| \na^{2K+4-j} Q \|_{L^\infty} \| \na^j g \|_{L^2} \| \Delta^{K+2} g \|_{L^2} \notag \\
    & \le  \left( 2(1-\mu) Q(0) + \frac{1}{100} \right) \| g \|_{\dot H^{2K+4}}^2 + C  \|g \|_{H^{2K+3}}^2. 
     \label{5.2.4}
\end{align}

    Consequently, combining \eqref{5.2.1}, \eqref{5.2.2}, \eqref{5.2.3}, \eqref{5.2.4}, along with the choice of $\beta < \frac{1}{2}$ from \eqref{beta: def}, Lemma \ref{lem: solve ODE}, the selection of $A$ from \eqref{A: choice range} and $K := \frac{A}{4}$, one finds that
    \begin{align*}
        & \quad \left( \calL g,g \right)_{\dot H^{2K+4}}
         \le  \Big( -\frac{\beta}{2} \left( 4K+5 \right)  +\frac{2K+4}{3(1-\mu)}+1+\frac{3}{100}\Big) \| g \|_{\dot H^{2K+4}}^2 + C\norm{g}_{L^2}^2 \\
        & =\Big(-\frac{A+8}{4j_0} + \frac{3\beta}{2}    +1+ \frac{3}{100} \Big)\| g \|_{\dot H^{2K+4}}^2 + C\norm{g}_{L^2}^2
         \le - \frac{1}{8} \| g \|_{\dot H^{2K+4}}^2 + C \| g \|_{L^2}^2,
    \end{align*}
    and thus, we have completed the proof of \eqref{coercivity in H^K}.
\end{proof}

\section{Nonlinear stability}
\label{sec: nonlinear sta}
In this section, building upon the coercivity properties of the operator $\calL$ established in Section \ref{sec: linear theory}, we proceed to analyze the nonlinear stability of $Q$. Then, based on this nonlinear stability, we will conclude this section by constructing a finite-time blowup solution to  \eqref{equation: KS with damping} for any $\mu \in \left[ 0,\frac{1}{3} \right)$ with finite mass and nonnegative density.

\subsection{Ansatz and modulation}\label{subsec:mod} 
Recalling the ansatz $\Psi = Q+ \ep$, where $\ep$ is \textit{radially symmetric} and solves the equation \eqref{linearized eq},  we further decompose $\ep$ as motivated by Proposition \ref{prop: coer}:
\be
\ep(\tau,y) = \epu(\tau,y) + \eps(\tau,y),
\text{ with } \epu(\tau,y) = \sum_{j=0}^K c_j(\tau) \chi(y) |y|^{2j},
\label{decomposition of Psi}
\ee
where $\chi$ is a radial smooth cut-off function on $B(0,1)$ defined in \eqref{def: cut-off function}, and $K = \frac{A}{4} \in \ZZ$ is as in Proposition \ref{prop: core H^K}. The coefficients $\{c_j \}_{j=0}^K$ are chosen such that the component $\eps$ satisfies the vanishing condition at the origin
\be
\partial_r^{2j} \ep_s (\tau,0) =0, \quad \; \forall \; 0 \le j \le K.
\label{stable part: modulation condition}
\ee
In particular, we split $\epu$ as
\be
\ep_u(\tau) = \ep_{u,real} + \ep_{u,fake} \;,
\label{Psi: decomposition}
\ee
where
\begin{equation}\label{epu: real & fake}
    \begin{cases}
        \ep_{u,real}(\tau,y) := \sum_{j=0}^{j_0} c_j(\tau) \chi(y) |y|^{2j},\\
    \ep_{u,fake}(\tau, y) := \sum_{j=j_0+1}^K c_{j} \chi(y) |y|^{2j}.
    \end{cases}
\end{equation}

\begin{remark}
   Recalling that the singular weight introduced in Proposition \ref{prop: coer} might not be sharp, the decomposition \eqref{decomposition of Psi} allows for stable components to be included in $\epu$. One can distinguish the unstable and stable parts as in \eqref{epu: real & fake}. For further intuition regarding decomposition \eqref{epu: real & fake}, we refer the readers to the modulation ODE system \eqref{ODE system for unstable part}.
\end{remark}

\subsubsection{Coefficients of the Taylor expansion of $\calL \epu$} With the vanishing condition \eqref{stable part: modulation condition}, one can derive the modulation equations for $\{c_j \}_{j=0}^K$. 
A crucial step in this process is to compute the Taylor expansion at the origin of each term appearing in \eqref{linearized eq}. As a preliminary, we focus in this section on determining the Taylor coefficients of $\calL \epu$ at the origin.

Specifically, recalling the definition of  $\calL$ from \eqref{linearized op}, and Taylor expansions of $(Q,f_Q)$ at the origin given in \eqref{(Q,f), expansion}, we obtain for any $r \in (0,\epsilon]$,
\begin{align*}
    & \quad \calL \epu 
     = - (\epu + \beta r \partial_r \epu) + f_Q \left(r \partial_r \epu \right) + r\partial_r Q \left( \frac{1}{r^3} \int_0^r \epu (s) s^2 ds \right) + 2(1-\mu) Q \epu \\
    & = -\sum_{j=0}^K c_j r^{2j}  - \beta  \sum_{j=0}^K 2j c_j r^{2j} + \left(\sum_{j=0}^\infty [f_Q]_{j} r^{2j} \right) \left( \sum_{j=0}^K 2j c_j r^{2j} \right) \\
  & \quad + \left(\sum_{j=0}^\infty 2j [Q]_{j} r^{2j} \right) \left( \sum_{j=0}^K  \frac{c_j}{2j+3} r^{2j} \right)  + 2(1-\mu) \left( \sum_{j=0}^\infty [Q]_{j}  r^{2j}\right) \left( \sum_{j=0}^K c_j r^{2j} \right).
\end{align*}
Applying \eqref{recurrence relation 1}, \eqref{recurrence Qj} and $[Q]_{j_0}=-1$, this yields that
\[
[\calL \epu]_j = -c_j - 2 \beta j c_j + 2j[f_Q]_0 c_j + 2(1-\mu) [Q]_0c_j 
= \frac{j_0 -j}{j_0} c_j, \qquad \forall \; 0 \le j < j_0,
\]
and
\begin{align*}
[\calL \ep]_{j_0} 
& = -c_{j_0} - 2 \beta j_0 c_{j_0} + 2j_0 [f_Q]_0 c_{j_0} + 2j_0 [Q]_{j_0} \frac{c_0}{3} + 2(1-\mu) [Q]_0 c_{j_0} + 2(1-\mu) [Q]_{j_0} c_0 \\
& 
=\sigma_{0,j_0} c_0, \quad \text{ where } \quad \sigma_{0,j_0} =  - \left( \frac{2}{3} j_0 + 2(1-\mu) \right).
\end{align*}
Similarly, for $j_0 +1 \le j \le K$, there exists $\{ \sigma_{i,j} \} =\{ \sigma_{i,j} (\mu,j_0) \} \subset \RR$ such that
\begin{align*}
    [\calL \ep]_{j}
    = \frac{j_0-j}{j_0} c_j + \sum_{i=0}^{j-1} \sigma_{i,j} c_i, \qquad \forall \; j_0+1 \le  j \le K.
\end{align*}
In summary, $[\calL \epu]_j$, the $2j$-th order coefficient of the Taylor expansion of $\calL \epu$ at the origin, satisfies
\be
[\calL \epu]_j
=
\begin{cases}
    \frac{j_0-j}{j_0} c_j, & 0 \le j < j_0, \\
    \frac{j_0-j}{j_0} c_j+ \sigma_{0,j_0} c_0, & j=j_0, \\
     \frac{j_0-j}{j_0} c_j + \sum_{i=0}^{j-1} \sigma_{i,j} c_i, & j_0+1 \le j \le K.
\end{cases}
\label{L epu: Taylor coefficients}
\ee


\subsubsection{Modulation equations.} Next, we derive the modulation equations for $\{c_j\}_{j=0}^K$ under the restriction given in \eqref{stable part: modulation condition}, building on the previous preliminary results. Concretely, with the decomposition of $\ep$ in \eqref{decomposition of Psi} and the equation \eqref{linearized eq},
\begin{align}
    \partial_\tau \eps
     & =  \calL \eps + N(\eps)  
     + \na \epu \cdot \na \Dein \eps + \na \eps \cdot \na \Dein \epu + 2(1-\mu) \epu \eps + G[\lambda, \Psi, \epu],
     \label{eq: eps}
\end{align}
where the \textit{modulation term} $G[\lambda,\Psi,\epu]$ is defined as
\be
G[\lambda, \Psi, \epu] := \lambda^{2-4\beta} \Delta \Psi - \sum_{j=0}^K \dot c_j \chi(r) r^{2j} + \calL \epu + N(\epu).
\label{G: def}
\ee
Since $\ep_s = O(r^{2K+2})$ at the origin as indicated in \eqref{stable part: modulation condition}, and by the definition of $\calL$ given in \eqref{linearized op}, $\calL \eps = O(r^{2K+2})$ at the origin, the following holds
\[
\partial_\tau \eps - \left( \calL \eps + N(\eps) + \na \epu \cdot \na \Dein \eps + \na \eps \cdot \na \Dein \epu + 2(1-\mu) \epu \eps \right) = O(r^{2K+2}),
\]
which requires the modulation term $G[\lambda,\Psi, \epu] = O(r^{2K+2})$ at the origin. Noting that $G[\lambda, \Psi, \epu]$ can be expanded as follows:
\begin{align}
    & \quad G[\lambda, \Psi ,\epu]
      = \lambda^{2-4 \beta} \Delta \Psi - \sum_{j=0}^K \dot c_j \chi r^{2j} + \calL \epu + N(\epu) \notag\\
    & = \lambda^{2-4\beta} \sum_{j=0}^K [\Delta \Psi ]_j \chi r^{2j} 
    - \sum_{j=0}^K \dot c_j \chi r^{2j} 
    + \sum_{j=0}^K [\calL \epu]_j \chi r^{2j} + \sum_{j=0}^K [N(\epu)]_j \chi  r^{2j}
    \label{G: lower term}
    \\
    & \quad + \lambda^{2-4\beta} \left( \left(\Delta Q + \epu \right) -\sum_{j=0}^K [\Delta Q + \Delta \epu ]_j \chi r^{2j} \right)
    + \lambda^{2-4\beta} \left( \Delta \eps  - [\Delta \eps]_K \chi r^{2K} \right) \notag \\
    & \quad 
    + \left( \calL \epu - \sum_{j=0}^K [\calL \epu]_j \chi r^{2j} \right) +N(\epu) -  \sum_{j=0}^K [N(\epu)]_j \chi  r^{2j} \notag,
\end{align}
where \eqref{G: lower term} has fewer orders of vanishing at the origin. Hence \eqref{G: lower term} should be imposed to vanish at the origin, then together with \eqref{L epu: Taylor coefficients}, this yields the following modulation equations onto the coefficients $\{c_j\}_{j=0}^K$:
\be
\begin{cases}
    \dot c_j =\frac{j_0 -j}{j_0} c_j + \lambda^{2-4 \beta} [\Delta \Psi]_j +  [N(\epu)]_{j}, & 0 \le j < j_0, \\
    \dot c_{j_0} =  \sigma_{0,j_0}c_0 +\lambda^{2-4 \beta} [\Delta \Psi]_{j_0}  +
    [N(\epu)]_j
    , & j =j_0, \\
    \dot c_{j} =  \frac{j_0 -j}{j_0} c_j + \sum_{i=0}^{j-1} \sigma_{i,j} c_i + \lambda^{2-4 \beta} [\Delta \Psi]_{j}  + [N(\epu)]_j, & j_0 < j \le K.
\end{cases}
\label{ODE system for unstable part}
\ee
In conclusion, we obtain an ODE-PDE system in terms of $\left(\{ c_j \}_{j=0}^K, \eps\right)$, which couples equations \eqref{eq: eps} and \eqref{ODE system for unstable part}. 
Moreover, the modulation term $G[\lambda, \Psi ,\epu]$ in \eqref{eq: eps} can be further expressed as follows:
\begin{align}
     G[\lambda, \Psi ,\epu]
    & =  \lambda^{2-4\beta} \left( \left(\Delta Q + \epu \right) -\sum_{j=0}^K [\Delta Q + \Delta \epu ]_j \chi r^{2j} \right) \notag
    + \lambda^{2-4\beta} \left( \Delta \eps  - [\Delta \eps]_K \chi r^{2K} \right) \\
    & \quad 
    + \left( \calL \epu - \sum_{j=0}^K [\calL \epu]_j \chi r^{2j} \right) +N(\epu) - \sum_{j=0}^K [N(\epu)]_j \chi r^{2j}.
    \label{G: new expression}
\end{align}


\subsection{Bootstrap argument.}
 We take $\delta_g \ll 1$ satisfying
    \be
    \delta_g \ll \min \Big\{ \frac{1}{8}, 2-4\beta, \frac{1}{j_0},  \frac{1}{|\sigma_{0,j_0}|}, A^{-1} , B  \Big\},
    \label{delta g: restriction}
    \ee
and introduce the function
\be
d_{real}(\tau)
:= \sqrt{ \frac{1}{2}\sum_{j=1}^{j_0-1} c_j^2 + \frac{10}{\delta_g^2} c_0^2 + \frac{1}{4 |\sigma_{0,j_0}|} c_{j_0}^2 },
\label{bootrap real unstable: norm}
\ee
which describes the behavior of $\ep_{u,real}$. The main result is as follows:
\begin{proposition}[Bootstrap]
\label{prop: bootstrap}
   There exists $0 < \delta_g \ll 1$ satisfying \eqref{delta g: restriction} such that there exists $(\delta_0,\delta_1, \delta_2, \delta_3,  \delta_{j_0+1}, \delta_{j_0+2} ..., \delta_K)$ with
    \be
    \delta_0  \ll \delta_3 \ll \delta_{j_0+1} \ll \delta_{j_0+2} \ll \delta_{j_0+3} \ll ... \ll \delta_{K} \ll \delta_1 \ll \delta_2 \ll \delta_3^\frac{1}{2} \ll \delta_g \ll Q(2),
    \label{delta i: restriction}
    \ee
    such that for any $\lambda(0) = \lambda_0$, $\ep_{s}(0) \in L_{w}^2 \cap \dot H_{rad}^{2K+6} (\RR^3)$ and $\{ c_j(0) \}_{j=j_0+1}^K$  \footnote{With this regularity assumption on initial data, together with \eqref{ss coordinte} and \eqref{ss renormalization}, by the standard fixed point arguments as in \cite{zbMATH01532872} or \cite[Appendix A]{ksnsblowup}, the local wellposedness can be ensured and the related solution to \eqref{equation: KS with damping} satisfying $\rho \in C_t^0 \left( [0,T_{max}), H_x^{2K+6}(\RR^3)  \right) \cap C_t^1\left([0,T_{max}), H_x^{2K+4}(\RR^3) \right)$.} satisfying
    \be
    |\lambda_0| + |\lambda_0|^{2-4\beta} + 
    \| \ep_{s}(0) \|_{ L_{w}^2 (\RR^3)} +  
    \| \ep_{s}(0) \|_{\dot H^{2K+4}(\RR^3)} + \sum_{j=j_0+1}^K |c_j(0)| \le \delta_0,
    \label{bootstrap: initial condition}
    \ee
    there exists $\{c_j(0) \}_{j=0}^{j_0}$ such that the radial solution to \eqref{renormalization KS} with initial datum
    \[
    (\Psi_0, \lambda_0) = \left (Q+ \sum_{j=0}^{j_0} c_j(0) \chi |y|^{2j} + \sum_{j=j_0+1}^K c_j(0) \chi |y|^{2j} + \ep_{s0}, \lambda_0 \right),
    \]
    globally exists and can be split into \eqref{decomposition of Psi} satisfying the following for all $\tau \ge 0$:


    \noindent $\bullet$ (Control the $L^2$ base norm of stable part $\eps$)
    \be 
    \| \ep_{s}(\tau) \|_{L_{w}^2} \le \delta_1 e^{- \frac{1}{2} \delta_g \tau}.
    \label{bootstrap assum: L2 stable}
    \ee

    \noindent $\bullet$ (Control the higher regularity of stable part $\eps$ via $\dot H^{2K+4}$ norm)
    \be
    \| \eps(\tau) \|_{\dot H^{2K+4}} \le \delta_2 e^{-\frac{1}{2} \delta_g \tau}.
    \label{bootstrap assum: Hm stable}
    \ee

    \noindent $\bullet$ (Control the real unstable part $\ep_{u,real}$)
    \be
    d_{real}(\tau) \le \delta_3 e^{-\frac{7}{10} \delta_g \tau}.
    \label{bootstrap assum: real unstable}
    \ee
    
    \noindent $\bullet$ (Control the fake unstable part $\ep_{u,fake}$)
    \be
    |c_j(\tau)| \le \delta_j e^{-\frac{7}{10} \delta_g \tau}, \quad \forall \; j_0+1 \le j \le K.
    \label{bootstrap assum: fake unstable}
    \ee
\end{proposition}

\vspace{0.5mm}


\begin{remark}
In what follows, the estimates \eqref{delta: choice 1}, \eqref{delta: choice 2}, \eqref{delta: choice 3}, and \eqref{outergoing-flux property} yield the requirements on $\{\delta_i\}$ summarized in \eqref{delta i: restriction}. 
Notably, the constants $C>0$ appearing below, which  might vary from line to line if necessary,  are all independent of $\{\delta_i\}$. Therefore,  we can choose appropriate $\{\delta_i\}$  in a manner to close Proposition \ref{prop: bootstrap}.
\end{remark}


\begin{remark}
Proposition \ref{prop: bootstrap} is the center of the  chapter. As in \cite{CollotsuperHeateq,MerleblowupNLSdefocusing}, Proposition \ref{prop: bootstrap} will be proven via contradiction using the topological argument as follows: given $\left(\lambda_0, \ep_{u,fake}(0), \eps(0) \right)$ satisfying \eqref{bootstrap: initial condition}, we assume that for any $\ep_{u,real}(\tau,y) = \sum_{j=0}^{j_0} c_j(\tau) \chi(y) |y|^{2j}$ satisfying \eqref{bootstrap assum: real unstable} when $\tau=0$, the exit time
\be
\tau^* = \sup \; \Big\{ \tau \ge 0: \big(d_{real}, \{ c_j \}_{j={j_0+1}}^N, \eps \big) \text{ satisfy  \eqref{bootstrap assum: L2 stable}-\eqref{bootstrap assum: fake unstable} simultaneously on } [0,\tau] \Big\}
\label{exit time}
\ee
is finite. We then look for a contradiction under the assumptions of Proposition \ref{prop: bootstrap}. Subsequently, we study the flow satisfying \eqref{bootstrap assum: L2 stable}-\eqref{bootstrap assum: fake unstable} on $[0,\tau^*]$. Specifically, we will show that the bounds in \eqref{bootstrap assum: L2 stable}, \eqref{bootstrap assum: Hm stable}, and \eqref{bootstrap assum: fake unstable} can be further improved within the bootstrap regime. This implies that the only possible scenario for the solution to exit the bootstrap regime is for the real unstable condition \eqref{bootstrap assum: real unstable} to fail as $\tau> \tau^*$. Moreover, using the outer-going flux property of $d_{real}$ at the exit time $\tau = \tau^*$, we conclude a contradiction via Brouwer's fixed point theorem.
\end{remark}


\subsection{A priori estimates}

\subsubsection{Preliminaries}

In the section, as preliminaries, we are devoted to the estimate of $[\Delta \Psi]_j$ with $0 \le j \le K$, which is the coefficient of Taylor expansion of $\Delta \Psi$ with the $2j$-th order at the origin. And the main result is as follows:
\begin{lemma}
\label{lemma: preliminaries, Psi}
    Under the bootstrap assumption of Proposition \ref{prop: bootstrap}, as for the function $\Psi$ defined in \eqref{ss renormalization}, there exists a uniform constant $C=C(K)>0$ such that the quantity $[\Delta\Psi]_j:= \frac{1}{(2j)!} \partial_r^{2j} \Delta \Psi (0)$ satisfies
    \be
    \big| [\Delta\Psi]_j \big| \le
    \begin{cases}
        C(K), & 0 \le j < K, \\
        C(K) + C(K) \| \eps \|_{H^{2K+4}}, & j=K.
    \end{cases}
    \label{Delta Psi: estimate on Taylor coeff}
    \ee
\end{lemma}

\begin{proof}
Recall the decomposition of $\Psi$ defined in \eqref{decomposition of Psi},
\[
[\Delta \Psi]_j = \frac{1}{(2j)!} \partial_r^{2j} [\Delta \Psi] (0)
= \frac{1}{(2j)!} \partial_r^{2j} \Delta Q (0) + \frac{1}{(2j)!} \partial_r^{2j} \Delta \epu(0) + \frac{1}{(2j)!} \partial_r^{2j}\Delta \eps (0),
\]
where, by bootstrap assumptions \eqref{bootstrap assum: real unstable} and \eqref{bootstrap assum: fake unstable}, there exists a constant $C=C(K)>0$ such that
\[
\Bigg|\frac{1}{(2j)!} \partial_r^{2j} [\Delta Q] (0) \Bigg|+ \Bigg| \frac{1}{(2j)!} \partial_r^{2j} (\Delta \epu) (0) \Bigg| \le C(K), \quad \forall \; 0 \le j \le 2K.
\]
 
For $\partial_r^{2j} \Delta \eps(\tau,0)$, note that $\eps = O(r^{2K+2})$ at the origin,
\[
\partial_r^{2j} \Delta \eps(0) = 0, \quad \forall \; 0 \le j \le K-1.
\]
In addition, for $\partial_r^{2K} \Delta \eps(\tau,0)$, by Sobolev inequality, there exists $C=C(K)>0$ such that
\begin{align}
    |\partial_r^{2K} \Delta \eps(\tau,0)| & 
      \le C  \big| [\eps(\tau)]_{K+1} \big|
    \le C |\na^{2K+2} \eps (\tau,0)| \notag
    \\
    &  \le C\| \na^{2K+2} \eps(\tau) \|_{L^\infty} \le C \| \eps(\tau) \|_{H^{2K+4}}.
    \label{Taylor expansion: Delta eps}
\end{align}
Consequently, combining all of the arguments above immediately yields \eqref{Delta Psi: estimate on Taylor coeff}.
\end{proof}


\begin{lemma}[Estimates of terms related to $\epu$]
\label{lemma: preliminaries epu}
    Under the bootstrap assumptions of Proposition \ref{prop: bootstrap}, for the function $\epu$ defined in \eqref{decomposition of Psi}, $N(\epu)$ is compactly supported on $B(0,2)$ and satisfies
    \be
   \sum_{j=0}^K \Big| [N(\epu)(\tau)]_j \Big| + \Big\| N(\epu)(\tau) \Big\|_{H^{2K+4}} \le C \sum_{j=0}^K |c_j(\tau)|^2, \quad \forall \; \tau \in [0,\tau^*],
    \label{nonlinear term: epu}
    \ee
     for some uniform constant $C=C(K)>0$. In addition, $\calL \epu \in H^{2K+4}$ and satisfies
    \be
    \sum_{j=0}^K \Big| [\calL \epu(\tau)]_j \Big| + \big\| \calL \epu(\tau) \big\|_{H^{2K+4}} \le C \sum_{j=0}^K |c_j(\tau)|, \quad \forall \; \tau \in [0,\tau^*],
    \label{linear term: epu}
    \ee 
    for some uniform constant $C=C(K,Q)>0$.
\end{lemma}

\begin{proof}
Recalling the definition of $\epu$ given in \eqref{decomposition of Psi}, and $N(\epu) = \na \Dein \epu \cdot \na \epu + (1-\mu) \epu^2$, we check
\begin{align*}
   N(\epu) 
    &= (r \partial_r \epu) \frac{1}{r^3} \int_0^r \epu(s) s^2 ds 
    + (1-\mu) \epu^2  \\
    & = \sum_{j_1,j_2=0}^K \left(\frac{2j_1 c_{j_1} c_{j_2}}{2j_2+3}
    + (1-\mu) c_{j_1} c_{j_2}  \right) r^{2j_1+2j_2} \\
    & = \sum_{j=0}^{2K} \left(  \sum_{j_1+j_2 =j}\frac{2j_1 c_{j_1} c_{j_2}}{2j_2+3} + (1-\mu) c_{j_1} c_{j_2}\right) r^{2j},  \quad \forall \; r \le \frac{1}{8}.
\end{align*}
This yields 
\begin{align*}
    \Big| [N(\epu)]_i \Big|
    & =  \Bigg| \sum_{j_1+j_2 =j}\frac{2j_1 c_{j_1} c_{j_2}}{2j_2+3} + (1-\mu) c_{j_1} c_{j_2} \Bigg| 
    \le C(K) \sum_{j=0}^K |c_j|^2, \quad \forall \; 0 \le i \le K.
\end{align*}
In addition, by using Gagliardo-Nirenberg inequality and  $\text{supp } \epu \in B(0,2)$,
\begin{align*}
\| N(\epu) \|_{H^{2K+4}}
& \le C | \epu \|_{H^{2K+5}}^2
\le C \sum_{j=0}^{K} |c_j|^2,
\end{align*}
which concludes \eqref{nonlinear term: epu}.
To verify \eqref{linear term: epu}, it is a direct result of \eqref{L epu: Taylor coefficients} that there exists a constant $C=C(K,Q)>0$ such that
\[
\Big| [\calL \epu]_i \Big| \le C(K,Q) \sum_{j=0}^K |c_j|, \quad \forall \; 0 \le i \le K.
\]
Additionally, recall \eqref{nonlocal term: formula}, Lemma \ref{lem: solve ODE} and $\text{supp } \epu \subset B(0,2)$, similar to the argument in \eqref{5.2.3} and \eqref{5.2.4}, by using Gagliardo-Nirenberg inequality, there exists 
a constant $C=C(K,Q)>0$ such that
\begin{align*}
    \big\| \calL \epu \big\|_{H^{2K+4}}  
    & \le  \Big\| -\left( \epu + \beta y \cdot \na \epu  \right) + \na \epu \cdot \na \Dein Q + 2(1-\mu) Q \epu \Big\|_{H^{2K+4}(B(0,2))} \\
    &  \quad + \| \na \Dein \epu \cdot \na Q \|_{H^{2K+4}} \\
    & \le C \| Q \|_{H^{2K+5}}\| \epu \|_{H^{2K+5}} \le C \sum_{j=0}^K |c_j|.
\end{align*}
This completes the proof of \eqref{linear term: epu}.
\end{proof}

\

\subsubsection{$L_w^2$ estimate of $\eps$.}
This section is to improve the $L_w^2(\RR^3)$ estimate of $\eps$ under the bootstrap assumptions of Proposition \ref{prop: bootstrap}. And the main result is as follows:
\begin{lemma}[$L_w^2$ estimate of $\eps$]
\label{lemma: L2 estimate of eps}
    Under the assumptions of Proposition \ref{prop: bootstrap}, there exists a constant $C=C(Q, A,B,\delta_g)>0$ such that
    \begin{align}
        \frac{d}{d\tau} \| \eps \|_{L_w^2}^2
        \le 
     - \delta_g \| \eps \|_{L_w^2}^2  +  C \left(\lambda^{4-8\beta} +  d_{real}^2 +\sum_{j=j_0+1}^K |c_j|^2  \right) \quad \forall \; \tau \in [0,\tau^*].
    \label{L2 estimate of eps}
    \end{align}
    In particular, the bootstrap assumption \eqref{bootstrap assum: L2 stable} can be improved to
    \[
    \| \eps (\tau) \|_{L_w^2} \le \frac{1}{2} \delta_1 e^{-\frac{\delta_g}{2} \tau}, \quad \forall \; \tau \in [0,\tau^*].
    \]
\end{lemma}


The proof of Lemma \ref{lemma: L2 estimate of eps} is lengthy; thus, we separate the $L_w^2$ estimate of the modulation term $G[\lambda, \Psi, \epu]$ defined in \eqref{G: def}. The estimate is as follows:
\begin{lemma}[Estimate on modulation term \text{$G[\lambda,\Psi,\epu]$}]
\label{estimate of G}
    Under the bootstrap assumption of Proposition \ref{prop: bootstrap}, as for $G[\lambda, \Psi, \epu]$ defined in \eqref{G: def},
    there exists a uniform constant $C=C(Q,A,B)>0$ such that
    \be
    \| G [\lambda, \Psi, \epu] \|_{L_w^2} \le C \lambda^{2-4\beta}  + C \sum_{j=0}^K |c_j|.
    \label{estimate of error term: singular weight}
    \ee
\end{lemma}
\begin{proof}[Proof of Lemma \text{\ref{estimate of G}}]
Recall \eqref{G: new expression}, $G[\lambda,\Psi, \epu] = O(r^{2K+2})$ at the origin, then by applying
 Taylor expansion with the form of integral residue at the origin onto $G[\lambda,\Psi,\epu]$,
\begin{align*}
     \big \| G[\lambda, \Psi, \epu] \big \|_{L_w^2(|y| \le 1)}^2
     & \le C \int_{|y| \le 1} |G[\lambda,\Psi, \epu]|^2 \frac{1}{|y|^{4K}} dy  \\
     & \le C \big\| D^{2K} G[\lambda, \Psi, \epu] \big\|_{L^\infty}^2 \le 
     C \| G[\lambda, \Psi, \epu] \|_{H^{2K+2}}^2.
\end{align*}
For the case with $|y| \ge 1$,
\begin{align*}
    \big \| G[\lambda, \Psi, \epu] \big \|_{L_w^2(|y| \ge 1)}
    & \le C \big \| G[\lambda, \Psi, \epu] \big \|_{L^2(|y| \ge 1)}  \le C  \| G[\lambda, \Psi, \epu] \|_{H^{2K+2}}.
\end{align*}

Consequently, together with the definition of $G[\lambda, \Psi,\epu]$ in \eqref{G: new expression}, Lemma \ref{lemma: preliminaries, Psi}, \eqref{Taylor expansion: Delta eps}, and Lemma \ref{lemma: preliminaries epu}, this concludes that
\begin{align*}
  & \quad  \| G[\lambda, \Psi, \epu] \|_{L_w^2} \le 
     C \| G[\lambda, \Psi, \epu] \|_{H^{2K+2}} \\
     & \le C\lambda^{2-4\beta} \left( \| \Delta Q + \epu \|_{H^{2K+2}} +\| \Delta \eps \|_{H^{2K+2}}+ \sum_{j=0}^K \big|[\Delta Q + \epu]_j \big| + [\Delta \eps]_K \right) \\
    &   \qquad +C \| \calL \epu \|_{H^{2K+2}} + \sum_{j=0}^K \big|[\calL \epu]_j \big | + C \| N(\epu) \|_{H^{2K+2}} + C \sum_{j=0}^K \big|[N(\epu)]_j \big| \\
    & \le C \lambda^{2-4\beta} \left(1+ \| \eps \|_{H^{2K+4}} \right) + C \left( \sum_{j=0}^K |c_j| + |c_j|^2 \right)
    \le C  \lambda^{2-4\beta}  + C  \sum_{j=0}^K |c_j|.
\end{align*}
for some uniform constant $C>0$, and thus we have concluded the proof.
\end{proof}


 Next, we are devoted to the proof of Lemma \ref{lemma: L2 estimate of eps}.
 
\begin{proof}[Proof of Lemma \ref{lemma: L2 estimate of eps}]
Recall that $\eps$ solves the equation \eqref{eq: eps},
    \begin{align*}
        \frac{1}{2} \frac{d}{d\tau} \| \eps \|_{L_w^2}^2
          = (\partial_\tau \eps, \eps)_{L_w^2} 
          = I + I I + III + IV,
    \end{align*}
    with
    \begin{align*}
        & I: = \left( \calL \eps, \eps \right)_{L_w^2}, \quad 
         II:= \left(\na \epu \cdot \na \Dein \eps + \na \eps \cdot \na \Dein \epu + 2(1-\mu) \epu \eps, \eps \right)_{L_w^2}, \\
        & III
        := \left( N(\eps), \eps \right)_{L_w^2},
        \quad  IV:= \left(G[\lambda, \Psi, \epu], \eps \right)_{L_w^2}.
    \end{align*}

    \noindent \textit{Step 1. Estimate of the small linear term $II$.} The small linear term $II$ can be written as $II:=II_1+II_2+ II_3$ with
    \[
    II_1 : =\left(\na \epu \cdot \na \Dein \eps , \eps \right)_{L_w^2}, \quad 
    II_2 := \left(\na \eps \cdot \na \Dein \epu, \eps \right)_{L_w^2}, \quad 
    II_3:= \left( 2(1-\mu) \epu \eps, \eps \right)_{L_w^2}.
    \]
    First of all, repeating \eqref{I NLO 1}, together with the fact that $\text{supp }\epu \subset B(0,2)$, there exists $C= C(A)>0$ such that $II_1$ can be controlled by
\begin{align*}
    II_1 \le C \big\| |y|^{-\frac12} \partial_r \epu \big\|_{L^2} \| \eps \|_{L_w^2}^2 \le C \| \na \epu \|_{L^\infty} \| \eps \|_{L_w^2}^2.
\end{align*}

   
For $II_2$, direct computation shows
\begin{align}
    II_2 
    & = \int \left( \na \eps \cdot \na \Dein \epu \right) \eps w dy  = \frac{1}{2} \int \na \eps^2 \cdot \na \Dein \epu w dy \notag \\
    & = -\frac{1}{2} \int \eps^2  \epu w dy - \frac{1}{2} \int \eps^2 \na \Dein \epu \cdot \na w dy \le C \| \epu \|_{L^\infty} \| \eps \|_{L_w^2}^2,
    \label{L2: weight norm II 2}
\end{align}
where the last inequality holds by Cauchy-Schwarz inequality together with the pointwise estimate
\begin{align*}
    |\na \Dein \epu \cdot \na w |
    & = \Bigg| \left( \frac{1}{r^2} \int_0^r \epu (s) s^2 ds \right) \left( \partial_r w  \right) \Bigg|
    \le C(A) \| \epu \|_{L^\infty} w.
\end{align*}

For $II_3$, it can be directly controlled by
\begin{align*}
    II_3 & \le \Big| \left( 2(1-\mu) \epu \eps , \eps \right)_{L_w^2} \Big|
     \le 2(1-\mu) \| \epu \|_{L^\infty} \| \eps \|_{L_w^2}^2.
\end{align*}


In sum, the small linear term $II$ can be estimated by
\begin{align*}
 II \le C \| \epu\|_{W^{1,\infty}} 
 \| \eps\|_{L_w^2}^2.
\end{align*}


\vspace{0.3cm}
\noindent \textit{Step 2. Estimate of the nonlinear term $III$.} 
We begin by performing integration by parts and using a similar argument in \eqref{L2: weight norm II 2}, it then follows that there exists $C=C(A)>0$ such that
\begin{align*}
    III & =\left( \na \eps \cdot \na \Dein \eps + (1-\mu) \eps^2, \eps  \right)_{L_w^2}  \le C \| \eps \|_{L^\infty} \| \eps \|_{L_w^2}^2.
\end{align*}


\vspace{0.3cm}


\noindent \textit{Step 3. Summary of the estimates.} Combining all of the estimates above, \eqref{L: coer}, \eqref{delta g: restriction}, \eqref{delta i: restriction} and \eqref{estimate of error term: singular weight}, and applying Young's inequality, we obtain that there exists a constant $C= C(Q,A,B,\delta_g) >0$ such that
\begin{align*}
    \frac{1}{2} \frac{d}{d\tau} \| \eps \|_{L_w^2}^2
    & \le -\frac{1}{8} \| \eps \|_{L_w^2}^2 + C \left( \| \epu \|_{W^{1,\infty}} + \| \eps \|_{L^\infty} \right) \| \eps \|_{L_w^2}^2 + C \left( \lambda^{2-4\beta} +\sum_{j=0}^{K} |c_j| \right) \| \eps \|_{L_w^2} \\
    & \le - \frac{\delta_g}{2} \| \eps \|_{L_w^2}^2 + C \left( \lambda^{4-8\beta} + \sum_{j=0}^K |c_j|^2 \right),
\end{align*}
which concludes \eqref{L2 estimate of eps}. Hence, recalling the bootstrap assumptions \eqref{bootstrap assum: L2 stable}, \eqref{bootstrap assum: Hm stable}, \eqref{bootstrap assum: real unstable} and \eqref{bootstrap assum: fake unstable}, and by Gronwall's inequality,
\begin{align}
    & \quad \| \eps(\tau) \|_{L_w^2}^2 
    \le  e^{-\delta_g \tau} \| \eps(0) \|_{L_w^2}^2
    + C \int_0^\tau e^{-\delta_g (\tau -s)} \left(  \lambda^{4-8\beta}(s) + d_{real}^2(s) + \sum_{j=j_0+1}^K |c_j(s)|^2 \right) ds \notag \\
    & \le  e^{-\delta_g \tau} \| \eps(0) \|_{L_w^2}^2 + C \int_0^\tau e^{-\delta_g (\tau -s)} \left( \lambda_0^{4-8\beta} e^{-(2-4\beta) s} + \left( \delta_3^2 + \sum_{j=j_0+1}^K \delta_j^2 \right) e^{-\frac{7}{5} \delta_g s} \right) ds \notag \\
    & \le \left[ \delta_0^2 + C \left( \lambda_0^{4-8\beta} + \delta_3^2 + \sum_{j=j_0+1}^K \delta_j^2 \right)  \right] e^{-\delta_g \tau}, \quad \forall \; \tau \in (0,\tau^*], 
    \label{delta: choice 1}
\end{align}
for some constant $C=C(Q, A,B,\delta_g)>0$ independent on each $\delta_i$. Ttogether with \eqref{delta i: restriction} and \eqref{bootstrap: initial condition}, this yields that
\[
\| \eps (\tau) \|_{L_w^2} \le \frac{1}{2} \delta_1 e^{-\frac{1}{2} \delta_g \tau}, \quad \forall \; \tau \in [0,\tau^*],
\]
hence we have concluded the proof.
\end{proof}





\subsubsection{$\dot H^{2K+4}$ estimate of $\eps$.} This section is to improve the $\dot H^{2K+4}(\RR^3)$ estimate of $\eps$ under the bootstrap assumptions of Proposition \ref{prop: bootstrap}. The main result is as follows:



\begin{lemma}[$\dot H^{2K+4}$ estimate of $\eps$]
\label{lemma: Hm estimate of eps}
Under the assumptions of Proposition \ref{prop: bootstrap}, there exists a constant $C=C(Q, A,B,\delta_g)>0$ such that the following inequality hold uniformly in $\tau \in [0,\tau^*]$:
\be
\frac{d}{d\tau} \| \eps \|_{\dot H^{2K+4}}^2 \le -  \frac{1}{16} \| \eps \|_{\dot H^{2K+4}}^2 + C \| \eps \|_{L^2}^2
    +C\left( \| \eps \|_{H^{2K+4}}^4 + \lambda^{4-8\beta} + \sum_{j=0}^{K} |c_j|^2 \right).
\label{stable part: higher regu}
\ee
In particular, the bootstrap assumption \eqref{bootstrap assum: Hm stable} can be improved to
\[
\| \eps (\tau) \|_{\dot H^{2K+4}} \le \frac{1}{2} \delta_2 e^{-\frac{\delta_g}{2} \tau}, \quad \forall \; \tau \in [0,\tau^*].
\]
\end{lemma}

\begin{proof}
    Recall that $\eps$ solves the equation \eqref{eq: eps},
    \begin{align*}
        &  \frac{1}{2} \frac{d}{d\tau} \| \eps \|_{\dot H^{2K+4}}^2
         = I + II + III + IV,
    \end{align*}
    with
    \begin{align*}
         &  I : = \left ( \Delta^{K+2}\calL \eps,\Delta^{K+2} \eps\right )_{L^2}, \\
         & II:= \left( \Delta^{K+2} \left( \na \epu \cdot \na \Dein \eps + \na \eps \cdot \na \Dein \epu + 2(1-\mu) \epu \eps \right), \Delta^{K+2} \eps \right)_{L^2}, \\
         &III:= \left(\Delta^{K+2}N(\eps),\Delta^{K+2} \eps\right )_{L^2}, \quad   
         IV:= \left(\Delta^{K+2}G[\lambda, \Psi, \epu],\Delta^{K+2} \eps\right )_{L^2}.
    \end{align*}

    \noindent \underline{\textit{Estimate of small linear term $II$.}} For the small linear term $II$, since $\epu \in C_0^\infty(\RR^3)$ with support in $B(0,2)$, together with integration by parts, Sobolev inequality, Gagliardo-Nirenberg inequality and \eqref{nonlocal term: formula}, there exists uniform constant $C=C(K,\mu)>0$ such that
    \begin{align}
         II
        & \le  \left( \Delta^{K+2} \left( \na \eps \cdot \na \Dein \epu \right), \Delta^{K+2} \eps \right)_{L^2}
        + \left( \Delta^{K+2} \left( \na \epu \cdot \na \Dein \eps + 2(1-\mu) \epu \eps \right), \Delta^{K+2} \eps \right)_{L^2} \notag \\
        & \le \left( \na \Delta^{K+2} \eps \cdot \na \Dein \epu, \Delta^{K+2} \eps \right)_{L^2}
        + C \sum_{j=1}^{2K+4} \| \na^{2K+5-j} \eps \|_{L^2} \| \na^{j+1} \Dein \epu \|_{L^\infty} \| \eps \|_{\dot H^{2K+4}}  \notag \\
        & \quad +C \| \na^{2K+5} \epu \|_{L^2} \| \na \Dein \eps \|_{L^\infty(B(0,2))}
        + C \sum_{j=1}^{2K+4}\| \na^{2K+5-j} \epu \|_{L^\infty} \| \na^{j+1} \Dein \eps \|_{L^2} \notag \\
        & \le C \| \epu \|_{H^{2K+6}} \| \eps \|_{H^{2K+4}}^2.
         \label{Hk: III}
    \end{align}


    \noindent \underline{\textit{Estimate of nonlinear term $III$.}} For $III$, by integration by parts, there exists a uniform constant $C=C(K,\mu)>0$ such that
    \begin{align}
        III
        & = \left(\Delta^{K+2} \left( \na \eps \cdot \na \Dein \eps \right),\Delta^{K+2} \eps\right )_{L^2} + (1-\mu)\left(\Delta^{K+2} (\eps^2),\Delta^{K+2} \eps\right )_{L^2} \notag \\
       % & \le \left( \na \Delta^{K+2} \eps \cdot \na \Dein \eps,\Delta^{K+2} \eps\right )_{L^2} 
      %  + C \sum_{j=1}^{2K+4} \int |\na^{2K+5-j} \eps| |\na^{j+1} \Dein \eps| |\Delta^{K+2} \eps| dy 
       % \notag 
       % \\
      %  & \quad + C \int  |\eps| |\na^{2K+4} \eps|^2  dy  +
      %  C \sum_{j=1}^{2K+3} \int|\na^{2K+4 -j} \eps| |\na^j \eps| |\Delta^{K+2} \eps| dy 
      %  \notag
      %  \\
        & \le  C  \left( \| \eps \|_{L^\infty} + \| \na^2 \Dein \eps \|_{L^\infty}  \right)  \| \eps \|_{H^{2K+4}}^2
        +  C \sum_{j=2}^{2K+4} \| \eps \|_{H^{2K+6-j}} \| \eps \|_{H^{j}} \| \eps \|_{\dot H^{2K+4}}
        \notag
        \\
        & \quad +C \sum_{j=1}^{2K+3} \| \eps \|_{H^{2K+5-j}} \| \eps \|_{H^{j+1}} \| \eps \|_{\dot H^{2K+4}} \notag\\
        & \le C \| \eps \|_{H^{2K+4}}^3.
        \label{HK: II}
    \end{align}
    
    \noindent \underline{\textit{Estimate of the modulation term $IV$.}} For the modulation term $IV$, recalling \eqref{G: new expression}, \eqref{Taylor expansion: Delta eps}, \eqref{nonlinear term: epu} and \eqref{linear term: epu},
    there exists a uniform constant $C>0$ such that
    \begin{align*}
        \Big\| G[\lambda,\Psi, \epu] - \lambda^{2-4\beta} \Delta \eps \Big\|_{\dot H^{2K+4}}
        \le C \lambda^{2-4\beta} + C \sum_{j=0}^K |c_j|,
    \end{align*}
    which, by the non-negativity of $\lambda$ (see \eqref{lambda: form}), yields that
    \begin{align}
        IV & = \left( \Delta^{K+2} G[\lambda,\Psi, \epu], \Delta^{K+2} \eps \right)_{L^2} \notag \\
        & =  \lambda^{2-4 \beta} \left( \Delta^{K+2} \Delta \eps, \Delta^{K+2} \eps \right)_{L^2} + \left( \Delta^{K+2} \left( G[\lambda,\Psi, \epu]-\lambda^{2-4\beta} \Delta \eps \right), \Delta^{K+2} \eps \right)_{L^2}
        \notag
        \\
        & = - \lambda^{2-4\beta} \| \na \Delta^{K+2} \eps \|_{L^2} +
        \left( \Delta^{K+2} \left( G[\lambda,\Psi, \epu]-\lambda^{2-4\beta} \Delta \eps \right), \Delta^{K+2} \eps \right)_{L^2} 
        \notag
        \\
        & \le C \left( \lambda^{2-4\beta} +  \sum_{j=0}^K |c_j| \right) \| \eps \|_{\dot H^{2K+4}}.
        \label{HK: IV}
    \end{align}

    \noindent \underline{\textit{Conclusion of the estimates.}} Noting that $I$ has been handled in Proposition \ref{prop: core H^K}, combining \eqref{coercivity in H^K}, \eqref{HK: II}, \eqref{Hk: III} and \eqref{HK: IV} concludes that
    \begin{align*}
    \frac{d}{d\tau} \frac{1}{2} \| \eps \|_{\dot H^{2K+4}}^2
    & \le - \frac{1}{8} \| \eps \|_{\dot H^{2K+4}}^2 + C \| \eps \|_{L^2}^2 \\
    & \quad \;+C\left( \| \eps \|_{H^{2K+4}}^2  + \lambda^{2-4\beta} + \sum_{j=0}^{K} |c_j| \right) \| \eps \|_{H^{2K+4}},
    \end{align*}
    which, together with Young's inequality, yields \eqref{stable part: higher regu}. Hence, recalling the bootstrap assumptions \eqref{bootstrap assum: L2 stable}, \eqref{bootstrap assum: Hm stable}, \eqref{bootstrap assum: real unstable} and \eqref{bootstrap assum: fake unstable}, by Gronwall's inequality,
    \begin{align}
        & \quad \| \eps(\tau) \|_{\dot H^{2K+4}}^2 \notag \\
        & \le \| \eps(0) \|_{\dot H^{2K+4}}^2 e^{-\frac{1}{16} \tau}
        +C \left(\delta_1^2 + \delta_2^4 + \delta_3^2 + \delta_0^{4-8\beta} + \sum_{j=0}^K \delta_j^2  \right) \int_0^\tau e^{-\frac{1}{16} (\tau-s)} e^{-\delta_g s} ds \notag \\
        & \le C \left(\delta_0^2 +\delta_1^2 + \delta_2^4 + \delta_3^2 + \delta_0^{4-8\beta} + \sum_{j=0}^K \delta_j^2  \right)  e^{-\delta_g \tau}, \quad \forall \; \tau \in [0,\tau^*].
        \label{delta: choice 2}
    \end{align}
    Combining the assumptions on the coefficients \eqref{delta g: restriction} and \eqref{delta i: restriction}, this yields that
    \[
    \| \eps(\tau) \|_{\dot H^{2K+4}} \le \frac{1}{2} \delta_2 e^{-\frac{1}{2} \delta_g \tau}, \qquad \forall \; \tau \in [0,\tau^*],
    \]
    and hence we have concluded the result.
\end{proof}

\subsubsection{Estimate of $\ep_{u,fake}$.}
This section is dedicated to improving the bootstrap assumption \eqref{bootstrap assum: fake unstable} under the bootstrap assumptions of Proposition \ref{prop: bootstrap}. The main result is stated as follows:

\begin{lemma}[Estimate of $\ep_{u,fake}$]
\label{lemma: estimate of unstable fake}
    Under the assumptions of Proposition \ref{prop: bootstrap}, for any $j_0+1 \le j \le K$, there exists a constant $C=C(\mu, K,j_0, \beta)>0$ such that
    \begin{align}
        \frac{d}{d\tau} c_j^2 \le - \frac{1}{j_0} c_j^2 +   C \lambda^{8 -4\beta} + C \sum_{i=0}^{j-1} |c_i|^2 + C \sum_{i=0}^K |c_i|^4, \quad \forall \; \tau \in [0,\tau^*].
        \label{fake unstable: estimate}
    \end{align}
    In particular, the bootstrap assumption \eqref{bootstrap assum: fake unstable} can be improved to
    \be
    |c_j (\tau)| \le \frac{1}{2} \delta_j e^{-\frac{7\delta_g}{10} \tau}, \quad \forall \; \tau \in [0,\tau^*].
    \label{fake unstable: improvement of bootstrap}
    \ee
\end{lemma}

\begin{proof}
Recalling \eqref{ODE system for unstable part}, $c_j$ solves the ODE
\[
\dot c_{j} =  \frac{j_0 -j}{j_0} c_j + \lambda^{2-4 \beta} [\Delta \Psi]_{j} +  \sum_{i=0}^{j-1} \sigma_{i,j} c_i + [N(\epu)]_{j}, \quad \text{  for any } j_0 < j \le K.
\]
Then by Young's inequality, \eqref{Delta Psi: estimate on Taylor coeff} and \eqref{nonlinear term: epu}, there exists $C=C(K, j_0, \mu)>0$ such that
\begin{align*}
    \frac{1}{2}\frac{d}{d\tau}  c_j^2 
     = c_j \dot c_j &= c_j \left( \frac{j_0 -j}{j_0} c_j + \lambda^{2-4 \beta} [\Delta \Psi]_{j} + \sum_{i=0}^{j-1} \sigma_{i,j} c_i + [N(\epu)]_j \right) \\
    & = \frac{j_0-j}{j_0} c_j^2 + \lambda^{2-4\beta}  [\Delta \Psi]_j c_j + \sum_{i=0}^{j-1} \sigma_{i,j} c_i c_j + [N(\epu)]_j c_j \\
    & \le - \frac{1}{2j_0} c_j^2 +  C \lambda^{8 -4\beta} + C \sum_{i=0}^{j-1} |c_i|^2 + C \sum_{i=0}^K |c_i|^4.
\end{align*}

By Gronwall's inequality, \eqref{delta g: restriction}  \eqref{delta i: restriction},  \eqref{bootstrap: initial condition}, and bootstrap assumption \eqref{bootstrap assum: real unstable} and \eqref{bootstrap assum: fake unstable}, 
there exists a constant $C= C(K, j_0,\beta)>0$ such that
\begin{align}
    c_j^2(\tau) 
    & \le e^{-\frac{1}{j_0} \tau} c_{j}^2(0) 
    + C \int_0^\tau e^{-\frac{1}{j_0} (\tau-s)} \Bigg[ \lambda_0^{4-8\beta} e^{-(2-4\beta) s}  + 
    \left( \delta_3^2+
    \sum_{i=j_0+1}^{j-1} \delta_i^2 \right) e^{-\frac{7}{5} \delta_g s}  \notag \\
    & \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad + \left( \delta_3^4 + \sum_{i=j_0+1}^K \delta_i^4 \right) e^{-\frac{14}{5} \delta_g s} \Bigg] ds \notag \\
    & \le  e^{-\frac{1}{j_0} \tau} c_{j}^2(0) + C \left( \lambda_0^{4-8\beta} + \delta_3^2 + \sum_{j_0+1 \le i \le j-1} \delta_i^2  + \delta_3^4 + \sum_{i=j_0+1}^K \delta_i^4 \right) e^{-\frac{7}{5} \delta_g \tau}
    \notag
    \\
    & \le C \left( \delta_0^2 + \lambda_0^{4-8\beta} + \delta_3^2 + \sum_{i=j_0+1}^{j-1} \delta_i^2 \right) e^{-\frac{7}{5}\delta_g \tau} \le \frac{1}{4} \delta_j^2 e^{-\frac{7}{5} \delta_g \tau}, \;\; \forall \; \tau \in [0,\tau^*],
    \label{delta: choice 3}
\end{align}
which concludes the proof.
\end{proof}

\subsection{Control of real unstable part.}

\mbox{}

\begin{proof}[Proof of Proposition \ref{prop: bootstrap}]
    
    \mbox{}

    \noindent \underline{\textit{Improvement of the bootstrap assumptions.}} Arguing by contradiction, suppose that there exists an initial triple $(\lambda_0, \ep_{u,fake}(0), \eps(0))$ satisfying \eqref{bootstrap: initial condition} such that for any $\ep_{u,fake}(0)$ with $d_{real}(0) \le \delta_3$, the exit time $\tau^*$ defined in \eqref{exit time} is always finite. Then, by Lemma \ref{lemma: L2 estimate of eps}, Lemma \ref{lemma: Hm estimate of eps} and Lemma \ref{lemma: estimate of unstable fake}, combining with the continuity of the solution to system \eqref{renormalization KS} with respect to $\tau$, there exists $0 < \epsilon_{\tau^*} \ll 1$ such that \eqref{bootstrap assum: L2 stable}, \eqref{bootstrap assum: Hm stable} and \eqref{bootstrap assum: fake unstable} hold for all $\tau \in [0,\tau^* + \epsilon_{\tau^*}]$.
    
\vspace{0.3cm}

\noindent \underline{\textit{Outer-going flux property.}}
In light of the preceding argument, the only possible mechanism by which the solution exits the bootstrap regime is the failure of the bootstrap assumption for the real unstable component $\ep_{u,real}$, specifically when this assumption ceases to hold on $[0,\tau]$ for some $\tau > \tau^*$. Moreover, by the local well-posedness of the system \eqref{equation: KS with damping}, it follows that the mapping $\tau \mapsto d_{real}(\tau)$ is continuous. If we define the set
\[
B(\tau) := \Big\{ \{c_j\}_{j=0}^{j_0} \in \RR^{j_0+1}: \sqrt{ \frac{1}{2}\sum_{j=1}^{j_0-1} c_j^2 + \frac{10}{\delta_g^2} c_0^2 + \frac{1}{4 |\sigma_{0,j_0}| } c_{j_0}^2} \le \delta_3 e^{-\frac{7}{10} \delta_g \tau} \Big\},
\]
then by the contradiction assumption, the following holds
\[
\begin{cases}
    \{ c_j(\tau) \}_{j=0}^{j_0} \in B(\tau), & \forall \; \tau \in [0,\tau^*], \\
    \{ c_j(\tau) \}_{j=0}^{j_0} \in \partial B(\tau), & \tau = \tau^*.
\end{cases}
\]
 Recalling the modulation ODE system satisfied by the coefficients $\{c_j\}_{j=0}^{j_0}$ as given in \eqref{ODE system for unstable part}, and invoking Young's inequality in conjunction with Lemma \ref{lemma: preliminaries, Psi} and Lemma \ref{lemma: preliminaries epu}, there exists a constant $C=C(\delta_g, |\sigma_{0,j_0}|,K,j_0)>0$ independent of $\{\delta_i\}$, such that the quantity $d_{real}$ defined in \eqref{bootrap real unstable: norm} satisfies
\begin{align*}
    & \quad \frac{d}{d\tau}d_{real}^2(\tau)
    = \sum_{j=1}^{j_0-1} c_j \dot c_j + \frac{20}{\delta_g^2} c_0 \dot c_0+ \frac{1}{2 |\sigma_{0,j_0}|} c_{j_0} \dot c_{j_0}  \\
    & = \sum_{j=1}^{j_0-1} \frac{j_0-j}{j_0} c_j^2 + \frac{20}{\delta_g^2} c_0^2 + \frac{1}{2} c_0 c_{j_0}  + \lambda^{2-4\beta}\left( \sum_{j=1}^{j_0-1} c_j  [\Delta \Psi]_j + \frac{20}{\delta_g^2} c_0 [\Delta \Psi]_0 + \frac{1}{2 |\sigma_{0,j_0}|}c_{j_0} [\Delta \Psi]_{j_0} \right) \\
    & \qquad + \sum_{j=1}^{j_0 -1} [N(\epu)]_j c_j + \frac{20}{\delta_g^2} c_0 [N(\epu)]_0 + \frac{1}{2 |\sigma_{0,j_0}|} c_{j_0} [N(\epu)]_{j_0} \\
    & \ge - C \lambda^{4-8\beta}\sum_{j=0}^{j_0} \Big|[\Delta \Psi]_j \Big|^2 - \frac{\delta_g^2}{160} c_{j_0}^2 - C \sum_{j=0}^K \big| [N(\epu)]_{j} \big|^2 \\
    &\ge - C \lambda^{4-8\beta}
    - \frac{\delta_g^2 |\sigma_{0,j_0}|}{40} d_{real}^2
     - Cd_{real}^4  - C \sum_{j=j_0+1}^K |c_j|^4.
\end{align*}
Consequently, under the contradiction assumption that $e^{\frac{7}{10}\delta_g \tau^*}d_{real}(\tau^*) = \delta_3$, 
and in light of bootstrap assumptions \eqref{bootstrap: initial condition}, \eqref{bootstrap assum: real unstable}, and \eqref{bootstrap assum: fake unstable}, together with coefficient restrictions \eqref{delta g: restriction} and \eqref{delta i: restriction}, we deduce the outer-going flux property on $\partial B(\tau^*)$:
\begin{align}
    & \quad \frac{d}{d\tau} \left( e^{\frac{7}{5} \delta_g \tau} d_{real}^2(\tau) \right) \Bigg|_{\tau = \tau^*}
    = \left( \frac{7}{5} \delta_g e^{\frac{7}{5} \delta_g \tau} d_{real}^2(\tau) + e^{\frac{7}{5} \delta_g \tau} \frac{d}{d\tau} d_{real}^2(\tau) \right) \Big|_{\tau = \tau^*} \notag\\
    & \ge  \frac{7}{5} \delta_g e^{\frac{7}{5} \delta_g \tau^*} d_{real}^2(\tau^*)
    - C \lambda_0^{4-8\beta}e^{\frac{7}{5} \delta_g \tau^*} e^{-(2-4\beta) \tau^*} - \frac{\delta_g^2 |\sigma_{0,j_0}|}{40} e^{\frac{7}{5} \delta_g \tau^*} d_{real}^2(\tau^*) \notag\\
    & \qquad \qquad 
    -C e^{\frac{7}{5} \delta_g \tau^*} d_{real}^4(\tau^*) -  C \sum_{j=j_0+1}^K e^{\frac{7}{5} \delta_g \tau^*} |c_j(\tau^*)|^4 \notag
    \\
    & \ge \frac{7}{5} \delta_g \delta_3^2 - C \lambda_0^{4-8\beta} - \frac{\delta_g^2 |\sigma_{0,j_0}|}{40} \delta_3^2 
    -C \delta_3^4 - C \sum_{j=j_0+1}^K \delta_j^4
    \ge \delta_g \delta_3^2>0.
    \label{outergoing-flux property}
\end{align}


\vspace{0.3cm}
\noindent \underline{\textit{Brouwer's topological argument.}} 
Firstly, for any $\delta >0$, we define the following convex subset on $\RR^{j_0+1}$:
\[
\calB_{real}(0,\delta)
:= \left\{ \{ c_j \}_{j=0}^{j_0} \in \RR^{j_0+1}:  \sqrt{ \frac{1}{2}\sum_{j=1}^{j_0-1} c_j^2 + \frac{10}{\delta_g^2} c_0^2 + \frac{1}{4 |\sigma_{0,j_0}|} c_{j_0}^2} < \delta  \right\}.
\]
By the local well-posedness theory for \eqref{equation: KS with damping} and contradiction assumption \eqref{exit time}, 
we establish the continuity of the map $\ep_{u,real} (0) \mapsto \ep_{u,real}(\tau^*(\ep_{u,real}(0)))$, where $\tau^*(\ep_{u,real}(0))$ denotes the exit time associated with 
$\left( \lambda_0, \ep_{u,real}(0), \ep_{u,fake}(0), \eps(0) \right)$ satisfying the initial condition \eqref{bootstrap: initial condition}. Accordingly, we define a mapping $\Phi: \overline{\calB_{real} (0,1)} \mapsto \partial \calB_{real} (0,1) $ as follows:
\begin{align*}
 \qquad  \{d_j\}_{j=0}^{j_0} \in \overline{\calB_{real} (0,1)}
&\mapsto \{c_{j}(0)\}_{j=0}^{j_0} := \{ \delta_3 d_j\}_{j=0}^{j_0}  \in \overline{\calB_{\RR^{j_0+1}} (0,\delta_3)} \\
&  \mapsto  \ep_{u,real}(0,y) =  \sum_{j=0}^{j_0} c_j(0) \chi(y) |y|^{2j}  \\
& \mapsto \ep_{u,real}(\tau^*,y) =\sum_{j=0}^{j_0} c_j(\tau^*) \chi(y) |y|^{2j} \\
&
 \mapsto \{ d_j(\tau^*) \}_{j=0}^{j_0} := \Big\{  \frac{1}{\delta_3}e^{\frac{7}{10} \delta_g \tau^*}c_j(\tau^*) \Big\}_{j=0}^{j_0} \in  \partial \calB_{real}(0,1),
\end{align*}
whose continuity is ensured by the local well-posedness of \eqref{equation: KS with damping}. In particular, when $\{d_j\}_{j=0}^{j_0} \in \partial \calB_{real} (0,1)$, by the outer-going flux property of the flow as indicated in \eqref{outergoing-flux property}, $\tau =0$ is exactly the exit time, and it leads to $\Phi = Id$ on the boundary $\partial \calB_{real}(0,1)$. However, with the continuity of $\Phi$ on the nonempty compact convex set $\overline{\calB_{real} (0,1)}$, we conclude that $-\Phi$ has a fixed point on the boundary $\partial \calB_{real}(0,1)$, which contradicts to the assertion that $\Phi =Id$ on the boundary. Consequently, the proof of Proposition \ref{prop: bootstrap} has been completed.
\end{proof}


\subsection{Existence of finite blowup solution to \eqref{equation: KS with damping} with finite mass.} This section is devoted to the study of the existence of the finite-time blowup solution to \eqref{equation: KS with damping} for any fixed $0 \le \mu < \frac{1}{3}$ and concludes the  chapter.

\begin{proof}[Proof of \textcolor{black}{Theorem \ref{thm: existence of blowup}}]
    Firstly, for any fixed $\mu \in \left[0,\frac{1}{3} \right)$, we choose $Q$ constructed in Lemma \ref{lem: solve ODE} and fix the weight $w$ as specified in Proposition \ref{prop: coer}. Then as indicated in Proposition \ref{prop: bootstrap}, there exist $\delta_g \ll 1$ and $\{ \delta_i \}$ satisfying \eqref{delta g: restriction} and \eqref{delta i: restriction}, such that the result shown in Proposition \ref{prop: bootstrap} holds.
    
    \noindent \underline{\textit{Construction of nonnegative initial data with finite mass.}}
    Firstly, since $Q\in H^{2K+4}$ as guaranteed by Lemma \ref{lem: solve ODE}, we can choose $\lambda_0 \ll \delta_0$ sufficiently small and $R_2 \gg 1$ sufficiently large such that the following estimates hold:
    \be
    \| (\chi_{R_2} -1) Q \|_{L_w^2} + \| (\chi_{R_2} -1) Q \|_{\dot H^{2K+4}} \ll \delta_0,
    \label{cut off: smallness}
    \ee
    where $\chi_{R_2}$ is a cut-off function on $B(0,R_2)$ defined by \eqref{def: cut-off on B(0,R)}.
    It then follows that there exists $\{ c_j(0) \}_{j=0}^{j_0}$ such that Proposition \ref{prop: bootstrap} holds with the initial datum
    \be
    \left(\lambda_0, \ep_s(0,y), \ep_{u,real}(0,y), \ep_{u,fake}(0,y) \right)
    := \left(\lambda_0, (\chi_{R_2} -1) Q, \sum_{j=0}^{j_0} c_j(0) \chi(y) |y|^{2j} ,0\right).
    \label{blowup to KS: initial data}
    \ee
    In other words, there exists $\ep_{u,real}(0,y)$ such that the solution to \eqref{renormalization KS} with initial data 
    \begin{align*}
    \Psi_0 &= Q + \eps(0) + \ep_{u,real}(0) + \ep_{u,fake}(0)
    =\chi_{R_2}Q + \sum_{j=0}^{j_0} c_{j}(0) \chi(y) |y|^{2j} \subset C_0^\infty(\RR^3),
    \end{align*}
    globally exists in $\tau$ and satisfies \eqref{bootstrap assum: L2 stable}-\eqref{bootstrap assum: fake unstable} on $[0,+\infty)$, and the corresponding solution $\Psi(\tau)$ can be decomposed into $\Psi(\tau) = Q + \ep(\tau)$ with
    \begin{align*}
        \| \ep(\tau) \|_{H^{2K+4}}
         & \le  \| \epu(\tau) \|_{H^{2K+4}} + \| \eps(\tau) \|_{H^{2K+4}} \\
        & \le C \left( \delta_1 + \delta_2 + \delta_3 + \sum_{j=j_0+1}^K \delta_j \right) e^{-\frac{1}{2} \delta_g \tau}, \quad \forall \; \tau >0,
    \end{align*}
    for some universal $C>0$. In addition, in view of the fact that $Q$ is radially decreasing, together with the condition \eqref{delta i: restriction}, we obtain that
    \[
    \begin{cases}
     \Psi_0(y) \ge Q(2) - C \sum_{j=0}^{j_0}|c_j(0)| \ge \frac{1}{2} Q(2) >0, &  \forall \; |y| \le 2, 
     \vspace{0.2cm}
     \\
    \Psi_0(y) = \chi_{R_2}(y)Q(y) \ge 0, & \forall \; |y| \ge 2,
    \end{cases}
    \]
    which yields the non-negativity of $\Psi_0$. Now, returning to the original equation \eqref{equation: KS with damping}, and recalling \eqref{ss coordinte}, \eqref{ss renormalization} and \eqref{lambda: form}, 
    the nonnegativity of initial density $\rho_0$ can be guaranteed:
    \[
    \rho_0(x) = \frac{1}{\lambda_0^2} \Psi_0\left( \frac{x}{\lambda_0^{2\beta}} \right) \in C_0^\infty(\RR^3).
    \]

    \noindent \underline{\textit{Finite time blowup.}} Recalling \eqref{ss coordinte}, we know that
    \begin{align*}
        \frac{d\lambda}{dt} = \frac{d\lambda}{d\tau} \frac{d\tau}{dt}
        = -\frac{\lambda}{2} \frac{1}{\lambda^2} = - \frac{1}{2\lambda}, \quad \text{with } \lambda(0) = \lambda_0,
    \end{align*}
    which implies that $\lambda(t)$ blows up at $T=\lambda_0^2$ and $\lambda(t)$ is given by
    \[
    \lambda(t) = \sqrt{T-t} = \sqrt{\lambda_0^2 -t}, \quad \forall \; t \in [0,T).
    \]
    Consequently, the solution to \eqref{equation: KS with damping} with initial data $ \rho_0$ is of form
    \[
    \rho(t,x) = \frac{1}{T-t} \left( Q + \e \right)\left(t, \frac{x}{(T-t)^{\beta}}\right),
    \]
    with
    \[
    \| \ep(\tau) \|_{H^{2K+4}} \le \epsilon_0 (T-t)^{\frac{\delta_g}{2}},
    \]
    for some $0 < \epsilon_0 \ll 1$. Consequently, we have concluded the proof of Theorem \ref{thm: existence of blowup}.

    
\end{proof}



\endgroup



